Updated T2K measurement of neutrino oscillation parameters with the first data from the Gadolinium-loaded far detector

The T2K experiment presents updated measurements of neutrino oscillation parameters using $21.4(16.3)\times10^{20}$ protons on target (POT) in (anti-)neutrino mode at the far detector, Super-Kamiokande. This analysis uses an additional neutrino dataset of $1.7 \times 10^{20}$ POT compared to the previous result, and for the very first time, data collected with Super-Kamiokande doped with Gadolinium (Gd). Significant improvements were introduced in the far detector selection and systematic error treatment. Both semi-frequentist and Bayesian analyses are presented, including results on $\sin^{2} \theta_{23}$, $\Delta m^2_{32} $, $\sin^{2} \theta_{13}$ and $\delta_{CP}$. Both analyses favor normal mass ordering with a nearly maximal CP-violating phase and are compatible with neutrino maximal mixing, slightly favouring the upper $\theta_{23}$ octant.

==> FD_old.tex <==
When a neutrino interaction produces charged particles, PMTs in the far detector collect the Cherenkov light emitted within the designated trigger window of the event. Seen as ring-like patterns on the cylindrical inner surface of the FD, the Cherenkov light is then used to reconstruct information about the charged particles produced. Notably, we identify the primary lepton from a neutrino interaction by looking for diffuse rings as a result of scattering in the case of electrons,  while muons yield rings with well-defined edges. 

Secondary particles, such as Michel electrons, generate delayed PMT hits. Previously, only the timing of the delayed hits was used to identify the Michel electrons.  Neutron captures also produce delayed hits, typically beyond the muon decay time of 2.2 $\mu$s (at characteristic times of 200~$\mu$s in water and 30~$\mu$s with Gd). Because neutron captures produce much less light than Michel electrons, we had previously seen low contamination, of about $5\%$, from neutron captures among Michel electron candidates. In the latest data taking for this work, with Gd-doping and the subsequent increase in the sensitivity to neutron captures, the Michel electron identification algorithm faced a misidentification rate of $70\%$.  To address this issue, as Figure \ref{fig:decaye} shows, we have introduced a selection-cut on the previously used measure of the timing associated with the production of a Michel electron, and the number of delayed PMT hits within $50$~ns of this time, thereby, reducing the misidentification rate to below $1\%$.

The new Michel electron selection-cut minimally impacts the neutrino event selection rates and makes the newly collected data comparable to the previous such that the event rates are within $2 - 6\%$ of prior selections. Six signal-enriched samples are used in this analysis, the same as in the previous analysis \cite{OA22shortPaper}. Five of these are identified by a single ring-like pattern from the prompt PMT hits. These are $\mu$-like and  $e$-like single-ring events collected with the beam running in the $\nu$ and $\bar\nu$ modes, and the single ring $e$-like sample with one decay electron (1Re1de), collected with only for the $\nu$ beam. The sixth sample contains both single and multi-ring topologies, to enhance our sensitivity to $\nu_\mu$CC1$\pi^+$ interactions from the $\nu$ beam. Table \ref{tab:run1-11_data} summarizes the neutrino interaction events across SK selections.  

\begin{table}
    \caption{The total number of data events for each SK selection for all runs upto this work.}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
\hline
Beam mode & Selection &  Run 1-11 POT & Events in Data \\
\hline
$\nu$ & 1R$\mu$     & $21.428\times10^{20}$ &  357 \\

& 1Re &  & 102  \\
&1Re1d.e &  & 15 \\
&$\nu_{\mu}$CC1$\pi$ &  & 140 \\
\hline
$\bar\nu$ & 1R$\mu$     & $16.346\times10^{20}$ & 137 \\
& 1Re      &  & 16 \\  %16.34556\times10^{20}
\hline

\end{tabular}

    \label{tab:run1-11_data}
\end{table}

\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.45\linewidth]{SK_figs/Decaye_cut/n50dt_Run1to10.pdf}\includegraphics[width=0.45\linewidth]{SK_figs/Decaye_cut/n50dt_Run11.pdf}
    \caption{Distribution of decay electron candidates selected by the previous Michel electron identification algorithm for the data collected in the pure-water phase (left) and Gd-doped water (right), with respect to the the number of PMT hits, on the x-axis, in a 50~ns time window around the time of producing the Michel electron candidate, on the y-axis. The magenta line represents the new selection-cut boundary, candidates below the line are identified as true Michel electrons.}
    \label{fig:decaye}
\end{figure}

\subsubsection{The new FD response model}
\label{sec:fd_sys}
%Similar to previous analyses, detector modeling errors on FD samples are evaluated through a fit on Super-K atmospheric neutrinos. set of effective error parameters that 

Similar to previous analyses \cite{T2K:2021xwb}, a fit on the atmospheric neutrinos at Super-K is used to estimate the FD mis-modelling via a set of effective error parameters that affect the sample selection criteria. 


%which shift ($\alpha$ parameters) and smear ($\beta$\ parameters) the likelihood-based cuts on different particle PIDs that are used in the sample selection cuts.
A Markov Chain Monte Carlo (MCMC)~\cite{MCMC-metro, MCMC-hasting} is used to optimize the same underlying probability distributions for data and MC, and measure the discrepancies between the two. The resulted covariance matrix binned in T2K FD sample kinematics is used for the oscillation parameter fits. In this work a few major updates are applied to the FD model for the inclusion of the new multi-ring neutrino sample, including the data binning scheme and the correlation between single- and multi-ring samples. The fitting process is also integrated better so that the irregular parameter likelihood surfaces are better represented.



\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.8\linewidth]{SK_figs/Matrix/SKErrorMatrix.pdf}
    \caption{Fractional uncertainties on different FD samples represented as the square root of the diagonal elements of the detector covariance matrix.}
    \label{fig:decaye}
\end{figure}

%\begin{itemize}
%    \item Removal of the effective error parameters' spatial dependence~\cite{t2k:2015prd} that does not work for the newly added multi-ring neutrino samples
%    \item Removal of the intermediate binning step~\cite{} that overlooked the correlation among MCMC parameters and the irregularity of parameters' likelihood surface
%    \item New binning in neutrino events' visible energy for the MCMC optimization
%    \item Inclusion of external constraints on $\pi^0$ and $\pi^{\pm}$ interactions in water~\cite{t2k:2015prd} as free parameters in the MCMC optimization
%\end{itemize}

%Additionally, better atmospheric flux spectra~\cite{} and neutrino interaction models~\cite{} are used as the inputs for MCMC.

Thanks to the better constraints via the atmospheric fit, the FD response error sizes of all T2K samples are reduced in this analysis. The change in uncertainties between the SK detector matrix used in the previous analysis (red) and the current analysis (blue) are shown in fig.~\ref{fig:SKpred_newmat}.

\begin{figure}[hb!]
\centering
        \subfloat[\centering $\nu_{e}$ appearance sample]{\includegraphics[width=0.45\textwidth, page=3]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf}}
        \qquad
        \subfloat[\centering $\bar\nu_{e}$ appearance sample]{\includegraphics[width=0.45\textwidth, page=4]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf}}
        %\includegraphics[width=0.49\textwidth, page=3]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf} &
        %\includegraphics[width=0.49\textwidth, page=4]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf} \\
        %\includegraphics[width=0.49\textwidth, page=5]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf} &
        %\includegraphics[width=0.49\textwidth, page=6]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf}
%\includegraphics[width=0.78\textwidth]{SK_figs/oldnewSKdet.png}
\caption{The change in uncertainties between the SK detector matrix used in the previous analysis (red)~\cite{OA22shortPaper} and this analysis (blue).} %As expected we see a slight tightening of errors at low reconstructed energy values.}%{\textcolor{blue}{A.L. taken from TN462 screenshot: recover vector image.}}
\label{fig:SKpred_newmat}
\end{figure}
%On the other hand, the MR diagonals do not vary much as compared to the other samples due to the rather similar parameterization for the MR sample in the \textit{Frankenmatrix} and OA2023.

%\begin{figure}[h]
%\centering
%    \makebox[\linewidth][c]{
%    \includegraphics[width=1.0\textwidth]{SK_figs/Matrix/diagonals.png}
%    \includegraphics[width=0.7\textwidth]{SK_figs/DiagErrorMom.pdf}\\
%    \includegraphics[width=0.99\textwidth]{SK_figs/DiagErrorErec.pdf}
%    }
%    \caption{The square root of the diagonal elements of the \textit{Frankenmatrix} (black) and OA2023 matrix (red). \textcolor{green}{The most top binning shows the reconstructed samples, while the one below shows the true interaction channel. The most bottom bins show the reconstructed energy.}}
%    \label{fig:sk_matrices_diag}
%\end{figure}


%In the fit of atmospheric neutrinos before OA2023, the \{$\alpha$, $\beta$\} parameters had detector spatial dependencies that were developed only for 1R samples and will not work for the MR samples. On the other hand, the missing dependency on E$_{vis}$ for the old \{$\alpha$, $\beta$\} led to strong correlations among the E$_{rec}$ (or $p$) bins in the final OA matrix. Thus, in this new analysis, the fit dimension separating the detector into different regions is replaced by an E$_{vis}$ dimension for the \{$\alpha$, $\beta$\} of both 1R and MR samples. 

%Back in OA2022, a temporary solution---the so-called \textit{Frankenmatrix}---was adopted to include errors for the MR sample.
%This \textit{Frankenmatrix} was created where the \{$\alpha$, $\beta$\} for 1R and MR samples were optimized separately using the already existing inputs that were developed independently.
%The lack of migration between the 1R and MR samples in this approach resulted in an unrealistic uncertainty matrix, with mild correlations only from the external constraints.
%This is automatically improved by the simultaneous fit of both 1R and MR samples performed for the current analysis.
%In addition to the new variables and visible final-state topologies for MR samples, the use of the $\pi^0$ and $\pi^{\pm}$ hybrid samples is also updated in this new matrix. \textcolor{red}{Unlike the previous treatment where the data-MC comparison of these hybrid samples were applied as external constraints on the \{$\alpha,\,\beta$\} parameters in the intermediate Toy MC that is removed, they are applied as prior constraints for the relevant \{$\alpha,\,\beta$\} parameters in the MCMC fits as explained in~\cite{TN482}.}

%Another important update is the removal of an intermediate matrix.
%Previously, the efficiency distributions from the nominal atmospheric MC as caused by the cut variables in the fit are used to construct an intermediate matrix binned in E$_{vis}$ and visible final topology.
%The error parameters were then thrown from this matrix, along with the BANFF post-fit and external constraints, to generate the uncertainty matrix based on the T2K MC.
%However, such a process inevitably loses the information on individual error parameters from the MCMC chains while overlooking the irregularity of the efficiency distributions.
%Therefore, we decided to remove this intermediate matrix and throw the error parameters directly from the MCMC. 

%All these improvements lead to the new constraints on detector systematic errors shown in the next section. 

%These changes introduced for OA2023 and future analyses are summarized in \cref{tab:sk-covmat-changes}.
%\begin{center}
%\begingroup
%\setlength\LTleft{-1.5cm}
%\captionsetup[table]{skip=5pt}
%\centering
%\begin{longtable}{p{4cm} | p{5cm} | p{5cm}}
%    \hline
%    \hline
%    & Prior to OA2023 & OA2023+\\
%    \hline & \\[-1mm]
% \hline
%   \multirow{4}{*}{Fitting} & 4 cut variables & 7 cut variables \\
%                               & 6 visible final topologies & 8 visible final topologies \\
%                               & 6 detector regions & no detector region binning\\
%                               & no E$_{vis}$ binning & 5 E$_{vis}$ binning\\
%    \hline
%    Intermediate matrix & Based on the ``efficiencies" of core sample cuts, binned in E$_{vis}$ & Removed \\
%    \hline
%    Toy MC & Throwing from the intermediate matrix & Throwing from the MCMC posterior distributions \\
%    \hline
%    1R\&MR correlation & The \textit{Frankenmatrix} & Fully correlated \\
%    \hline
%    External errors & Constraints on e.g. NC, $\mu$ decay, Michel $e$ tagging applied in parallel with the fit & Partially removed -or- constrained in the fit\\
%    \hline
%    Hybrid samples & Implemented as ``external constraints'' in parallel with the fit & Included in the fit \\
%    \hline
%    \hline
%    \caption{Major updates of SK detector uncertainties for OA2023+.}
%    \label{tab:sk-covmat-changes}
%\end{longtable}
%\endgroup
%\end{center}

%\subsubsection{Results on detector systematics constraints}

%\cref{fig:sk_matrices} shows the \textit{Frankenmatrix} to the left and the new matrix for OA2023 right.
%In both matrices, the blocks are ordered by FHC 1R$e$, FHC 1R$\mu$, RHC 1R$e$, RHC 1R$\mu$, FHC 1R$e$+1d.e., and MR from left to right. Each sample block is further binned by E$_{rec}$ and neutrino interaction/oscillation channels.
%
%\begin{figure}[H]
%\centering
%\includegraphics[width=0.75\textwidth]{SK_figs/Matrix/SKJointErrorMatrix_Total_270122_OA2021_erec_plot.pdf}
%
%\includegraphics[width=0.75\textwidth]{SK_figs/Matrix/SKJointErrorMatrix_OA2023_V1_erec_plot.pdf}
%    \caption{The OA2022 \textit{Frankenmatrix} to the top and the new OA2023 matrix from the full atmospheric fit to the bottom. Both matrices have the same binning of T2K samples and $E_{rec}$.}
%    \label{fig:sk_matrices}
%\end{figure}

%\begin{figure}[H]
%\centering
%    \makebox[\linewidth][c]{\includegraphics[width=1.0\textwidth]{SK_figs/Matrix/OAmatrix.png}}
%    \caption{The OA2022 \textit{Frankenmatrix} to the left and the new OA2023 matrix from the full atmospheric fit to the right. Both matrices have the same binning of T2K samples and E$_{rec}$.}
%    \label{fig:sk_matrices}
%\end{figure}
%\todo{Remake these plots to be prettier and have a consistent colour theme}

%The missed correlation between 1R and MR samples in the \textit{Frankenmatrix} is recovered in the new matrix thanks to the full atmospheric fit.
%Meanwhile, the strong correlation among E$_{rec}$ bins in each T2K sample is also reduced because of the new E$_{vis}$ dependencies of the \{$\alpha$, $\beta$\} parameters.

%\subsection{Impact on the Monte Carlo predictions uncertainties at SK}
%\todo{compare the new and old MC predictions at SK}
%\subsubsection{New MC prediction at SK}
%\subsubsection{Impact of new SK det cov on predictions}


==> FakeDataStudySummary.tex <==
\section{Fake data studies}
\label{sec:FDS}

\subsection{Summary of Fake Data Impacts in OA2022}
As described in TN441, several fake data studies were performed for OA2022 to evaluate the impact of alternative nuclear and cross-section models, as well as some data-driven studies and other additional effects on the oscillation analysis. Biases on quoted intervals for each atmospheric oscillation parameters are computed and the impact on the Physics conclusion on CP violation is checked. A list of these studies together with the computed biases for both Asimov A22 and B22 sets~\ref{tbl:osc_param} are shown in \cref{tab:SummaryAllScaled}.
In this table, the 'scaled Asimov' method is used, meaning that the impact of the fake data study on the total number of events is retrieved to focus on the effect coming from migration between samples or distortions of spectra.

It was found that none of the studies impacted our conclusions on the exclusion of CP conservation at more than 90\%. However, it was found that an additional error on the atmospheric $\Delta m^2$ was necessary to be applied in the form of a Gaussian smearing with sigma $S^{A22}_{All} = 2.7\times10^{-5}$~eV$^2$. At this precision level, the same value was found for standard and scaled Asimov fits, due to small differences compensating each other. This is to be compared to the error on $\Delta m^2$ in the data fit. For example, from the global best fit, the total error on $\Delta m^2$ was $3.4\times10^{-5}$~eV$^2$. The effect of the fake data accumulated is therefore the same order of magnitude than the total fit error.

Due to a bug introduced at the level of the NEUT software used to model all interactions, concerning the pion final state interactions, an additional contribution to this smearing factor was computed. As a result the final full value of smearing for this analysis is $3.1\times10^{-5}$~eV$^2$ on $\Delta m^2_{32}$.
\begin{table}[htb!]
\setlength\LTleft{-1.5cm}
\centering
\renewcommand{\arraystretch}{1.3}
   \newcommand{\paren}[1]{\ensuremath{\left(#1\right)} }
    \resizebox{\textwidth}{!}{
\begin{tabular}{ c | c | c | c | c || c | c | c | c  }
\hline \hline
& \multicolumn{4}{c|}{A22} & \multicolumn{4}{c}{B22} \\ \hline
Fake Data Study & $B_{\Delta m_{32}^2}^\textrm{syst.}$ & $R_{\Delta m_{32}^2}^{2\sigma}$ & $B_{sin^2 \theta_{32}}^\textrm{syst.}$ & $R_{sin^2 \theta_{32}}^{2\sigma}$ & $B_{\Delta m_{32}^2}^\textrm{syst.}$ & $R_{\Delta m_{32}^2}^{2\sigma}$ & $B_{sin^2 \theta_{32}}^\textrm{syst.}$ & $R_{sin^2 \theta_{32}}^{2\sigma}$ \\ \hline \hline

Z-exp Lower & -6\% & 1.00 & 2\% & 1.0 & -7\% & 1.00 & --- & 1.00  \\

Z-exp CV & --- & 1.00 & --- & 1.0 & -0.803\% & 0.996 & 0.367\% & 0.999 \\

Z-exp Upper & -20\% & 1.0 & --- & 1.00 & -20\% & 1.0 & -2\% & 1.00 \\ \hline

3Comp Lower & 2\% & 1.0 & --- & 1.00 & 3\% & 1.0 & -2\% & 1.0 \\

3Comp CV & -4\% & 1.00 & 2\% & 1.00 & -1\% & 1.00 & --- & 1.00  \\

3Comp Upper & -6\% & 1.01 & 8\% & 1.01 & -4\% & 1.01 & 3\% & 1.02 \\ \hline

LFG & -44\% & 1.00 & --- & 0.98 & -46\% & 1.00 & -1\% & 1.0 \\

CRPA & 90\% & 0.93 & -21\% & 1.02 & 94\% & 1.0 & -22\% & 0.98 \\

Removal Energy & -1\% & 1.0 & -1\% & 1.0 & --- & 1.00 & --- & 1.0 \\

Removal Energy cubic interpolation & -17\% & 1.01 & 6\% & 1.02 & -16.6\% & 1.01 & 2\% & 1.03 \\ 

Removal Energy linear interpolation & -5\% & 1.01 & 4\% & 1.02 &  -0.1\% & 1.01 & 3\% & 1.02 \\ \hline

$1\pi$ Low $Q^{2}$ & 20\% & 0.99 & 17\% & 1.02 & 22\% & 1.0 & 10\% & 1.04 \\

$1\pi$ Kin. $-3\sigma$ & 19\% & 1.00 & -3\% & 1.00 & 19\% & 1.00 & -3\% & 1.0 \\

$1\pi$ Kin. $+3\sigma$ & -8\% & 1.0 & 2\% & 1.01 & -5\% & 1.0 & 3\% & 1.01 \\

Martini $1\pi$ & -18\% & 1.0 & -3\% & 1.0 & -16\% & 1.0 & -2\% & 0.99 \\ \hline

Radiative Corrections. & 17\% & 0.98 & -7\% & 0.98 & 15\% & 1.0 & -5\% & 0.97 \\ \hline

Data-driven non-QE & -76\% & 0.99 & 7\% & 1.02 & -71\% & 0.99 & 2\% & 1.03  \\

Data-driven $1\pi$ & -7\% & 1.01 & -2\% & 1.00 & -9\% & 1.01 & -3\% & 1.0 \\ 

Pion SI & 52\% & --- & -10\% & 0.99 &  49\% & 0.99 & -10\% & 0.98 \\

\hline\hline
\end{tabular}}
\caption{Summary of all biases computed for $\Delta m_{32}^2$ and $\sin^2 \theta_{32}$ from the scaled Asimov  FDS fits for both Asimov sets. Values in this table are truncated and those that are negligible are removed for ease of reading.}
\label{tab:SummaryAllScaled}
%It was decided to keep the same value for the statistical update and not redo all studies since changes to the analysis are small.
\end{table}
\subsection{Additional checks for the $1$Re-$1$d.e. sample}
%\todo{add hybrid study from Lucile}
Since the last oscillation analysis, there has been extensive work in other working groups performing joint-fits with other experiments i.e. the T2K+SK and T2K+NOvA groups.
In particular, T2K+SK has observed potential tensions with the T2K-ND prediction and atmospheric samples with one or multiple decay electrons in the low lepton momentum bins.
To reduce bias caused by the data-MC disagreement in these regions, additional systematics were added to the T2K+SK cross-section model.
Details of this are reported in T2K+SK technical note TN456.
It was not recommended that the T2K-only oscillation analysis also add these systematics, but it was thought to be sensible to check how sensitive the results of the analysis would be to a similar effect.
To assess this, two studies were performed; a fake data study and a hybrid study.

%\todo{introduce why we are doing it here, it is not a normal FDS rather a posteriori, not model changing}
%\todo{add intro on FDS and put it at the end of this section}
\subsubsection{A new Fake Data Study for the 1Re - 1d.e. sample \label{sec:FDS}}

%An excess of events in data, of more than 100\% can be observed in the neutrino low momentum region ($<200$~MeV) of the 1Re-1d.e. sample. 
%This has first been noticed in the context of the T2K-SK combined fit with atmospheric data.
%In that context it was studied in details and changes in the models have been introduced to address that excess.
%However, these changes have not been applied to the standard T2K analysis.
%It is expected that the impact will be negligible as this is not a region of high statistics and impact on the T2K oscillation analysis. As a result, a complementary fake data study (FDS) was performed to check the impact on this analysis.
To study the impact of an excess of events at low lepton momentum in the analysis, fake data inputs were made where the only modification is an increase in the MC prediction in the $1$Re-$1$d.e. sample below $200$~MeV i.e. in the single, lowest bin of lepton momentum.
An increase of $100\%$ was chosen to study this impact which is roughly the scale of the difference between the MC prediction and data in the SK atmospheric samples whilst also being of the order of difference seen between the data and the MC in the $1$Re-$1$d.e. sample in this analysis.
The post-ND fit MC prediction at Asimov A22 (red histogram) and the fake data inputs (histogram with error bars) for the $1$Re-$1$d.e. sample can be seen in \cref{fig:Mom1Re-1d.e.}. 
The produced Asimov sets were fitted as real data to the nominal model following our standard FDS procedure described in T2K-TN-441~\cite{TN441}.
The biases on oscillation parameters are reported in \cref{tab:SummaryAllScaled}.
%\cref{tab:SummaryAllScaled}.
%
%The relevant biases for the criteria established (T2K-TN-441~\cite{TN441} and T2K-TN-444~\cite{TN444}) to take into account a fake data study are written {\textcolor{blue}{in blue (not anymore?).}}
%
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.47\textwidth,keepaspectratio]{FDS_figs/Data_data23over_A22_RC_wSyst_nue1RD_x.pdf}
%
\includegraphics[width=0.47\textwidth,keepaspectratio]{FDS_figs/Data_data23over_RweightedA22_RC_wSyst_nue1RD_x.pdf}
\end{center}
\caption{Reconstructed momentum distribution of the 1Re-1d.e. sample data (blue) and MC-events overlaid (red) for the nominal MC (left) and the reweighted MC for the fake data study (right).}
\label{fig:Mom1Re-1d.e.}
\end{figure}
%
%To perform this study, the MC events with reconstructed momentum smaller than 200 MeV have been reweighted by a factor 2 to produce Asimov A22 and B22 sets of Asimov data. A factor 2 was used since it allows to obtain compatibility between reweighted MC and data within statistical errors (on both MC and data) without tuning too much the study to the observed data in the SK atmospheric samples.
%The reconstructed momentum distribution of the reweighted MC, together with the data is shown in the bottom plot of figure {fig:Mom1Re-1d.e.}.
%\begin{table}[!h]
%\setlength\LTleft{-1.5cm}
%\begin{center}
%    \caption{Table of the biases on $\sin^2\theta_{23}$, $\Delta m^2_{32}$, and $\delta_{CP}$ for the low momentum excess FDS for both Asimovs sets with respect to the Nominal. For Asimov B22, results at the lower and upper octant minima are shown.}
%    \label{tab:LowMomXcessbiases}
%    \includegraphics[width=15cm,keepaspectratio]{FDS_figs/CI_bias_LowMomXcess_wrt_Nominal.pdf}
%    \end{center}
%\end{table}
%\todo{leave this table in the main TN and just make a reference/summary}

The impact of this fake data study is somewhat negligible on the disappearance parameters and in particular, no additional smearing on $\Delta m^2$ is needed as it does not change the already computed value of $3\times10^{-5}$ at this level of precision.
However, the impact on the $\delta_{CP}$ data fit conclusion has to be assessed as well.
To check this, we want to understand how much our constraint would be weakened if we take into account the change in our sensitivity in the fake data fit compared to our real data fit.

We first define the $\Delta\chi^2$ difference in the FDS as:
\begin{equation*}
    \Delta\chi^2_{diff}(\delta_{CP}) = \Delta\chi^2_{nom}(\delta_{CP}) - \Delta\chi^2_{FDS}(\delta_{CP}).
\end{equation*}
Here $\Delta\chi^2_{nom}(\delta_{CP})$ and $\Delta\chi^2_{FDS}(\delta_{CP})$ are the $\Delta\chi^2$ curves in the nominal and fake data fits respectively.
Using this function, we make a shifted $\Delta\chi^2$ curve for the data:
\begin{equation*}
    \Delta\chi^2_{shift}(\delta_{CP}) = \Delta\chi^2_{data}(\delta_{CP}) + \Delta\chi^2_{diff}(\delta_{CP}).
\end{equation*}
Here $\Delta\chi^2_{data}(\delta_{cp})$ is the $\Delta\chi^2$ curve from the fit to the data. The confidence intervals are then calculated with $\Delta\chi^2_{shift}(\delta_{cp})$ and the intervals are compared to those from data. We use the confidence intervals taken from the Feldman-Cousins critical $\Delta\chi^2$ values. The difference in the $\Delta\chi^{2}$ between the real data and the FDS as well as the resulting change in the $\Delta\chi^{2}$ can be seen in \cref{fig:FDSdCPopposite} in the left and right plots respectively. The 90\% exclusion of CP symmetry does not fully stand anymore as the 90\% confidence interval includes the $-\pi$ value: [-3.156, -0.202]. 

As a conclusion, taking into account this known data excess in the low momentum bin of the 1Re-1d.e. sample, and without any further information on its cause, we can not claim the exclusion of CP conservation at 90\%. A further study without the 1Re-1d.e. sample was conducted in P-Theta (T2K-TN-461~\cite{TN461}) and showed similar conclusions.
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.45\textwidth]{FDS_figs/cont_diff_oppositecomputation.pdf}
    \includegraphics[width=0.45\textwidth]{FDS_figs/contour_dCP_oppositecomputation.pdf}
    \caption{Computed $\Delta \chi^2$ from the fake data study (left) and comparison of the likelihood curves (right) for the data fit (blue) and the data fit corrected (orange).}
    \label{fig:FDSdCPopposite}
\end{figure}

%\FloatBarrier
\subsubsection{``Hybrid'' study for the 1Re-1d.e. sample}
An alternative way of visualizing the impact of the low-momentum excess in the 1Re-1d.e. sample is to perform the data fit with all samples except the 1Re-1d.e. sample, which is replaced by the MC prediction at the data best fit. In that way, the low momentum excess is constrained to be only understood within the fitter underlying model. Note that this is an alternative way to show the impact of this low excess on oscillation contours compared to the FDS shown in \cref{fig:FDSdCPopposite}. It allows to preserve the data statistical power in every samples except the 1R1decay-e, and show the direct impact of the data difference with the post-fit model in the sole 1R1decay-e sample. Thus, it encompass potential statistical fluctuations, as well as potential difference in the systematic or oscillation model in this particular sample. An important difference though is that the FDS is performed using the MC-nominal (Asimov) prediction for the 1Re-1d.e. sample (\textit{i.e.} the prior), while the following hybrid data fit uses instead the MC-prediction at best fit (\textit{i.e.} the posterior). The impact of the hybrid study compared to the FDS described above is shown in \cref{fig:LowMomXcessHybridFDS1D}. \textcolor{blue}{The $\Delta \chi^2$ in the hybrid study goes in the same direction as the FDS (blue vs black line).

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{FDS_figs/HybridvsFDS.pdf}
    \caption{1D likelihood surfaces for $\delta_{CP}$ with the reactor constraint on $\sin \theta_{13}$ both normal ordering for the hybrid data set (blue), the nominal data set (orange) and data fit corrected by the FDS effect (black).}
    \label{fig:LowMomXcessHybridFDS1D}
\end{figure}

==> Forewords.tex <==
\section*{Foreword}
\label{sec:fwds}

This is the first Physics Analysis Summary (PAS) written as part of the Oscillation Analysis.
The introduction of PASs is intended to provide the T2K member with a condensed but thorough overview of the physics content of a new analysis.
The goal is to ease the review process and allow it to be more accessible and effective without requiring the ``fine details'' of the analysis.
Therefore, the description and presentation of changes to the analysis is done in a more general way and then reference to the usual Technical Notes (TN) for a deeper level of documentation.
Profiting from the feedback from the collaboration we hope to gradually fine-tune this document to get closer to these intentions. More on the goals of PAS notes can be found in~\cite{PAS}.

==> Introduction.tex <==
\section{Introduction}
\label{sec:intro}
% 

This PAS summarizes the physics content of the 2023 Oscillation Analysis (OA2023). The TNs that accompany this analysis release are shown in \cref{tab:TNs}. Some of the TNs related to this analysis are the same as for the previous analysis (OA2022) as the inputs or methodology used are unchanged.

\textcolor{blue}{The T2K oscillation analysis uses three distinct and complementary fitters named BANFF, P-Theta, and MaCh3. %666 Over the last few years, a new fitting framework called GUNDAM, an acronym of \textit{Generalized and Unified Neutrino Data Analysis Methods}, has been developed. It is used for the ND data analysis and its performances and validation are described in detail in T2K-TN-458~\cite{TN458}. GUNDAM was included in this analysis to have at least one analysis in which both fitters are run in parallel before OA2024 where only GUNDAM will be used.}

The P-Theta fitter uses the ND-postfit central values and covariance matrix to fit the SK samples and produces both frequentist and Bayesian results. MaCh3 can perform ND fits and simultaneous fits of the ND and SK data samples using Markov Chain Monte Carlo and produces a Bayesian result. The basic differences between the MaCh3 and P-Theta fitters are described in \cref{tab:fitterdiff}. \textcolor{green}{Though these different approaches, the fitter are carefully validated and tested against each other it order to make sure they produce only minor differences between their results, and that the source of these differences are fully understood and quantified.} The different approaches and methods of the fitters allow for the effects of the near-detector fit binning, non-gaussianities, or far-detector binning on the sensitivity and data results to be diagnosed and cross-checked. 
Generally, the P-Theta and MaCh3 results agree very well and any differences are understood.
A selection of the results from BANFF,
%666/GUNDAM
MaCh3, and P-Theta are shown in this note to highlight the main changes to this analysis with respect to the previous one.
The full results of all the fitters can be found in their respective TNs.

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
\hline
\hline
    TN OA2022  & TN OA2023  & Topic  \\
\hline
    414~\cite{TN414}     & Same & NIWG \\ 
\hline
    429~\cite{TN429}     & 462~\cite{TN462} & MaCh3 \\ 
\hline
    430~\cite{TN430}     & 461~\cite{TN461} & P-Theta \\ 
\hline
    423~\cite{TN423}     & 474~\cite{TN474} & ND280 \\ 
\hline
    441~\cite{TN441}     & Same & Fake Data Studies \\ 
\hline
    399~\cite{TN399}     & 465 & Super-K selection and Data Quality \\ 
\hline
    448~\cite{TN448}     & 469~\cite{TN469} & Super-K detector syst. \\
\hline
    \textcolor{orange}{401~\cite{TN401}}     & \textcolor{orange}{Same} & \textcolor{orange}{Flux syst.} \\
\hline
\hline
    \end{tabular}
    \caption{Summary of TNs associated to the previous and this OA analysis.}
    \label{tab:TNs}
\end{table}

The significant changes to this analysis with respect to OA2022 are the following:
\begin{itemize}
\item an increase in sample statistics at the Far Detector (FD) with the addition of Run 11 data ($\simeq +9$\% increase of the previous Forward Horn Current sample). This is the first data set with Gd-loading, at the 0.01\% level. A summary of the POT used in the far detector analysis is available in Tab.~1 of TN465~\cite{TN465}. The evolution of collected POT is shown in Fig.~\ref{fig:pot} (from TN465 Fig.~1.);
\item an update in the FD selection for Michel decay-electrons motivated by the interplay with an increased number of delayed signals from neutron captures in the new 0.01\% Gd SK phase~\cite{TN465};
\item the introduction of a new detector covariance matrix for FD, including correlations between the $\nu_{\mu}$CC$1\pi^+$-like sample and the single ring samples for the first time, as well as a better treatment of all systematic uncertainties.
The largest net effect is a significant reduction of the e-like sample errors;
\item the introduction of a new Fake Data Study (FDS).
This study tests the robustness of the results concerning the data ``excess'' seen in the FD sample with an $e$-like ring accompanied by a Michel decay-electron (``1Re-1d.e.'') at energies below $\sim~200$~MeV. This FDS is presented briefly in Sec.~\ref{sec:FDS} and described thoroughly in~\cite{TN461};
\item \textcolor{orange}{small changes to the flux inputs due to the inclusion of Run 11 flux at the FD. The method for evaluating the flux parameters and the flux covariance matrix has remained unchanged from what was used for OA2022, and has been extensively described in~\cite{TN401}. As is customary when a new run is included, the addition of Run 11 FD flux means that the flux covariance matrix was updated. The proton beam profile, horn alignment, horn current and off-axis angle components of the covariance matrix have changed, taking into account the relative Run 11 POT and also keeping track of which of these systematic effects are correlated among which groups of FD runs based on the underlying changes to beamline configuration, as described in~\cite{TN401}.}
\end{itemize}

\begin{table}[htbp]
	\centering
	\begin{tabular}{ l c c | c | c c }
    \hline
    \hline
		Run     &  Run    & Run  & Beam      & \multicolumn{2}{c}{POT $(\times10^{19})$} \\
		number   &  start  & end  & mode & ND & FD \\
		\hline
		1 & Jan. 2010 & Jun. 2010 & $\nu$ & ---     & 3.26 \\
		2 & Nov. 2010 & Mar. 2011 & $\nu$ & 7.93    & 11.22 \\
		3 & Mar. 2012 & Jun. 2012 & $\nu$ & 15.81   & 15.99 \\
		4 & Oct. 2012 & May 2013  & $\nu$ & 34.26   & 35.97 \\
		5 & May 2014  & Jun. 2014 & $\overline{\nu}$ & 4.35    & 5.12 \\
		  &           &           & $\nu$ & ---     & 2.44 \\
		6 & Oct. 2014 & Jun. 2015 & $\overline{\nu}$ & 34.09   & 35.46 \\
		  &           &           & $\nu$ & ---     & 1.92 \\
		7 & Feb. 2016 & May 2016  & $\overline{\nu}$ & 24.38   & 34.98 \\
		  &           &           & $\nu$ & ---     & 4.84 \\
		8 & Oct. 2016 & Apr. 2017 & $\nu$ & 57.31   & 71.69 \\
		9 & Oct. 2017 & May 2018  & $\overline{\nu}$ & 20.54   & 87.88 \\
		  &           &           & $\nu$ & ---     & 2.04 \\
		10& Oct. 2019 & Feb. 2020 & $\nu$& ---     & 47.26 \\
        11& Mar. 2021 & Apr. 2021 & $\nu$& ---     & 17.6 \\
		\hline
		\multicolumn{3}{c|}{Total} & $\nu$ & 115.31 & 214.23 \\
		\multicolumn{3}{c|}{Total} & $\overline{\nu}$ & 83.36  & 163.44 \\
		\hline
		\multicolumn{3}{c|}{Total} & $\nu+\overline{\nu}$ & 198.67 & 377.67 \\
	\hline
	\hline
	\end{tabular}
	\caption{Collected protons-on-target (POT) for each T2K run included in the analysis of T2K data at the ND and FD.}
	\label{tab:pot_2020}
\end{table}



%
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{intro_figs/POT_run11.png}
    \caption{POT used for the FD analysis (TM465 Fig.1).}
    \label{fig:pot}
\end{figure}
It should be noted that the samples considered for the Near Detector (ND) constrain have not been updated with respect to OA2022 (22 samples in total, see Tab. I in~\cite{TN423}) apart from a minor update of the predictions solely due to the changed flux prediction (see \cref{sec:nd}).

The major factors at play in the modification of our performances with OA2023 are the increase in the data statistics used, the modification of uncertainties at the FD, and the inclusion of a new FDS. The effects of each of these factors are illustrated in \cref{fig:A22novelties} which shows the sensitivity to $\delta_{CP}$ (left) and $\Delta m^{2}_{32}$ vs. $\sin^{2}\theta_{23}$ (right) at the A22 Asimov point (defined in Tab.~\ref{tbl:osc_param}) using the P-Theta analysis.
One observes how the previous analysis sensitivity (violet) is improved by using the new SK-detector uncertainties (blue).
This is then improved further by using the new data (orange).
The change in sensitivity due to the increase in data statistics can be seen to be similar to the improvement in sensitivity due to the new SK-detector uncertainties by using the old SK detector uncertainties with the new statistics (green).
The total increase in $\Delta \chi^2$ around $\pi/2$ is a bit less than 2 units (roughly from 13 to 15).

\begin{table}[htb]
  \centering
  \caption{Reference values of the neutrino oscillation parameters for various oscillation parameter sets 
    and earth matter density. The columns are changed compared to the previous oscillation sets A, B in TN397.}
  \label{tbl:osc_param}
\begin{tabular}{l | c | c  }
\hline
\hline
Parameters & {\color{red}A22} & {\color{red} B22}  \\
\hline
\hline
\Dmtwoone & \multicolumn{2}{c}{$7.53 \times 10^{-5} \,\mathrm{eV^2}$} \\
\Dmthreetwo (NH) / \absDmthreeone (IH) & \multicolumn{2}{c}{$ {\color{red} 2.494} \times 10^{-3} \,\mathrm{eV^2}$} \\
\hline
\stwothree & {\color{red} 0.561} & 0.45  \\
\hline
\sonetwo (\stonetwo) & \multicolumn{2}{c}{0.307 (0.851)} \\
\sonethree (\stonethree) & \multicolumn{2}{c}{ {\color{red} 0.0220 (0.0861)} } \\
\hline
\dcp & $-1.601$ & 0  \\
\hline
Earth matter density & \multicolumn{2}{c}{$2.6 \, \mathrm{g/cm^3}$} \\
Baseline length & \multicolumn{2}{c}{$295 \, \mathrm{km}$} \\
\hline
Mass hierarchy & \multicolumn{2}{c|}{Normal}  \\
\hline
\hline
\end{tabular}
\end{table}

%The net results of the OA2023 can be roughly summarized as an overall increase in the sensitivity to $\delta_{CP}$ by xx units of $\Delta \chi^2$... a reduction of the error on ... \todo{summarise the main changes concisely}

The changes introduced by the new release of the OA analysis can also be appreciated in the summary plot of \cref{fig:summary} which shows the variations of central values and $1\sigma$ intervals for P-Theta and MaCh3 for the OA2022 and OA2023 analyses.
\begin{figure}[h]
\begin{center}
\includegraphics[width=1.1\textwidth,keepaspectratio]{intro_figs/ptheta_OA22-23_v3.pdf}
\end{center}
\caption{A comparison of OA2023 and OA2022 with the previous results for $\sin^2\theta_{13}$ (top left), $\delta_{CP}$ (top right),
the atmospheric SK $\Delta m^2$ (bottom left) and $\sin^2\theta_{23}$ (bottom right). Results are shown with and without the reactor constraint (RC). %\textcolor{blue}{TODO: cross check numbers, for MaCh3 there should be more digits.}
}
\label{fig:summary}
\end{figure}

\begin{table}[htb]
\centering
\begin{tabular}{ c | c | c | c | c | c }
\hline \hline
& Fitted & ND & FD & Marginalisation & oscillation \\
& samples & binning & binning & method & probability weights \\
\hline
P-Theta & SK 6 samples & \textcolor{blue}{rectilinear} & $p_{e}$ \& $\theta_{e}$ (e) & MC sampling & bin-by-bin \\
 &  &  & $p_{\mu}$ \& $E_{\nu}$ ($\mu$) & & \\
 \hline
MaCh3 & SK 6 samples & \textcolor{blue}{non rectilinear} & $E_{\nu}$ \& $\theta_{e}$ (e) & MCMC & event by event\\
 &  \& ND samples &  & $E_{\nu}$ ($\mu$) & & \\
\hline\hline
\end{tabular}
\caption{Summary of the basic features of the P-Theta and MaCh3 fitters.}
\label{tab:fitterdiff}
\end{table}

\subsection{Overview of the contents}
%
\cref{sec:nd} describes the residual updates concerning the ND, while the more substantial changes related to the FD are detailed in \cref{sec:sk}.%, with changes in the selection of decay electrons in \cref{sec:sksel} and changes in the FD detector covariance matrix in \cref{sec:skmat}.
%
The results on oscillation parameters obtained with the MaCh3 and P-Theta fitters are given in \cref{sec:OscResults} as follows:
\begin{itemize}

\item Sensitivity (Asimov fits) fit results are shown in \cref{sec:asimovfits}. We also show the impact of the different factors from last year's analysis (sample statistics, SK errors, selection, etc.) on the atmospheric and $\delta_{CP}$ parameters (\cref{fig:A22novelties}).
%
\item Data fit results with real data are shown in \cref{sec:datafits}, with and without reactor constraint (RC) for $\delta_{CP}$, $\Delta m^2_{32}$ vs $\sin^2\theta_{23}$. We also compare the results of P-Theta with the ND detector post-fit covariance matrix from the MaCh3 ND fit instead of the BANFF one. The reevaluation of Feldman-Cousins (FC) critical values for $\delta_{CP}$ and $\sin^2\theta_{23}$ for P-Theta is also reported in \cref{tab:FC_CI_all}. The goodness-of-fit for the analysis is also reported briefly here and compared to OA2022.
%
\item The final best-fit points and confidence regions on oscillation parameters are given for P-Theta in \cref{tab:Bestfit_PTheta} (with and without RC) and in \cref{table:MaCh3CI} for the MaCh3 analysis (credible intervals with and without RC).
%
\item Summary of the effects of FDSs already considered in OA2022 and of the additional FDS related to the 1Re-1d.e. discrepancy at low energy (\cref{sec:FDS}). Here we also discuss some updates that were necessary after the discovery of a bug in the sign of the $\Delta \chi^2$ correction to be applied to the data that was discovered in Nov. 2023 and the related changes in the conclusions. %\todo{should this be discussed here or should the FDS TN go back to review again? I think it might be quite messy to include it here.}

\end{itemize}

==> ND280.tex <==
\section{Changes in the ND constraint}
\label{sec:nd}

The samples on which the ND constraint is calculated and the methodology is the same as for OA2022. The only changes come from the beam prediction that has been re-tuned using Run 11 data. They are taken into account by employing a new flux release (tuned21bv2) which includes the overall flux uncertainty also incorporating the contribution coming from the Run 11 protons on target (PoT).

%\subsection{Modifications related to the Run 11 flux update}
% Andrea: commented title of subsection following the suggestion oj J Lagoda

%\subsubsection*{Impact of new flux weights on systematics compared to OA2022}
Due to the COVID-19 pandemic, ND280 was not operated during run 11 data taking, so no new data is included in the near detector analysis. However, the inclusion of Run 11 data impacts the flux predictions at near and far detectors, which could be constrained by adding beamline data for that run period. For a detailed discussion of the flux release see T2K-TN-354 which describes the 21bv2 flux release~\cite{TN354}. Therefore, at the ND level, the near detector analysis described in T2K-TN-423~\cite{TN423} has been re-ran using the Run 1-11 flux covariance, and the results are described in T2K-TN-474~\cite{TN474}. As expected, the impact due to the new flux constraint is negligible.

%666 \subsection{A new ND fitter: GUNDAM}
%\label{sec:GUNDAM_NDsec}

%Over the last few years, a new fitting framework called GUNDAM has been implemented and is described in detail in T2K-TN-458~\cite{TN458}. We show some comparisons between the performances of the new GUNDAM fitter to MaCh3 and BANFF for the OA2022 ND analysis. All validation and results are compatible among the three fitters. The central result of the analysis of P-Theta (that needs an external ND constraint as an input) uses the BANFF results. A comparison has also been made with results obtained using the GUNDAM output showing very good agreement in terms of compatibility in the confidence regions for oscillation parameters.

%\textcolor{blue}{It has been employed at the ND for this analysis and cross-checked against the results of the other fitters BANFF and MaCh3. Overall a good agreement is found among these fitters and it is reported in \cref{sec:GUNDAM}.} 

%Not in last PAS, to keep commented even adding back: GUNDAM The output of GUNDAM has been employed in this analysis only to show the compatibility with the official fitters and is shown in \cref{sec:GUNDAM}.}

%\clearpage   

==> OscillationAnalysisResults.tex <==
\section{Oscillation Analysis Results}
\label{sec:OscResults}
%\FloatBarrier
The following section of the PAS highlights the main results on oscillation parameters from the MaCh3 and P-Theta fitters.
The section begins with the sensitivity of the analysis at the Asimov A22 values of the oscillation parameters. These are the values close to the past T2K best fit: $\sin^2\theta_{12}=0.307$, $\sin^2\theta_{23}=0.561$, $\sin^2\theta_{13}=0.0220$, $\Delta m^2_{12} = 7.53\times10^{-5}$~eV$^2$, $\Delta m^2_{32}=2.494\times 10^{-3}$~eV$^2$, $\delta_{CP}=-1.601$.
These sensitivities have a dual purpose in the fact that they aid in understanding what the expected change in the data fit results might be compared to the previous analysis and also to validate the fitters against each other.
The highlights of the data-fit results are then shown after the Asimov fits.
The full results and a detailed description of the cross-fitter validations can be found in \cite{TN461} and \cite{TN462}.
 
\subsection{Asimov fits for Run 1-11}
\label{sec:asimovfits}

% stolen from TN430
Rather than averaging over the results of many toy data sets throwing the systematic parameters, the sensitivities presented
are derived from a fit to a single data set generated with all of the systematic parameters at
their central values. This is referred to as the ``Asimov'' data set, a single data set representative
of the distribution of possible data sets. Within the fit itself, the systematic parameters are
marginalized. The sensitivity calculated in this way is therefore the ``Asimov Sensitivity''. This
method saves a great deal of computation time.

The agreement in the number of events predicted by the fitters (MaCh3 and P-Theta) at the FD is carefully checked at Asimov A22 oscillation parameters values. Once the fitters agree, as verified, then fits to these predictions are performed and the output of the fitters in terms of oscillation parameters are compared. 

The results of this comparison can be seen in \cref{fig:A22dCP} for $\delta_{CP}$ and in \cref{fig:A22_2D} for the $\Delta m^{2}_{32}/\sin^2\theta_{23}$ plane.
It should be noted that for this 1D comparison, the output posterior probability from MaCh3 has been converted into a $\Delta\chi^{2}$ surface. At large values of $\Delta\chi^{2}$ there are not enough MCMC steps for this to be done. At lower values (below 12 units of $\Delta\chi^{2}$) excellent agreement between the fitters can be seen.

The conclusion of this comparison is that known differences between fitters related to the methods are visible, but an overall satisfying agreement is found.
\textcolor{blue}{The differences in Asimov sensitivities between p-theta and MaCh3 were studied in TN-429 \cite{TN429}, and were found to be driven by the sample binning at SK and the ND constraint. We have not repeated this study for the Asimov fits for this analysis but the same checks were performed on the data fit results in this analysis (see figures \crefrange{fig:datadCP}{fig:data_2DwoRC}).}
\begin{figure}[h]
\begin{center}
%\includegraphics[width=7.5cm,keepaspectratio]{Asimov_figs/1DContours_AsimovFit_NH_wRC.pdf}
%\includegraphics[width=7.5cm,keepaspectratio]{Asimov_figs/1DContours_AsimovFit_IH_wRC.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Asimov_figs/asimov_comp_dcp_wRC_NO.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Asimov_figs/asimov_comp_dcp_wRC_IO.pdf}
\end{center}
\caption{1D $\chi^2$ curves for $\delta_{CP}$ with A22 Asimov set sensitivities for both fitters with the reactor constraint applied, for normal (left) and inverted (right) orderings.}% The spiked features in the MaCh3 curve is due to few MCMC steps in this unlikely region of $\delta_{CP}$. %\textcolor{blue}{A.L. screenshot from TN 462 v1.0.0.}
}
\label{fig:A22dCP}
\end{figure}
%\todo{Henry will update this.}

\begin{figure}[h]
\begin{center}
\includegraphics[width=7.5cm,keepaspectratio]{Asimov_figs/th23dm32_NH_wRC.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Asimov_figs/PThetaMaCh3Comp_dm2_th23_IH_wRC.pdf}
\end{center}
\caption{2D contours of $\sin^2\theta_{23}$ vs. $\Delta m^{2}_{32}$ with A22 Asimov set sensitivities for both fitters, for normal (left) and inverted (right) orderings. \textcolor{blue}{The agreement is seen to be at a similar level to the previous analysis.}}
\label{fig:A22_2D}
\end{figure}
%\FloatBarrier

As previously mentioned, Asimov fits are also used to compare the expected sensitivity of an analysis to previous ones.
To evaluate the impact of the changes in this analysis compared to the previous analysis, sensitivity studies using the A22 set were conducted for various scenarios with the P-Theta fitter.
In \cref{fig:A22novelties}, the purple curve is the previous analysis' sensitivity (OA21), the orange curve is this OA2023 sensitivity, the green curve is OA2023 sensitivity with the previous SK detector error matrix, and the blue curve is this OA2023 sensitivity without the Run 11 POT.
It can be concluded that the sensitivity has been improved slightly and that the addition of the Run 11 POT is comparable to the improvement seen due to the reduced error from the SK detector matrix.
The best-fit value for $\Delta m^{2}_{32}$ is slightly shifted towards higher values, most probably through correlations with $\sin^2\theta_{23}$.
The sensitivity of the analysis to the octant of $\sin^2\theta_{23}$ is visibly improved and the best fit is also shifted slightly towards higher values with the new analysis.
The $\delta_{CP}$ sensitivity, is improved by a bit more than 1 unit of $\chi^2$, in particular the ability to reject the wrong sign of the phase.
For all parameters, the improvement in sensitivity comes more or less equally from the addition of the new data and the new error SK detector matrix.
Further studies, described in TN461, show that it is the reduced error on the 1Re-1d.e. sample in the new matrix that has a significant impact more than the additional correlations.
\begin{figure}[h]
\begin{center}
%\includegraphics[width=7.5cm,keepaspectratio]{Pthetasensi_figs/contour_dCP.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Pthetasensi_figs/contour_dCP_inkscape_fix_Legend.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Pthetasensi_figs/contour_dm2_32_th23-3.pdf}
\end{center}
\caption{Sensitivity plots at A22 using p-theta, with reactor constraints and with systematic parameters, adding the Statistical update specific items one by one. The purple curve is the OA21 sensitivity, the orange curve is the OA2023 sensitivity, the green curve is the OA2023 sensitivity with the previous SK detector error matrix, and the blue curve is this OA2023 sensitivity without the Run 11 POT.}
\label{fig:A22novelties}
\end{figure}
%\todo{start with the above fig? move the Legend?}
%\todo{start with the above fig?} % Legend fixed with inkscape (Andrea)
\FloatBarrier
\subsection{Data fits for Run 1-11}
\label{sec:datafits}
The statistics of the collected samples in the data
for Run 1-11 that passed all the selection cuts~\cite{TN399}, \cite{TN465} are given in \cref{tab:eventsamples}. The samples corresponding to OA2022 are also shown for reference. The best fit of P-Theta with post fit errors (TN461) is given in the last line.

\begin{table}[h]
    \centering
{{\small
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    \hline
&\multicolumn{2}{|c|}{1R$\mu$} & \multicolumn{2}{|c|}{1Re}& 1R $\nu_e$CC1$\pi^+$ & MR $\nu_\mu$CC1$\pi^+$ &Total\\
\hline
         & FHC & RHC & FHC & RHC & FHC & FHC &\\ \hline
         OA22 & 318 $\pm$ 18 & 137 $\pm$ 12 & 94 $\pm$ 10 & 16 $\pm$ 4 & 14 $\pm$ 4 & 134 $\pm$ 12 & 713 $\pm$ 27 \\\hline
         OA23 & 357 $\pm$ 19 & 137 $\pm$ 12 & 102 $\pm$ 10 & 16 $\pm$ 4 & 15 $\pm$ 4 & 140 $\pm$ 12& 767 $\pm$ 28\\\hline
         OA23 P-$\theta$ b.f. & $419 \pm 13$ & $147 \pm 7$ & $112.1 \pm 5.5$ & $18.0 \pm 1.2$ & $9.9 \pm 0.6$ & $123 \pm 5$ & \\         
         \hline
         \hline
    \end{tabular}
    \caption{Data samples at the FD. The P-theta best fit prediction with ND post-fit systematic uncertainties shown in the last line is taken from Tab.~22 of TN461. The quoted uncertainties on the predictions are the total systematic while for data they are Poisson statistical errors.}
    \label{tab:eventsamples}
}}
\end{table}

These results are also summarized in a graphical form in Fig.~\ref{fig:dataset_pre}, where we show the number of events collected at SK for Run 1-11 split into the six samples and predictions for different $\delta_{CP}$ for the P-theta fitter. The error band on the prediction represents the pre-fit uncertainty.
\begin{figure}
    \centering
    \includegraphics[width=1.05\textwidth]{Datafits_figs/T2K_FDdataMC_1.pdf}
    \caption{Events collected at SK for Run 1-11 split into the six samples and predictions for different $\delta_{CP}$ for the P-theta fitter. The error band on the prediction represents the pre-fit (before ND fit) systematic uncertainty. Inputs are from Tab.~23 of TN461.}
    \label{fig:dataset_pre}
\end{figure}
Figure \ref{fig:dataset_post} shows the same information for the best fit prediction and ND post-fit errors.
\begin{figure}
    \centering
    \includegraphics[width=0.52\textwidth]{Datafits_figs/T2K_FDdataMC_0.pdf}%
        \includegraphics[width=0.52\textwidth]{Datafits_figs/T2K_FDdataMC_2.pdf}
    \caption{Events collected at SK for Run 1-11 split into the six samples. Left: the predictions of P-theta are superimposed for different values of $\delta_{CP}$ and the best fit one. Right: the best fit prediction is shown with a band showing the post-fit systematic uncertainty. Inputs are from Tab.~22 of TN461.}
    \label{fig:dataset_post}
\end{figure}

The fitted data distributions of the reconstructed neutrino energy at the FD are shown in \cref{fig:SKspectra} for the 1R$\mu$, 1R$e$ samples (in both FHC and RHC) and for the FHC 1R$e$1d.e. and FHC $\nu_\mu$ CC1$\pi$ samples with the MaCh3 posterior predictive distributions superimposed (from TN462, Fig.~18).

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{Datafits_figs/spectra_1.png}%
    \includegraphics[width=0.4\textwidth]{Datafits_figs/spectra_2.png}
    \includegraphics[width=0.4\textwidth]{Datafits_figs/spectra_3.png}%
    \includegraphics[width=0.4\textwidth]{Datafits_figs/spectra_4.png}
    \includegraphics[width=0.4\textwidth]{Datafits_figs/spectra_5.png}%
    \includegraphics[width=0.4\textwidth]{Datafits_figs/spectra_6.png}
    \caption{Event spectra at SK with Run 1-11.  Post-fit distribution (blue) and one sigma error band (red) with data (black) for each SK selection overlaid. Posterior predictive distributions are made using a Markov chain from a joint SK and ND fit where all parameters are sampled. The post-fit distribution is calculated by taking the mean from the posterior predictive distribution in each bin. Similarly, the one-sigma error band is calculated by taking the RMS of the posterior predictive distribution in each bin.}
    \label{fig:SKspectra}
\end{figure}
The distributions in momentum and angle of the leptons can be found in the P-Theta TN, \cite{TN461}, Fig.~12.
%This section contains a selection of results from fits to data from Runs 1-11.
%We have performed fits using a Gaussian prior as well as fits with a flat prior, so called ``with reactor constraint'' (wRC) and ``without reactor constraint'' (woRC) respectively.

The fits with the reactor constraint provide the greatest sensitivity owing to the decreased uncertainty on $\sin^{2}\theta_{13}$ compared to T2Ks constraint on the parameter.
In the Asimov fits, a Gaussian prior on $\sin^{2}\theta_{13}$ from the PDG was used. However, we also perform the data fit without the constraint to highlight the sensitivity of T2K data alone.

In \cref{sec:contours_dataRC} results from both MaCh3 and P-Theta are shown on $\delta_{CP}$ 
%in \cref{fig:datadCP} 
and in the $\delta_{CP}$ vs. $\sin^{2}\theta_{13}$ and $\Delta m^{2}_{32}$ vs. $\sin^{2}\theta_{23}$ planes 
%in \cref{fig:data_2D}. 
The equivalent results after releasing the external constraint on $\theta_{13}$ are given in \cref{sec:contours_dataNORC}.
%
The best-fit points, errors, and Feldman-Cousins corrected intervals from P-Theta are given in \cref{sec:bestfits_data}.



\subsubsection{Data fit results with reactor constraint}
\label{sec:contours_dataRC}

The comparison between fitters with reactor constraint can be seen in \cref{fig:datadCP,fig:data_2D_A,fig:data_2D_B} for $\delta_{CP}$, $\Delta m^2_{32}$ vs. $\sin^2\theta_{23}$ and $\delta_{CP}$ vs. $\sin^2\theta_{13}$, respectively.
\begin{figure}[h]
\begin{center}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/dcp_fixed_binning_no_wRC.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/dcp_fixed_binning_io_wRC.pdf}
\end{center}
\caption{1D $\chi^2$ curves for $\delta_{CP}$ data fit for both fitters, for normal (left) and inverted (right) orderings.}
\label{fig:datadCP}
\end{figure}
%\todo{"capping" at 20 for Mach3?} lack of sufficient MCMC steps statistics
\begin{figure}[h]
\begin{center}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/dm32_th23_comp_no_wRC.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/comp_disap_IO_wRC.pdf}
\end{center}
\caption{2D data fit contours in the $\sin^2\theta_{23}/\Delta m^2$ plane for both fitters, for normal (left) and inverted (right) orderings.}
\label{fig:data_2D_A}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/MaCh3PThetaComp_dcp_th13_datafit_NO_wRC.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/dcp_th13_comp_io_wRC.pdf}
\end{center}
\caption{2D data fit contours in the $\sin^2\theta_{13}/\delta_{CP}$ plane for both fitters, for normal (left) and inverted (right) orderings.}
\label{fig:data_2D_B}
\end{figure}
There is an overall satisfying agreement between fitters even though it is not perfect, especially in the inverted mass ordering. To study the differences, a third data fit is presented, called ``Mach3-like P-Theta'' in the Legend of the figures. It consists of using the P-Theta fitter with Near detector inputs from MaCh3 instead of BANFF and with MaCh3 binning at the SK level. As can be seen from the figures, in that case, the agreement with the standard MaCh3 analysis is much better. Therefore, the differences are understood and come mostly from the ND fit method (Bayesian MCMC for MaCh3, global gradient descent for BANFF), as well as sample binning at both ND and FD.

%\FloatBarrier
\subsubsection{Data fit results without reactor constraint}
\label{sec:contours_dataNORC}
The 1D likelihood curves obtained for $\delta_{CP}$ are shown in \cref{fig:datadCPwoRC}, and the 2D appearance contours in \cref{fig:datadCPth13woRC}.
These results highlight the role that the reactor constraint on $\sin^{2}\theta_{13}$ has as the sensitivity to $\delta_{CP}$ is very reduced: the $\chi^2$ difference between the most favored and most disfavored values in normal ordering is around 6 instead of 15.
The lower sensitivity of T2K to $\sin^2\theta_{13}$ can be seen as the obtained likelihood distribution is very wide in comparison with the standard analysis contours presented in the plots of \cref{fig:data_2D_B}.
There is an important correlation between $\sin^{2}\theta_{23}$ and $\sin^{2}\theta_{13}$ which is also clear and results in a different preference for the octant of $\sin^{2}\theta_{23}$ to when the reactor constraint is being applied. 
Here we see the lower octant of $\sin \theta_{23}$ is favored over the upper octant and the preference is very mild compared to the fit with reactor constraints as can be seen in the 2D contours in \cref{fig:data_2DwoRC}.
Those conclusions are similar to what has been observed in previous analyses.
%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/MaCh3_PTheta_NH_woRC_1DContours.pdf}
%\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/MaCh3_PTheta_IH_woRC_1DContours.pdf}
%\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/datafit_comp_dcp_woRC_NO.pdf}
%\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/datafit_comp_dcp_woRC_IO.pdf}
%\end{center}
%\caption{1D $\chi^2$ curves for $\delta_{CP}$ data fit for both fitters, for normal (left) and inverted (right) orderings, without reactor constraint.}
%\label{fig:datadCPwoRC}
%\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/MaCh3_PthetaComp_dcpth13_NH_woRC.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/MaCh3_PthetaComp_dcpth13_IH_woRC.pdf}
\end{center}
\caption{2D data fit contours in the $\sin^2\theta_{13}$/$\delta_{CP}$ plane for both fitters, for normal (left) and inverted (right) orderings, without reactor constraint.}
\label{fig:datadCPth13woRC}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/MaCh3_PthetaComp_dm2th23_NH_woRC.pdf}
\includegraphics[width=7.5cm,keepaspectratio]{Datafits_figs/MaCh3_PthetaComp_dm2th23_IH_woRC.pdf}
\end{center}
\caption{2D data fit contours in the $\sin^2\theta_{23}/\Delta m^2$ plane for both fitters, for normal (left) and inverted (right) orderings, without reactor constraint.}
\label{fig:data_2DwoRC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%
%\FloatBarrier
\subsubsection{Best fit points and errors}
\label{sec:bestfits_data}
The results on the constraint on oscillation parameters $\sin^2\theta_{13}$, $\delta_{CP}$, $\Delta m^2_{32}$ (NO)/$\Delta m^2_{31}$ (IO), $\sin^2\theta_{23}$ can also be presented, in a more quantitative way, as best fit values and $1\sigma$ errors. \cref{tab:Bestfit_PTheta} show these results from the P-Theta fitter for fits with and without reactor constraint. The best fit points are extracted, not from the standard P-Theta analysis, but with a dedicated global MINUIT fit.
The asymmetric errors are however computed from the $1\sigma$ confidence intervals from the standard analysis.
For $\mathrm{sin^2(\theta_{23})}$ with reactor constraint in normal ordering and for both ordering without reactor constraint the 90\% interval is used as the $1\sigma$ interval is split into two small intervals.
For the result using reactor constraint, intervals deduced from the Feldman-Cousins studies critical $\chi^2$ values are used for $\delta_{CP}$ and $\mathrm{sin^2(\theta_{23})}$.
A full description of how the Feldman-Cousins critical values are calculated is given in T2K-TN-461~\cite{TN461}. 
%Andrea (comment from Justyna)
\textcolor{blue}{The  
$\Delta\chi^2$ of the data fit for $\delta_{CP}$ and $\sin^2 \theta_{23}$ for both normal (blue) and inverted
(orange) orderings are shown respectively in the left and right plots of Fig.~\ref{fig:FCFinalplotdCP}. The Feldman-Cousin corrected confidence intervals are displayed in different textures. The intervals of the same figure are given in Tab.~\ref{tab:FC_CI_all}.}

%Brief description of Feldman Cousins corrected intervals
\begin{table}
    \centering
    \begin{tabular}{c|c|c|c|c}
        \hline
        \hline
    &NO w RC & IO w RC & NO w/o RC& IO w/o RC\\
     \hline
         $\mathrm{sin^2(\theta_{13})/10^{-3}}$ &$21.9^{+0.9}_{-0.5}$&$22.0^{+1.0}_{-0.4}$ 
         &$27.8^{+1.8}_{-6.9}$&$31.0^{+1.8}_{-7.4}$ \\
         \hline
         $\delta_{CP}$,  & $-2.08^{+1.33}_{-0.61}$ & $-1.41^{+0.64}_{-0.82}$ 
         & $-2.21^{+1.62}_{-0.75}$ & $-1.29^{+0.63}_{-0.99}$\\
         $\Delta m^2_{32}$ (NO)/$\Delta m^2_{31}$ (IO) &$2.521^{+0.037}_{-0.050}$
         &$-2.486^{+0.043}_{-0.044}$ 
&$2.521^{+0.039}_{-0.050}$ &$-2.489^{+0.042}_{-0.046}$\\       
         $\mathrm{sin^2(\theta_{23})}$  & $0.568^{+0.024}_{-0.125}$ & $0.567^{+0.021}_{-0.048}$ 
         &$0.458^{+0.130}_{-0.021}$ & $0.458^{+0.127}_{-0.021}$\\ 
         \hline
         -2 ln L & 649.06& 651.013 & 648.837& 649.655\\
         -2 $\Delta$ln L & 0. & 1.953 & 0. & 0.818\\
          \hline
          \hline
    \end{tabular}
    \caption{Best fit values for the OA2023 analysis with the P-Theta fitter, with reactor constraints, global best fit is in normal ordering. Units for mass splittings are
    $10^{-3}\mathrm{eV^2/c^4}$. For $\sin^2\theta_{23}$ with reactor constraint in normal ordering and for both ordering without reactor constraint the 90\% interval is used as the 1$\sigma$ interval is split into two small intervals.} 
    \label{tab:Bestfit_PTheta}
\end{table}

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.5\textwidth,keepaspectratio]{FCstudies_figs/contour_dCP_NoTag_wCI_all_errorBand.pdf}%
\includegraphics[width=0.5\textwidth,keepaspectratio]{FCstudies_figs/contour_th23_NoTag_wCI_all_errorBand.pdf}
\end{center}
\caption{$\Delta\chi{^2}$ of the data fit for $\delta_{CP}$ (left) and $\sin^2\theta_{23}$ (right) for both normal (blue) and inverted (orange) orderings. The Feldman-Cousin corrected confidence intervals are displayed in different textures. }
\label{fig:FCFinalplotdCP}
\end{figure}

\begin{table}
\begin{center}
\begin{tabular}{c|c|c}
\hline
\hline
%~&\multicolumn{2}{|cc|}{$\sin^2\theta_{23}$}\\
%\multicolumn{3}{|cc|}{ciao}\\
%\hline
Confidence level & NO & IO \\
\hline
&\multicolumn{2}{c}{$\sin^2{\theta_{23}}$}\\
\hline
$1\sigma$ & [0.464, 0.482] $\cup$ [0.532, 0.582] &  \\\hline
$90\%$    & [0.443, 0.592] & [0.530, 0.586] \\\hline
$2\sigma$ & [0.436, 0.598] & [0.466, 0.592] \\
\hline
\hline
&\multicolumn{2}{c}{$\delta_{CP}$}\\
\hline
$1\sigma$ & [-2.69, -0.75] &  \\\hline
$90\%$    & [-3.04, -0.34] &  [-2.07, -0.91]\\\hline
$2\sigma$ & [-$\pi$, -0.13] $\cup$ [3.06, $\pi$] & [-2.34, -0.67] \\\hline
$3\sigma$ & [-$\pi$, 0.43] $\cup$ [2.54, $\pi$]  & [-2.92, -0.08] \\
\hline
\hline
\end{tabular}
\end{center}
\caption{Feldman-Cousins confidence intervals for $\sin^2{\theta_{23}}$ and $\delta_{CP}$.}\label{tab:FC_CI_all}
\end{table}

%\FloatBarrier
Similar results from the MaCh3 fitter are shown in \cref{table:MaCh3CI} in terms of credible intervals for the analysis with and without reactor constraints. One observes that the intervals have only very minor differences with respect to p-theta ones, and these differences are understood to come from the same source of those observed during plot comparison in \cref{fig:datadCPth13woRC}, \cref{fig:data_2DwoRC}.

\textcolor{blue}{The conclusions at this stage of the analysis, i.e. before any fake data study described in \cref{sec:FDS}, are the exclusion of CP symmetry conservation at more than 90\% CL, a mild preference for normal ordering and upper octant of $\mathrm{sin^2(\theta_{23})}$, and a precision measurement of $\Delta m^2_{32}$ (NO)/$\Delta m^2_{31}$ (IO) with an error of the order of 2\%.}

\begin{table}
\centering
\renewcommand{\arraystretch}{0.75}
\resizebox{\textwidth}{!}{\begin{tabular}{c|c|c|c|c}
\hline
\hline
\multicolumn{5}{c}{w RC}\\
\hline
Parameter & $\delta_{CP}$ [rad.] & $\sin^{2}\theta_{23}$ & $\sin^{2}\theta_{13}$ & $\Delta m^{2}_{32}$ [$\times10^{-3}$ eV$^{2}$] \\
\hline
Central Value & -1.85 & 0.54 & 0.022 & 2.50 \\
1$\sigma$ C.I. & [-2.60, -1.01] & [0.49, 0.56] & [0.021, 0.023] & [2.42, 2.59] \\
2$\sigma$ C.I. & [ -$\pi$, -0.34] $\cup$ [3.10, $\pi$] & [0.46, 0.58] & [0.021, 0.023] & [-2.63, -2.47] $\cup$ [2.38, 2.62] \\
3$\sigma$ C.I. & [-$\pi$, 0.38] $\cup$ [2.51, $\pi$] & [0.44, 0.60] & [0.020, 0.024] & [-2.69, -2.40] $\cup$ [2.33, 2.67] \\
\hline
\multicolumn{5}{c}{w/o RC}\\
\hline
%Parameter & $\delta_{CP}$ [rad.] & $\sin^{2}\theta_{23}$ & $\sin^{2}\theta_{13}$ & $\Delta m^{2}_{32}$ [$\times10^{-3}$ eV$^{2}$] \\
%\hline
Central Value & -2.01 & 0.48 & 0.024 & 2.51 \\
1$\sigma$ C.I & [-2.83, -0.75] & [0.47, 0.55] & [0.021, 0.030] & [-2.59, -2.51] $\cup$ [2.44, 2.57] \\
2$\sigma$ C.I & [-$\pi$, 0.25] $\cup$ [2.51, $\pi$] & [0.45, 0.58] & [0.018, 0.036] & [-2.65, -2.45] $\cup$ [2.39, 2.62] \\
3$\sigma$ C.I & [-$\pi$, 1.19] $\cup$ [1.38, $\pi$] & [0.43, 0.60] & [0.015, 0.043] & [-2.71, -2.39] $\cup$ [2.33, 2.67] \\
\hline
\hline
\end{tabular}}
\caption{MaCh3 best fit values and 1$\sigma$, 2$\sigma$ and 3$\sigma$ credible interval ranges for oscillation parameters. 2D best fit values are taken from disappearance $(\sin^{2}\theta_{23}-\Delta m^{2}_{32})$ and appearance $(\delta_{CP}-\sin^{2}\theta_{13})$ contours whilst the credible intervals are taken from the 1D posteriors. Results are given for T2K+reactors (top) and T2K-only (bottom).}
\label{table:MaCh3CI}
\end{table}
%
%\todo{unify tables?}
%\begin{table}[h]
%    \centering
%    \caption{Best fit values for the OA2023 analysis with the P-Theta fitter, \textbf{without} reactor constraints, global best fit is in normal ordering}
%     \begin{tabular}{|c|c|c|}
%     \hline
%    &Normal ordering & Inverted ordering \\
%     \hline
%    & & \\
%          $\mathrm{sin^2(\theta_{13})/10^{-3}}$ &$(27.8^{+1.8}_{-6.9})$&$(31.0^{+1.8}_{-7.4})$ \\
%         & &\\
%         $\delta_{CP}$ & $-2.21^{+1.62}_{-0.75}$ & $-1.29^{+0.63}_{-0.99}$ \\
%         & &\\
%         $\Delta m^2_{32}$ (NO)/$\Delta m^2_{31}$ (IO) &$(2.521^{+0.039}_{-0.050})10^{-3}\mathrm{eV^2/c^4}$ &$(-2.489^{+0.042}_{-0.046})10^{-3}\mathrm{eV^2/c^4}$\\
%         & & \\
%         $\mathrm{sin^2(\theta_{23})}$  & $0.458^{+0.130}_{-0.021}$ & $0.458^{+0.127}_{-0.021}$\\ 
%         & & \\
%         \hline
%         -2 ln L & 648.837& 649.655\\
%         -2 $\Delta$ln L & 0. & 0.818\\
%          \hline
%    \end{tabular}
%    \label{tab:BestfitwoRC_PTheta}
%\end{table}
%\FloatBarrier
%\begin{table}[H]
%\centering
%\renewcommand{\arraystretch}{0.75}
%\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|}
%\hline
%\multicolumn{5}{|c|}{NO(?) w/o RC}\\
%\hline
%Parameter & $\delta_{CP}$ [rad.] & $\sin^{2}\theta_{23}$ & $\sin^{2}\theta_{13}$ & $\Delta m^{2}_{32}$ [$\times10^{-3}$ eV$^{2}$] \\
%\hline
%2D Best Fit Value & -2.01 & 0.48 & 0.024 & 2.51 \\
%68\% (1$\sigma$) C.I. range & [-2.83, -0.75] & [0.47, 0.55] & [0.021,0.030] & [-2.59, -2.51] $\cup$ [2.44, 2.57] \\
%95.4 (2$\sigma$) C.I. & [-$\pi$, 0.25] $\cup$ [2.51, $\pi$] & [0.45, 0.58] & [0.018, 0.036] & [-2.65, -2.45] $\cup$ [2.39, 2.62] \\
%99.73 (3$\sigma$) C.I. & [-$\pi$, 1.19] $\cup$ [1.38, $\pi$] & [0.43, 0.60] & [0.015, 0.043] & [-2.71, -2.39] $\cup$ [2.33, 2.67] \\
%\hline
%\end{tabular}}
%\caption{T2K only: best fit values and 1$\sigma$, 2$\sigma$ and 3$\sigma$ credible interval ranges for oscillation parameters. 2D best fit values are taken from disappearance $(\sin^{2}\theta_{23}-\Delta m^{2}_{32})$ and appearance $(\delta_{cp}-\sin^{2}\theta_{13})$ contours whilst the credible intervals are taken from the 1D posteriors.}
%\label{table:MaCh3CI_woRC}
%\end{table}
%\FloatBarrier
%\subsubsection{Feldman-Cousins studies with P-Theta}
%\label{sec:FC}
%\todo{necessary for PAS? eventually put the difference with run 1-10?}
%\todo{highlight change in oscillation results with respect to previous anaysis for data?}
%As for the previous years, P-Theta ran Feldman-Cousins studies for the two parameters that have non-Gaussian $\chi^2$ curves: $\delta_{CP}$ and $\sin^2{\theta_{23}}$.
%\paragraph{$\delta_{CP}$}
%\mbox{}\\
%\mbox{}\\
%The critical $\Delta\chi^2$ values for $\delta_{CP}$ are computed using 50,000~toy MC experiments generated for fixed values of $\delta_{CP}$ and randomly generated values of the other oscillation parameters. \\$\delta_{CP}$ is generated at values of $\delta_{CP}/\pi =\{-0.75, -0.5, -0.25, 0, 0.125, 0.25, 0.5, 0.75, 0.825, 1\}$. $\theta_{13}$ is generated following the results of the reactor experiments.
%The atmospheric parameters are generated according to the result of an Asimov fit for true values of the oscillation parameters corresponding to the best-fit points. The $\Delta m^2_{32}$ ($\Delta m^2_{31}$ ) distribution is smeared according to the Fake Data studies procedure mentioned before. The obtained critical value distributions can be found in \cref{fig:FCCritvaluesdCP} for both orderings and are used to compute the $\delta_{CP}$ confidence interval with correct coverage. details of the study are available in TN 461. The obtained intervals for both orderings are presented visually on \cref{fig:FCFinalplotdCP} and numerically in \cref{tab:FCIntervals}. As said before, we obtain an exclusion of CP conservation at more than 90\% but less than 2 $\sigma$.
%\begin{figure}[ht]
%\begin{center}
%\includegraphics[width=7.5cm,keepaspectratio]{FCstudies_figs/CriticalChi2_plots_NH_4.pdf}
%\includegraphics[width=7.5cm,keepaspectratio]{FCstudies_figs/CriticalChi2_plots_IH_4.pdf}
%\end{center}
%\caption[Critical $\chi{^2}$ values as a function of  true $\delta_{CP}$ values]{Critical $\chi{^2}$ values as a function of true $\delta_{CP}$ computed  with 50000 toy experiments, for 10 values of $\delta_{CP}$, and 4 levels of confidence. Multiple lines represent statistical error bands. Green dotted lines show the standard levels of confidence under the Gaussian assumption. Results are given for Normal (left) and Inverted (right) orderings.}
%\label{fig:FCCritvaluesdCP}
%\end{figure}

%\begin{table}[h]
%\begin{center}
%\begin{tabular}{|c|c|c|}
%\hline
%Confidence level & Interval (NH) & Interval (IH) \\
%\hline
%$1\sigma$ & [-2.69,-0.75] &  \\\hline
%$90\%$    & [-3.04,-0.34] &  [-2.07,-0.91]\\\hline
%$2\sigma$ & [-$\pi$,-0.13] $\cup$ [3.06,$\pi$] & [-2.34,-0.67] \\\hline
%$3\sigma$ & [-$\pi$,0.43] $\cup$ [2.54,$\pi$]  & [-2.92,-0.08] \\
%\hline
%\end{tabular}
%\end{center}
%\caption{Feldman-Cousins confidence intervals for $\delta_{CP}$.}\label{tab:FCIntervals}
%\end{table}

%\FloatBarrier
%\paragraph{$\sin^2{\theta_{23}}$}
%\mbox{}\\
%\mbox{}\\
%Analogously we construct Feldman-Cousins confidence intervals for $\sin^2{\theta_{23}}$. Here, we produce 22~sets of toys with true values of $\sin^2{\theta_{23}}$ placed on 11~evenly spaced points between 0.42 and 0.62 for both mass hierarchies. For each point we throw 20000~toys, for the other oscillation parameters according to the $(\Delta m^2_{32},\delta_\mathrm{CP})$ (NH) and $(\left|\Delta m^2_{31}\right|,\delta_\mathrm{CP})$ (IH) distributions for the best-fit Asimov, and for $\sin^2{2\theta_{13}}$ according to the reactor constraint, where the $\Delta m^2_{32}$ ($\Delta m^2_{31}$) distributions are smeared.


%ETA - commenting this out, I think a lot of the FC stuff is a bit too technical for the PAS
%\begin{figure}[ht]
%\begin{center}
%\includegraphics[width=7.5cm,keepaspectratio]{FCstudies_figs/CriticalChi2_plots_NH_3.pdf}
%\includegraphics[width=7.5cm,keepaspectratio]{FCstudies_figs/CriticalChi2_plots_IH_3.pdf}
%\end{center}
%\caption[Critical $\chi{^2}$ values as a function of  true $\sin^2\theta_{23}$ values]{Critical $\chi{^2}$ values as a function of true $\sin^2\theta_{23}$ computed  with 20000 toy experiments, for 11 values of $\sin^2\theta_{23}$, and 3 levels of confidence. Multiple lines represent statistical error bands. Green dotted lines show the standard levels of confidence under the Gaussian assumption. Results are given for Normal (left) and Inverted (right) orderings.}
%\label{fig:FCCritvaluessin223}
%\end{figure}

% sin2th23 dChi2 surface using FC calculated intervals
%\begin{figure}[ht]
%\begin{center}
%\includegraphics[width=12cm,keepaspectratio]{FCstudies_figs/contour_th23_runversion_wCI_all_errorBand.pdf}
%\end{center}
%\caption{$\chi{^2}$ of the data fit for $\sin^2\theta_{23}$ for both normal (blue) and inverted (orange) orderings. The computed confidence intervals are displayed in different textures. }
%\label{fig:FCFinalplotsin223}
%\end{figure}
%The obtained $\chi^2$ critical values are shown in \cref{fig:FCCritvaluessin223}.

%\FloatBarrier

\subsubsection{Octant and mass ordering preferences: Bayes factors}
It is also possible to make statements about discrete hypotheses such as the Mass Ordering (MO) and octant of $\sin^{2}\theta_{23}$ preferences from the analysis.
A natural way to do this is with the use of Bayes factors from the MaCh3 posterior distributions.
These are calculated by comparing the number of MCMC steps in a particular region of the posterior.
The number of steps is proportional to the probability of the true value being contained in that region and thus gives a measure of a model preference.
The fraction of posterior contained in each MO, octant and each of these conditional on each other, for fits with reactor constraint are shown in \cref{table:Prob_wRC}.
The corresponding Bayes factors are $\mathfrak{B}(NH/IH) = 3.35$ and $\mathfrak{B}(UO/LO) = 2.57$.
The Jeffrey's scale \cite{Jeffrey} for these is ``barely worth mentioning'' and thus these Bayes factors are not at a sufficient level to make physics conclusions with. Still, upper octant (72\%) and normal ordering (77\%) are mildly preferred.\\
Regarding the octant, the interplay between $\sin^{2} \theta_{13}$ and $\sin^{2} \theta_{23}$ is also illustrated in Figure~\ref{fig:Alldata_2D_sinsin}. One observes that without reactor constraint, there is a slight (but not significance) preference for the lower octant driven by the $\nu_{e}$ sample. In this same sample, there is a natural anti-correlation between $\sin^{2} \theta_{13}$ and $\sin^{2} \theta_{23}$ that is observed on the plot. Fixing $\sin^{2} \theta_{13}$ with the reactor constraint, one observes that this correlation naturally disappears and that higher octant is then slightly favoured in order to compensate the lower $\nu_{e}$ rate induced by the lower value of $\sin^{2} \theta_{13}$ from reactor constraint compared to T2K.

% Probabilities, model comparison for w/-RC
\begin{table}
\centering
\begin{tabular}{c|c c |c}
\hline
\hline
 & $\sin^{2}\theta_{23}  < 0.5$ & $\sin^{2}\theta_{23}  > 0.5$ & Sum\\
\hline
NO ($\Delta m_{32}^{2} > 0$)& 0.23 & 0.54 & 0.77\\
IO ($\Delta m_{32}^{2} < 0$)& 0.05 & 0.18 & 0.23\\
\hline
Sum &0.28 & 0.72 & 1.00\\
\hline
\hline
\end{tabular}
\caption{Model comparison probabilities for normal and inverted hierarchies, as well as upper and lower octants, from the posterior with reactor constraint.}
\label{table:Prob_wRC}
\end{table}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.49\textwidth]{Datafits_figs/contour_th13_th23_wRC_NH.pdf}
    \includegraphics[width=0.49\textwidth]{Datafits_figs/contour_th13_th23_woRC_NH.pdf}
    \caption{2D likelihood surfaces in the $\sin^2 \theta_{23}$/$\sin^2 \theta_{13}$ planes with the reactor constraint on $\sin^2 \theta_{13}$ (left) and without (right) for normal ordering,  for the data fit. }
    \label{fig:Alldata_2D_sinsin}
\end{figure}

\subsubsection{MaCh3 goodness of fit}

Another key check for any analysis is on the goodness of fit of the post-fit prediction to the fitted data.
This can be done in either fitter using slightly different methods.

Below are the post-fit p-value constructed from MaCh3.
These are called posterior predictive p-values (PPPV). They are constructed as follows: sampling from the Markov chain we get a set of parameter values; we create a prediction from these parameters and calculate the likelihood of this prediction compared to a Poisson fluctuation of this prediction. We also calculate the likelihood of this prediction compared to the real data.
The PPPV is then calculated from the fraction of samples for which the likelihood of the real data is less than the likelihood of the Poisson-fluctuated prediction.
This process is described in more detail in T2K-TN-462~\cite{TN462} and older MaCh3 notes.

For each PPPV, we calculate a ``rate only'' version where only the event rate is used compare to the real data or fluctuated data (i.e. as if the analysis had only one bin for each sample) and a ``rate$+$shape'' version where the likelihood is summed across all bins used in the analysis.

The total PPPV as well as those broken down by samples are given below. The PPPVs from the previous analysis are also included in the table below for comparison but good agreement is seen. In general, the data shows a reasonable agreement (PPPV $\geq$ 0.05) with respect to the model posteriors, confirming the validity of our model to fit the data. The only exception is the 1 ring $\mu$-like samples, which small PPPV = 0.02 has been observed since several years in our analyses. Though relatively large, this disagreement mostly disappear when adding the shape information, and has also been tested against several alternative scenarios in the past. These two results confort the interpretation of this low rate-only p-value as a sole statistical effect, though this interpretation will be of course continuously tested in the coming years of the experiments.\\
Moreover, there are some changes with respect to the previous analysis, in particular the large change in the rate$+$shape p-value in the FHC $\nu_{\mu}$CC$1\pi$ sample which is most likely due to the new SK detector matrix and the inclusion of correlations between this sample and the single-ring samples as well as the other changes made to the matrix.

\begin{table}[H]
\centering
\begin{tabular}{c|c|c|c|c}
\hline
\hline
  \multirow{2}{*}{\textbf{Sample / p-value}}         & \multicolumn{2}{c|}{\textbf{rate+shape}}  & \multicolumn{2}{c}{\textbf{rate-only}} \\
  \cline{2-5}
        & OA2023 & OA2022 & OA2023 & OA2022 \\
\hline
\hline
%FHC 1R$\mu$  &  0.33  & 0.30 & 0.0236 & 0.02 \\
FHC 1R$\mu$  &  0.33  & 0.30 & 0.024 & 0.02 \\
\hline
RHC 1R$\mu$  &  0.83  & 0.84 & 0.57 & 0.66 \\
\hline
FHC $\nu_{\mu}$CC1$\pi$  & 0.43 & 0.96 &  0.25 & 0.30\\
\hline
%FHC 1R$e$  & 0.1228 & 0.12 & 0.48 & 0.51 \\
FHC 1R$e$  & 0.12 & 0.12 & 0.48 & 0.51 \\
\hline
RHC 1R$e$  &  0.64 & 0.66 & 0.47 & 0.39 \\
\hline
FHC 1R$e$1d.e  & 0.73  & 0.89 & 0.12  & 0.26 \\
\hline\hline
%\textbf{Total}  & 0.5136 & 0.84 & 0.06 & 0.10 \\
\textbf{Total}  & 0.51 & 0.84 & 0.06 & 0.10 \\
\hline
\hline
\end{tabular} \\
\caption{Breakdown of posterior predictive p-values, quoted separately for bin-by-bin (rate+shape) and total rate (rate-only), used as a test for the compatibility between the best-fit model and the data, using T2K + reactor constraint fit.}
\label{table:GOF_wRC}
\end{table}

==> SK.tex <==
\section{Changes in the FD}
\label{sec:sk}
%\todo{Add in an introduction. Just syaing that nothing has changed in terms of the samples we include in the analysis.}
%\todo{DONE BQ: It is very good to explain what has changed, but we may wish this TN to be almost self-consistent. Same as for other sections, I propose to have a small intro explaining the samples very briefly.}
In this analysis, we have used the same six FD samples used for OA2022, with the only changes being related to a change in the selection (decay-e cut) and the re-evaluation of detector systematics. As a reminder, these samples are:
\begin{itemize}
\item the 1 ring electron and muon in both Forward and Reverse Horn-Current (FHC/RHC-1Re, FHC/RHC)-1R$\mu$).
\item the FHC 1 ring electron with one additional decay-electron (FHC 1Re-1d.e.).
\item the FHC $\nu_{\mu}$ CC$1\pi^+$-like sample (FHC $\nu_{\mu}$CC$1\pi^+$-like).
\end{itemize}
These 6 samples' detailed descriptions can be found in~\cite{TN465} and are illustrated in \cref{fig:SKpred_newmat}.
The two changes, the new decay-e cut, and the new  SK detector systematics will be described in the following sections.

\subsection{New decay-electron cut to remove contamination from neutron captures}
\label{sec:sksel}
We select events into the samples for the OA partly on the basis of the number of electrons from muon decays recorded in an event.
The reconstruction software, fiTQun~\cite{FitQUN1}, infers the number of decay electrons mainly from the time at which the photo-multiplier tubes (PMTs) detect the Cherenkov light emitted due to the decay electrons.

All Run 1-10 data were collected with the SK detector containing ultra-pure water.
%, while Run 11 being the first time this was not the case.
Run 11 data were collected after Gadolinium (Gd) loading at SK at the concentration of $0.01\%$.
The introduction of Gd to SK creates a potential source of confusion for the decay-electron tagging due to its neutron capture capabilities. 
The delayed de-excitation of a Gd-nucleus after a neutron capture could be confused with the delayed signal of a decay electron.
As part of this analysis, the mis-ID of neutron captures as decay electrons was studied, and the contamination from neutron captures in Run~11 was found to be $70\%$ (see TN465, Sec. 3.2~\cite{TN465}).
Thus, a more accurate method to identify decay electrons has been developed.
Interestingly, in Runs~1-10 (i.e. in pure water) approximately $5\%$ of the decay-electrons identified by fiTQun were actually neutron captures on Hydrogen.
Therefore, the improved decay electron reconstruction has been applied to all runs.
The implementation and optimization of the new decay electron tagging are briefly described below with details given in T2K-TN-465~\cite{TN465}.

Typically, neutron captures produce less visible light than decay electrons. Moreover, the actual capture time of neutrons ($\lambda = 200~\mu$s for water, and $30~\mu$s for Gd) is generally longer than the muon lifetime ($2.2~\mu$s in its own reference frame). %\todo{DONE B.Q: Shall we also say few words about the lifetime of a muon and n-capture, to explain the later time constant is bigger?}
Therefore, in addition to the timing information, we made considerations on the number of PMTs that detect the Cherenkov radiation from the decay electrons.
We now recognize a decay-electron as any decay-electron candidate identified by fiTQun at a time, \textit{dt}, after the creation of the main Cherenkov ring in an event, if,
\begin{itemize}
    \item \equation{\textit{dt} $<1.5~\mu$s} or,
    \item \equation{\textit{dt}} $<20~\mu$s and, for $N$ PMTs hit in a $50$ns time window for the candidate, \equation{\textit{dt} $< (0.25N - 7.5)~\mu$s}.
\end{itemize}  
An instance of applying the cut is shown in \cref{fig:decayecut}.
In Run~1-11, the efficiency of identifying true decay-electrons is $99\%$ with a neutron impurity of less than $1\%$.
Consequently, we see up to a $2\%$ change in the event rates of CCQE-like (single ring) samples, and about a $6\%$ decrease in the $\nu_{\mu}$ CC$1\pi^+$-like samples.
The results are summarized in \cref{tab:gdmigration}. It is important to stress that the numbers reported in this table are obtained \textcolor{red}{with the same T2K event selection cuts usually applied for each sample in the oscillation analysis}, except the \textcolor{blue}{on visible energy and reconstructed neutrino energy}. This explains the difference w.r.t. \cref{tab:eventsamples}.
 
\begin{figure}[H]
    \centering
\includegraphics[width=0.6\linewidth]{SK_figs/Decaye_cut/cut.png}
    \caption{ Distribution of decay-electron candidates identified by fiTQun over the two-dimensional space of N$50$ -- the number of hit PMTs in $50$ns time window for a candidate, and \textit{dt} -- the time of recording the candidate after the creation of the main Cherenkov ring. The sample used here was that of the Run 1-10 $\nu_\mu$ CCQE events. Neutron captures (in gray) are almost entirely removed by rejecting the candidates above the cut (magenta line), and mostly the decay electrons (in blue) are selected. }  
    \label{fig:decayecut}
\end{figure}

\begin{table}[H]
    \centering
%    \begin{tabular}{|p{1.7 cm}|p{1.2cm}|p{1.2cm}|p{1.6cm}|p{1.2cm}|p{1.2cm}|p{1.7cm}|}
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
    \hline
        &  \multicolumn{3}{c}{Run 1-10 n. of events} & \multicolumn{3}{|c}{Run 11 n. of events} \\
        \cline{2-7}
%        \multirow{2}{*}{Sample} & w/o cut & w cut & change $\%$  & w/o cut & w cut & change $\%$ \\
        Sample & w/o cut & w cut & change  & w/o cut & w cut & change \\
        \hline
        $\nu_e$CCQE & 99& 99& - & 5& 7& 40\%\\
        \hline
        $\bar\nu_e$CCQE & 20& 20& - & -& -& -\\
        \hline
        $\nu_e$ CC$1\pi^+$ & 14& 14& -& 2& 1& -50\%\\
        \hline
        $\nu_{\mu}$CCQE& 335& 337& 1\%& 35& 35& -\\
        \hline
        $\bar\nu_{\mu}$CCQE& 140& 140& -& -& -& -\\
        \hline
        $\nu_{\mu}$CC$1\pi^+$-like (1 decay e)& 62& 62& -& 5& 5& -\\
        \hline
        $\nu_{\mu}$CC$1\pi^+$-like (2 decay e)& 73& 70& -4\%& 6& 4& -33\%\\
        \hline
        \hline
    \end{tabular}
    \caption{Change in the event rates on applying the new decay-electron cut on the Run~1-11 data. Samples are listed by the dominant neutrino interaction modes present in them. These were selected from the official minituples which are generated with less conservative cuts than those used in the OA.\\POT in $10^{20}$, for Run~1-10 forward horn current (FHC): $19.7$, Run~5-9 reverse horn current: $16.2$, and Run 11 FHC: $0.176$.}
    \label{tab:gdmigration}
\end{table}


\subsection{New detector covariance matrix}
\label{sec:skmat}

Similar to previous analyses, a fit on the atmospheric neutrinos at SK is used to estimate the possible SK detector mis-modelling via a set of effective error parameters which shift ($\alpha$ parameters) and smear ($\beta$\ parameters) the likelihood-based cuts on different particle PIDs that are used in the sample selection cuts.
We utilize a Bayesian approach (MCMC) to optimize the same underlying probability distributions for data and MC and measure the discrepancies between the two.
This section summarizes the updates in SK detector error estimation related to the inclusion of a new MR sample, as well as the resulting new constraints of detector systematic errors.
More details can be found in T2K-TN-482~\cite{TN482} and a bi-weekly talk given here \cite{RogerBiWeekly}. 

\subsubsection{Description of changes in procedure}

In the fit of atmospheric neutrinos before OA2023, the \{$\alpha$, $\beta$\} parameters had detector spatial dependencies that were developed only for 1R samples and will not work for the MR samples.
On the other hand, the missing dependency on E$_{vis}$ for the old \{$\alpha$, $\beta$\} led to strong correlations among the E$_{rec}$ (or $p$) bins in the final OA matrix.
Thus, in this new analysis, the fit dimension separating the detector into different regions is replaced by an E$_{vis}$ dimension for the \{$\alpha$, $\beta$\} of both 1R and MR samples. 

Back in OA2022, a temporary solution---the so-called \textit{Frankenmatrix}---was adopted to include errors for the MR sample.
This \textit{Frankenmatrix} was created where the \{$\alpha$, $\beta$\} for 1R and MR samples were optimized separately using the already existing inputs that were developed independently.
The lack of migration between the 1R and MR samples in this approach resulted in an unrealistic uncertainty matrix, with mild correlations only from the external constraints.
This is automatically improved by the simultaneous fit of both 1R and MR samples performed for the current analysis.
In addition to the new variables and visible final-state topologies for MR samples, the use of the $\pi^0$ and $\pi^{\pm}$ hybrid samples is also updated in this new matrix. \textcolor{red}{Unlike the previous treatment where the data-MC comparison of these hybrid samples were applied as external constraints on the \{$\alpha,\,\beta$\} parameters in the intermediate Toy MC that is removed, they are applied as prior constraints for the relevant \{$\alpha,\,\beta$\} parameters in the MCMC fits as explained in~\cite{TN482}.}

Another important update is the removal of an intermediate matrix.
Previously, the efficiency distributions from the nominal atmospheric MC as caused by the cut variables in the fit are used to construct an intermediate matrix binned in E$_{vis}$ and visible final topology.
The error parameters were then thrown from this matrix, along with the BANFF post-fit and external constraints, to generate the uncertainty matrix based on the T2K MC.
However, such a process inevitably loses the information on individual error parameters from the MCMC chains while overlooking the irregularity of the efficiency distributions.
Therefore, we decided to remove this intermediate matrix and throw the error parameters directly from the MCMC. 
 
Besides the aforementioned changes, better atmospheric flux spectra and neutrino interaction (BANFF 2020) models are used as the inputs for MCMC.
All these improvements lead to the new constraints on detector systematic errors shown in the next section. 

These changes introduced for OA2023 and future analyses are summarized in \cref{tab:sk-covmat-changes}.
\begin{center}
%\begingroup
%\setlength\LTleft{-1.5cm}
%\captionsetup[table]{skip=5pt}
%\centering
\begin{longtable}{p{4cm} | p{5cm} | p{5cm}}
    \hline
    \hline
    & Prior to OA2023 & OA2023+\\
%    \hline & \\[-1mm]
 \hline
    \multirow{4}{*}{Fitting} & 4 cut variables & 7 cut variables \\
                               & 6 visible final topologies & 8 visible final topologies \\
                               & 6 detector regions & no detector region binning\\
                               & no E$_{vis}$ binning & 5 E$_{vis}$ binning\\
    \hline
    Intermediate matrix & Based on the ``efficiencies" of core sample cuts, binned in E$_{vis}$ & Removed \\
    \hline
    Toy MC & Throwing from the intermediate matrix & Throwing from the MCMC posterior distributions \\
    \hline
    1R\&MR correlation & The \textit{Frankenmatrix} & Fully correlated \\
    \hline
    External errors & Constraints on e.g. NC, $\mu$ decay, Michel $e$ tagging applied in parallel with the fit & Partially removed -or- constrained in the fit\\
    \hline
    Hybrid samples & Implemented as ``external constraints'' in parallel with the fit & Included in the fit \\
    \hline
    \hline
    \caption{Major updates of SK detector uncertainties for OA2023+.}
    \label{tab:sk-covmat-changes}
\end{longtable}
%\endgroup
\end{center}

\subsubsection{Results on detector systematics constraints}

\cref{fig:sk_matrices} shows the \textit{Frankenmatrix} to the left and the new matrix for OA2023 right.
In both matrices, the blocks are ordered by FHC 1R$e$, FHC 1R$\mu$, RHC 1R$e$, RHC 1R$\mu$, FHC 1R$e$+1d.e., and MR from left to right. Each sample block is further binned by E$_{rec}$ and neutrino interaction/oscillation channels.
%
\begin{figure}[H]
\centering
\includegraphics[width=0.75\textwidth]{SK_figs/Matrix/SKJointErrorMatrix_Total_270122_OA2021_erec_plot.pdf}
%
\includegraphics[width=0.75\textwidth]{SK_figs/Matrix/SKJointErrorMatrix_OA2023_V1_erec_plot.pdf}
    \caption{The OA2022 \textit{Frankenmatrix} to the top and the new OA2023 matrix from the full atmospheric fit to the bottom. Both matrices have the same binning of T2K samples and $E_{rec}$.}
    \label{fig:sk_matrices}
\end{figure}

%\begin{figure}[H]
%\centering
%    \makebox[\linewidth][c]{\includegraphics[width=1.0\textwidth]{SK_figs/Matrix/OAmatrix.png}}
%    \caption{The OA2022 \textit{Frankenmatrix} to the left and the new OA2023 matrix from the full atmospheric fit to the right. Both matrices have the same binning of T2K samples and E$_{rec}$.}
%    \label{fig:sk_matrices}
%\end{figure}
%\todo{Remake these plots to be prettier and have a consistent colour theme}

The missed correlation between 1R and MR samples in the \textit{Frankenmatrix} is recovered in the new matrix thanks to the full atmospheric fit.
Meanwhile, the strong correlation among E$_{rec}$ bins in each T2K sample is also reduced because of the new E$_{vis}$ dependencies of the \{$\alpha$, $\beta$\} parameters.

\cref{fig:sk_matrices_diag} shows the square roots of the matrices' diagonals.
Reduced errors of background events, e.g. NC interactions, consistently exist in all T2K samples thanks to the better constraints via the atmospheric fit instead of external sources.
The error sizes of the FHC 1R$e$-1d.e. sample are also reduced to be closer to those of the FHC 1R$e$ sample as expected since these two samples have the same primary particle topology.
This improvement is attributed to the removal of the intermediate matrix, which allows finer details such as the pion momentum spectrum to be included in the throws via the visible final topology and E$_{vis}$ bins.
On the other hand, the MR diagonals do not vary much as compared to the other samples due to the rather similar parameterization for the MR sample in the \textit{Frankenmatrix} and OA2023.

\begin{figure}[h]
\centering
%    \makebox[\linewidth][c]{
%    \includegraphics[width=1.0\textwidth]{SK_figs/Matrix/diagonals.png}
%    \includegraphics[width=0.7\textwidth]{SK_figs/DiagErrorMom.pdf}\\
    \includegraphics[width=0.99\textwidth]{SK_figs/DiagErrorErec.pdf}
%    }
    \caption{The square root of the diagonal elements of the \textit{Frankenmatrix} (black) and OA2023 matrix (red). \textcolor{green}{The most top binning shows the reconstructed samples, while the one below shows the true interaction channel. The most bottom bins show the reconstructed energy.}}
    \label{fig:sk_matrices_diag}
\end{figure}

\subsection{Impact on the Monte Carlo predictions uncertainties at SK}
%\todo{compare the new and old MC predictions at SK}
%\subsubsection{New MC prediction at SK}
%\subsubsection{Impact of new SK det cov on predictions}
The change in uncertainties between the SK detector matrix used in the
previous analysis (red) and the current analysis (blue) are shown in \cref{fig:SKpred_newmat} (from TN 462). As expected we see a slight tightening of errors at low reconstructed energy values for all samples and a
reduction of error across the full energy spectrum for multi-ring samples.
%
\begin{figure}[h]
\centering
    \begin{tabular}{c c}
        \includegraphics[width=0.49\textwidth, page=1]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf} &
        \includegraphics[width=0.49\textwidth, page=2]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf} \\
        \includegraphics[width=0.49\textwidth, page=3]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf} &
        \includegraphics[width=0.49\textwidth, page=4]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf} \\
        \includegraphics[width=0.49\textwidth, page=5]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf} &
        \includegraphics[width=0.49\textwidth, page=6]{SK_figs/SK_det_Old_and_New_all_samples_ratio_plots.pdf}
    \end{tabular}
%\includegraphics[width=0.78\textwidth]{SK_figs/oldnewSKdet.png}
\caption{The change in uncertainties between the SK detector matrix used in the previous analysis (red) and the current analysis (blue). As expected we see a slight tightening of errors at low reconstructed energy values for all samples and a reduction of error across the full energy spectrum for multi-ring samples.}%{\textcolor{blue}{A.L. taken from TN462 screenshot: recover vector image.}}
\label{fig:SKpred_newmat}
\end{figure}
%\todo{put spectra at FD with error bands with old and new det matrix (search in presentations of Lucile/Denis)}

==> Summary.tex <==
\section{Summary and Conclusions}
\label{sec:summary}


%We show in \cref{fig:summary_nature} a comparison of $\nu_e$-like samples
%at SK with.
%\begin{figure}
%    \centering
%    \includegraphics[width=0.505\textwidth]{summary_figs/nature_1-10.png}%
%    \includegraphics[width=0.49\textwidth]{summary_figs/nature_1-11.png}
%    \caption{"Nature-style" plots for OA2023. From TN462.}
%    \label{fig:summary_nature}
%\end{figure}


%Taken from P-Theta: being changed:

This analysis is the first with the SK Run 11 data (9\% increase in FHC statistics) and with the new decay electron cut and reduced SK systematic errors on the 1Re1.d.e sample. The near detector constraint is the same as for the previous analysis (22 samples and ND280 runs 2–9). The data sample corresponds to 21.428~$\times$~10$^{20}$
POT in FHC mode and $16.346~\times~10^{20}$~POT in RHC mode at SK, and for the ND $11.531 \times 10^{20}$ POT in FHC and $8.336 \times 10^{20}$ POT in RHC beam modes.
The following six SK samples (FHC/RHC 1R$\mu$, FHC/RHC 1Re, FHC 1R $\nu_e$ CC1$\pi^+$ and FHC MR $\nu_\mu$ CC1$\pi$) from Run 1-11 have been analyzed together in a fit to four oscillation parameters \Dmthreetwo, \stwothree, \sonethree, and \dcp.
%666 The BANFF constraint from the ND fit of Run 2-9 was used for the main result but another fitter, GUNDAM has also been tested on the same ND dataset providing very close results both at the level of predicted events at the FD (see \cite{TN458}). The analysis is performed with two fitters (MaCh3 and P-Theta). We have shown that both fitters are based on very different approaches, provide consistent results both for the A22 Asimov data-set (\cref{sec:asimovfits}) and for the Run 1-11 data (\cref{sec:datafits}).

As in previous analyses, a \Dmthreetwo ($|$\Dmthreeone$|$ for IO) smearing is applied to account for changes in the $\Delta\chi^2$ distributions observed in fake data studies~\cite{TN441}. Additional studies have shown that the overall improvement in sensitivity on all parameters comes more or less equally from the increase in statistics and the reduced SK detection errors on 1Re-1d.e.

In the P-Theta analysis, the error on \Dmthreetwo~is improved by 20\% reaching an overall 2\% level with  
$\Delta m^2_{32}$ (NO)= $(2.521^{+0.037}_{-0.050})\times10^{-3}~\mathrm{eV^2/c^4}$ and $\Delta m^2_{31}$ (IO)$= (-2.486^{+0.043}_{-0.044})\times10^{-3}~\mathrm{eV^2/c^4}$ 
at a 1$\sigma$ level. For MaCh3 the uncertainty does not seem to reduce so significantly.

%The most notable change is the weaker constraint of \dcp, partly due to the various model changes, but for the most part due to the rather small number of e-like events in the run~10 data. 
%The constraint on \dcp~ has not changed compared to the previous analysis. 
\textcolor{blue}{The conclusion on values of \dcp~ has not changed compared to the previous analysis: if we consider the impact of FDS we cannot exclude CP conservation at 90\% CL. In this iteration, we have included a FDS to test the observed excess of events in the low momentum bin of the 1Re-1d.e. sample. Also this study confirms we cannot exclude CP conservation at 90\% CL. The Feldman-Cousins $2\sigma$ CL for \dcp~ is [-$\pi$, -0.13] $\cup$ [3.06, $\pi$] at NH, not excluding the CP-conserving value of \dcp $= \pi$ like in the previous analysis (\cref{fig:FDSdCPopposite}).}
%
The corresponding $3\sigma$ confidence interval is still closed at [-$\pi$, 0.43] $\cup$ [2.54, $\pi$]. The constraint on \dcp is still stronger than our sensitivity, but the constraint on both \Dmthreetwo~ and \stwothree~ is slightly weaker than the sensitivity. The overall comparison with MaCh3 is shown in \cref{fig:summary}. As previously the upper octant is slightly preferred with RC while the lower octant is preferred using T2K data only. With respect to OA2022 the fitted $\sin^2\theta_{13}$ moves consistently a little up in the T2K-only data and $\sin^2\theta_{23}$ moves a little away from 0.5 both with and without the RC.

%The Feldman Cousins $1\sigma$ confidence interval on \stwothree is $[0.464,0.482] \cup [0.532,0.582]$ for NH, excluding maximal-mixing at this confidence level.
%As the previous analysis, we see both octants within the $1\sigma$ confidence regions.\\
%The impact of the numuCC1pi sample was checked again this year, and as in the previous analysis, it is very small on Asimov contours but visible on data fit contours. As a reminder, this is expected as most of the events in this sample are above the oscillation maximum in terms of reconstructed energy.

Finally, we show in \cref{fig:summary_datafit_Mach3} a comparison of oscillation parameters contours with MaCh3 between the current analysis and the previous one based on Run 1-10 for a subset of variables (full plot set in T2K-TN-462~\cite{TN462}.
A mild reduction in the error on $\delta_{CP}$ can be observed while the best fit remains very stable.
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{summary_figs/comparison_datanew-dataold.png}
    \caption{Comparison of oscillation parameter contours between the data fits, with the reactor constraint, of MaCh3 from the previous and current analyses. (Top) disappearance contours (bottom) appearance contours (left) normal hierarchy (right) inverted hierarchy. %\textcolor{blue}{Compare to Fig.1 and check consistency...}
    }
    \label{fig:summary_datafit_Mach3}
\end{figure}



==> authorlist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% T2K author list generated on Tue Jul 22 01:49:51 2025
% setting: extra = False
%         author list from archive (starting March 14 2025 until July 16 2025)
%         exemption(s) granted to: ashida,rgonzjim,jgrosa,gdmegias,jac,jgm,hmatthias,njachowicz,akumar,edatkin,martind,kniewczas,scap,vedantha,fcadoux,fsanchez,evila,amunoz,nova,pdunne,dlast,adrienblanchet,mkabirne,barker,morgan_wascko,bdl,vlglagolev,slava,mtzanov,kutter,lmachado,litchfieldp,egoodman,yyang,kiseevavi,akaboth,kmahtani,dseppala,acraplet,alex,kudenko,oleg,erofeev,kurochka,matveev,shaykhiev,greina,asrivast,nicklatham,nakahata,rubbiaa,laveder,mezzetto,Forza,mgrassi,damartin,denhaff,wilking
% Number of authors = 401
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Authors with their affiliation numbers
\author[1]{K.\,Abe}
\author[1]{S.\,Abe}
\author[2]{R.\,Akutsu}
\author[3]{H.\,Alarakia--Charles}
\author[4]{Y.I.\,Alj Hakim}
\author[5]{S.\,Alonso Monsalve}
\author[6]{L.\,Anthony}
\author[7]{S.\,Aoki}
\author[6]{K.A.\,Apte}
\author[8]{T.\,Arai}
\author[9]{T.\,Arihara}
\author[10]{S.\,Arimoto}
\author[11]{Y.\,Ashida}
\author[6]{E.T.\,Atkin}
\author[12]{N.\,Babu}
\author[13]{V.\,Baranov}
\author[14]{G.J.\,Barker}
\author[15]{G.\,Barr}
\author[15]{D.\,Barrow}
\author[16]{P.\,Bates}
\author[15]{L.\,Bathe--Peters}
\author[17]{M.\,Batkiewicz--Kwasniak}
\author[15]{N.\,Baudis}
\author[18]{V.\,Berardi}
\author[11]{L.\,Berns}
\author[12]{S.\,Bhattacharjee}
\author[19]{A.\,Blanchet}
\author[20,21]{A.\,Blondel}
\author[22]{P.M.M.\,Boistier}
\author[22]{S.\,Bolognesi}
\author[21]{S.\,Bordoni}
\author[14]{S.B.\,Boyd}
\author[23]{C.\,Bronner}
\author[24]{A.\,Bubak}
\author[25]{M.\,Buizza Avanzini}
\author[26]{J.A.\,Caballero}
\author[21]{F.\,Cadoux}
\author[18]{N.F.\,Calabria}
\author[27]{S.\,Cao}
\author[21]{S.\,Cap}
\author[25]{D.\,Carabadjac\thanks{also at Universit\'e Paris-Saclay}}
\author[4]{S.L.\,Cartwright}
\author[28]{M.P.\,Casado\thanks{also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain}}
\author[18]{M.G.\,Catanesi}
\author[29]{J.\,Chakrani}
\author[20]{A.\,Chalumeau}
\author[30]{D.\,Cherdack}
\author[31]{A.\,Chvirova}
\author[16]{J.\,Coleman}
\author[32]{G.\,Collazuol}
\author[33]{F.\,Cormier}
\author[6]{A.A.L.\,Craplet}
\author[34]{A.\,Cudd}
\author[32]{D.\,D'ago}
\author[20]{C.\,Dalmazzone}
\author[22]{T.\,Daret}
\author[35]{P.\,Dasgupta}
\author[36]{C.\,Davis}
\author[13]{Yu.I.\,Davydov}
\author[37]{P.\,de Perio}
\author[38]{G.\,De Rosa}
\author[3]{T.\,Dealtry}
\author[39]{C.\,Densham}
\author[31]{A.\,Dergacheva}
\author[40]{R.\,Dharmapal Banerjee}
\author[41]{F.\,Di Lodovico}
\author[20]{G.\,Diaz Lopez}
\author[19]{S.\,Dolan}
\author[21]{D.\,Douqa}
\author[15]{T.A.\,Doyle}
\author[25]{O.\,Drapier}
\author[15]{K.E.\,Duffy}
\author[20]{J.\,Dumarchez}
\author[6]{P.\,Dunne}
\author[42]{K.\,Dygnarowicz}
\author[8]{A.\,Eguchi}
\author[43]{J.\,Elias}
\author[22]{S.\,Emery--Schrenk}
\author[31]{G.\,Erofeev}
\author[25]{A.\,Ershova}
\author[22]{G.\,Eurin}
\author[31]{D.\,Fedorova}
\author[31]{S.\,Fedotov}
\author[32]{M.\,Feltre}
\author[10]{L.\,Feng}
\author[8]{D.\,Ferlewicz}
\author[3]{A.J.\,Finch}
\author[39]{M.D.\,Fitton}
\author[32]{C.\,Forza}
\author[2]{M.\,Friend\thanks{also at J-PARC, Tokai, Japan}}
\author[2]{Y.\,Fujii\thanks{also at J-PARC, Tokai, Japan}}
\author[44]{Y.\,Fukuda}
\author[9]{Y.\,Furui}
\author[45]{J.\,Garc\'ia--Marcos}
\author[36]{A.C.\,Germer}
\author[21]{L.\,Giannessi}
\author[20]{C.\,Giganti}
\author[46]{M.\,Girgus}
\author[13]{V.\,Glagolev}
\author[47]{M.\,Gonin}
\author[26]{R.\,Gonz\'alez Jim\'enez}
\author[26]{J.\,Gonz\'alez Rosa}
\author[48]{E.A.G.\,Goodman}
\author[31]{K.\,Gorshanov}
\author[47]{P.\,Govindaraj}
\author[32]{M.\,Grassi}
\author[20]{M.\,Guigue}
\author[49]{F.Y.\,Guo}
\author[14]{D.R.\,Hadley}
\author[10,50]{S.\,Han}
\author[51]{D.A.\,Harris}
\author[3,39]{R.J.\,Harris}
\author[2]{T.\,Hasegawa\thanks{also at J-PARC, Tokai, Japan}}
\author[19]{C.M.\,Hasnip}
\author[22]{S.\,Hassani}
\author[2]{N.C.\,Hastings}
\author[1,37]{Y.\,Hayato}
\author[11]{I.\,Heitkamp}
\author[22]{D.\,Henaff}
\author[2]{Y.\,Hino}
\author[24]{J.\,Holeczek}
\author[39]{A.\,Holin}
\author[15]{T.\,Holvey}
\author[52]{N.T.\,Hong Van}
\author[53]{T.\,Honjo}
\author[45]{M.C.F.\,Hooft}
\author[1]{K.\,Hosokawa}
\author[10]{J.\,Hu}
\author[11]{A.K.\,Ichikawa}
\author[1]{K.\,Ieki}
\author[1]{M.\,Ikeda}
\author[11]{T.H.\,Ishida}
\author[2]{T.\,Ishida\thanks{also at J-PARC, Tokai, Japan}}
\author[54]{M.\,Ishitsuka}
\author[7]{H.\,Ito}
\author[23]{S.\,Ito}
\author[31]{A.\,Izmaylov}
\author[45]{N.\,Jachowicz}
\author[16]{S.J.\,Jenkins}
\author[19]{C.\,Jes\'us--Valls}
\author[49]{M.\,Jia}
\author[49]{J.J.\,Jiang}
\author[49]{J.Y.\,Ji}
\author[3]{T.P.\,Jones}
\author[6]{P.\,Jonsson}
\author[22]{S.\,Joshi}
\author[6]{M.\,Kabirnezhad}
\author[55]{A.C.\,Kaboth}
\author[9]{H.\,Kakuno}
\author[1]{J.\,Kameda}
\author[21]{S.\,Karpova}
\author[21]{V.S.\,Kasturi}
\author[1]{Y.\,Kataoka}
\author[41]{T.\,Katori}
\author[56]{A.\,Kawabata}
\author[53]{Y.\,Kawamura}
\author[10]{M.\,Kawaue}
\author[57]{E.\,Kearns\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}
\author[31]{M.\,Khabibullin}
\author[31]{A.\,Khotjantsev}
\author[10]{T.\,Kikawa}
\author[41]{S.\,King}
\author[13]{V.\,Kiseeva}
\author[24]{J.\,Kisiel}
\author[6]{A.\,Klustov\'a}
\author[4]{L.\,Kneale}
\author[8]{H.\,Kobayashi}
\author[11]{Sota.R\,Kobayashi}
\author[58]{L.\,Koch}
\author[8]{S.\,Kodama}
\author[31]{M.\,Kolupanova}
\author[33]{A.\,Konaka}
\author[3]{L.L.\,Kormos}
\author[59]{Y.\,Koshio\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}
\author[60]{K.\,Kowalik}
\author[31]{Y.\,Kudenko\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}}
\author[23]{Y.\,Kudo}
\author[45]{A.\,Kumar Jha}
\author[42]{R.\,Kurjata}
\author[31]{V.\,Kurochka}
\author[12]{T.\,Kutter}
\author[61]{L.\,Labarga}
\author[43]{M.\,Lachat}
\author[5]{K.\,Lachner}
\author[60]{J.\,Lagoda}
\author[24]{S.M.\,Lakshmi}
\author[14]{M.\,Lamers James}
\author[38]{A.\,Langella}
\author[55]{D.H.\,Langridge}
\author[22]{J.--F.\,Laporte}
\author[43]{D.\,Last}
\author[41]{N.\,Latham}
\author[32]{M.\,Laveder}
\author[38]{L.\,Lavitola}
\author[3]{M.\,Lawe}
\author[62]{D.\,Leon Silverio}
\author[32]{S.\,Levorato}
\author[41]{S.V.\,Lewis}
\author[5]{B.\,Li}
\author[6]{C.\,Lin}
\author[48]{R.P.\,Litchfield}
\author[49]{S.L.\,Liu}
\author[15]{W.\,Li}
\author[32]{A.\,Longhin}
\author[41]{A.\,Lopez Moreno}
\author[63]{L.\,Ludovici}
\author[14]{X.\,Lu}
\author[28]{T.\,Lux}
\author[48]{L.N.\,Machado}
\author[18]{L.\,Magaletti}
\author[64]{K.\,Mahn}
\author[49]{K.K.\,Mahtani}
\author[43]{S.\,Manly}
\author[34]{A.D.\,Marino}
\author[6]{D.G.R.\,Martin}
\author[62]{D.A.\,Martinez Caicedo}
\author[28]{L.\,Martinez}
\author[20]{M.\,Martini\thanks{also at IPSA-DRII, France}}
\author[2]{T.\,Matsubara}
\author[65]{R.\,Matsumoto}
\author[31]{V.\,Matveev}
\author[36]{C.\,Mauger}
\author[16]{K.\,Mavrokoridis}
\author[16]{N.\,McCauley}
\author[43]{K.S.\,McFarland}
\author[49]{C.\,McGrew}
\author[6]{J.\,McKean}
\author[31]{A.\,Mefodiev}
\author[26]{G.D.\,Megias}
\author[64]{L.\,Mellet}
\author[16]{C.\,Metelko}
\author[32]{M.\,Mezzetto}
\author[1]{S.\,Miki}
\author[48]{V.\,Mikola}
\author[28]{E.W.\,Miller}
\author[23]{A.\,Minamino}
\author[31]{O.\,Mineev}
\author[1,66]{S.\,Mine}
\author[57]{J.\,Mirabito}
\author[1]{M.\,Miura\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}
\author[1]{S.\,Moriyama\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}
\author[23]{S.\,Moriyama}
\author[48]{P.\,Morrison}
\author[25]{Th.A.\,Mueller}
\author[30]{D.\,Munford}
\author[25,47]{A.\,Mu\~noz}
\author[19]{L.\,Munteanu}
\author[35]{Y.\,Nagai}
\author[2]{T.\,Nakadaira\thanks{also at J-PARC, Tokai, Japan}}
\author[8]{K.\,Nakagiri}
\author[1,37]{M.\,Nakahata}
\author[8]{Y.\,Nakajima}
\author[11]{K.D.\,Nakamura}
\author[11]{A.\,Nakano}
\author[67]{Y.\,Nakano}
\author[1,37]{S.\,Nakayama}
\author[10,37]{T.\,Nakaya}
\author[2]{K.\,Nakayoshi\thanks{also at J-PARC, Tokai, Japan}}
\author[6]{C.E.R.\,Naseby}
\author[68]{D.T.\,Nguyen}
\author[25]{V.Q.\,Nguyen}
\author[45]{K.\,Niewczas}
\author[2]{S.\,Nishimori}
\author[56]{Y.\,Nishimura}
\author[1]{Y.\,Noguchi}
\author[60]{T.\,Nosek}
\author[39]{F.\,Nova}
\author[6]{J.C.\,Nugent}
\author[3]{H.M.\,O'Keeffe}
\author[58]{L.\,O'Sullivan}
\author[56]{R.\,Okazaki}
\author[8]{W.\,Okinaga}
\author[50,37]{K.\,Okumura}
\author[53]{T.\,Okusawa}
\author[10]{N.\,Onda}
\author[18]{N.\,Ospina}
\author[25]{L.\,Osu}
\author[10]{N.\,Otani}
\author[2]{Y.\,Oyama\thanks{also at J-PARC, Tokai, Japan}}
\author[69]{V.\,Paolone}
\author[6]{J.\,Pasternak}
\author[16]{D.\,Payne}
\author[4]{T.P.D.\,Peacock}
\author[6]{M.\,Pfaff}
\author[39]{L.\,Pickering}
\author[20]{B.\,Popov\thanks{also at JINR, Dubna, Russia}}
\author[2]{A.J.\,Portocarrero Yrey}
\author[46]{M.\,Posiadala--Zezula}
\author[46]{Y.S.\,Prabhu}
\author[40]{H.\,Prasad}
\author[32]{F.\,Pupilli}
\author[47,25]{B.\,Quilain}
\author[27]{P.T.\,Quyen\thanks{also at the Graduate University of Science and Technology, Vietnam Academy of Science and Technology}}
\author[18]{E.\,Radicioni}
\author[51]{B.\,Radics}
\author[36]{M.A.\,Ramirez}
\author[41]{R.\,Ramsden}
\author[3]{P.N.\,Ratoff}
\author[34]{M.\,Reh}
\author[58]{G.\,Reina}
\author[49]{C.\,Riccio}
\author[48]{D.W.\,Riley}
\author[60]{E.\,Rondio}
\author[70]{S.\,Roth}
\author[51]{N.\,Roy}
\author[5]{A.\,Rubbia}
\author[20]{L.\,Russo}
\author[42]{A.\,Rychter}
\author[20]{W.\,Saenz}
\author[2]{K.\,Sakashita\thanks{also at J-PARC, Tokai, Japan}}
\author[21]{S.\,Samani}
\author[21]{F.\,S\'anchez}
\author[16]{E.M.\,Sandford}
\author[54]{Y.\,Sato}
\author[12]{T.\,Schefke}
\author[71]{K.\,Scholberg\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}
\author[6]{M.\,Scott}
\author[53]{Y.\,Seiya\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}}
\author[2]{T.\,Sekiguchi\thanks{also at J-PARC, Tokai, Japan}}
\author[1,37]{H.\,Sekiya\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}
\author[9]{T.\,Sekiya}
\author[64]{D.\,Seppala}
\author[5]{D.\,Sgalaberna}
\author[31]{A.\,Shaikhiev}
\author[1,37]{M.\,Shiozawa}
\author[59]{Y.\,Shiraishi}
\author[31]{A.\,Shvartsman}
\author[31]{N.\,Skrobova}
\author[55]{K.\,Skwarczynski}
\author[70]{D.\,Smyczek}
\author[66]{M.\,Smy}
\author[40]{J.T.\,Sobczyk}
\author[66,37]{H.\,Sobel}
\author[48]{F.J.P.\,Soler}
\author[3]{A.J.\,Speers}
\author[18]{R.\,Spina}
\author[58]{A.\,Srivastava}
\author[4]{P.\,Stowell}
\author[31]{Y.\,Stroke}
\author[13]{I.A.\,Suslov}
\author[7]{A.\,Suzuki}
\author[2]{S.Y.\,Suzuki\thanks{also at J-PARC, Tokai, Japan}}
\author[2]{M.\,Tada\thanks{also at J-PARC, Tokai, Japan}}
\author[11]{S.\,Tairafune}
\author[1]{A.\,Takeda}
\author[7,37]{Y.\,Takeuchi}
\author[59]{K.\,Takeya}
\author[1]{H.K.\,Tanaka\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}
\author[2]{H.\,Tanigawa}
\author[13]{V.V.\,Tereshchenko}
\author[70]{N.\,Thamm}
\author[16]{C.\,Touramanis}
\author[10]{N.\,Tran}
\author[2]{T.\,Tsukamoto\thanks{also at J-PARC, Tokai, Japan}}
\author[12]{M.\,Tzanov}
\author[6]{Y.\,Uchida}
\author[37,66]{M.\,Vagins}
\author[28]{M.\,Varghese}
\author[13]{I.\,Vasilyev}
\author[22]{G.\,Vasseur}
\author[19,21]{E.\,Villa}
\author[20]{U.\,Virginet}
\author[39]{T.\,Vladisavljevic}
\author[17]{T.\,Wachala}
\author[7]{S.--i.\,Wada}
\author[11]{D.\,Wakabayashi}
\author[4]{H.T.\,Wallace}
\author[64]{J.G.\,Walsh}
\author[39,15]{D.\,Wark}
\author[15,39]{M.O.\,Wascko}
\author[58]{A.\,Weber}
\author[10]{R.\,Wendell}
\author[72]{M.J.\,Wilking}
\author[29]{C.\,Wilkinson}
\author[41]{J.R.\,Wilson}
\author[29]{K.\,Wood}
\author[6]{C.\,Wret}
\author[73]{J.\,Xia}
\author[53]{K.\,Yamamoto\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}}
\author[53]{T.\,Yamamoto}
\author[49]{C.\,Yanagisawa\thanks{also at BMCC/CUNY, Science Department, New York, New York, U.S.A.}}
\author[15]{Y.\,Yang}
\author[1]{T.\,Yano}
\author[31]{N.\,Yershov}
\author[49]{U.\,Yevarouskaya}
\author[8]{M.\,Yokoyama\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}
\author[8]{Y.\,Yoshimoto}
\author[10]{N.\,Yoshimura}
\author[51]{R.\,Zaki}
\author[17]{A.\,Zalewska}
\author[60]{J.\,Zalipska}
\author[17]{G.\,Zarnecki}
\author[33,74]{J.\,Zhang}
\author[5]{X.Y.\,Zhao}
\author[49]{H.\,Zheng}
\author[7]{H.\,Zhong}
\author[6]{T.\,Zhu}
\author[42]{M.\,Ziembicki}
\author[34]{E.D.\,Zimmerman}
\author[20]{M.\,Zito}
\author[41]{S.\,Zsoldos}

% Affiliations
\affil[1]{University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}
\affil[2]{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}
\affil[3]{Lancaster University, Physics Department, Lancaster, United Kingdom}
\affil[4]{University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom}
\affil[5]{ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland}
\affil[6]{Imperial College London, Department of Physics, London, United Kingdom}
\affil[7]{Kobe University, Kobe, Japan}
\affil[8]{University of Tokyo, Department of Physics, Tokyo, Japan}
\affil[9]{Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}
\affil[10]{Kyoto University, Department of Physics, Kyoto, Japan}
\affil[11]{Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan}
\affil[12]{Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}
\affil[13]{Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia}
\affil[14]{University of Warwick, Department of Physics, Coventry, United Kingdom}
\affil[15]{Oxford University, Department of Physics, Oxford, United Kingdom}
\affil[16]{University of Liverpool, Department of Physics, Liverpool, United Kingdom}
\affil[17]{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}
\affil[18]{INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}
\affil[19]{CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland}
\affil[20]{Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}
\affil[21]{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}
\affil[22]{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affil[23]{Yokohama National University, Department of Physics, Yokohama, Japan}
\affil[24]{University of Silesia, Institute of Physics, Katowice, Poland}
\affil[25]{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France}
\affil[26]{Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain}
\affil[27]{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}
\affil[28]{Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}
\affil[29]{Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.}
\affil[30]{University of Houston, Department of Physics, Houston, Texas, U.S.A.}
\affil[31]{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}
\affil[32]{INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}
\affil[33]{TRIUMF, Vancouver, British Columbia, Canada}
\affil[34]{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}
\affil[35]{E\"{o}tv\"{o}s Lor\'{a}nd University, Department of Atomic Physics, Budapest, Hungary}
\affil[36]{University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.}
\affil[37]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}
\affil[38]{INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}
\affil[39]{STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}
\affil[40]{Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}
\affil[41]{King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom}
\affil[42]{Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland}
\affil[43]{University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}
\affil[44]{Miyagi University of Education, Department of Physics, Sendai, Japan}
\affil[45]{Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium}
\affil[46]{University of Warsaw, Faculty of Physics, Warsaw, Poland}
\affil[47]{ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}
\affil[48]{University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom}
\affil[49]{State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}
\affil[50]{University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}
\affil[51]{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}

==> authorlist_20260923.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% T2K author list generated on Mon Sep 28 14:55:29 2026
% setting: extra = False
%         author list from archive (starting March 14 2025 until October 06 2026)
%         exemption(s) granted to: jacdz,akumar,alexrd,mccauley,mbuizza,munteanu,khomutov,melbaz,ateklu,alpinist,jgrosa,gdmegias,jac,jgm,hmatthias,edatkin,martind,kniewczas,adrienblanchet,mkabirne,morgan_wascko,bdl,vlglagolev,slava,kiseevavi,kurochka,shaykhiev,rubbiaa,laveder,damartin,wilking,ateklu,alpinist,naokiotani,tvngoc,ashida,rgonzjim,jgrosa,gdmegias,jac,jgm,hmatthias,njachowicz,akumar,edatkin,martind,kniewczas,scap,vedantha,fsanchez,evila,amunoz,nova,pdunne,dlast,adrienblanchet,mkabirne,barker,morgan_wascko,bdl,vlglagolev,slava,mtzanov,kutter,lmachado,litchfieldp,egoodman,yyang,kiseevavi,akaboth,kmahtani,dseppala,acraplet,alex,kudenko,oleg,erofeev,kurochka,matveev,shaykhiev,greina,asrivast,nicklatham,nakahata,rubbiaa,laveder,mezzetto,Forza,mgrassi,damartin,denhaff,wilking
% Number of authors = 442
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\INSTHD}{\affiliation{University Autonoma Madrid, Department of Theoretical Physics, 28049 Madrid, Spain}}
\newcommand{\INSTFE}{\affiliation{Boston University, Department of Physics, Boston, Massachusetts, U.S.A.}}
\newcommand{\INSTD}{\affiliation{University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada}}
\newcommand{\INSTGA}{\affiliation{University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.}}
\newcommand{\INSTI}{\affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}}
\newcommand{\INSTGB}{\affiliation{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}}
\newcommand{\INSTFH}{\affiliation{Duke University, Department of Physics, Durham, North Carolina, U.S.A.}}
\newcommand{\INSTEF}{\affiliation{ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland}}
\newcommand{\INSTIG}{\affiliation{VNU University of Science, Vietnam National University, Hanoi, Vietnam}}
\newcommand{\INSTIE}{\affiliation{CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland}}
\newcommand{\INSTEG}{\affiliation{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}}
\newcommand{\INSTHJ}{\affiliation{University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom}}
\newcommand{\INSTJG}{\affiliation{Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium}}
\newcommand{\INSTDG}{\affiliation{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}}
\newcommand{\INSTCB}{\affiliation{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}}
\newcommand{\INSTIB}{\affiliation{University of Houston, Department of Physics, Houston, Texas, U.S.A.}}
\newcommand{\INSTED}{\affiliation{Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}}
\newcommand{\INSTJC}{\affiliation{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Staudingerweg 7, 55128 Mainz, Germany}}
\newcommand{\INSTHH}{\affiliation{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}}
\newcommand{\INSTEI}{\affiliation{Imperial College London, Department of Physics, London, United Kingdom}}
\newcommand{\INSTGF}{\affiliation{INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}}
\newcommand{\INSTBE}{\affiliation{INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}}
\newcommand{\INSTBF}{\affiliation{INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}}
\newcommand{\INSTBD}{\affiliation{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy}}
\newcommand{\INSTEB}{\affiliation{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}}
\newcommand{\INSTHI}{\affiliation{International Centre of Physics, Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), 10 Dao Tan, Ba Dinh, Hanoi, Vietnam}}
\newcommand{\INSTJD}{\affiliation{ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}}
\newcommand{\INSTHA}{\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}}
\newcommand{\INSTID}{\affiliation{Keio University, Department of Physics, Kanagawa, Japan}}
\newcommand{\INSTIF}{\affiliation{King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom}}
\newcommand{\INSTCC}{\affiliation{Kobe University, Kobe, Japan}}
\newcommand{\INSTCD}{\affiliation{Kyoto University, Department of Physics, Kyoto, Japan}}
\newcommand{\INSTEJ}{\affiliation{Lancaster University, School of Physics and Astronomy, Lancaster, United Kingdom}}
\newcommand{\INSTII}{\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.}}
\newcommand{\INSTBA}{\affiliation{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France}}
\newcommand{\INSTFC}{\affiliation{University of Liverpool, Department of Physics, Liverpool, United Kingdom}}
\newcommand{\INSTFI}{\affiliation{Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}}
\newcommand{\INSTIH}{\affiliation{Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia}}
\newcommand{\INSTHB}{\affiliation{Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.}}
\newcommand{\INSTCE}{\affiliation{Miyagi University of Education, Department of Physics, Sendai, Japan}}
\newcommand{\INSTDF}{\affiliation{National Centre for Nuclear Research, Warsaw, Poland}}
\newcommand{\INSTFJ}{\affiliation{State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}}
\newcommand{\INSTEH}{\affiliation{STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}}
\newcommand{\INSTGJ}{\affiliation{Okayama University, Department of Physics, Okayama, Japan}}
\newcommand{\INSTCF}{\affiliation{Osaka Metropolitan University, Department of Physics, Osaka, Japan}}
\newcommand{\INSTGG}{\affiliation{Oxford University, Department of Physics, Oxford, United Kingdom}}
\newcommand{\INSTIC}{\affiliation{University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.}}
\newcommand{\INSTGC}{\affiliation{University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.}}
\newcommand{\INSTGD}{\affiliation{University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}}
\newcommand{\INSTHC}{\affiliation{Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom}}
\newcommand{\INSTBC}{\affiliation{RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany}}
\newcommand{\INSTJF}{\affiliation{School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota, U.S.A.}}
\newcommand{\INSTJB}{\affiliation{Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain}}
\newcommand{\INSTFB}{\affiliation{University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom}}
\newcommand{\INSTDI}{\affiliation{University of Silesia, Institute of Physics, Katowice, Poland}}
\newcommand{\INSTIA}{\affiliation{SLAC National Accelerator Laboratory, Stanford University, Menlo Park, California, U.S.A.}}
\newcommand{\INSTBB}{\affiliation{Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}}
\newcommand{\INSTJE}{\affiliation{South Dakota School of Mines and Technology, 501 East Saint Joseph Street, Rapid City, SD 57701, United States}}
\newcommand{\INSTCH}{\affiliation{University of Tokyo, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTBJ}{\affiliation{University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}}
\newcommand{\INSTCG}{\affiliation{University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}}
\newcommand{\INSTHF}{\affiliation{Institute of Science Tokyo, Department of Physics, Tokyo}}
\newcommand{\INSTGI}{\affiliation{Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTHG}{\affiliation{Tokyo University of Science, Faculty of Science and Technology, Department of Physics, Noda, Chiba, Japan}}
\newcommand{\INSTB}{\affiliation{TRIUMF, Vancouver, British Columbia, Canada}}
\newcommand{\INSTJH}{\affiliation{University of Toyama, Faculty of Science, Toyama, Japan}}
\newcommand{\INSTJJ}{\affiliation{University of Tsukuba, Faculty of Pure and Applied Sciences, Tsukuba, Ibaraki, Japan}}
\newcommand{\INSTDJ}{\affiliation{University of Warsaw, Faculty of Physics, Warsaw, Poland}}
\newcommand{\INSTDH}{\affiliation{Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland}}
\newcommand{\INSTIJ}{\affiliation{Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan}}
\newcommand{\INSTFD}{\affiliation{University of Warwick, Department of Physics, Coventry, United Kingdom}}
\newcommand{\INSTEA}{\affiliation{Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}}
\newcommand{\INSTHE}{\affiliation{Yokohama National University, Department of Physics, Yokohama, Japan}}
\newcommand{\INSTH}{\affiliation{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}}

\INSTHD
\INSTFE
\INSTD
\INSTGA
\INSTI
\INSTGB
\INSTFH
\INSTEF
\INSTIG
\INSTIE
\INSTEG
\INSTHJ
\INSTJG
\INSTDG
\INSTCB
\INSTIB
\INSTED
\INSTJC
\INSTHH
\INSTEI
\INSTGF
\INSTBE
\INSTBF
\INSTBD
\INSTEB
\INSTHI
\INSTJD
\INSTHA
\INSTID
\INSTIF
\INSTCC
\INSTCD
\INSTEJ
\INSTII
\INSTBA
\INSTFC
\INSTFI
\INSTIH
\INSTHB
\INSTCE
\INSTDF
\INSTFJ
\INSTEH
\INSTGJ
\INSTCF
\INSTGG
\INSTIC
\INSTGC
\INSTGD
\INSTHC
\INSTBC
\INSTJF
\INSTJB
\INSTFB
\INSTDI
\INSTIA
\INSTBB
\INSTJE
\INSTCH
\INSTBJ
\INSTCG
\INSTHF
\INSTGI
\INSTHG
\INSTB
\INSTJH
\INSTJJ
\INSTDJ
\INSTDH
\INSTIJ
\INSTFD
\INSTEA
\INSTHE
\INSTH

\author{K.\,Abe}\INSTBJ
\author{S.\,Abe}\INSTBJ
\author{H.\,Adhikary}\INSTDJ
\author{R.\,Akutsu}\INSTCB
\author{H.\,Alarakia-Charles}\INSTEJ
\author{Y.I.\,Alj Hakim}\INSTFB
\author{S.\,Alonso Monsalve}\INSTEF
\author{L.\,Anthony}\INSTEI
\author{S.\,Aoki}\INSTCC
\author{K.A.\,Apte}\INSTEI
\author{T.\,Arai}\INSTCH
\author{T.\,Arihara}\INSTGI
\author{S.\,Arimoto}\INSTCD
\author{Y.\,Asami}\INSTGI
\author{Y.\,Asaoka}\INSTBJ
\author{Y.\,Ashida}\INSTIJ
\author{E.T.\,Atkin}\INSTEI
\author{N.\,Babu}\INSTFI
\author{V.\,Baranov}\INSTIH
\author{G.J.\,Barker}\INSTFD
\author{G.\,Barr}\INSTGG
\author{D.\,Barrow}\INSTGG
\author{P.\,Bates}\INSTFC
\author{L.\,Bathe-Peters}\INSTGG
\author{M.\,Batkiewicz-Kwasniak}\INSTDG
\author{N.\,Baudis}\INSTGG
\author{A.\,Beliakova}\INSTEB
\author{V.\,Berardi}\INSTGF
\author{L.\,Berns}\INSTIJ
\author{S.\,Bhattacharjee}\INSTFI
\author{A.\,Blanchet}\INSTBB
\author{A.\,Blondel}\INSTBB\INSTEG
\author{L.\,B{\o}e}\INSTIB
\author{P.M.M.\,Boistier}\INSTI
\author{S.\,Bolognesi}\INSTI
\author{B.\,Bombin}\INSTEB
\author{S.\,Bordoni }\INSTEG
\author{S.B.\,Boyd}\INSTFD
\author{C.\,Bronner}\INSTHE
\author{A.\,Bubak}\INSTDI
\author{M.\,Buizza Avanzini}\INSTBA
\author{J.A.\,Caballero}\INSTJB
\author{N.F.\,Calabria}\INSTGF
\author{S.\,Cao}\INSTHH
\author{S.\,Cap}\INSTEG
\author{D.\,Carabadjac}\thanks{also at Universit\'e Paris-Saclay}\INSTBA
\author{S.L.\,Cartwright}\INSTFB
\author{M.P.\,Casado}\thanks{also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain}\INSTED
\author{M.G.\,Catanesi}\INSTGF
\author{J.\,Chakrani}\INSTII
\author{A.\,Chalumeau}\INSTBB
\author{D.\,Cherdack}\INSTIB
\author{A.\,Chvirova}\INSTEB
\author{J.\,Coleman}\INSTFC
\author{G.\,Collazuol}\INSTBF
\author{F.\,Cormier}\INSTB
\author{A.A.L.\,Craplet}\INSTEI
\author{A.\,Cudd}\INSTGB
\author{D.\,D'Ago}\INSTBF
\author{C.\,Dalmazzone}\INSTBB
\author{T.\,Daret}\INSTI
\author{P.\,Dasgupta}\INSTED
\author{C.\,Davis}\INSTIC
\author{Yu.I.\,Davydov}\INSTIH
\author{P.\,de Perio}\INSTHA
\author{G.\,De Rosa}\INSTBE
\author{T.\,Dealtry}\INSTEJ
\author{C.\,Densham}\INSTEH
\author{A.\,Dergacheva}\INSTEB
\author{R.\,Dharmapal Banerjee}\INSTEA
\author{F.\,Di Lodovico}\INSTIF
\author{G.\,Diaz Lopez}\INSTBB
\author{S.\,Dolan}\INSTIE
\author{D.\,Douqa}\INSTEG
\author{T.A.\,Doyle}\INSTGG
\author{O.\,Drapier}\INSTBA
\author{K.E.\,Duffy}\INSTGG
\author{J.\,Dumarchez}\INSTBB
\author{P.\,Dunne}\INSTEI
\author{K.\,Dygnarowicz}\INSTDH
\author{A.\,Eguchi}\INSTCH
\author{M.\,El Baz}\INSTEG
\author{J.\,Elias}\INSTGD
\author{S.\,Emery-Schrenk}\INSTI
\author{G.\,Erofeev}\INSTEB
\author{A.\,Ershova}\INSTBA
\author{G.\,Eurin}\INSTI
\author{M.\,Fani}\INSTJF
\author{D.\,Fedorova}\INSTEB
\author{S.\,Fedotov}\INSTEB
\author{M.\,Feltre}\INSTBF
\author{C.\,Fengler}\INSTGG
\author{L.\,Feng}\INSTCD
\author{D.\,Ferlewicz}\INSTBB
\author{A.J.\,Finch}\INSTEJ
\author{M.D.\,Fitton}\INSTEH
\author{C.\,Forza}\INSTBF
\author{M.\,Friend}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{Y.\,Fujii}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{Y.\,Fukuda}\INSTCE
\author{N.\,Funayama}\INSTCF
\author{Y.\,Furui}\INSTGI
\author{A.N.\,Gaci\~no Olmedo}\INSTBB
\author{J.\,Garc\'ia-Marcos}\INSTJG
\author{A.C.\,Germer}\INSTIC
\author{L.\,Giannessi}\INSTEG
\author{C.\,Giganti}\INSTBB
\author{M.\,Girgus}\INSTDJ
\author{V.\,Glagolev}\INSTIH
\author{P.\,Golak}\INSTDJ
\author{M.\,Gonin}\INSTJD
\author{R.\,Gonzalez Jimenez}\INSTJB
\author{J.\,Gonz\'alez Rosa}\INSTJB
\author{E.A.G.\,Goodman}\INSTHJ
\author{K.\,Gorshanov}\INSTEB
\author{P.\,Govindaraj}\INSTDJ
\author{M.\,Grassi}\INSTBF
\author{M.\,Guigue}\INSTBB
\author{F.Y.\,Guo}\INSTFJ
\author{D.R.\,Hadley}\INSTFD
\author{S.\,Han}\INSTCD\INSTCG
\author{D.A.\,Harris}\INSTH
\author{R.J.\,Harris}\INSTEJ\INSTEH
\author{M.\,Hartz}\INSTB\INSTHA
\author{K.\,Hasegawa}\INSTCD
\author{T.\,Hasegawa}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{C.M.\,Hasnip}\INSTIE
\author{S.\,Hassani}\INSTI
\author{N.C.\,Hastings}\INSTCB
\author{K.\,Hayashi}\INSTCD
\author{Y.\,Hayato}\INSTBJ\INSTHA
\author{I.\,Heitkamp}\INSTIJ
\author{D.\,Henaff}\INSTI
\author{Y.\,Hino}\INSTCB
\author{K.\,Hiraide}\INSTBJ\INSTHA
\author{J.\,Holeczek}\INSTDI
\author{A.\,Holin}\INSTEH
\author{T.\,Holvey}\INSTGG
\author{N.T.\,Hong Van}\INSTHI
\author{T.\,Honjo}\INSTCF
\author{M.C.F.\,Hooft}\INSTJG
\author{K.\,Hosokawa}\INSTBJ
\author{R.\,Huang}\INSTII
\author{J.\,Hu}\INSTCD
\author{A.K.\,Ichikawa}\INSTIJ
\author{K.\,Ieki}\INSTBJ
\author{M.\,Ikeda}\INSTBJ
\author{K.\,Indo}\INSTCD
\author{T.H.\,Ishida}\INSTIJ
\author{T.\,Ishida}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Ishitsuka}\INSTHG
\author{H.\,Ito}\INSTCC
\author{S.\,Ito}\INSTHE
\author{A.\,Izmaylov}\INSTEB
\author{N.\,Jachowicz}\INSTJG
\author{B.\,Jargowsky}\INSTFE
\author{S.J.\,Jenkins}\INSTFC
\author{C.\,Jes\'us-Valls}\INSTIE
\author{M.\,Jia}\INSTFJ
\author{J.J.\,Jiang}\INSTFJ
\author{J.Y.\,Ji}\INSTFJ
\author{T.P.\,Jones}\INSTEJ
\author{P.\,Jonsson}\INSTEI
\author{S.\,Joshi}\INSTFJ
\author{C.K.\,Jung}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFJ
\author{M.\,Kabirnezhad}\INSTGG
\author{A.C.\,Kaboth}\INSTHC
\author{K.\,Kadota}\INSTCC
\author{H.\,Kakuno}\INSTGI
\author{A.\,Kamata}\INSTGI
\author{J.\,Kameda}\INSTBJ
\author{S.\,Karpova}\INSTEG
\author{V.S.\,Kasturi}\INSTEG
\author{Y.\,Kataoka}\INSTBJ
\author{T.\,Katori}\INSTIF
\author{A.\,Kawabata}\INSTID
\author{R.\,Kawabe}\INSTCF
\author{Y.\,Kawamura}\INSTCF
\author{M.\,Kawaue}\INSTCD
\author{E.\,Kearns}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFE
\author{M.\,Khabibullin}\INSTEB
\author{N.V.\,Khomutov}\INSTIH
\author{A.\,Khotjantsev}\INSTEB
\author{T.\,Kikawa}\INSTCD
\author{S.\,King}\INSTIF
\author{V.\,Kiseeva}\INSTIH
\author{J.\,Kisiel}\INSTDI
\author{A.\,Klustov\'a}\INSTEI
\author{L.\,Kneale}\INSTFB
\author{H.\,Kobayashi}\INSTCH
\author{S.R.\,Kobayashi}\INSTIJ
\author{T.\,Kobayashi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{L.\,Koch}\INSTJC
\author{S.\,Kodama}\INSTCH
\author{M.\,Kolupanova}\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}\INSTEB
\author{A.\,Konaka}\INSTB
\author{L.L.\,Kormos}\INSTEJ
\author{Y.\,Koshio}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTGJ
\author{K.\,Kowalik}\INSTDF
\author{R.\,Kralik}\INSTIF
\author{Y.\,Kudenko}\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}\INSTEB
\author{Y.\,Kudo}\INSTHE
\author{A.\,Kumar Jha}\INSTJG
\author{R.\,Kurjata}\INSTDH
\author{V.\,Kurochka}\INSTEB
\author{T.\,Kutter}\INSTFI
\author{L.\,Labarga}\INSTHD
\author{M.\,Lachat}\INSTGD
\author{K.\,Lachner}\INSTEF
\author{J.\,Lagoda}\INSTDF
\author{S.M.\,Lakshmi}\INSTDI
\author{M.\,Lamers James}\INSTFD
\author{A.\,Langella}\INSTBE
\author{D.H.\,Langridge}\INSTHC
\author{J.-F.\,Laporte}\INSTI
\author{D.\,Last}\INSTGD
\author{N.\,Latham}\INSTIF
\author{M.\,Laveder}\INSTBF
\author{L.\,Lavitola}\INSTBE
\author{M.\,Lawe}\INSTEJ
\author{A.\,Leclerc}\INSTI
\author{N.\,Lemaire}\INSTBA
\author{D.\,Leon Silverio}\INSTJE
\author{T.\,Leplumey}\INSTBA
\author{S.\,Levorato}\INSTBF
\author{S.V.\,Lewis}\INSTIF
\author{B.\,Li}\INSTEF
\author{C.\,Lin}\INSTEI
\author{R.P.\,Litchfield}\INSTHJ
\author{S.L.\,Liu}\INSTFJ
\author{W.\,Li}\INSTGG
\author{A.\,Longhin}\INSTBF
\author{A.\,Lopez Moreno}\INSTIF
\author{L.\,Ludovici}\INSTBD
\author{X.\,Lu}\INSTFD
\author{T.\,Lux}\INSTED
\author{L.N.\,Machado}\INSTHJ
\author{L.\,Magaletti}\INSTGF
\author{K.\,Mahn}\INSTHB
\author{K.K.\,Mahtani}\INSTFJ
\author{S.\,Manly}\INSTGD
\author{A.D.\,Marino}\INSTGB
\author{D.G.R.\,Martin}\INSTEI
\author{D.A.\,Martinez Caicedo}\INSTJE
\author{L.\,Martinez}\INSTED
\author{M.\,Martini}\thanks{also at IPSA-DRII, France}\INSTBB
\author{N.\,Mashin}\INSTEB
\author{T.\,Matsubara}\INSTCB
\author{R.\,Matsumoto}\INSTHF
\author{V.\,Matveev}\INSTEB
\author{C.\,Mauger}\INSTIC
\author{K.\,Mavrokoridis}\INSTFC
\author{N.\,McCauley}\INSTFC
\author{K.S.\,McFarland}\INSTGD
\author{C.\,McGrew}\INSTFJ
\author{J.\,McKean}\INSTCD
\author{A.\,Mefodiev}\INSTEB
\author{G.D.\,Megias }\INSTJB
\author{L.\,Mellet}\INSTHB
\author{C.\,Metelko}\INSTFC
\author{M.\,Mezzetto}\INSTBF
\author{S.\,Miki}\INSTBJ
\author{V.\,Mikola}\INSTHJ
\author{E.W.\,Miller}\INSTEI
\author{A.\,Minamino}\INSTHE
\author{O.\,Mineev}\INSTEB
\author{S.\,Mine}\INSTBJ\INSTGA
\author{J.\,Mirabito}\INSTFE
\author{M.\,Miura}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{S.\,Moriyama}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{S.\,Moriyama}\INSTHE
\author{P.\,Morrison}\INSTHJ
\author{Th.A.\,Mueller}\INSTBA
\author{D.\,Munford}\INSTIB
\author{A.\,Mu\~noz}\INSTJC
\author{L.\,Munteanu}\INSTIE
\author{Y.\,Nagai}\INSTCB
\author{T.\,Nakadaira}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{K.\,Nakagiri}\INSTBJ
\author{M.\,Nakahata}\INSTBJ\INSTHA
\author{Y.\,Nakajima}\INSTCH
\author{K.D.\,Nakamura}\INSTIJ
\author{A.\,Nakano}\INSTIJ
\author{Y.\,Nakano}\INSTJH
\author{S.\,Nakayama}\INSTBJ\INSTHA
\author{T.\,Nakaya}\INSTCD\INSTHA
\author{K.\,Nakayoshi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{C.E.R.\,Naseby}\INSTEI
\author{D.T.\,Nguyen}\INSTIG
\author{V.Q.\,Nguyen}\INSTBA
\author{K.\,Niewczas}\INSTBA\INSTJG
\author{S.\,Nishimori}\INSTCH
\author{Y.\,Nishimura}\INSTID
\author{Y.\,Noguchi}\INSTBJ
\author{T.\,Nosek}\INSTDF
\author{F.\,Nova}\INSTEH
\author{J.C.\,Nugent}\INSTEI
\author{H.M.\,O'Keeffe}\INSTEJ
\author{L.\,O'Sullivan}\INSTJC
\author{R.\,Okazaki}\INSTID
\author{W.\,Okinaga}\INSTCH
\author{K.\,Okumura}\INSTCG\INSTHA
\author{T.\,Okusawa}\INSTCF
\author{N.\,Onda}\INSTCD
\author{N.\,Ospina}\INSTGF
\author{L.\,Osu}\INSTBA
\author{N.\,Otani}\INSTCD
\author{Y.\,Oyama}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{V.\,Paolone}\INSTGC
\author{J.\,Pasternak}\INSTEI
\author{D.\,Payne}\INSTFC
\author{T.P.D.\,Peacock}\INSTFB
\author{M.\,Pfaff}\INSTEI
\author{L.\,Pickering}\INSTEH
\author{J.-B.\,Plan\c{c}on}\INSTBA
\author{P.\,Podlaski}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{B.\,Popov}\thanks{also at JINR, Dubna, Russia}\INSTBB
\author{A.J.\,Portocarrero Yrey}\INSTCB
\author{M.\,Posiadala-Zezula}\INSTDJ
\author{Y.S.\,Prabhu}\INSTDJ
\author{H.\,Prasad}\INSTEA
\author{F.\,Pupilli}\INSTBF
\author{B.\,Quilain}\INSTJD\INSTBA
\author{P.T.\,Quyen}\thanks{also at the Graduate University of Science and Technology, Vietnam Academy of Science and Technology}\INSTHH
\author{E.\,Radicioni}\INSTGF
\author{B.\,Radics}\INSTH
\author{M.A.\,Ramirez Delgado}\INSTIC
\author{R.\,Ramsden}\INSTIF
\author{P.N.\,Ratoff}\INSTEJ
\author{M.\,Reh}\INSTGB
\author{G.\,Reina}\INSTJC
\author{L.\,Restrepo}\INSTBB
\author{C.\,Riccio}\INSTFJ
\author{D.W.\,Riley}\INSTHJ
\author{E.\,Rondio}\INSTDF
\author{D.\,Ross}\INSTHB
\author{S.\,Roth}\INSTBC
\author{N.\,Roy}\INSTH
\author{A.\,Rubbia}\INSTEF
\author{L.\,Russo}\INSTBB
\author{A.\,Rychter}\INSTDH
\author{W.\,Saenz}\INSTBB
\author{K.\,Sakashita}\thanks{also at J-PARC, Tokai, Japan}\INSTJJ\INSTCB
\author{S.\,Samani}\INSTEG
\author{F.\,S\'anchez}\INSTEG
\author{E.M.\,Sandford}\INSTFC
\author{Y.\,Sato}\INSTHG
\author{T.\,Schefke}\INSTFI
\author{K.\,Scholberg}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTFH
\author{M.\,Scott}\INSTEI
\author{Y.\,Seiya}\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}\INSTCF
\author{T.\,Sekiguchi}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{H.\,Sekiya}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ\INSTHA
\author{M.\,Sekiyama}\INSTCH
\author{T.\,Sekiya}\INSTGI
\author{D.\,Seppala}\INSTHB
\author{D.\,Sgalaberna}\INSTEF
\author{A.\,Shaikhiev}\INSTEB
\author{M.\,Shiozawa}\INSTBJ\INSTHA
\author{Y.\,Shiraishi}\INSTGJ
\author{N.\,Shvarev}\INSTEB
\author{A.\,Shvartsman}\INSTEB
\author{V.\,Siccardi}\INSTIF
\author{N.\,Skrobova}\INSTEB
\author{K.\,Skwarczynski}\INSTHC
\author{D.\,Smyczek}\INSTBC
\author{M.\,Smy}\INSTGA
\author{J.T.\,Sobczyk}\INSTEA
\author{H.\,Sobel}\INSTGA\INSTHA
\author{F.J.P.\,Soler}\INSTHJ
\author{A.J.\,Speers}\INSTEJ
\author{R.\,Spina}\INSTGF
\author{A.\,Srivastava}\INSTJC
\author{P.\,Stowell}\INSTFB
\author{Y.\,Stroke}\INSTEB
\author{I.A.\,Suslov}\INSTIH
\author{A.\,Suzuki}\INSTCC
\author{M.\,Suzuki}\INSTHE
\author{S.Y.\,Suzuki}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Tada}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{S.\,Tairafune}\INSTIJ
\author{A.\,Takeda}\INSTBJ
\author{Y.\,Takeuchi}\INSTCC\INSTHA
\author{K.\,Takeya}\INSTGJ
\author{H.K.\,Tanaka}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTBJ
\author{H.\,Tanigawa}\INSTID
\author{A.\,Teklu}\INSTFJ
\author{V.V.\,Tereshchenko}\INSTIH
\author{N.\,Thamm}\INSTBC
\author{C.\,Touramanis}\INSTFC
\author{N.\,Tran}\INSTHH
\author{T.\,Tsukamoto}\thanks{also at J-PARC, Tokai, Japan}\INSTCB
\author{M.\,Tzanov}\INSTFI
\author{Y.\,Uchida}\INSTEI
\author{M.\,Vagins}\INSTHA\INSTGA
\author{M.\,Varghese}\INSTED
\author{I.\,Vasilyev}\INSTIH
\author{G.\,Vasseur}\INSTI
\author{E.\,Villa}\INSTEF
\author{U.\,Virginet}\INSTBB
\author{T.\,Vladisavljevic}\INSTEH
\author{T.\,Wachala}\INSTDG
\author{S.-i.\,Wada}\INSTCC
\author{D.\,Wakabayashi}\INSTIJ
\author{H.T.\,Wallace}\INSTFB
\author{J.G.\,Walsh}\INSTHB
\author{D.\,Wark}\INSTEH\INSTGG
\author{M.O.\,Wascko}\INSTGG\INSTEH
\author{A.\,Weber}\INSTJC
\author{R.\,Wendell}\INSTCD
\author{M.J.\,Wilking}\INSTJF
\author{C.\,Wilkinson}\INSTII
\author{J.R.\,Wilson}\INSTIF
\author{C.\,Winterstein}\INSTI
\author{K.\,Wood}\INSTII
\author{C.\,Wret}\INSTEI
\author{J.\,Xia}\INSTIA
\author{Z.\,Xie}\INSTJF
\author{K.\,Yamamoto}\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}\INSTCF
\author{T.\,Yamamoto}\INSTCF
\author{T.\,Yamazumi}\INSTCH
\author{C.\,Yanagisawa}\thanks{also at BMCC/CUNY, Science Department, New York, New York, U.S.A.}\INSTFJ
\author{Y.\,Yang}\INSTGG
\author{T.\,Yano}\INSTBJ
\author{N.\,Yershov}\INSTEB
\author{U.\,Yevarouskaya}\INSTFJ
\author{M.\,Yokoyama}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}\INSTCH
\author{Y.\,Yoshimoto}\INSTCH
\author{N.\,Yoshimura}\INSTCD
\author{R.\,Zaki}\INSTH
\author{A.\,Zalewska}\INSTDG
\author{J.\,Zalipska}\INSTDF
\author{G.\,Zarnecki}\INSTDG
\author{J.\,Zhang}\INSTB\INSTD
\author{X.Y.\,Zhao}\INSTEI
\author{H.\,Zheng}\INSTFJ
\author{H.\,Zhong}\INSTCC
\author{T.\,Zhu}\INSTEI
\author{M.\,Ziembicki}\INSTDH
\author{E.D.\,Zimmerman}\INSTGB
\author{M.\,Zito}\INSTBB
\author{S.\,Zsoldos}\INSTIF

\collaboration{The T2K Collaboration}\noaffiliation

==> authorlist_PTEP_442_all_alsoat_numbered.tex <==
% T2K author list in ptephy_v1 PTEP format
% All 'Also at' notes converted to numbered affiliations.
% 442 authors / 80 affiliations
\author{
\name{\fname{K.} \surname{Abe}}{60}
\name{\fname{S.} \surname{Abe}}{60}
\name{\fname{H.} \surname{Adhikary}}{68}
\name{\fname{R.} \surname{Akutsu}}{15}
\name{\fname{H.} \surname{Alarakia-Charles}}{33}
\name{\fname{Y.I.} \surname{Alj Hakim}}{54}
\name{\fname{S.} \surname{Alonso Monsalve}}{8}
\name{\fname{L.} \surname{Anthony}}{20}
\name{\fname{S.} \surname{Aoki}}{31}
\name{\fname{K.A.} \surname{Apte}}{20}
\name{\fname{T.} \surname{Arai}}{59}
\name{\fname{T.} \surname{Arihara}}{63}
\name{\fname{S.} \surname{Arimoto}}{32}
\name{\fname{Y.} \surname{Asami}}{63}
\name{\fname{Y.} \surname{Asaoka}}{60}
\name{\fname{Y.} \surname{Ashida}}{70}
\name{\fname{E.T.} \surname{Atkin}}{20}
\name{\fname{N.} \surname{Babu}}{37}
\name{\fname{V.} \surname{Baranov}}{38}
\name{\fname{G.J.} \surname{Barker}}{71}
\name{\fname{G.} \surname{Barr}}{46}
\name{\fname{D.} \surname{Barrow}}{46}
\name{\fname{P.} \surname{Bates}}{36}
\name{\fname{L.} \surname{Bathe-Peters}}{46}
\name{\fname{M.} \surname{Batkiewicz-Kwasniak}}{14}
\name{\fname{N.} \surname{Baudis}}{46}
\name{\fname{A.} \surname{Beliakova}}{25}
\name{\fname{V.} \surname{Berardi}}{21}
\name{\fname{L.} \surname{Berns}}{70}
\name{\fname{S.} \surname{Bhattacharjee}}{37}
\name{\fname{A.} \surname{Blanchet}}{57}
\name{\fname{A.} \surname{Blondel}}{57,11}
\name{\fname{L.} \surname{B{\o}e}}{16}
\name{\fname{P.M.M.} \surname{Boistier}}{5}
\name{\fname{S.} \surname{Bolognesi}}{5}
\name{\fname{B.} \surname{Bombin}}{25}
\name{\fname{S.} \surname{Bordoni}}{11}
\name{\fname{S.B.} \surname{Boyd}}{71}
\name{\fname{C.} \surname{Bronner}}{73}
\name{\fname{A.} \surname{Bubak}}{55}
\name{\fname{M.} \surname{Buizza Avanzini}}{35}
\name{\fname{J.A.} \surname{Caballero}}{53}
\name{\fname{N.F.} \surname{Calabria}}{21}
\name{\fname{S.} \surname{Cao}}{19}
\name{\fname{S.} \surname{Cap}}{11}
\name{\fname{D.} \surname{Carabadjac}}{35,5}
\name{\fname{S.L.} \surname{Cartwright}}{54}
\name{\fname{M.P.} \surname{Casado}}{17,75}
\name{\fname{M.G.} \surname{Catanesi}}{21}
\name{\fname{J.} \surname{Chakrani}}{34}
\name{\fname{A.} \surname{Chalumeau}}{57}
\name{\fname{D.} \surname{Cherdack}}{16}
\name{\fname{A.} \surname{Chvirova}}{25}
\name{\fname{J.} \surname{Coleman}}{36}
\name{\fname{G.} \surname{Collazuol}}{23}
\name{\fname{F.} \surname{Cormier}}{65}
\name{\fname{A.A.L.} \surname{Craplet}}{20}
\name{\fname{A.} \surname{Cudd}}{6}
\name{\fname{D.} \surname{D'Ago}}{23}
\name{\fname{C.} \surname{Dalmazzone}}{57}
\name{\fname{T.} \surname{Daret}}{5}
\name{\fname{P.} \surname{Dasgupta}}{17}
\name{\fname{C.} \surname{Davis}}{47}
\name{\fname{Yu.I.} \surname{Davydov}}{38}
\name{\fname{P.} \surname{de Perio}}{28}
\name{\fname{G.} \surname{De Rosa}}{22}
\name{\fname{T.} \surname{Dealtry}}{33}
\name{\fname{C.} \surname{Densham}}{43}
\name{\fname{A.} \surname{Dergacheva}}{25}
\name{\fname{R.} \surname{Dharmapal Banerjee}}{72}
\name{\fname{F.} \surname{Di Lodovico}}{30}
\name{\fname{G.} \surname{Diaz Lopez}}{57}
\name{\fname{S.} \surname{Dolan}}{10}
\name{\fname{D.} \surname{Douqa}}{11}
\name{\fname{T.A.} \surname{Doyle}}{46}
\name{\fname{O.} \surname{Drapier}}{35}
\name{\fname{K.E.} \surname{Duffy}}{46}
\name{\fname{J.} \surname{Dumarchez}}{57}
\name{\fname{P.} \surname{Dunne}}{20}
\name{\fname{K.} \surname{Dygnarowicz}}{69}
\name{\fname{A.} \surname{Eguchi}}{59}
\name{\fname{M.} \surname{El Baz}}{11}
\name{\fname{J.} \surname{Elias}}{49}
\name{\fname{S.} \surname{Emery-Schrenk}}{5}
\name{\fname{G.} \surname{Erofeev}}{25}
\name{\fname{A.} \surname{Ershova}}{35}
\name{\fname{G.} \surname{Eurin}}{5}
\name{\fname{M.} \surname{Fani}}{52}
\name{\fname{D.} \surname{Fedorova}}{25}
\name{\fname{S.} \surname{Fedotov}}{25}
\name{\fname{M.} \surname{Feltre}}{23}
\name{\fname{C.} \surname{Fengler}}{46}
\name{\fname{L.} \surname{Feng}}{32}
\name{\fname{D.} \surname{Ferlewicz}}{57}
\name{\fname{A.J.} \surname{Finch}}{33}
\name{\fname{M.D.} \surname{Fitton}}{43}
\name{\fname{C.} \surname{Forza}}{23}
\name{\fname{M.} \surname{Friend}}{15,76}
\name{\fname{Y.} \surname{Fujii}}{15,76}
\name{\fname{Y.} \surname{Fukuda}}{40}
\name{\fname{N.} \surname{Funayama}}{45}
\name{\fname{Y.} \surname{Furui}}{63}
\name{\fname{A.N.} \surname{Gaci\~no Olmedo}}{57}
\name{\fname{J.} \surname{Garc\'ia-Marcos}}{13}
\name{\fname{A.C.} \surname{Germer}}{47}
\name{\fname{L.} \surname{Giannessi}}{11}
\name{\fname{C.} \surname{Giganti}}{57}
\name{\fname{M.} \surname{Girgus}}{68}
\name{\fname{V.} \surname{Glagolev}}{38}
\name{\fname{P.} \surname{Golak}}{68}
\name{\fname{M.} \surname{Gonin}}{27}
\name{\fname{R.} \surname{Gonzalez Jimenez}}{53}
\name{\fname{J.} \surname{Gonz\'alez Rosa}}{53}
\name{\fname{E.A.G.} \surname{Goodman}}{12}
\name{\fname{K.} \surname{Gorshanov}}{25}
\name{\fname{P.} \surname{Govindaraj}}{68}
\name{\fname{M.} \surname{Grassi}}{23}
\name{\fname{M.} \surname{Guigue}}{57}
\name{\fname{F.Y.} \surname{Guo}}{42}
\name{\fname{D.R.} \surname{Hadley}}{71}
\name{\fname{S.} \surname{Han}}{32,61}
\name{\fname{D.A.} \surname{Harris}}{74}
\name{\fname{R.J.} \surname{Harris}}{33,43}
\name{\fname{M.} \surname{Hartz}}{65,28}
\name{\fname{K.} \surname{Hasegawa}}{32}
\name{\fname{T.} \surname{Hasegawa}}{15,76}
\name{\fname{C.M.} \surname{Hasnip}}{10}
\name{\fname{S.} \surname{Hassani}}{5}
\name{\fname{N.C.} \surname{Hastings}}{15}
\name{\fname{K.} \surname{Hayashi}}{32}
\name{\fname{Y.} \surname{Hayato}}{60,28}
\name{\fname{I.} \surname{Heitkamp}}{70}
\name{\fname{D.} \surname{Henaff}}{5}
\name{\fname{Y.} \surname{Hino}}{15}
\name{\fname{K.} \surname{Hiraide}}{60,28}
\name{\fname{J.} \surname{Holeczek}}{55}
\name{\fname{A.} \surname{Holin}}{43}
\name{\fname{T.} \surname{Holvey}}{46}
\name{\fname{N.T.} \surname{Hong Van}}{26}
\name{\fname{T.} \surname{Honjo}}{45}
\name{\fname{M.C.F.} \surname{Hooft}}{13}
\name{\fname{K.} \surname{Hosokawa}}{60}
\name{\fname{R.} \surname{Huang}}{34}
\name{\fname{J.} \surname{Hu}}{32}
\name{\fname{A.K.} \surname{Ichikawa}}{70}
\name{\fname{K.} \surname{Ieki}}{60}
\name{\fname{M.} \surname{Ikeda}}{60}
\name{\fname{K.} \surname{Indo}}{32}
\name{\fname{T.H.} \surname{Ishida}}{70}
\name{\fname{T.} \surname{Ishida}}{15,76}
\name{\fname{M.} \surname{Ishitsuka}}{64}
\name{\fname{H.} \surname{Ito}}{31}
\name{\fname{S.} \surname{Ito}}{73}
\name{\fname{A.} \surname{Izmaylov}}{25}
\name{\fname{N.} \surname{Jachowicz}}{13}
\name{\fname{B.} \surname{Jargowsky}}{2}
\name{\fname{S.J.} \surname{Jenkins}}{36}
\name{\fname{C.} \surname{Jes\'us-Valls}}{10}
\name{\fname{M.} \surname{Jia}}{42}
\name{\fname{J.J.} \surname{Jiang}}{42}
\name{\fname{J.Y.} \surname{Ji}}{42}
\name{\fname{T.P.} \surname{Jones}}{33}
\name{\fname{P.} \surname{Jonsson}}{20}
\name{\fname{S.} \surname{Joshi}}{42}
\name{\fname{C.K.} \surname{Jung}}{42}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Kabirnezhad}}{46}
\name{\fname{A.C.} \surname{Kaboth}}{50}
\name{\fname{K.} \surname{Kadota}}{31}
\name{\fname{H.} \surname{Kakuno}}{63}
\name{\fname{A.} \surname{Kamata}}{63}
\name{\fname{J.} \surname{Kameda}}{60}
\name{\fname{S.} \surname{Karpova}}{11}
\name{\fname{V.S.} \surname{Kasturi}}{11}
\name{\fname{Y.} \surname{Kataoka}}{60}
\name{\fname{T.} \surname{Katori}}{30}
\name{\fname{A.} \surname{Kawabata}}{29}
\name{\fname{R.} \surname{Kawabe}}{45}
\name{\fname{Y.} \surname{Kawamura}}{45}
\name{\fname{M.} \surname{Kawaue}}{32}
\name{\fname{E.} \surname{Kearns}}{2}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Khabibullin}}{25}
\name{\fname{N.V.} \surname{Khomutov}}{38}
\name{\fname{A.} \surname{Khotjantsev}}{25}
\name{\fname{T.} \surname{Kikawa}}{32}
\name{\fname{S.} \surname{King}}{30}
\name{\fname{V.} \surname{Kiseeva}}{38}
\name{\fname{J.} \surname{Kisiel}}{55}
\name{\fname{A.} \surname{Klustov\'a}}{20}
\name{\fname{L.} \surname{Kneale}}{54}
\name{\fname{H.} \surname{Kobayashi}}{59}
\name{\fname{S.R.} \surname{Kobayashi}}{70}
\name{\fname{T.} \surname{Kobayashi}}{15,76}
\name{\fname{L.} \surname{Koch}}{18}
\name{\fname{S.} \surname{Kodama}}{59}
\name{\fname{M.} \surname{Kolupanova}}{25,77}
\name{\fname{A.} \surname{Konaka}}{65}
\name{\fname{L.L.} \surname{Kormos}}{33}
\name{\fname{Y.} \surname{Koshio}}{44}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{K.} \surname{Kowalik}}{41}
\name{\fname{R.} \surname{Kralik}}{30}
\name{\fname{Y.} \surname{Kudenko}}{25,77}
\name{\fname{Y.} \surname{Kudo}}{73}
\name{\fname{A.} \surname{Kumar Jha}}{13}
\name{\fname{R.} \surname{Kurjata}}{69}
\name{\fname{V.} \surname{Kurochka}}{25}
\name{\fname{T.} \surname{Kutter}}{37}
\name{\fname{L.} \surname{Labarga}}{1}
\name{\fname{M.} \surname{Lachat}}{49}
\name{\fname{K.} \surname{Lachner}}{8}
\name{\fname{J.} \surname{Lagoda}}{41}
\name{\fname{S.M.} \surname{Lakshmi}}{55}
\name{\fname{M.} \surname{Lamers James}}{71}
\name{\fname{A.} \surname{Langella}}{22}
\name{\fname{D.H.} \surname{Langridge}}{50}
\name{\fname{J.-F.} \surname{Laporte}}{5}
\name{\fname{D.} \surname{Last}}{49}
\name{\fname{N.} \surname{Latham}}{30}
\name{\fname{M.} \surname{Laveder}}{23}
\name{\fname{L.} \surname{Lavitola}}{22}
\name{\fname{M.} \surname{Lawe}}{33}
\name{\fname{A.} \surname{Leclerc}}{5}
\name{\fname{N.} \surname{Lemaire}}{35}
\name{\fname{D.} \surname{Leon Silverio}}{58}
\name{\fname{T.} \surname{Leplumey}}{35}
\name{\fname{S.} \surname{Levorato}}{23}
\name{\fname{S.V.} \surname{Lewis}}{30}
\name{\fname{B.} \surname{Li}}{8}
\name{\fname{C.} \surname{Lin}}{20}
\name{\fname{R.P.} \surname{Litchfield}}{12}
\name{\fname{S.L.} \surname{Liu}}{42}
\name{\fname{W.} \surname{Li}}{46}
\name{\fname{A.} \surname{Longhin}}{23}
\name{\fname{A.} \surname{Lopez Moreno}}{30}
\name{\fname{L.} \surname{Ludovici}}{24}
\name{\fname{X.} \surname{Lu}}{71}
\name{\fname{T.} \surname{Lux}}{17}
\name{\fname{L.N.} \surname{Machado}}{12}
\name{\fname{L.} \surname{Magaletti}}{21}
\name{\fname{K.} \surname{Mahn}}{39}
\name{\fname{K.K.} \surname{Mahtani}}{42}
\name{\fname{S.} \surname{Manly}}{49}
\name{\fname{A.D.} \surname{Marino}}{6}
\name{\fname{D.G.R.} \surname{Martin}}{20}
\name{\fname{D.A.} \surname{Martinez Caicedo}}{58}
\name{\fname{L.} \surname{Martinez}}{17}
\name{\fname{M.} \surname{Martini}}{57,78}
\name{\fname{N.} \surname{Mashin}}{25}
\name{\fname{T.} \surname{Matsubara}}{15}
\name{\fname{R.} \surname{Matsumoto}}{62}
\name{\fname{V.} \surname{Matveev}}{25}
\name{\fname{C.} \surname{Mauger}}{47}
\name{\fname{K.} \surname{Mavrokoridis}}{36}
\name{\fname{N.} \surname{McCauley}}{36}
\name{\fname{K.S.} \surname{McFarland}}{49}
\name{\fname{C.} \surname{McGrew}}{42}
\name{\fname{J.} \surname{McKean}}{32}
\name{\fname{A.} \surname{Mefodiev}}{25}
\name{\fname{G.D.} \surname{Megias}}{53}
\name{\fname{L.} \surname{Mellet}}{39}
\name{\fname{C.} \surname{Metelko}}{36}
\name{\fname{M.} \surname{Mezzetto}}{23}
\name{\fname{S.} \surname{Miki}}{60}
\name{\fname{V.} \surname{Mikola}}{12}
\name{\fname{E.W.} \surname{Miller}}{20}
\name{\fname{A.} \surname{Minamino}}{73}
\name{\fname{O.} \surname{Mineev}}{25}
\name{\fname{S.} \surname{Mine}}{60,4}
\name{\fname{J.} \surname{Mirabito}}{2}
\name{\fname{M.} \surname{Miura}}{60}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{60}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{73}
\name{\fname{P.} \surname{Morrison}}{12}
\name{\fname{Th.A.} \surname{Mueller}}{35}
\name{\fname{D.} \surname{Munford}}{16}
\name{\fname{A.} \surname{Mu\~noz}}{18}
\name{\fname{L.} \surname{Munteanu}}{10}
\name{\fname{Y.} \surname{Nagai}}{15}
\name{\fname{T.} \surname{Nakadaira}}{15,76}
\name{\fname{K.} \surname{Nakagiri}}{60}
\name{\fname{M.} \surname{Nakahata}}{60,28}
\name{\fname{Y.} \surname{Nakajima}}{59}
\name{\fname{K.D.} \surname{Nakamura}}{70}
\name{\fname{A.} \surname{Nakano}}{70}
\name{\fname{Y.} \surname{Nakano}}{66}
\name{\fname{S.} \surname{Nakayama}}{60,28}
\name{\fname{T.} \surname{Nakaya}}{32,28}
\name{\fname{K.} \surname{Nakayoshi}}{15,76}
\name{\fname{C.E.R.} \surname{Naseby}}{20}
\name{\fname{D.T.} \surname{Nguyen}}{9}
\name{\fname{V.Q.} \surname{Nguyen}}{35}
\name{\fname{K.} \surname{Niewczas}}{35,13}
\name{\fname{S.} \surname{Nishimori}}{59}
\name{\fname{Y.} \surname{Nishimura}}{29}
\name{\fname{Y.} \surname{Noguchi}}{60}
\name{\fname{T.} \surname{Nosek}}{41}
\name{\fname{F.} \surname{Nova}}{43}
\name{\fname{J.C.} \surname{Nugent}}{20}
\name{\fname{H.M.} \surname{O'Keeffe}}{33}
\name{\fname{L.} \surname{O'Sullivan}}{18}
\name{\fname{R.} \surname{Okazaki}}{29}
\name{\fname{W.} \surname{Okinaga}}{59}
\name{\fname{K.} \surname{Okumura}}{61,28}
\name{\fname{T.} \surname{Okusawa}}{45}
\name{\fname{N.} \surname{Onda}}{32}
\name{\fname{N.} \surname{Ospina}}{21}
\name{\fname{L.} \surname{Osu}}{35}
\name{\fname{N.} \surname{Otani}}{32}
\name{\fname{Y.} \surname{Oyama}}{15,76}
\name{\fname{V.} \surname{Paolone}}{48}
\name{\fname{J.} \surname{Pasternak}}{20}
\name{\fname{D.} \surname{Payne}}{36}
\name{\fname{T.P.D.} \surname{Peacock}}{54}
\name{\fname{M.} \surname{Pfaff}}{20}
\name{\fname{L.} \surname{Pickering}}{43}
\name{\fname{J.-B.} \surname{Plan\c{c}on}}{35}
\name{\fname{P.} \surname{Podlaski}}{15,76}
\name{\fname{B.} \surname{Popov}}{57,46}
\name{\fname{A.J.} \surname{Portocarrero Yrey}}{15}
\name{\fname{M.} \surname{Posiadala-Zezula}}{68}
\name{\fname{Y.S.} \surname{Prabhu}}{68}
\name{\fname{H.} \surname{Prasad}}{72}
\name{\fname{F.} \surname{Pupilli}}{23}
\name{\fname{B.} \surname{Quilain}}{27,35}
\name{\fname{P.T.} \surname{Quyen}}{19,79}
\name{\fname{E.} \surname{Radicioni}}{21}
\name{\fname{B.} \surname{Radics}}{74}
\name{\fname{M.A.} \surname{Ramirez Delgado}}{47}
\name{\fname{R.} \surname{Ramsden}}{30}
\name{\fname{P.N.} \surname{Ratoff}}{33}
\name{\fname{M.} \surname{Reh}}{6}
\name{\fname{G.} \surname{Reina}}{18}
\name{\fname{L.} \surname{Restrepo}}{57}
\name{\fname{C.} \surname{Riccio}}{42}
\name{\fname{D.W.} \surname{Riley}}{12}
\name{\fname{E.} \surname{Rondio}}{41}
\name{\fname{D.} \surname{Ross}}{39}
\name{\fname{S.} \surname{Roth}}{51}
\name{\fname{N.} \surname{Roy}}{74}
\name{\fname{A.} \surname{Rubbia}}{8}
\name{\fname{L.} \surname{Russo}}{57}
\name{\fname{A.} \surname{Rychter}}{69}
\name{\fname{W.} \surname{Saenz}}{57}
\name{\fname{K.} \surname{Sakashita}}{67,15,76}
\name{\fname{S.} \surname{Samani}}{11}
\name{\fname{F.} \surname{S\'anchez}}{11}
\name{\fname{E.M.} \surname{Sandford}}{36}
\name{\fname{Y.} \surname{Sato}}{64}
\name{\fname{T.} \surname{Schefke}}{37}
\name{\fname{K.} \surname{Scholberg}}{7}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Scott}}{20}
\name{\fname{Y.} \surname{Seiya}}{45,53}
\name{\fname{T.} \surname{Sekiguchi}}{15,76}
\name{\fname{H.} \surname{Sekiya}}{60,28}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Sekiyama}}{59}
\name{\fname{T.} \surname{Sekiya}}{63}
\name{\fname{D.} \surname{Seppala}}{39}
\name{\fname{D.} \surname{Sgalaberna}}{8}
\name{\fname{A.} \surname{Shaikhiev}}{25}
\name{\fname{M.} \surname{Shiozawa}}{60,28}
\name{\fname{Y.} \surname{Shiraishi}}{44}
\name{\fname{N.} \surname{Shvarev}}{25}
\name{\fname{A.} \surname{Shvartsman}}{25}
\name{\fname{V.} \surname{Siccardi}}{30}
\name{\fname{N.} \surname{Skrobova}}{25}
\name{\fname{K.} \surname{Skwarczynski}}{50}
\name{\fname{D.} \surname{Smyczek}}{51}
\name{\fname{M.} \surname{Smy}}{4}
\name{\fname{J.T.} \surname{Sobczyk}}{72}
\name{\fname{H.} \surname{Sobel}}{4,28}
\name{\fname{F.J.P.} \surname{Soler}}{12}
\name{\fname{A.J.} \surname{Speers}}{33}
\name{\fname{R.} \surname{Spina}}{21}
\name{\fname{A.} \surname{Srivastava}}{18}
\name{\fname{P.} \surname{Stowell}}{54}
\name{\fname{Y.} \surname{Stroke}}{25}
\name{\fname{I.A.} \surname{Suslov}}{38}
\name{\fname{A.} \surname{Suzuki}}{31}
\name{\fname{M.} \surname{Suzuki}}{73}
\name{\fname{S.Y.} \surname{Suzuki}}{15,76}
\name{\fname{M.} \surname{Tada}}{15,76}
\name{\fname{S.} \surname{Tairafune}}{70}
\name{\fname{A.} \surname{Takeda}}{60}
\name{\fname{Y.} \surname{Takeuchi}}{31,28}
\name{\fname{K.} \surname{Takeya}}{44}
\name{\fname{H.K.} \surname{Tanaka}}{60}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{H.} \surname{Tanigawa}}{29}
\name{\fname{A.} \surname{Teklu}}{42}
\name{\fname{V.V.} \surname{Tereshchenko}}{38}
\name{\fname{N.} \surname{Thamm}}{51}
\name{\fname{C.} \surname{Touramanis}}{36}
\name{\fname{N.} \surname{Tran}}{19}
\name{\fname{T.} \surname{Tsukamoto}}{15,76}
\name{\fname{M.} \surname{Tzanov}}{37}
\name{\fname{Y.} \surname{Uchida}}{20}
\name{\fname{M.} \surname{Vagins}}{28,4}
\name{\fname{M.} \surname{Varghese}}{17}
\name{\fname{I.} \surname{Vasilyev}}{38}
\name{\fname{G.} \surname{Vasseur}}{5}
\name{\fname{E.} \surname{Villa}}{8}
\name{\fname{U.} \surname{Virginet}}{57}
\name{\fname{T.} \surname{Vladisavljevic}}{43}
\name{\fname{T.} \surname{Wachala}}{14}
\name{\fname{S.-i.} \surname{Wada}}{31}
\name{\fname{D.} \surname{Wakabayashi}}{70}
\name{\fname{H.T.} \surname{Wallace}}{54}
\name{\fname{J.G.} \surname{Walsh}}{39}
\name{\fname{D.} \surname{Wark}}{43,46}
\name{\fname{M.O.} \surname{Wascko}}{46,43}
\name{\fname{A.} \surname{Weber}}{18}
\name{\fname{R.} \surname{Wendell}}{32}
\name{\fname{M.J.} \surname{Wilking}}{52}
\name{\fname{C.} \surname{Wilkinson}}{34}
\name{\fname{J.R.} \surname{Wilson}}{30}
\name{\fname{C.} \surname{Winterstein}}{5}
\name{\fname{K.} \surname{Wood}}{34}
\name{\fname{C.} \surname{Wret}}{20}
\name{\fname{J.} \surname{Xia}}{56}
\name{\fname{Z.} \surname{Xie}}{52}
\name{\fname{K.} \surname{Yamamoto}}{45,53}
\name{\fname{T.} \surname{Yamamoto}}{45}
\name{\fname{T.} \surname{Yamazumi}}{59}
\name{\fname{C.} \surname{Yanagisawa}}{42,80}
\name{\fname{Y.} \surname{Yang}}{46}
\name{\fname{T.} \surname{Yano}}{60}
\name{\fname{N.} \surname{Yershov}}{25}
\name{\fname{U.} \surname{Yevarouskaya}}{42}
\name{\fname{M.} \surname{Yokoyama}}{59}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{Y.} \surname{Yoshimoto}}{59}
\name{\fname{N.} \surname{Yoshimura}}{32}
\name{\fname{R.} \surname{Zaki}}{74}
\name{\fname{A.} \surname{Zalewska}}{14}
\name{\fname{J.} \surname{Zalipska}}{41}
\name{\fname{G.} \surname{Zarnecki}}{14}
\name{\fname{J.} \surname{Zhang}}{65,3}
\name{\fname{X.Y.} \surname{Zhao}}{20}
\name{\fname{H.} \surname{Zheng}}{42}
\name{\fname{H.} \surname{Zhong}}{31}
\name{\fname{T.} \surname{Zhu}}{20}
\name{\fname{M.} \surname{Ziembicki}}{69}
\name{\fname{E.D.} \surname{Zimmerman}}{6}
\name{\fname{M.} \surname{Zito}}{57}
\name{\fname{S.} \surname{Zsoldos}}{30}
}

\address{
$^{1}$ University Autonoma Madrid, Department of Theoretical Physics, 28049 Madrid, Spain\par
$^{2}$ Boston University, Department of Physics, Boston, Massachusetts, U.S.A.\par
$^{3}$ University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada\par
$^{4}$ University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.\par
$^{5}$ IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France\par
$^{6}$ University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.\par
$^{7}$ Duke University, Department of Physics, Durham, North Carolina, U.S.A.\par
$^{8}$ ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland\par
$^{9}$ VNU University of Science, Vietnam National University, Hanoi, Vietnam\par
$^{10}$ CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland\par
$^{11}$ University of Geneva, Section de Physique, DPNC, Geneva, Switzerland\par
$^{12}$ University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom\par
$^{13}$ Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium\par
$^{14}$ H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland\par
$^{15}$ High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan\par
$^{16}$ University of Houston, Department of Physics, Houston, Texas, U.S.A.\par
$^{17}$ Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain\par
$^{18}$ Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Staudingerweg 7, 55128 Mainz, Germany\par
$^{19}$ Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam\par
$^{20}$ Imperial College London, Department of Physics, London, United Kingdom\par
$^{21}$ INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy\par
$^{22}$ INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy\par
$^{23}$ INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy\par
$^{24}$ INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy\par
$^{25}$ Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia\par
$^{26}$ International Centre of Physics, Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), 10 Dao Tan, Ba Dinh, Hanoi, Vietnam\par
$^{27}$ ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan\par
$^{28}$ Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan\par
$^{29}$ Keio University, Department of Physics, Kanagawa, Japan\par
$^{30}$ King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom\par
$^{31}$ Kobe University, Kobe, Japan\par
$^{32}$ Kyoto University, Department of Physics, Kyoto, Japan\par
$^{33}$ Lancaster University, School of Physics and Astronomy, Lancaster, United Kingdom\par
$^{34}$ Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.\par
$^{35}$ Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France\par
$^{36}$ University of Liverpool, Department of Physics, Liverpool, United Kingdom\par
$^{37}$ Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.\par
$^{38}$ Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia\par
$^{39}$ Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.\par
$^{40}$ Miyagi University of Education, Department of Physics, Sendai, Japan\par
$^{41}$ National Centre for Nuclear Research, Warsaw, Poland\par
$^{42}$ State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.\par
$^{43}$ STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom\par
$^{44}$ Okayama University, Department of Physics, Okayama, Japan\par
$^{45}$ Osaka Metropolitan University, Department of Physics, Osaka, Japan\par
$^{46}$ Oxford University, Department of Physics, Oxford, United Kingdom\par
$^{47}$ University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.\par
$^{48}$ University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.\par
$^{49}$ University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.\par
$^{50}$ Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom\par
$^{51}$ RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany\par
$^{52}$ School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota, U.S.A.\par
$^{53}$ Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain\par
$^{54}$ University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom\par
$^{55}$ University of Silesia, Institute of Physics, Katowice, Poland\par
$^{56}$ SLAC National Accelerator Laboratory, Stanford University, Menlo Park, California, U.S.A.\par
$^{57}$ Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France\par
$^{58}$ South Dakota School of Mines and Technology, 501 East Saint Joseph Street, Rapid City, SD 57701, United States\par
$^{59}$ University of Tokyo, Department of Physics, Tokyo, Japan\par
$^{60}$ University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan\par
$^{61}$ University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan\par
$^{62}$ Institute of Science Tokyo, Department of Physics, Tokyo\par
$^{63}$ Tokyo Metropolitan University, Department of Physics, Tokyo, Japan\par
$^{64}$ Tokyo University of Science, Faculty of Science and Technology, Department of Physics, Noda, Chiba, Japan\par
$^{65}$ TRIUMF, Vancouver, British Columbia, Canada\par
$^{66}$ University of Toyama, Faculty of Science, Toyama, Japan\par
$^{67}$ University of Tsukuba, Faculty of Pure and Applied Sciences, Tsukuba, Ibaraki, Japan\par
$^{68}$ University of Warsaw, Faculty of Physics, Warsaw, Poland\par
$^{69}$ Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland\par
$^{70}$ Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan\par
$^{71}$ University of Warwick, Department of Physics, Coventry, United Kingdom\par
$^{72}$ Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland\par
$^{73}$ Yokohama National University, Department of Physics, Yokohama, Japan\par
$^{74}$ York University, Department of Physics and Astronomy, Toronto, Ontario, Canada\par
$^{75}$ Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain\par
$^{76}$ J-PARC, Tokai, Japan\par
$^{77}$ Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia\par
$^{78}$ IPSA-DRII, France\par
$^{79}$ the Graduate University of Science and Technology, Vietnam Academy of Science and Technology\par
$^{80}$ BMCC/CUNY, Science Department, New York, New York, U.S.A.\par
}


==> authorlist_PTEP_442_primary_only.tex <==
% T2K author list in ptephy_v1 PTEP format
% Primary affiliations only; 'Also at' affiliations removed for testing.
% 442 authors / 74 primary affiliations
\author{
\name{\fname{K.} \surname{Abe}}{60}
\name{\fname{S.} \surname{Abe}}{60}
\name{\fname{H.} \surname{Adhikary}}{68}
\name{\fname{R.} \surname{Akutsu}}{15}
\name{\fname{H.} \surname{Alarakia-Charles}}{33}
\name{\fname{Y.I.} \surname{Alj Hakim}}{54}
\name{\fname{S.} \surname{Alonso Monsalve}}{8}
\name{\fname{L.} \surname{Anthony}}{20}
\name{\fname{S.} \surname{Aoki}}{31}
\name{\fname{K.A.} \surname{Apte}}{20}
\name{\fname{T.} \surname{Arai}}{59}
\name{\fname{T.} \surname{Arihara}}{63}
\name{\fname{S.} \surname{Arimoto}}{32}
\name{\fname{Y.} \surname{Asami}}{63}
\name{\fname{Y.} \surname{Asaoka}}{60}
\name{\fname{Y.} \surname{Ashida}}{70}
\name{\fname{E.T.} \surname{Atkin}}{20}
\name{\fname{N.} \surname{Babu}}{37}
\name{\fname{V.} \surname{Baranov}}{38}
\name{\fname{G.J.} \surname{Barker}}{71}
\name{\fname{G.} \surname{Barr}}{46}
\name{\fname{D.} \surname{Barrow}}{46}
\name{\fname{P.} \surname{Bates}}{36}
\name{\fname{L.} \surname{Bathe-Peters}}{46}
\name{\fname{M.} \surname{Batkiewicz-Kwasniak}}{14}
\name{\fname{N.} \surname{Baudis}}{46}
\name{\fname{A.} \surname{Beliakova}}{25}
\name{\fname{V.} \surname{Berardi}}{21}
\name{\fname{L.} \surname{Berns}}{70}
\name{\fname{S.} \surname{Bhattacharjee}}{37}
\name{\fname{A.} \surname{Blanchet}}{57}
\name{\fname{A.} \surname{Blondel}}{57,11}
\name{\fname{L.} \surname{B{\o}e}}{16}
\name{\fname{P.M.M.} \surname{Boistier}}{5}
\name{\fname{S.} \surname{Bolognesi}}{5}
\name{\fname{B.} \surname{Bombin}}{25}
\name{\fname{S.} \surname{Bordoni}}{11}
\name{\fname{S.B.} \surname{Boyd}}{71}
\name{\fname{C.} \surname{Bronner}}{73}
\name{\fname{A.} \surname{Bubak}}{55}
\name{\fname{M.} \surname{Buizza Avanzini}}{35}
\name{\fname{J.A.} \surname{Caballero}}{53}
\name{\fname{N.F.} \surname{Calabria}}{21}
\name{\fname{S.} \surname{Cao}}{19}
\name{\fname{S.} \surname{Cap}}{11}
\name{\fname{D.} \surname{Carabadjac}}{35,5}
\name{\fname{S.L.} \surname{Cartwright}}{54}
\name{\fname{M.P.} \surname{Casado}}{17}
\name{\fname{M.G.} \surname{Catanesi}}{21}
\name{\fname{J.} \surname{Chakrani}}{34}
\name{\fname{A.} \surname{Chalumeau}}{57}
\name{\fname{D.} \surname{Cherdack}}{16}
\name{\fname{A.} \surname{Chvirova}}{25}
\name{\fname{J.} \surname{Coleman}}{36}
\name{\fname{G.} \surname{Collazuol}}{23}
\name{\fname{F.} \surname{Cormier}}{65}
\name{\fname{A.A.L.} \surname{Craplet}}{20}
\name{\fname{A.} \surname{Cudd}}{6}
\name{\fname{D.} \surname{D'Ago}}{23}
\name{\fname{C.} \surname{Dalmazzone}}{57}
\name{\fname{T.} \surname{Daret}}{5}
\name{\fname{P.} \surname{Dasgupta}}{17}
\name{\fname{C.} \surname{Davis}}{47}
\name{\fname{Yu.I.} \surname{Davydov}}{38}
\name{\fname{P.} \surname{de Perio}}{28}
\name{\fname{G.} \surname{De Rosa}}{22}
\name{\fname{T.} \surname{Dealtry}}{33}
\name{\fname{C.} \surname{Densham}}{43}
\name{\fname{A.} \surname{Dergacheva}}{25}
\name{\fname{R.} \surname{Dharmapal Banerjee}}{72}
\name{\fname{F.} \surname{Di Lodovico}}{30}
\name{\fname{G.} \surname{Diaz Lopez}}{57}
\name{\fname{S.} \surname{Dolan}}{10}
\name{\fname{D.} \surname{Douqa}}{11}
\name{\fname{T.A.} \surname{Doyle}}{46}
\name{\fname{O.} \surname{Drapier}}{35}
\name{\fname{K.E.} \surname{Duffy}}{46}
\name{\fname{J.} \surname{Dumarchez}}{57}
\name{\fname{P.} \surname{Dunne}}{20}
\name{\fname{K.} \surname{Dygnarowicz}}{69}
\name{\fname{A.} \surname{Eguchi}}{59}
\name{\fname{M.} \surname{El Baz}}{11}
\name{\fname{J.} \surname{Elias}}{49}
\name{\fname{S.} \surname{Emery-Schrenk}}{5}
\name{\fname{G.} \surname{Erofeev}}{25}
\name{\fname{A.} \surname{Ershova}}{35}
\name{\fname{G.} \surname{Eurin}}{5}
\name{\fname{M.} \surname{Fani}}{52}
\name{\fname{D.} \surname{Fedorova}}{25}
\name{\fname{S.} \surname{Fedotov}}{25}
\name{\fname{M.} \surname{Feltre}}{23}
\name{\fname{C.} \surname{Fengler}}{46}
\name{\fname{L.} \surname{Feng}}{32}
\name{\fname{D.} \surname{Ferlewicz}}{57}
\name{\fname{A.J.} \surname{Finch}}{33}
\name{\fname{M.D.} \surname{Fitton}}{43}
\name{\fname{C.} \surname{Forza}}{23}
\name{\fname{M.} \surname{Friend}}{15}
\name{\fname{Y.} \surname{Fujii}}{15}
\name{\fname{Y.} \surname{Fukuda}}{40}
\name{\fname{N.} \surname{Funayama}}{45}
\name{\fname{Y.} \surname{Furui}}{63}
\name{\fname{A.N.} \surname{Gaci\~no Olmedo}}{57}
\name{\fname{J.} \surname{Garc\'ia-Marcos}}{13}
\name{\fname{A.C.} \surname{Germer}}{47}
\name{\fname{L.} \surname{Giannessi}}{11}
\name{\fname{C.} \surname{Giganti}}{57}
\name{\fname{M.} \surname{Girgus}}{68}
\name{\fname{V.} \surname{Glagolev}}{38}
\name{\fname{P.} \surname{Golak}}{68}
\name{\fname{M.} \surname{Gonin}}{27}
\name{\fname{R.} \surname{Gonzalez Jimenez}}{53}
\name{\fname{J.} \surname{Gonz\'alez Rosa}}{53}
\name{\fname{E.A.G.} \surname{Goodman}}{12}
\name{\fname{K.} \surname{Gorshanov}}{25}
\name{\fname{P.} \surname{Govindaraj}}{68}
\name{\fname{M.} \surname{Grassi}}{23}
\name{\fname{M.} \surname{Guigue}}{57}
\name{\fname{F.Y.} \surname{Guo}}{42}
\name{\fname{D.R.} \surname{Hadley}}{71}
\name{\fname{S.} \surname{Han}}{32,61}
\name{\fname{D.A.} \surname{Harris}}{74}
\name{\fname{R.J.} \surname{Harris}}{33,43}
\name{\fname{M.} \surname{Hartz}}{65,28}
\name{\fname{K.} \surname{Hasegawa}}{32}
\name{\fname{T.} \surname{Hasegawa}}{15}
\name{\fname{C.M.} \surname{Hasnip}}{10}
\name{\fname{S.} \surname{Hassani}}{5}
\name{\fname{N.C.} \surname{Hastings}}{15}
\name{\fname{K.} \surname{Hayashi}}{32}
\name{\fname{Y.} \surname{Hayato}}{60,28}
\name{\fname{I.} \surname{Heitkamp}}{70}
\name{\fname{D.} \surname{Henaff}}{5}
\name{\fname{Y.} \surname{Hino}}{15}
\name{\fname{K.} \surname{Hiraide}}{60,28}
\name{\fname{J.} \surname{Holeczek}}{55}
\name{\fname{A.} \surname{Holin}}{43}
\name{\fname{T.} \surname{Holvey}}{46}
\name{\fname{N.T.} \surname{Hong Van}}{26}
\name{\fname{T.} \surname{Honjo}}{45}
\name{\fname{M.C.F.} \surname{Hooft}}{13}
\name{\fname{K.} \surname{Hosokawa}}{60}
\name{\fname{R.} \surname{Huang}}{34}
\name{\fname{J.} \surname{Hu}}{32}
\name{\fname{A.K.} \surname{Ichikawa}}{70}
\name{\fname{K.} \surname{Ieki}}{60}
\name{\fname{M.} \surname{Ikeda}}{60}
\name{\fname{K.} \surname{Indo}}{32}
\name{\fname{T.H.} \surname{Ishida}}{70}
\name{\fname{T.} \surname{Ishida}}{15}
\name{\fname{M.} \surname{Ishitsuka}}{64}
\name{\fname{H.} \surname{Ito}}{31}
\name{\fname{S.} \surname{Ito}}{73}
\name{\fname{A.} \surname{Izmaylov}}{25}
\name{\fname{N.} \surname{Jachowicz}}{13}
\name{\fname{B.} \surname{Jargowsky}}{2}
\name{\fname{S.J.} \surname{Jenkins}}{36}
\name{\fname{C.} \surname{Jes\'us-Valls}}{10}
\name{\fname{M.} \surname{Jia}}{42}
\name{\fname{J.J.} \surname{Jiang}}{42}
\name{\fname{J.Y.} \surname{Ji}}{42}
\name{\fname{T.P.} \surname{Jones}}{33}
\name{\fname{P.} \surname{Jonsson}}{20}
\name{\fname{S.} \surname{Joshi}}{42}
\name{\fname{C.K.} \surname{Jung}}{42}%\%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Kabirnezhad}}{46}
\name{\fname{A.C.} \surname{Kaboth}}{50}
\name{\fname{K.} \surname{Kadota}}{31}
\name{\fname{H.} \surname{Kakuno}}{63}
\name{\fname{A.} \surname{Kamata}}{63}
\name{\fname{J.} \surname{Kameda}}{60}
\name{\fname{S.} \surname{Karpova}}{11}
\name{\fname{V.S.} \surname{Kasturi}}{11}
\name{\fname{Y.} \surname{Kataoka}}{60}
\name{\fname{T.} \surname{Katori}}{30}
\name{\fname{A.} \surname{Kawabata}}{29}
\name{\fname{R.} \surname{Kawabe}}{45}
\name{\fname{Y.} \surname{Kawamura}}{45}
\name{\fname{M.} \surname{Kawaue}}{32}
\name{\fname{E.} \surname{Kearns}}{2}%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Khabibullin}}{25}
\name{\fname{N.V.} \surname{Khomutov}}{38}
\name{\fname{A.} \surname{Khotjantsev}}{25}
\name{\fname{T.} \surname{Kikawa}}{32}
\name{\fname{S.} \surname{King}}{30}
\name{\fname{V.} \surname{Kiseeva}}{38}
\name{\fname{J.} \surname{Kisiel}}{55}
\name{\fname{A.} \surname{Klustov\'a}}{20}
\name{\fname{L.} \surname{Kneale}}{54}
\name{\fname{H.} \surname{Kobayashi}}{59}
\name{\fname{S.R.} \surname{Kobayashi}}{70}
\name{\fname{T.} \surname{Kobayashi}}{15}
\name{\fname{L.} \surname{Koch}}{18}
\name{\fname{S.} \surname{Kodama}}{59}
\name{\fname{M.} \surname{Kolupanova}}{25}
\name{\fname{A.} \surname{Konaka}}{65}
\name{\fname{L.L.} \surname{Kormos}}{33}
\name{\fname{Y.} \surname{Koshio}}{44}%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{K.} \surname{Kowalik}}{41}
\name{\fname{R.} \surname{Kralik}}{30}
\name{\fname{Y.} \surname{Kudenko}}{25}
\name{\fname{Y.} \surname{Kudo}}{73}
\name{\fname{A.} \surname{Kumar Jha}}{13}
\name{\fname{R.} \surname{Kurjata}}{69}
\name{\fname{V.} \surname{Kurochka}}{25}
\name{\fname{T.} \surname{Kutter}}{37}
\name{\fname{L.} \surname{Labarga}}{1}
\name{\fname{M.} \surname{Lachat}}{49}
\name{\fname{K.} \surname{Lachner}}{8}
\name{\fname{J.} \surname{Lagoda}}{41}
\name{\fname{S.M.} \surname{Lakshmi}}{55}
\name{\fname{M.} \surname{Lamers James}}{71}
\name{\fname{A.} \surname{Langella}}{22}
\name{\fname{D.H.} \surname{Langridge}}{50}
\name{\fname{J.-F.} \surname{Laporte}}{5}
\name{\fname{D.} \surname{Last}}{49}
\name{\fname{N.} \surname{Latham}}{30}
\name{\fname{M.} \surname{Laveder}}{23}
\name{\fname{L.} \surname{Lavitola}}{22}
\name{\fname{M.} \surname{Lawe}}{33}
\name{\fname{A.} \surname{Leclerc}}{5}
\name{\fname{N.} \surname{Lemaire}}{35}
\name{\fname{D.} \surname{Leon Silverio}}{58}
\name{\fname{T.} \surname{Leplumey}}{35}
\name{\fname{S.} \surname{Levorato}}{23}
\name{\fname{S.V.} \surname{Lewis}}{30}
\name{\fname{B.} \surname{Li}}{8}
\name{\fname{C.} \surname{Lin}}{20}
\name{\fname{R.P.} \surname{Litchfield}}{12}
\name{\fname{S.L.} \surname{Liu}}{42}
\name{\fname{W.} \surname{Li}}{46}
\name{\fname{A.} \surname{Longhin}}{23}
\name{\fname{A.} \surname{Lopez Moreno}}{30}
\name{\fname{L.} \surname{Ludovici}}{24}
\name{\fname{X.} \surname{Lu}}{71}
\name{\fname{T.} \surname{Lux}}{17}
\name{\fname{L.N.} \surname{Machado}}{12}
\name{\fname{L.} \surname{Magaletti}}{21}
\name{\fname{K.} \surname{Mahn}}{39}
\name{\fname{K.K.} \surname{Mahtani}}{42}
\name{\fname{S.} \surname{Manly}}{49}
\name{\fname{A.D.} \surname{Marino}}{6}
\name{\fname{D.G.R.} \surname{Martin}}{20}
\name{\fname{D.A.} \surname{Martinez Caicedo}}{58}
\name{\fname{L.} \surname{Martinez}}{17}
\name{\fname{M.} \surname{Martini}}{57}
\name{\fname{N.} \surname{Mashin}}{25}
\name{\fname{T.} \surname{Matsubara}}{15}
\name{\fname{R.} \surname{Matsumoto}}{62}
\name{\fname{V.} \surname{Matveev}}{25}
\name{\fname{C.} \surname{Mauger}}{47}
\name{\fname{K.} \surname{Mavrokoridis}}{36}
\name{\fname{N.} \surname{McCauley}}{36}
\name{\fname{K.S.} \surname{McFarland}}{49}
\name{\fname{C.} \surname{McGrew}}{42}
\name{\fname{J.} \surname{McKean}}{32}
\name{\fname{A.} \surname{Mefodiev}}{25}
\name{\fname{G.D.} \surname{Megias}}{53}
\name{\fname{L.} \surname{Mellet}}{39}
\name{\fname{C.} \surname{Metelko}}{36}
\name{\fname{M.} \surname{Mezzetto}}{23}
\name{\fname{S.} \surname{Miki}}{60}
\name{\fname{V.} \surname{Mikola}}{12}
\name{\fname{E.W.} \surname{Miller}}{20}
\name{\fname{A.} \surname{Minamino}}{73}
\name{\fname{O.} \surname{Mineev}}{25}
\name{\fname{S.} \surname{Mine}}{60,4}
\name{\fname{J.} \surname{Mirabito}}{2}
\name{\fname{M.} \surname{Miura}}{60}%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{60}%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{73}
\name{\fname{P.} \surname{Morrison}}{12}
\name{\fname{Th.A.} \surname{Mueller}}{35}
\name{\fname{D.} \surname{Munford}}{16}
\name{\fname{A.} \surname{Mu\~noz}}{18}
\name{\fname{L.} \surname{Munteanu}}{10}
\name{\fname{Y.} \surname{Nagai}}{15}
\name{\fname{T.} \surname{Nakadaira}}{15}
\name{\fname{K.} \surname{Nakagiri}}{60}
\name{\fname{M.} \surname{Nakahata}}{60,28}
\name{\fname{Y.} \surname{Nakajima}}{59}
\name{\fname{K.D.} \surname{Nakamura}}{70}
\name{\fname{A.} \surname{Nakano}}{70}
\name{\fname{Y.} \surname{Nakano}}{66}
\name{\fname{S.} \surname{Nakayama}}{60,28}
\name{\fname{T.} \surname{Nakaya}}{32,28}
\name{\fname{K.} \surname{Nakayoshi}}{15}
\name{\fname{C.E.R.} \surname{Naseby}}{20}
\name{\fname{D.T.} \surname{Nguyen}}{9}
\name{\fname{V.Q.} \surname{Nguyen}}{35}
\name{\fname{K.} \surname{Niewczas}}{35,13}
\name{\fname{S.} \surname{Nishimori}}{59}
\name{\fname{Y.} \surname{Nishimura}}{29}
\name{\fname{Y.} \surname{Noguchi}}{60}
\name{\fname{T.} \surname{Nosek}}{41}
\name{\fname{F.} \surname{Nova}}{43}
\name{\fname{J.C.} \surname{Nugent}}{20}
\name{\fname{H.M.} \surname{O'Keeffe}}{33}
\name{\fname{L.} \surname{O'Sullivan}}{18}
\name{\fname{R.} \surname{Okazaki}}{29}
\name{\fname{W.} \surname{Okinaga}}{59}
\name{\fname{K.} \surname{Okumura}}{61,28}
\name{\fname{T.} \surname{Okusawa}}{45}
\name{\fname{N.} \surname{Onda}}{32}
\name{\fname{N.} \surname{Ospina}}{21}
\name{\fname{L.} \surname{Osu}}{35}
\name{\fname{N.} \surname{Otani}}{32}
\name{\fname{Y.} \surname{Oyama}}{15}
\name{\fname{V.} \surname{Paolone}}{48}
\name{\fname{J.} \surname{Pasternak}}{20}
\name{\fname{D.} \surname{Payne}}{36}
\name{\fname{T.P.D.} \surname{Peacock}}{54}
\name{\fname{M.} \surname{Pfaff}}{20}
\name{\fname{L.} \surname{Pickering}}{43}
\name{\fname{J.-B.} \surname{Plan\c{c}on}}{35}
\name{\fname{P.} \surname{Podlaski}}{15}
\name{\fname{B.} \surname{Popov}}{57,46}
\name{\fname{A.J.} \surname{Portocarrero Yrey}}{15}
\name{\fname{M.} \surname{Posiadala-Zezula}}{68}
\name{\fname{Y.S.} \surname{Prabhu}}{68}
\name{\fname{H.} \surname{Prasad}}{72}
\name{\fname{F.} \surname{Pupilli}}{23}
\name{\fname{B.} \surname{Quilain}}{27,35}
\name{\fname{P.T.} \surname{Quyen}}{19}
\name{\fname{E.} \surname{Radicioni}}{21}
\name{\fname{B.} \surname{Radics}}{74}
\name{\fname{M.A.} \surname{Ramirez Delgado}}{47}
\name{\fname{R.} \surname{Ramsden}}{30}
\name{\fname{P.N.} \surname{Ratoff}}{33}
\name{\fname{M.} \surname{Reh}}{6}
\name{\fname{G.} \surname{Reina}}{18}
\name{\fname{L.} \surname{Restrepo}}{57}
\name{\fname{C.} \surname{Riccio}}{42}
\name{\fname{D.W.} \surname{Riley}}{12}
\name{\fname{E.} \surname{Rondio}}{41}
\name{\fname{D.} \surname{Ross}}{39}
\name{\fname{S.} \surname{Roth}}{51}
\name{\fname{N.} \surname{Roy}}{74}
\name{\fname{A.} \surname{Rubbia}}{8}
\name{\fname{L.} \surname{Russo}}{57}
\name{\fname{A.} \surname{Rychter}}{69}
\name{\fname{W.} \surname{Saenz}}{57}
\name{\fname{K.} \surname{Sakashita}}{67,15}
\name{\fname{S.} \surname{Samani}}{11}
\name{\fname{F.} \surname{S\'anchez}}{11}
\name{\fname{E.M.} \surname{Sandford}}{36}
\name{\fname{Y.} \surname{Sato}}{64}
\name{\fname{T.} \surname{Schefke}}{37}
\name{\fname{K.} \surname{Scholberg}}{7}%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Scott}}{20}
\name{\fname{Y.} \surname{Seiya}}{45,53}
\name{\fname{T.} \surname{Sekiguchi}}{15}
\name{\fname{H.} \surname{Sekiya}}{60,28}%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Sekiyama}}{59}
\name{\fname{T.} \surname{Sekiya}}{63}
\name{\fname{D.} \surname{Seppala}}{39}
\name{\fname{D.} \surname{Sgalaberna}}{8}
\name{\fname{A.} \surname{Shaikhiev}}{25}
\name{\fname{M.} \surname{Shiozawa}}{60,28}
\name{\fname{Y.} \surname{Shiraishi}}{44}
\name{\fname{N.} \surname{Shvarev}}{25}
\name{\fname{A.} \surname{Shvartsman}}{25}
\name{\fname{V.} \surname{Siccardi}}{30}
\name{\fname{N.} \surname{Skrobova}}{25}
\name{\fname{K.} \surname{Skwarczynski}}{50}
\name{\fname{D.} \surname{Smyczek}}{51}
\name{\fname{M.} \surname{Smy}}{4}
\name{\fname{J.T.} \surname{Sobczyk}}{72}
\name{\fname{H.} \surname{Sobel}}{4,28}
\name{\fname{F.J.P.} \surname{Soler}}{12}
\name{\fname{A.J.} \surname{Speers}}{33}
\name{\fname{R.} \surname{Spina}}{21}
\name{\fname{A.} \surname{Srivastava}}{18}
\name{\fname{P.} \surname{Stowell}}{54}
\name{\fname{Y.} \surname{Stroke}}{25}
\name{\fname{I.A.} \surname{Suslov}}{38}
\name{\fname{A.} \surname{Suzuki}}{31}
\name{\fname{M.} \surname{Suzuki}}{73}
\name{\fname{S.Y.} \surname{Suzuki}}{15}
\name{\fname{M.} \surname{Tada}}{15}
\name{\fname{S.} \surname{Tairafune}}{70}
\name{\fname{A.} \surname{Takeda}}{60}
\name{\fname{Y.} \surname{Takeuchi}}{31,28}
\name{\fname{K.} \surname{Takeya}}{44}
\name{\fname{H.K.} \surname{Tanaka}}{60}%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{H.} \surname{Tanigawa}}{29}
\name{\fname{A.} \surname{Teklu}}{42}
\name{\fname{V.V.} \surname{Tereshchenko}}{38}
\name{\fname{N.} \surname{Thamm}}{51}
\name{\fname{C.} \surname{Touramanis}}{36}
\name{\fname{N.} \surname{Tran}}{19}
\name{\fname{T.} \surname{Tsukamoto}}{15}
\name{\fname{M.} \surname{Tzanov}}{37}
\name{\fname{Y.} \surname{Uchida}}{20}
\name{\fname{M.} \surname{Vagins}}{28,4}
\name{\fname{M.} \surname{Varghese}}{17}
\name{\fname{I.} \surname{Vasilyev}}{38}
\name{\fname{G.} \surname{Vasseur}}{5}
\name{\fname{E.} \surname{Villa}}{8}
\name{\fname{U.} \surname{Virginet}}{57}
\name{\fname{T.} \surname{Vladisavljevic}}{43}
\name{\fname{T.} \surname{Wachala}}{14}
\name{\fname{S.-i.} \surname{Wada}}{31}
\name{\fname{D.} \surname{Wakabayashi}}{70}
\name{\fname{H.T.} \surname{Wallace}}{54}
\name{\fname{J.G.} \surname{Walsh}}{39}
\name{\fname{D.} \surname{Wark}}{43,46}
\name{\fname{M.O.} \surname{Wascko}}{46,43}
\name{\fname{A.} \surname{Weber}}{18}
\name{\fname{R.} \surname{Wendell}}{32}
\name{\fname{M.J.} \surname{Wilking}}{52}
\name{\fname{C.} \surname{Wilkinson}}{34}
\name{\fname{J.R.} \surname{Wilson}}{30}
\name{\fname{C.} \surname{Winterstein}}{5}
\name{\fname{K.} \surname{Wood}}{34}
\name{\fname{C.} \surname{Wret}}{20}
\name{\fname{J.} \surname{Xia}}{56}
\name{\fname{Z.} \surname{Xie}}{52}
\name{\fname{K.} \surname{Yamamoto}}{45,53}
\name{\fname{T.} \surname{Yamamoto}}{45}
\name{\fname{T.} \surname{Yamazumi}}{59}
\name{\fname{C.} \surname{Yanagisawa}}{42}
\name{\fname{Y.} \surname{Yang}}{46}
\name{\fname{T.} \surname{Yano}}{60}
\name{\fname{N.} \surname{Yershov}}{25}
\name{\fname{U.} \surname{Yevarouskaya}}{42}
\name{\fname{M.} \surname{Yokoyama}}{59}%thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{Y.} \surname{Yoshimoto}}{59}
\name{\fname{N.} \surname{Yoshimura}}{32}
\name{\fname{R.} \surname{Zaki}}{74}
\name{\fname{A.} \surname{Zalewska}}{14}
\name{\fname{J.} \surname{Zalipska}}{41}
\name{\fname{G.} \surname{Zarnecki}}{14}
\name{\fname{J.} \surname{Zhang}}{65,3}
\name{\fname{X.Y.} \surname{Zhao}}{20}
\name{\fname{H.} \surname{Zheng}}{42}
\name{\fname{H.} \surname{Zhong}}{31}
\name{\fname{T.} \surname{Zhu}}{20}
\name{\fname{M.} \surname{Ziembicki}}{69}
\name{\fname{E.D.} \surname{Zimmerman}}{6}
\name{\fname{M.} \surname{Zito}}{57}
\name{\fname{S.} \surname{Zsoldos}}{30}
}

\address{
\affil{1}{University Autonoma Madrid, Department of Theoretical Physics, 28049 Madrid, Spain}
\affil{2}{Boston University, Department of Physics, Boston, Massachusetts, U.S.A.}
\affil{3}{University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada}
\affil{4}{University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.}
\affil{5}{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affil{6}{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}
\affil{7}{Duke University, Department of Physics, Durham, North Carolina, U.S.A.}
\affil{8}{ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland}
\affil{9}{VNU University of Science, Vietnam National University, Hanoi, Vietnam}
\affil{10}{CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland}
\affil{11}{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}
\affil{12}{University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom}
\affil{13}{Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium}
\affil{14}{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}
\affil{15}{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}
\affil{16}{University of Houston, Department of Physics, Houston, Texas, U.S.A.}
\affil{17}{Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}
\affil{18}{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Staudingerweg 7, 55128 Mainz, Germany}
\affil{19}{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}
\affil{20}{Imperial College London, Department of Physics, London, United Kingdom}
\affil{21}{INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}
\affil{22}{INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}
\affil{23}{INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}
\affil{24}{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy}
\affil{25}{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}
\affil{26}{International Centre of Physics, Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), 10 Dao Tan, Ba Dinh, Hanoi, Vietnam}
\affil{27}{ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}
\affil{28}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}
\affil{29}{Keio University, Department of Physics, Kanagawa, Japan}
\affil{30}{King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom}
\affil{31}{Kobe University, Kobe, Japan}
\affil{32}{Kyoto University, Department of Physics, Kyoto, Japan}
\affil{33}{Lancaster University, School of Physics and Astronomy, Lancaster, United Kingdom}
\affil{34}{Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.}
\affil{35}{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France}
\affil{36}{University of Liverpool, Department of Physics, Liverpool, United Kingdom}
\affil{37}{Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}
\affil{38}{Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia}
\affil{39}{Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.}
\affil{40}{Miyagi University of Education, Department of Physics, Sendai, Japan}
\affil{41}{National Centre for Nuclear Research, Warsaw, Poland}
\affil{42}{State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}
\affil{43}{STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}
\affil{44}{Okayama University, Department of Physics, Okayama, Japan}
\affil{45}{Osaka Metropolitan University, Department of Physics, Osaka, Japan}
\affil{46}{Oxford University, Department of Physics, Oxford, United Kingdom}
\affil{47}{University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.}
\affil{48}{University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.}
\affil{49}{University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}
\affil{50}{Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom}
\affil{51}{RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany}
\affil{52}{School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota, U.S.A.}
\affil{53}{Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain}
\affil{54}{University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom}
\affil{55}{University of Silesia, Institute of Physics, Katowice, Poland}
\affil{56}{SLAC National Accelerator Laboratory, Stanford University, Menlo Park, California, U.S.A.}
\affil{57}{Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}
\affil{58}{South Dakota School of Mines and Technology, 501 East Saint Joseph Street, Rapid City, SD 57701, United States}
\affil{59}{University of Tokyo, Department of Physics, Tokyo, Japan}
\affil{60}{University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}
\affil{61}{University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}
\affil{62}{Institute of Science Tokyo, Department of Physics, Tokyo}
\affil{63}{Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}
\affil{64}{Tokyo University of Science, Faculty of Science and Technology, Department of Physics, Noda, Chiba, Japan}
\affil{65}{TRIUMF, Vancouver, British Columbia, Canada}
\affil{66}{University of Toyama, Faculty of Science, Toyama, Japan}
\affil{67}{University of Tsukuba, Faculty of Pure and Applied Sciences, Tsukuba, Ibaraki, Japan}
\affil{68}{University of Warsaw, Faculty of Physics, Warsaw, Poland}
\affil{69}{Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland}
\affil{70}{Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan}
\affil{71}{University of Warwick, Department of Physics, Coventry, United Kingdom}
\affil{72}{Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}
\affil{73}{Yokohama National University, Department of Physics, Yokohama, Japan}
\affil{74}{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}
}


==> authorlist_PTEP_442_restored_affil.tex <==
% T2K author list in ptephy_v1 PTEP format
% All 'Also at' notes converted to numbered affiliations.
% 442 authors / 80 affiliations
\author{
\name{\fname{K.} \surname{Abe}}{60}
\name{\fname{S.} \surname{Abe}}{60}
\name{\fname{H.} \surname{Adhikary}}{68}
\name{\fname{R.} \surname{Akutsu}}{15}
\name{\fname{H.} \surname{Alarakia-Charles}}{33}
\name{\fname{Y.I.} \surname{Alj Hakim}}{54}
\name{\fname{S.} \surname{Alonso Monsalve}}{8}
\name{\fname{L.} \surname{Anthony}}{20}
\name{\fname{S.} \surname{Aoki}}{31}
\name{\fname{K.A.} \surname{Apte}}{20}
\name{\fname{T.} \surname{Arai}}{59}
\name{\fname{T.} \surname{Arihara}}{63}
\name{\fname{S.} \surname{Arimoto}}{32}
\name{\fname{Y.} \surname{Asami}}{63}
\name{\fname{Y.} \surname{Asaoka}}{60}
\name{\fname{Y.} \surname{Ashida}}{70}
\name{\fname{E.T.} \surname{Atkin}}{20}
\name{\fname{N.} \surname{Babu}}{37}
\name{\fname{V.} \surname{Baranov}}{38}
\name{\fname{G.J.} \surname{Barker}}{71}
\name{\fname{G.} \surname{Barr}}{46}
\name{\fname{D.} \surname{Barrow}}{46}
\name{\fname{P.} \surname{Bates}}{36}
\name{\fname{L.} \surname{Bathe-Peters}}{46}
\name{\fname{M.} \surname{Batkiewicz-Kwasniak}}{14}
\name{\fname{N.} \surname{Baudis}}{46}
\name{\fname{A.} \surname{Beliakova}}{25}
\name{\fname{V.} \surname{Berardi}}{21}
\name{\fname{L.} \surname{Berns}}{70}
\name{\fname{S.} \surname{Bhattacharjee}}{37}
\name{\fname{A.} \surname{Blanchet}}{57}
\name{\fname{A.} \surname{Blondel}}{57,11}
\name{\fname{L.} \surname{B{\o}e}}{16}
\name{\fname{P.M.M.} \surname{Boistier}}{5}
\name{\fname{S.} \surname{Bolognesi}}{5}
\name{\fname{B.} \surname{Bombin}}{25}
\name{\fname{S.} \surname{Bordoni}}{11}
\name{\fname{S.B.} \surname{Boyd}}{71}
\name{\fname{C.} \surname{Bronner}}{73}
\name{\fname{A.} \surname{Bubak}}{55}
\name{\fname{M.} \surname{Buizza Avanzini}}{35}
\name{\fname{J.A.} \surname{Caballero}}{53}
\name{\fname{N.F.} \surname{Calabria}}{21}
\name{\fname{S.} \surname{Cao}}{19}
\name{\fname{S.} \surname{Cap}}{11}
\name{\fname{D.} \surname{Carabadjac}}{35,5}
\name{\fname{S.L.} \surname{Cartwright}}{54}
\name{\fname{M.P.} \surname{Casado}}{17,75}
\name{\fname{M.G.} \surname{Catanesi}}{21}
\name{\fname{J.} \surname{Chakrani}}{34}
\name{\fname{A.} \surname{Chalumeau}}{57}
\name{\fname{D.} \surname{Cherdack}}{16}
\name{\fname{A.} \surname{Chvirova}}{25}
\name{\fname{J.} \surname{Coleman}}{36}
\name{\fname{G.} \surname{Collazuol}}{23}
\name{\fname{F.} \surname{Cormier}}{65}
\name{\fname{A.A.L.} \surname{Craplet}}{20}
\name{\fname{A.} \surname{Cudd}}{6}
\name{\fname{D.} \surname{D'Ago}}{23}
\name{\fname{C.} \surname{Dalmazzone}}{57}
\name{\fname{T.} \surname{Daret}}{5}
\name{\fname{P.} \surname{Dasgupta}}{17}
\name{\fname{C.} \surname{Davis}}{47}
\name{\fname{Yu.I.} \surname{Davydov}}{38}
\name{\fname{P.} \surname{de Perio}}{28}
\name{\fname{G.} \surname{De Rosa}}{22}
\name{\fname{T.} \surname{Dealtry}}{33}
\name{\fname{C.} \surname{Densham}}{43}
\name{\fname{A.} \surname{Dergacheva}}{25}
\name{\fname{R.} \surname{Dharmapal Banerjee}}{72}
\name{\fname{F.} \surname{Di Lodovico}}{30}
\name{\fname{G.} \surname{Diaz Lopez}}{57}
\name{\fname{S.} \surname{Dolan}}{10}
\name{\fname{D.} \surname{Douqa}}{11}
\name{\fname{T.A.} \surname{Doyle}}{46}
\name{\fname{O.} \surname{Drapier}}{35}
\name{\fname{K.E.} \surname{Duffy}}{46}
\name{\fname{J.} \surname{Dumarchez}}{57}
\name{\fname{P.} \surname{Dunne}}{20}
\name{\fname{K.} \surname{Dygnarowicz}}{69}
\name{\fname{A.} \surname{Eguchi}}{59}
\name{\fname{M.} \surname{El Baz}}{11}
\name{\fname{J.} \surname{Elias}}{49}
\name{\fname{S.} \surname{Emery-Schrenk}}{5}
\name{\fname{G.} \surname{Erofeev}}{25}
\name{\fname{A.} \surname{Ershova}}{35}
\name{\fname{G.} \surname{Eurin}}{5}
\name{\fname{M.} \surname{Fani}}{52}
\name{\fname{D.} \surname{Fedorova}}{25}
\name{\fname{S.} \surname{Fedotov}}{25}
\name{\fname{M.} \surname{Feltre}}{23}
\name{\fname{C.} \surname{Fengler}}{46}
\name{\fname{L.} \surname{Feng}}{32}
\name{\fname{D.} \surname{Ferlewicz}}{57}
\name{\fname{A.J.} \surname{Finch}}{33}
\name{\fname{M.D.} \surname{Fitton}}{43}
\name{\fname{C.} \surname{Forza}}{23}
\name{\fname{M.} \surname{Friend}}{15,76}
\name{\fname{Y.} \surname{Fujii}}{15,76}
\name{\fname{Y.} \surname{Fukuda}}{40}
\name{\fname{N.} \surname{Funayama}}{45}
\name{\fname{Y.} \surname{Furui}}{63}
\name{\fname{A.N.} \surname{Gaci\~no Olmedo}}{57}
\name{\fname{J.} \surname{Garc\'ia-Marcos}}{13}
\name{\fname{A.C.} \surname{Germer}}{47}
\name{\fname{L.} \surname{Giannessi}}{11}
\name{\fname{C.} \surname{Giganti}}{57}
\name{\fname{M.} \surname{Girgus}}{68}
\name{\fname{V.} \surname{Glagolev}}{38}
\name{\fname{P.} \surname{Golak}}{68}
\name{\fname{M.} \surname{Gonin}}{27}
\name{\fname{R.} \surname{Gonzalez Jimenez}}{53}
\name{\fname{J.} \surname{Gonz\'alez Rosa}}{53}
\name{\fname{E.A.G.} \surname{Goodman}}{12}
\name{\fname{K.} \surname{Gorshanov}}{25}
\name{\fname{P.} \surname{Govindaraj}}{68}
\name{\fname{M.} \surname{Grassi}}{23}
\name{\fname{M.} \surname{Guigue}}{57}
\name{\fname{F.Y.} \surname{Guo}}{42}
\name{\fname{D.R.} \surname{Hadley}}{71}
\name{\fname{S.} \surname{Han}}{32,61}
\name{\fname{D.A.} \surname{Harris}}{74}
\name{\fname{R.J.} \surname{Harris}}{33,43}
\name{\fname{M.} \surname{Hartz}}{65,28}
\name{\fname{K.} \surname{Hasegawa}}{32}
\name{\fname{T.} \surname{Hasegawa}}{15,76}
\name{\fname{C.M.} \surname{Hasnip}}{10}
\name{\fname{S.} \surname{Hassani}}{5}
\name{\fname{N.C.} \surname{Hastings}}{15}
\name{\fname{K.} \surname{Hayashi}}{32}
\name{\fname{Y.} \surname{Hayato}}{60,28}
\name{\fname{I.} \surname{Heitkamp}}{70}
\name{\fname{D.} \surname{Henaff}}{5}
\name{\fname{Y.} \surname{Hino}}{15}
\name{\fname{K.} \surname{Hiraide}}{60,28}
\name{\fname{J.} \surname{Holeczek}}{55}
\name{\fname{A.} \surname{Holin}}{43}
\name{\fname{T.} \surname{Holvey}}{46}
\name{\fname{N.T.} \surname{Hong Van}}{26}
\name{\fname{T.} \surname{Honjo}}{45}
\name{\fname{M.C.F.} \surname{Hooft}}{13}
\name{\fname{K.} \surname{Hosokawa}}{60}
\name{\fname{R.} \surname{Huang}}{34}
\name{\fname{J.} \surname{Hu}}{32}
\name{\fname{A.K.} \surname{Ichikawa}}{70}
\name{\fname{K.} \surname{Ieki}}{60}
\name{\fname{M.} \surname{Ikeda}}{60}
\name{\fname{K.} \surname{Indo}}{32}
\name{\fname{T.H.} \surname{Ishida}}{70}
\name{\fname{T.} \surname{Ishida}}{15,76}
\name{\fname{M.} \surname{Ishitsuka}}{64}
\name{\fname{H.} \surname{Ito}}{31}
\name{\fname{S.} \surname{Ito}}{73}
\name{\fname{A.} \surname{Izmaylov}}{25}
\name{\fname{N.} \surname{Jachowicz}}{13}
\name{\fname{B.} \surname{Jargowsky}}{2}
\name{\fname{S.J.} \surname{Jenkins}}{36}
\name{\fname{C.} \surname{Jes\'us-Valls}}{10}
\name{\fname{M.} \surname{Jia}}{42}
\name{\fname{J.J.} \surname{Jiang}}{42}
\name{\fname{J.Y.} \surname{Ji}}{42}
\name{\fname{T.P.} \surname{Jones}}{33}
\name{\fname{P.} \surname{Jonsson}}{20}
\name{\fname{S.} \surname{Joshi}}{42}
\name{\fname{C.K.} \surname{Jung}}{42}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Kabirnezhad}}{46}
\name{\fname{A.C.} \surname{Kaboth}}{50}
\name{\fname{K.} \surname{Kadota}}{31}
\name{\fname{H.} \surname{Kakuno}}{63}
\name{\fname{A.} \surname{Kamata}}{63}
\name{\fname{J.} \surname{Kameda}}{60}
\name{\fname{S.} \surname{Karpova}}{11}
\name{\fname{V.S.} \surname{Kasturi}}{11}
\name{\fname{Y.} \surname{Kataoka}}{60}
\name{\fname{T.} \surname{Katori}}{30}
\name{\fname{A.} \surname{Kawabata}}{29}
\name{\fname{R.} \surname{Kawabe}}{45}
\name{\fname{Y.} \surname{Kawamura}}{45}
\name{\fname{M.} \surname{Kawaue}}{32}
\name{\fname{E.} \surname{Kearns}}{2}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Khabibullin}}{25}
\name{\fname{N.V.} \surname{Khomutov}}{38}
\name{\fname{A.} \surname{Khotjantsev}}{25}
\name{\fname{T.} \surname{Kikawa}}{32}
\name{\fname{S.} \surname{King}}{30}
\name{\fname{V.} \surname{Kiseeva}}{38}
\name{\fname{J.} \surname{Kisiel}}{55}
\name{\fname{A.} \surname{Klustov\'a}}{20}
\name{\fname{L.} \surname{Kneale}}{54}
\name{\fname{H.} \surname{Kobayashi}}{59}
\name{\fname{S.R.} \surname{Kobayashi}}{70}
\name{\fname{T.} \surname{Kobayashi}}{15,76}
\name{\fname{L.} \surname{Koch}}{18}
\name{\fname{S.} \surname{Kodama}}{59}
\name{\fname{M.} \surname{Kolupanova}}{25,77}
\name{\fname{A.} \surname{Konaka}}{65}
\name{\fname{L.L.} \surname{Kormos}}{33}
\name{\fname{Y.} \surname{Koshio}}{44}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{K.} \surname{Kowalik}}{41}
\name{\fname{R.} \surname{Kralik}}{30}
\name{\fname{Y.} \surname{Kudenko}}{25,77}
\name{\fname{Y.} \surname{Kudo}}{73}
\name{\fname{A.} \surname{Kumar Jha}}{13}
\name{\fname{R.} \surname{Kurjata}}{69}
\name{\fname{V.} \surname{Kurochka}}{25}
\name{\fname{T.} \surname{Kutter}}{37}
\name{\fname{L.} \surname{Labarga}}{1}
\name{\fname{M.} \surname{Lachat}}{49}
\name{\fname{K.} \surname{Lachner}}{8}
\name{\fname{J.} \surname{Lagoda}}{41}
\name{\fname{S.M.} \surname{Lakshmi}}{55}
\name{\fname{M.} \surname{Lamers James}}{71}
\name{\fname{A.} \surname{Langella}}{22}
\name{\fname{D.H.} \surname{Langridge}}{50}
\name{\fname{J.-F.} \surname{Laporte}}{5}
\name{\fname{D.} \surname{Last}}{49}
\name{\fname{N.} \surname{Latham}}{30}
\name{\fname{M.} \surname{Laveder}}{23}
\name{\fname{L.} \surname{Lavitola}}{22}
\name{\fname{M.} \surname{Lawe}}{33}
\name{\fname{A.} \surname{Leclerc}}{5}
\name{\fname{N.} \surname{Lemaire}}{35}
\name{\fname{D.} \surname{Leon Silverio}}{58}
\name{\fname{T.} \surname{Leplumey}}{35}
\name{\fname{S.} \surname{Levorato}}{23}
\name{\fname{S.V.} \surname{Lewis}}{30}
\name{\fname{B.} \surname{Li}}{8}
\name{\fname{C.} \surname{Lin}}{20}
\name{\fname{R.P.} \surname{Litchfield}}{12}
\name{\fname{S.L.} \surname{Liu}}{42}
\name{\fname{W.} \surname{Li}}{46}
\name{\fname{A.} \surname{Longhin}}{23}
\name{\fname{A.} \surname{Lopez Moreno}}{30}
\name{\fname{L.} \surname{Ludovici}}{24}
\name{\fname{X.} \surname{Lu}}{71}
\name{\fname{T.} \surname{Lux}}{17}
\name{\fname{L.N.} \surname{Machado}}{12}
\name{\fname{L.} \surname{Magaletti}}{21}
\name{\fname{K.} \surname{Mahn}}{39}
\name{\fname{K.K.} \surname{Mahtani}}{42}
\name{\fname{S.} \surname{Manly}}{49}
\name{\fname{A.D.} \surname{Marino}}{6}
\name{\fname{D.G.R.} \surname{Martin}}{20}
\name{\fname{D.A.} \surname{Martinez Caicedo}}{58}
\name{\fname{L.} \surname{Martinez}}{17}
\name{\fname{M.} \surname{Martini}}{57,78}
\name{\fname{N.} \surname{Mashin}}{25}
\name{\fname{T.} \surname{Matsubara}}{15}
\name{\fname{R.} \surname{Matsumoto}}{62}
\name{\fname{V.} \surname{Matveev}}{25}
\name{\fname{C.} \surname{Mauger}}{47}
\name{\fname{K.} \surname{Mavrokoridis}}{36}
\name{\fname{N.} \surname{McCauley}}{36}
\name{\fname{K.S.} \surname{McFarland}}{49}
\name{\fname{C.} \surname{McGrew}}{42}
\name{\fname{J.} \surname{McKean}}{32}
\name{\fname{A.} \surname{Mefodiev}}{25}
\name{\fname{G.D.} \surname{Megias}}{53}
\name{\fname{L.} \surname{Mellet}}{39}
\name{\fname{C.} \surname{Metelko}}{36}
\name{\fname{M.} \surname{Mezzetto}}{23}
\name{\fname{S.} \surname{Miki}}{60}
\name{\fname{V.} \surname{Mikola}}{12}
\name{\fname{E.W.} \surname{Miller}}{20}
\name{\fname{A.} \surname{Minamino}}{73}
\name{\fname{O.} \surname{Mineev}}{25}
\name{\fname{S.} \surname{Mine}}{60,4}
\name{\fname{J.} \surname{Mirabito}}{2}
\name{\fname{M.} \surname{Miura}}{60}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{60}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{73}
\name{\fname{P.} \surname{Morrison}}{12}
\name{\fname{Th.A.} \surname{Mueller}}{35}
\name{\fname{D.} \surname{Munford}}{16}
\name{\fname{A.} \surname{Mu\~noz}}{18}
\name{\fname{L.} \surname{Munteanu}}{10}
\name{\fname{Y.} \surname{Nagai}}{15}
\name{\fname{T.} \surname{Nakadaira}}{15,76}
\name{\fname{K.} \surname{Nakagiri}}{60}
\name{\fname{M.} \surname{Nakahata}}{60,28}
\name{\fname{Y.} \surname{Nakajima}}{59}
\name{\fname{K.D.} \surname{Nakamura}}{70}
\name{\fname{A.} \surname{Nakano}}{70}
\name{\fname{Y.} \surname{Nakano}}{66}
\name{\fname{S.} \surname{Nakayama}}{60,28}
\name{\fname{T.} \surname{Nakaya}}{32,28}
\name{\fname{K.} \surname{Nakayoshi}}{15,76}
\name{\fname{C.E.R.} \surname{Naseby}}{20}
\name{\fname{D.T.} \surname{Nguyen}}{9}
\name{\fname{V.Q.} \surname{Nguyen}}{35}
\name{\fname{K.} \surname{Niewczas}}{35,13}
\name{\fname{S.} \surname{Nishimori}}{59}
\name{\fname{Y.} \surname{Nishimura}}{29}
\name{\fname{Y.} \surname{Noguchi}}{60}
\name{\fname{T.} \surname{Nosek}}{41}
\name{\fname{F.} \surname{Nova}}{43}
\name{\fname{J.C.} \surname{Nugent}}{20}
\name{\fname{H.M.} \surname{O'Keeffe}}{33}
\name{\fname{L.} \surname{O'Sullivan}}{18}
\name{\fname{R.} \surname{Okazaki}}{29}
\name{\fname{W.} \surname{Okinaga}}{59}
\name{\fname{K.} \surname{Okumura}}{61,28}
\name{\fname{T.} \surname{Okusawa}}{45}
\name{\fname{N.} \surname{Onda}}{32}
\name{\fname{N.} \surname{Ospina}}{21}
\name{\fname{L.} \surname{Osu}}{35}
\name{\fname{N.} \surname{Otani}}{32}
\name{\fname{Y.} \surname{Oyama}}{15,76}
\name{\fname{V.} \surname{Paolone}}{48}
\name{\fname{J.} \surname{Pasternak}}{20}
\name{\fname{D.} \surname{Payne}}{36}
\name{\fname{T.P.D.} \surname{Peacock}}{54}
\name{\fname{M.} \surname{Pfaff}}{20}
\name{\fname{L.} \surname{Pickering}}{43}
\name{\fname{J.-B.} \surname{Plan\c{c}on}}{35}
\name{\fname{P.} \surname{Podlaski}}{15,76}
\name{\fname{B.} \surname{Popov}}{57,46}
\name{\fname{A.J.} \surname{Portocarrero Yrey}}{15}
\name{\fname{M.} \surname{Posiadala-Zezula}}{68}
\name{\fname{Y.S.} \surname{Prabhu}}{68}
\name{\fname{H.} \surname{Prasad}}{72}
\name{\fname{F.} \surname{Pupilli}}{23}
\name{\fname{B.} \surname{Quilain}}{27,35}
\name{\fname{P.T.} \surname{Quyen}}{19,79}
\name{\fname{E.} \surname{Radicioni}}{21}
\name{\fname{B.} \surname{Radics}}{74}
\name{\fname{M.A.} \surname{Ramirez Delgado}}{47}
\name{\fname{R.} \surname{Ramsden}}{30}
\name{\fname{P.N.} \surname{Ratoff}}{33}
\name{\fname{M.} \surname{Reh}}{6}
\name{\fname{G.} \surname{Reina}}{18}
\name{\fname{L.} \surname{Restrepo}}{57}
\name{\fname{C.} \surname{Riccio}}{42}
\name{\fname{D.W.} \surname{Riley}}{12}
\name{\fname{E.} \surname{Rondio}}{41}
\name{\fname{D.} \surname{Ross}}{39}
\name{\fname{S.} \surname{Roth}}{51}
\name{\fname{N.} \surname{Roy}}{74}
\name{\fname{A.} \surname{Rubbia}}{8}
\name{\fname{L.} \surname{Russo}}{57}
\name{\fname{A.} \surname{Rychter}}{69}
\name{\fname{W.} \surname{Saenz}}{57}
\name{\fname{K.} \surname{Sakashita}}{67,15,76}
\name{\fname{S.} \surname{Samani}}{11}
\name{\fname{F.} \surname{S\'anchez}}{11}
\name{\fname{E.M.} \surname{Sandford}}{36}
\name{\fname{Y.} \surname{Sato}}{64}
\name{\fname{T.} \surname{Schefke}}{37}
\name{\fname{K.} \surname{Scholberg}}{7}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Scott}}{20}
\name{\fname{Y.} \surname{Seiya}}{45,53}
\name{\fname{T.} \surname{Sekiguchi}}{15,76}
\name{\fname{H.} \surname{Sekiya}}{60,28}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Sekiyama}}{59}
\name{\fname{T.} \surname{Sekiya}}{63}
\name{\fname{D.} \surname{Seppala}}{39}
\name{\fname{D.} \surname{Sgalaberna}}{8}
\name{\fname{A.} \surname{Shaikhiev}}{25}
\name{\fname{M.} \surname{Shiozawa}}{60,28}
\name{\fname{Y.} \surname{Shiraishi}}{44}
\name{\fname{N.} \surname{Shvarev}}{25}
\name{\fname{A.} \surname{Shvartsman}}{25}
\name{\fname{V.} \surname{Siccardi}}{30}
\name{\fname{N.} \surname{Skrobova}}{25}
\name{\fname{K.} \surname{Skwarczynski}}{50}
\name{\fname{D.} \surname{Smyczek}}{51}
\name{\fname{M.} \surname{Smy}}{4}
\name{\fname{J.T.} \surname{Sobczyk}}{72}
\name{\fname{H.} \surname{Sobel}}{4,28}
\name{\fname{F.J.P.} \surname{Soler}}{12}
\name{\fname{A.J.} \surname{Speers}}{33}
\name{\fname{R.} \surname{Spina}}{21}
\name{\fname{A.} \surname{Srivastava}}{18}
\name{\fname{P.} \surname{Stowell}}{54}
\name{\fname{Y.} \surname{Stroke}}{25}
\name{\fname{I.A.} \surname{Suslov}}{38}
\name{\fname{A.} \surname{Suzuki}}{31}
\name{\fname{M.} \surname{Suzuki}}{73}
\name{\fname{S.Y.} \surname{Suzuki}}{15,76}
\name{\fname{M.} \surname{Tada}}{15,76}
\name{\fname{S.} \surname{Tairafune}}{70}
\name{\fname{A.} \surname{Takeda}}{60}
\name{\fname{Y.} \surname{Takeuchi}}{31,28}
\name{\fname{K.} \surname{Takeya}}{44}
\name{\fname{H.K.} \surname{Tanaka}}{60}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{H.} \surname{Tanigawa}}{29}
\name{\fname{A.} \surname{Teklu}}{42}
\name{\fname{V.V.} \surname{Tereshchenko}}{38}
\name{\fname{N.} \surname{Thamm}}{51}
\name{\fname{C.} \surname{Touramanis}}{36}
\name{\fname{N.} \surname{Tran}}{19}
\name{\fname{T.} \surname{Tsukamoto}}{15,76}
\name{\fname{M.} \surname{Tzanov}}{37}
\name{\fname{Y.} \surname{Uchida}}{20}
\name{\fname{M.} \surname{Vagins}}{28,4}
\name{\fname{M.} \surname{Varghese}}{17}
\name{\fname{I.} \surname{Vasilyev}}{38}
\name{\fname{G.} \surname{Vasseur}}{5}
\name{\fname{E.} \surname{Villa}}{8}
\name{\fname{U.} \surname{Virginet}}{57}
\name{\fname{T.} \surname{Vladisavljevic}}{43}
\name{\fname{T.} \surname{Wachala}}{14}
\name{\fname{S.-i.} \surname{Wada}}{31}
\name{\fname{D.} \surname{Wakabayashi}}{70}
\name{\fname{H.T.} \surname{Wallace}}{54}
\name{\fname{J.G.} \surname{Walsh}}{39}
\name{\fname{D.} \surname{Wark}}{43,46}
\name{\fname{M.O.} \surname{Wascko}}{46,43}
\name{\fname{A.} \surname{Weber}}{18}
\name{\fname{R.} \surname{Wendell}}{32}
\name{\fname{M.J.} \surname{Wilking}}{52}
\name{\fname{C.} \surname{Wilkinson}}{34}
\name{\fname{J.R.} \surname{Wilson}}{30}
\name{\fname{C.} \surname{Winterstein}}{5}
\name{\fname{K.} \surname{Wood}}{34}
\name{\fname{C.} \surname{Wret}}{20}
\name{\fname{J.} \surname{Xia}}{56}
\name{\fname{Z.} \surname{Xie}}{52}
\name{\fname{K.} \surname{Yamamoto}}{45,53}
\name{\fname{T.} \surname{Yamamoto}}{45}
\name{\fname{T.} \surname{Yamazumi}}{59}
\name{\fname{C.} \surname{Yanagisawa}}{42,80}
\name{\fname{Y.} \surname{Yang}}{46}
\name{\fname{T.} \surname{Yano}}{60}
\name{\fname{N.} \surname{Yershov}}{25}
\name{\fname{U.} \surname{Yevarouskaya}}{42}
\name{\fname{M.} \surname{Yokoyama}}{59}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{Y.} \surname{Yoshimoto}}{59}
\name{\fname{N.} \surname{Yoshimura}}{32}
\name{\fname{R.} \surname{Zaki}}{74}
\name{\fname{A.} \surname{Zalewska}}{14}
\name{\fname{J.} \surname{Zalipska}}{41}
\name{\fname{G.} \surname{Zarnecki}}{14}
\name{\fname{J.} \surname{Zhang}}{65,3}
\name{\fname{X.Y.} \surname{Zhao}}{20}
\name{\fname{H.} \surname{Zheng}}{42}
\name{\fname{H.} \surname{Zhong}}{31}
\name{\fname{T.} \surname{Zhu}}{20}
\name{\fname{M.} \surname{Ziembicki}}{69}
\name{\fname{E.D.} \surname{Zimmerman}}{6}
\name{\fname{M.} \surname{Zito}}{57}
\name{\fname{S.} \surname{Zsoldos}}{30}
}

\address{
\affil{1}{University Autonoma Madrid, Department of Theoretical Physics, 28049 Madrid, Spain}
\affil{2}{Boston University, Department of Physics, Boston, Massachusetts, U.S.A.}
\affil{3}{University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada}
\affil{4}{University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.}
\affil{5}{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affil{6}{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}
\affil{7}{Duke University, Department of Physics, Durham, North Carolina, U.S.A.}
\affil{8}{ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland}
\affil{9}{VNU University of Science, Vietnam National University, Hanoi, Vietnam}
\affil{10}{CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland}
\affil{11}{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}
\affil{12}{University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom}
\affil{13}{Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium}
\affil{14}{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}
\affil{15}{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}
\affil{16}{University of Houston, Department of Physics, Houston, Texas, U.S.A.}
\affil{17}{Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}
\affil{18}{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Staudingerweg 7, 55128 Mainz, Germany}
\affil{19}{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}
\affil{20}{Imperial College London, Department of Physics, London, United Kingdom}
\affil{21}{INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}
\affil{22}{INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}
\affil{23}{INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}
\affil{24}{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy}
\affil{25}{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}
\affil{26}{International Centre of Physics, Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), 10 Dao Tan, Ba Dinh, Hanoi, Vietnam}
\affil{27}{ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}
\affil{28}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}
\affil{29}{Keio University, Department of Physics, Kanagawa, Japan}
\affil{30}{King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom}
\affil{31}{Kobe University, Kobe, Japan}
\affil{32}{Kyoto University, Department of Physics, Kyoto, Japan}
\affil{33}{Lancaster University, School of Physics and Astronomy, Lancaster, United Kingdom}
\affil{34}{Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.}
\affil{35}{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France}
\affil{36}{University of Liverpool, Department of Physics, Liverpool, United Kingdom}
\affil{37}{Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}
\affil{38}{Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia}
\affil{39}{Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.}
\affil{40}{Miyagi University of Education, Department of Physics, Sendai, Japan}
\affil{41}{National Centre for Nuclear Research, Warsaw, Poland}
\affil{42}{State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}
\affil{43}{STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}
\affil{44}{Okayama University, Department of Physics, Okayama, Japan}
\affil{45}{Osaka Metropolitan University, Department of Physics, Osaka, Japan}
\affil{46}{Oxford University, Department of Physics, Oxford, United Kingdom}
\affil{47}{University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.}
\affil{48}{University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.}
\affil{49}{University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}
\affil{50}{Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom}
\affil{51}{RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany}
\affil{52}{School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota, U.S.A.}
\affil{53}{Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain}
\affil{54}{University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom}
\affil{55}{University of Silesia, Institute of Physics, Katowice, Poland}
\affil{56}{SLAC National Accelerator Laboratory, Stanford University, Menlo Park, California, U.S.A.}
\affil{57}{Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}
\affil{58}{South Dakota School of Mines and Technology, 501 East Saint Joseph Street, Rapid City, SD 57701, United States}
\affil{59}{University of Tokyo, Department of Physics, Tokyo, Japan}
\affil{60}{University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}
\affil{61}{University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}
\affil{62}{Institute of Science Tokyo, Department of Physics, Tokyo}
\affil{63}{Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}
\affil{64}{Tokyo University of Science, Faculty of Science and Technology, Department of Physics, Noda, Chiba, Japan}
\affil{65}{TRIUMF, Vancouver, British Columbia, Canada}
\affil{66}{University of Toyama, Faculty of Science, Toyama, Japan}
\affil{67}{University of Tsukuba, Faculty of Pure and Applied Sciences, Tsukuba, Ibaraki, Japan}
\affil{68}{University of Warsaw, Faculty of Physics, Warsaw, Poland}
\affil{69}{Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland}
\affil{70}{Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan}
\affil{71}{University of Warwick, Department of Physics, Coventry, United Kingdom}
\affil{72}{Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}
\affil{73}{Yokohama National University, Department of Physics, Yokohama, Japan}
\affil{74}{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}
\affil{75}{Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain}
\affil{76}{J-PARC, Tokai, Japan}
\affil{77}{Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}
\affil{78}{IPSA-DRII, France}
\affil{79}{the Graduate University of Science and Technology, Vietnam Academy of Science and Technology}
\affil{80}{BMCC/CUNY, Science Department, New York, New York, U.S.A.}
}


==> authorlist_PTEP_442_with_affiliations.tex <==
% T2K author list in ptephy_v1 PTEP format
% 442 authors / 74 affiliations
% Affiliations are printed explicitly because ptephy_v1.cls does not define \affil.
\author{
\name{\fname{K.} \surname{Abe}}{60}
\name{\fname{S.} \surname{Abe}}{60}
\name{\fname{H.} \surname{Adhikary}}{68}
\name{\fname{R.} \surname{Akutsu}}{15}
\name{\fname{H.} \surname{Alarakia-Charles}}{33}
\name{\fname{Y.I.} \surname{Alj Hakim}}{54}
\name{\fname{S.} \surname{Alonso Monsalve}}{8}
\name{\fname{L.} \surname{Anthony}}{20}
\name{\fname{S.} \surname{Aoki}}{31}
\name{\fname{K.A.} \surname{Apte}}{20}
\name{\fname{T.} \surname{Arai}}{59}
\name{\fname{T.} \surname{Arihara}}{63}
\name{\fname{S.} \surname{Arimoto}}{32}
\name{\fname{Y.} \surname{Asami}}{63}
\name{\fname{Y.} \surname{Asaoka}}{60}
\name{\fname{Y.} \surname{Ashida}}{70}
\name{\fname{E.T.} \surname{Atkin}}{20}
\name{\fname{N.} \surname{Babu}}{37}
\name{\fname{V.} \surname{Baranov}}{38}
\name{\fname{G.J.} \surname{Barker}}{71}
\name{\fname{G.} \surname{Barr}}{46}
\name{\fname{D.} \surname{Barrow}}{46}
\name{\fname{P.} \surname{Bates}}{36}
\name{\fname{L.} \surname{Bathe-Peters}}{46}
\name{\fname{M.} \surname{Batkiewicz-Kwasniak}}{14}
\name{\fname{N.} \surname{Baudis}}{46}
\name{\fname{A.} \surname{Beliakova}}{25}
\name{\fname{V.} \surname{Berardi}}{21}
\name{\fname{L.} \surname{Berns}}{70}
\name{\fname{S.} \surname{Bhattacharjee}}{37}
\name{\fname{A.} \surname{Blanchet}}{57}
\name{\fname{A.} \surname{Blondel}}{57,11}
\name{\fname{L.} \surname{B{\o}e}}{16}
\name{\fname{P.M.M.} \surname{Boistier}}{5}
\name{\fname{S.} \surname{Bolognesi}}{5}
\name{\fname{B.} \surname{Bombin}}{25}
\name{\fname{S.} \surname{Bordoni}}{11}
\name{\fname{S.B.} \surname{Boyd}}{71}
\name{\fname{C.} \surname{Bronner}}{73}
\name{\fname{A.} \surname{Bubak}}{55}
\name{\fname{M.} \surname{Buizza Avanzini}}{35}
\name{\fname{J.A.} \surname{Caballero}}{53}
\name{\fname{N.F.} \surname{Calabria}}{21}
\name{\fname{S.} \surname{Cao}}{19}
\name{\fname{S.} \surname{Cap}}{11}
\name{\fname{D.} \surname{Carabadjac}}{35,}\thanks{also at Universit\'e Paris-Saclay}
\name{\fname{S.L.} \surname{Cartwright}}{54}
\name{\fname{M.P.} \surname{Casado}}{17,}\thanks{also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain}
\name{\fname{M.G.} \surname{Catanesi}}{21}
\name{\fname{J.} \surname{Chakrani}}{34}
\name{\fname{A.} \surname{Chalumeau}}{57}
\name{\fname{D.} \surname{Cherdack}}{16}
\name{\fname{A.} \surname{Chvirova}}{25}
\name{\fname{J.} \surname{Coleman}}{36}
\name{\fname{G.} \surname{Collazuol}}{23}
\name{\fname{F.} \surname{Cormier}}{65}
\name{\fname{A.A.L.} \surname{Craplet}}{20}
\name{\fname{A.} \surname{Cudd}}{6}
\name{\fname{D.} \surname{D'Ago}}{23}
\name{\fname{C.} \surname{Dalmazzone}}{57}
\name{\fname{T.} \surname{Daret}}{5}
\name{\fname{P.} \surname{Dasgupta}}{17}
\name{\fname{C.} \surname{Davis}}{47}
\name{\fname{Yu.I.} \surname{Davydov}}{38}
\name{\fname{P.} \surname{de Perio}}{28}
\name{\fname{G.} \surname{De Rosa}}{22}
\name{\fname{T.} \surname{Dealtry}}{33}
\name{\fname{C.} \surname{Densham}}{43}
\name{\fname{A.} \surname{Dergacheva}}{25}
\name{\fname{R.} \surname{Dharmapal Banerjee}}{72}
\name{\fname{F.} \surname{Di Lodovico}}{30}
\name{\fname{G.} \surname{Diaz Lopez}}{57}
\name{\fname{S.} \surname{Dolan}}{10}
\name{\fname{D.} \surname{Douqa}}{11}
\name{\fname{T.A.} \surname{Doyle}}{46}
\name{\fname{O.} \surname{Drapier}}{35}
\name{\fname{K.E.} \surname{Duffy}}{46}
\name{\fname{J.} \surname{Dumarchez}}{57}
\name{\fname{P.} \surname{Dunne}}{20}
\name{\fname{K.} \surname{Dygnarowicz}}{69}
\name{\fname{A.} \surname{Eguchi}}{59}
\name{\fname{M.} \surname{El Baz}}{11}
\name{\fname{J.} \surname{Elias}}{49}
\name{\fname{S.} \surname{Emery-Schrenk}}{5}
\name{\fname{G.} \surname{Erofeev}}{25}
\name{\fname{A.} \surname{Ershova}}{35}
\name{\fname{G.} \surname{Eurin}}{5}
\name{\fname{M.} \surname{Fani}}{52}
\name{\fname{D.} \surname{Fedorova}}{25}
\name{\fname{S.} \surname{Fedotov}}{25}
\name{\fname{M.} \surname{Feltre}}{23}
\name{\fname{C.} \surname{Fengler}}{46}
\name{\fname{L.} \surname{Feng}}{32}
\name{\fname{D.} \surname{Ferlewicz}}{57}
\name{\fname{A.J.} \surname{Finch}}{33}
\name{\fname{M.D.} \surname{Fitton}}{43}
\name{\fname{C.} \surname{Forza}}{23}
\name{\fname{M.} \surname{Friend}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{Y.} \surname{Fujii}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{Y.} \surname{Fukuda}}{40}
\name{\fname{N.} \surname{Funayama}}{45}
\name{\fname{Y.} \surname{Furui}}{63}
\name{\fname{A.N.} \surname{Gaci\~no Olmedo}}{57}
\name{\fname{J.} \surname{Garc\'ia-Marcos}}{13}
\name{\fname{A.C.} \surname{Germer}}{47}
\name{\fname{L.} \surname{Giannessi}}{11}
\name{\fname{C.} \surname{Giganti}}{57}
\name{\fname{M.} \surname{Girgus}}{68}
\name{\fname{V.} \surname{Glagolev}}{38}
\name{\fname{P.} \surname{Golak}}{68}
\name{\fname{M.} \surname{Gonin}}{27}
\name{\fname{R.} \surname{Gonzalez Jimenez}}{53}
\name{\fname{J.} \surname{Gonz\'alez Rosa}}{53}
\name{\fname{E.A.G.} \surname{Goodman}}{12}
\name{\fname{K.} \surname{Gorshanov}}{25}
\name{\fname{P.} \surname{Govindaraj}}{68}
\name{\fname{M.} \surname{Grassi}}{23}
\name{\fname{M.} \surname{Guigue}}{57}
\name{\fname{F.Y.} \surname{Guo}}{42}
\name{\fname{D.R.} \surname{Hadley}}{71}
\name{\fname{S.} \surname{Han}}{32,61}
\name{\fname{D.A.} \surname{Harris}}{74}
\name{\fname{R.J.} \surname{Harris}}{33,43}
\name{\fname{M.} \surname{Hartz}}{65,28}
\name{\fname{K.} \surname{Hasegawa}}{32}
\name{\fname{T.} \surname{Hasegawa}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{C.M.} \surname{Hasnip}}{10}
\name{\fname{S.} \surname{Hassani}}{5}
\name{\fname{N.C.} \surname{Hastings}}{15}
\name{\fname{K.} \surname{Hayashi}}{32}
\name{\fname{Y.} \surname{Hayato}}{60,28}
\name{\fname{I.} \surname{Heitkamp}}{70}
\name{\fname{D.} \surname{Henaff}}{5}
\name{\fname{Y.} \surname{Hino}}{15}
\name{\fname{K.} \surname{Hiraide}}{60,28}
\name{\fname{J.} \surname{Holeczek}}{55}
\name{\fname{A.} \surname{Holin}}{43}
\name{\fname{T.} \surname{Holvey}}{46}
\name{\fname{N.T.} \surname{Hong Van}}{26}
\name{\fname{T.} \surname{Honjo}}{45}
\name{\fname{M.C.F.} \surname{Hooft}}{13}
\name{\fname{K.} \surname{Hosokawa}}{60}
\name{\fname{R.} \surname{Huang}}{34}
\name{\fname{J.} \surname{Hu}}{32}
\name{\fname{A.K.} \surname{Ichikawa}}{70}
\name{\fname{K.} \surname{Ieki}}{60}
\name{\fname{M.} \surname{Ikeda}}{60}
\name{\fname{K.} \surname{Indo}}{32}
\name{\fname{T.H.} \surname{Ishida}}{70}
\name{\fname{T.} \surname{Ishida}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Ishitsuka}}{64}
\name{\fname{H.} \surname{Ito}}{31}
\name{\fname{S.} \surname{Ito}}{73}
\name{\fname{A.} \surname{Izmaylov}}{25}
\name{\fname{N.} \surname{Jachowicz}}{13}
\name{\fname{B.} \surname{Jargowsky}}{2}
\name{\fname{S.J.} \surname{Jenkins}}{36}
\name{\fname{C.} \surname{Jes\'us-Valls}}{10}
\name{\fname{M.} \surname{Jia}}{42}
\name{\fname{J.J.} \surname{Jiang}}{42}
\name{\fname{J.Y.} \surname{Ji}}{42}
\name{\fname{T.P.} \surname{Jones}}{33}
\name{\fname{P.} \surname{Jonsson}}{20}
\name{\fname{S.} \surname{Joshi}}{42}
\name{\fname{C.K.} \surname{Jung}}{42,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Kabirnezhad}}{46}
\name{\fname{A.C.} \surname{Kaboth}}{50}
\name{\fname{K.} \surname{Kadota}}{31}
\name{\fname{H.} \surname{Kakuno}}{63}
\name{\fname{A.} \surname{Kamata}}{63}
\name{\fname{J.} \surname{Kameda}}{60}
\name{\fname{S.} \surname{Karpova}}{11}
\name{\fname{V.S.} \surname{Kasturi}}{11}
\name{\fname{Y.} \surname{Kataoka}}{60}
\name{\fname{T.} \surname{Katori}}{30}
\name{\fname{A.} \surname{Kawabata}}{29}
\name{\fname{R.} \surname{Kawabe}}{45}
\name{\fname{Y.} \surname{Kawamura}}{45}
\name{\fname{M.} \surname{Kawaue}}{32}
\name{\fname{E.} \surname{Kearns}}{2,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Khabibullin}}{25}
\name{\fname{N.V.} \surname{Khomutov}}{38}
\name{\fname{A.} \surname{Khotjantsev}}{25}
\name{\fname{T.} \surname{Kikawa}}{32}
\name{\fname{S.} \surname{King}}{30}
\name{\fname{V.} \surname{Kiseeva}}{38}
\name{\fname{J.} \surname{Kisiel}}{55}
\name{\fname{A.} \surname{Klustov\'a}}{20}
\name{\fname{L.} \surname{Kneale}}{54}
\name{\fname{H.} \surname{Kobayashi}}{59}
\name{\fname{S.R.} \surname{Kobayashi}}{70}
\name{\fname{T.} \surname{Kobayashi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{L.} \surname{Koch}}{18}
\name{\fname{S.} \surname{Kodama}}{59}
\name{\fname{M.} \surname{Kolupanova}}{25,}\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}
\name{\fname{A.} \surname{Konaka}}{65}
\name{\fname{L.L.} \surname{Kormos}}{33}
\name{\fname{Y.} \surname{Koshio}}{44,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{K.} \surname{Kowalik}}{41}
\name{\fname{R.} \surname{Kralik}}{30}
\name{\fname{Y.} \surname{Kudenko}}{25,}\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}
\name{\fname{Y.} \surname{Kudo}}{73}
\name{\fname{A.} \surname{Kumar Jha}}{13}
\name{\fname{R.} \surname{Kurjata}}{69}
\name{\fname{V.} \surname{Kurochka}}{25}
\name{\fname{T.} \surname{Kutter}}{37}
\name{\fname{L.} \surname{Labarga}}{1}
\name{\fname{M.} \surname{Lachat}}{49}
\name{\fname{K.} \surname{Lachner}}{8}
\name{\fname{J.} \surname{Lagoda}}{41}
\name{\fname{S.M.} \surname{Lakshmi}}{55}
\name{\fname{M.} \surname{Lamers James}}{71}
\name{\fname{A.} \surname{Langella}}{22}
\name{\fname{D.H.} \surname{Langridge}}{50}
\name{\fname{J.-F.} \surname{Laporte}}{5}
\name{\fname{D.} \surname{Last}}{49}
\name{\fname{N.} \surname{Latham}}{30}
\name{\fname{M.} \surname{Laveder}}{23}
\name{\fname{L.} \surname{Lavitola}}{22}
\name{\fname{M.} \surname{Lawe}}{33}
\name{\fname{A.} \surname{Leclerc}}{5}
\name{\fname{N.} \surname{Lemaire}}{35}
\name{\fname{D.} \surname{Leon Silverio}}{58}
\name{\fname{T.} \surname{Leplumey}}{35}
\name{\fname{S.} \surname{Levorato}}{23}
\name{\fname{S.V.} \surname{Lewis}}{30}
\name{\fname{B.} \surname{Li}}{8}
\name{\fname{C.} \surname{Lin}}{20}
\name{\fname{R.P.} \surname{Litchfield}}{12}
\name{\fname{S.L.} \surname{Liu}}{42}
\name{\fname{W.} \surname{Li}}{46}
\name{\fname{A.} \surname{Longhin}}{23}
\name{\fname{A.} \surname{Lopez Moreno}}{30}
\name{\fname{L.} \surname{Ludovici}}{24}
\name{\fname{X.} \surname{Lu}}{71}
\name{\fname{T.} \surname{Lux}}{17}
\name{\fname{L.N.} \surname{Machado}}{12}
\name{\fname{L.} \surname{Magaletti}}{21}
\name{\fname{K.} \surname{Mahn}}{39}
\name{\fname{K.K.} \surname{Mahtani}}{42}
\name{\fname{S.} \surname{Manly}}{49}
\name{\fname{A.D.} \surname{Marino}}{6}
\name{\fname{D.G.R.} \surname{Martin}}{20}
\name{\fname{D.A.} \surname{Martinez Caicedo}}{58}
\name{\fname{L.} \surname{Martinez}}{17}
\name{\fname{M.} \surname{Martini}}{57,}\thanks{also at IPSA-DRII, France}
\name{\fname{N.} \surname{Mashin}}{25}
\name{\fname{T.} \surname{Matsubara}}{15}
\name{\fname{R.} \surname{Matsumoto}}{62}
\name{\fname{V.} \surname{Matveev}}{25}
\name{\fname{C.} \surname{Mauger}}{47}
\name{\fname{K.} \surname{Mavrokoridis}}{36}
\name{\fname{N.} \surname{McCauley}}{36}
\name{\fname{K.S.} \surname{McFarland}}{49}
\name{\fname{C.} \surname{McGrew}}{42}
\name{\fname{J.} \surname{McKean}}{32}
\name{\fname{A.} \surname{Mefodiev}}{25}
\name{\fname{G.D.} \surname{Megias}}{53}
\name{\fname{L.} \surname{Mellet}}{39}
\name{\fname{C.} \surname{Metelko}}{36}
\name{\fname{M.} \surname{Mezzetto}}{23}
\name{\fname{S.} \surname{Miki}}{60}
\name{\fname{V.} \surname{Mikola}}{12}
\name{\fname{E.W.} \surname{Miller}}{20}
\name{\fname{A.} \surname{Minamino}}{73}
\name{\fname{O.} \surname{Mineev}}{25}
\name{\fname{S.} \surname{Mine}}{60,4}
\name{\fname{J.} \surname{Mirabito}}{2}
\name{\fname{M.} \surname{Miura}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{73}
\name{\fname{P.} \surname{Morrison}}{12}
\name{\fname{Th.A.} \surname{Mueller}}{35}
\name{\fname{D.} \surname{Munford}}{16}
\name{\fname{A.} \surname{Mu\~noz}}{18}
\name{\fname{L.} \surname{Munteanu}}{10}
\name{\fname{Y.} \surname{Nagai}}{15}
\name{\fname{T.} \surname{Nakadaira}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{K.} \surname{Nakagiri}}{60}
\name{\fname{M.} \surname{Nakahata}}{60,28}
\name{\fname{Y.} \surname{Nakajima}}{59}
\name{\fname{K.D.} \surname{Nakamura}}{70}
\name{\fname{A.} \surname{Nakano}}{70}
\name{\fname{Y.} \surname{Nakano}}{66}
\name{\fname{S.} \surname{Nakayama}}{60,28}
\name{\fname{T.} \surname{Nakaya}}{32,28}
\name{\fname{K.} \surname{Nakayoshi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{C.E.R.} \surname{Naseby}}{20}
\name{\fname{D.T.} \surname{Nguyen}}{9}
\name{\fname{V.Q.} \surname{Nguyen}}{35}
\name{\fname{K.} \surname{Niewczas}}{35,13}
\name{\fname{S.} \surname{Nishimori}}{59}
\name{\fname{Y.} \surname{Nishimura}}{29}
\name{\fname{Y.} \surname{Noguchi}}{60}
\name{\fname{T.} \surname{Nosek}}{41}
\name{\fname{F.} \surname{Nova}}{43}
\name{\fname{J.C.} \surname{Nugent}}{20}
\name{\fname{H.M.} \surname{O'Keeffe}}{33}
\name{\fname{L.} \surname{O'Sullivan}}{18}
\name{\fname{R.} \surname{Okazaki}}{29}
\name{\fname{W.} \surname{Okinaga}}{59}
\name{\fname{K.} \surname{Okumura}}{61,28}
\name{\fname{T.} \surname{Okusawa}}{45}
\name{\fname{N.} \surname{Onda}}{32}
\name{\fname{N.} \surname{Ospina}}{21}
\name{\fname{L.} \surname{Osu}}{35}
\name{\fname{N.} \surname{Otani}}{32}
\name{\fname{Y.} \surname{Oyama}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{V.} \surname{Paolone}}{48}
\name{\fname{J.} \surname{Pasternak}}{20}
\name{\fname{D.} \surname{Payne}}{36}
\name{\fname{T.P.D.} \surname{Peacock}}{54}
\name{\fname{M.} \surname{Pfaff}}{20}
\name{\fname{L.} \surname{Pickering}}{43}
\name{\fname{J.-B.} \surname{Plan\c{c}on}}{35}
\name{\fname{P.} \surname{Podlaski}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{B.} \surname{Popov}}{57,}\thanks{also at JINR, Dubna, Russia}
\name{\fname{A.J.} \surname{Portocarrero Yrey}}{15}
\name{\fname{M.} \surname{Posiadala-Zezula}}{68}
\name{\fname{Y.S.} \surname{Prabhu}}{68}
\name{\fname{H.} \surname{Prasad}}{72}
\name{\fname{F.} \surname{Pupilli}}{23}
\name{\fname{B.} \surname{Quilain}}{27,35}
\name{\fname{P.T.} \surname{Quyen}}{19,}\thanks{also at the Graduate University of Science and Technology, Vietnam Academy of Science and Technology}
\name{\fname{E.} \surname{Radicioni}}{21}
\name{\fname{B.} \surname{Radics}}{74}
\name{\fname{M.A.} \surname{Ramirez Delgado}}{47}
\name{\fname{R.} \surname{Ramsden}}{30}
\name{\fname{P.N.} \surname{Ratoff}}{33}
\name{\fname{M.} \surname{Reh}}{6}
\name{\fname{G.} \surname{Reina}}{18}
\name{\fname{L.} \surname{Restrepo}}{57}
\name{\fname{C.} \surname{Riccio}}{42}
\name{\fname{D.W.} \surname{Riley}}{12}
\name{\fname{E.} \surname{Rondio}}{41}
\name{\fname{D.} \surname{Ross}}{39}
\name{\fname{S.} \surname{Roth}}{51}
\name{\fname{N.} \surname{Roy}}{74}
\name{\fname{A.} \surname{Rubbia}}{8}
\name{\fname{L.} \surname{Russo}}{57}
\name{\fname{A.} \surname{Rychter}}{69}
\name{\fname{W.} \surname{Saenz}}{57}
\name{\fname{K.} \surname{Sakashita}}{67,15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{S.} \surname{Samani}}{11}
\name{\fname{F.} \surname{S\'anchez}}{11}
\name{\fname{E.M.} \surname{Sandford}}{36}
\name{\fname{Y.} \surname{Sato}}{64}
\name{\fname{T.} \surname{Schefke}}{37}
\name{\fname{K.} \surname{Scholberg}}{7,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Scott}}{20}
\name{\fname{Y.} \surname{Seiya}}{45,}\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}
\name{\fname{T.} \surname{Sekiguchi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{H.} \surname{Sekiya}}{60,28,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Sekiyama}}{59}
\name{\fname{T.} \surname{Sekiya}}{63}
\name{\fname{D.} \surname{Seppala}}{39}
\name{\fname{D.} \surname{Sgalaberna}}{8}
\name{\fname{A.} \surname{Shaikhiev}}{25}
\name{\fname{M.} \surname{Shiozawa}}{60,28}
\name{\fname{Y.} \surname{Shiraishi}}{44}
\name{\fname{N.} \surname{Shvarev}}{25}
\name{\fname{A.} \surname{Shvartsman}}{25}
\name{\fname{V.} \surname{Siccardi}}{30}
\name{\fname{N.} \surname{Skrobova}}{25}
\name{\fname{K.} \surname{Skwarczynski}}{50}
\name{\fname{D.} \surname{Smyczek}}{51}
\name{\fname{M.} \surname{Smy}}{4}
\name{\fname{J.T.} \surname{Sobczyk}}{72}
\name{\fname{H.} \surname{Sobel}}{4,28}
\name{\fname{F.J.P.} \surname{Soler}}{12}
\name{\fname{A.J.} \surname{Speers}}{33}
\name{\fname{R.} \surname{Spina}}{21}
\name{\fname{A.} \surname{Srivastava}}{18}
\name{\fname{P.} \surname{Stowell}}{54}
\name{\fname{Y.} \surname{Stroke}}{25}
\name{\fname{I.A.} \surname{Suslov}}{38}
\name{\fname{A.} \surname{Suzuki}}{31}
\name{\fname{M.} \surname{Suzuki}}{73}
\name{\fname{S.Y.} \surname{Suzuki}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Tada}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{S.} \surname{Tairafune}}{70}
\name{\fname{A.} \surname{Takeda}}{60}
\name{\fname{Y.} \surname{Takeuchi}}{31,28}
\name{\fname{K.} \surname{Takeya}}{44}
\name{\fname{H.K.} \surname{Tanaka}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{H.} \surname{Tanigawa}}{29}
\name{\fname{A.} \surname{Teklu}}{42}
\name{\fname{V.V.} \surname{Tereshchenko}}{38}
\name{\fname{N.} \surname{Thamm}}{51}
\name{\fname{C.} \surname{Touramanis}}{36}
\name{\fname{N.} \surname{Tran}}{19}
\name{\fname{T.} \surname{Tsukamoto}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Tzanov}}{37}
\name{\fname{Y.} \surname{Uchida}}{20}
\name{\fname{M.} \surname{Vagins}}{28,4}
\name{\fname{M.} \surname{Varghese}}{17}
\name{\fname{I.} \surname{Vasilyev}}{38}
\name{\fname{G.} \surname{Vasseur}}{5}
\name{\fname{E.} \surname{Villa}}{8}
\name{\fname{U.} \surname{Virginet}}{57}
\name{\fname{T.} \surname{Vladisavljevic}}{43}
\name{\fname{T.} \surname{Wachala}}{14}
\name{\fname{S.-i.} \surname{Wada}}{31}
\name{\fname{D.} \surname{Wakabayashi}}{70}
\name{\fname{H.T.} \surname{Wallace}}{54}
\name{\fname{J.G.} \surname{Walsh}}{39}
\name{\fname{D.} \surname{Wark}}{43,46}
\name{\fname{M.O.} \surname{Wascko}}{46,43}
\name{\fname{A.} \surname{Weber}}{18}
\name{\fname{R.} \surname{Wendell}}{32}
\name{\fname{M.J.} \surname{Wilking}}{52}
\name{\fname{C.} \surname{Wilkinson}}{34}
\name{\fname{J.R.} \surname{Wilson}}{30}
\name{\fname{C.} \surname{Winterstein}}{5}
\name{\fname{K.} \surname{Wood}}{34}
\name{\fname{C.} \surname{Wret}}{20}
\name{\fname{J.} \surname{Xia}}{56}
\name{\fname{Z.} \surname{Xie}}{52}
\name{\fname{K.} \surname{Yamamoto}}{45,}\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}
\name{\fname{T.} \surname{Yamamoto}}{45}
\name{\fname{T.} \surname{Yamazumi}}{59}
\name{\fname{C.} \surname{Yanagisawa}}{42,}\thanks{also at BMCC/CUNY, Science Department, New York, New York, U.S.A.}
\name{\fname{Y.} \surname{Yang}}{46}
\name{\fname{T.} \surname{Yano}}{60}
\name{\fname{N.} \surname{Yershov}}{25}
\name{\fname{U.} \surname{Yevarouskaya}}{42}
\name{\fname{M.} \surname{Yokoyama}}{59,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{Y.} \surname{Yoshimoto}}{59}
\name{\fname{N.} \surname{Yoshimura}}{32}
\name{\fname{R.} \surname{Zaki}}{74}
\name{\fname{A.} \surname{Zalewska}}{14}
\name{\fname{J.} \surname{Zalipska}}{41}
\name{\fname{G.} \surname{Zarnecki}}{14}
\name{\fname{J.} \surname{Zhang}}{65,3}
\name{\fname{X.Y.} \surname{Zhao}}{20}
\name{\fname{H.} \surname{Zheng}}{42}
\name{\fname{H.} \surname{Zhong}}{31}
\name{\fname{T.} \surname{Zhu}}{20}
\name{\fname{M.} \surname{Ziembicki}}{69}
\name{\fname{E.D.} \surname{Zimmerman}}{6}
\name{\fname{M.} \surname{Zito}}{57}
\name{\fname{S.} \surname{Zsoldos}}{30}
}

\address{
$^{1}$ University Autonoma Madrid, Department of Theoretical Physics, 28049 Madrid, Spain\par
$^{2}$ Boston University, Department of Physics, Boston, Massachusetts, U.S.A.\par
$^{3}$ University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada\par
$^{4}$ University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.\par
$^{5}$ IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France\par
$^{6}$ University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.\par
$^{7}$ Duke University, Department of Physics, Durham, North Carolina, U.S.A.\par
$^{8}$ ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland\par
$^{9}$ VNU University of Science, Vietnam National University, Hanoi, Vietnam\par
$^{10}$ CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland\par
$^{11}$ University of Geneva, Section de Physique, DPNC, Geneva, Switzerland\par
$^{12}$ University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom\par
$^{13}$ Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium\par
$^{14}$ H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland\par
$^{15}$ High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan\par
$^{16}$ University of Houston, Department of Physics, Houston, Texas, U.S.A.\par
$^{17}$ Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain\par
$^{18}$ Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Staudingerweg 7, 55128 Mainz, Germany\par
$^{19}$ Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam\par
$^{20}$ Imperial College London, Department of Physics, London, United Kingdom\par
$^{21}$ INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy\par
$^{22}$ INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy\par
$^{23}$ INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy\par
$^{24}$ INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy\par
$^{25}$ Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia\par
$^{26}$ International Centre of Physics, Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), 10 Dao Tan, Ba Dinh, Hanoi, Vietnam\par
$^{27}$ ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan\par
$^{28}$ Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan\par
$^{29}$ Keio University, Department of Physics, Kanagawa, Japan\par
$^{30}$ King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom\par
$^{31}$ Kobe University, Kobe, Japan\par
$^{32}$ Kyoto University, Department of Physics, Kyoto, Japan\par
$^{33}$ Lancaster University, School of Physics and Astronomy, Lancaster, United Kingdom\par
$^{34}$ Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.\par
$^{35}$ Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France\par
$^{36}$ University of Liverpool, Department of Physics, Liverpool, United Kingdom\par
$^{37}$ Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.\par
$^{38}$ Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia\par
$^{39}$ Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.\par
$^{40}$ Miyagi University of Education, Department of Physics, Sendai, Japan\par
$^{41}$ National Centre for Nuclear Research, Warsaw, Poland\par
$^{42}$ State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.\par
$^{43}$ STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom\par
$^{44}$ Okayama University, Department of Physics, Okayama, Japan\par
$^{45}$ Osaka Metropolitan University, Department of Physics, Osaka, Japan\par
$^{46}$ Oxford University, Department of Physics, Oxford, United Kingdom\par
$^{47}$ University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.\par
$^{48}$ University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.\par
$^{49}$ University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.\par
$^{50}$ Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom\par
$^{51}$ RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany\par
$^{52}$ School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota, U.S.A.\par
$^{53}$ Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain\par
$^{54}$ University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom\par
$^{55}$ University of Silesia, Institute of Physics, Katowice, Poland\par
$^{56}$ SLAC National Accelerator Laboratory, Stanford University, Menlo Park, California, U.S.A.\par
$^{57}$ Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France\par
$^{58}$ South Dakota School of Mines and Technology, 501 East Saint Joseph Street, Rapid City, SD 57701, United States\par
$^{59}$ University of Tokyo, Department of Physics, Tokyo, Japan\par
$^{60}$ University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan\par
$^{61}$ University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan\par
$^{62}$ Institute of Science Tokyo, Department of Physics, Tokyo\par
$^{63}$ Tokyo Metropolitan University, Department of Physics, Tokyo, Japan\par
$^{64}$ Tokyo University of Science, Faculty of Science and Technology, Department of Physics, Noda, Chiba, Japan\par
$^{65}$ TRIUMF, Vancouver, British Columbia, Canada\par
$^{66}$ University of Toyama, Faculty of Science, Toyama, Japan\par
$^{67}$ University of Tsukuba, Faculty of Pure and Applied Sciences, Tsukuba, Ibaraki, Japan\par
$^{68}$ University of Warsaw, Faculty of Physics, Warsaw, Poland\par
$^{69}$ Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland\par
$^{70}$ Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan\par
$^{71}$ University of Warwick, Department of Physics, Coventry, United Kingdom\par
$^{72}$ Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland\par
$^{73}$ Yokohama National University, Department of Physics, Yokohama, Japan\par
$^{74}$ York University, Department of Physics and Astronomy, Toronto, Ontario, Canada\par
}


==> authorlist_PTEP_fixed.tex <==
% T2K author list converted to PTEP format
% Source: authorlist_20260923.tex
% Number of authors = 442

\author{
\name{\fname{K.} \surname{Abe}}{60}
\name{\fname{S.} \surname{Abe}}{60}
\name{\fname{H.} \surname{Adhikary}}{68}
\name{\fname{R.} \surname{Akutsu}}{15}
\name{\fname{H.} \surname{Alarakia-Charles}}{33}
\name{\fname{Y.I.} \surname{Alj Hakim}}{54}
\name{\fname{S.} \surname{Alonso Monsalve}}{8}
\name{\fname{L.} \surname{Anthony}}{20}
\name{\fname{S.} \surname{Aoki}}{31}
\name{\fname{K.A.} \surname{Apte}}{20}
\name{\fname{T.} \surname{Arai}}{59}
\name{\fname{T.} \surname{Arihara}}{63}
\name{\fname{S.} \surname{Arimoto}}{32}
\name{\fname{Y.} \surname{Asami}}{63}
\name{\fname{Y.} \surname{Asaoka}}{60}
\name{\fname{Y.} \surname{Ashida}}{70}
\name{\fname{E.T.} \surname{Atkin}}{20}
\name{\fname{N.} \surname{Babu}}{37}
\name{\fname{V.} \surname{Baranov}}{38}
\name{\fname{G.J.} \surname{Barker}}{71}
\name{\fname{G.} \surname{Barr}}{46}
\name{\fname{D.} \surname{Barrow}}{46}
\name{\fname{P.} \surname{Bates}}{36}
\name{\fname{L.} \surname{Bathe-Peters}}{46}
\name{\fname{M.} \surname{Batkiewicz-Kwasniak}}{14}
\name{\fname{N.} \surname{Baudis}}{46}
\name{\fname{A.} \surname{Beliakova}}{25}
\name{\fname{V.} \surname{Berardi}}{21}
\name{\fname{L.} \surname{Berns}}{70}
\name{\fname{S.} \surname{Bhattacharjee}}{37}
\name{\fname{A.} \surname{Blanchet}}{57}
\name{\fname{A.} \surname{Blondel}}{57,11}
\name{\fname{L.} \surname{B{\o}e}}{16}
\name{\fname{P.M.M.} \surname{Boistier}}{5}
\name{\fname{S.} \surname{Bolognesi}}{5}
\name{\fname{B.} \surname{Bombin}}{25}
\name{\fname{S.} \surname{Bordoni}}{11}
\name{\fname{S.B.} \surname{Boyd}}{71}
\name{\fname{C.} \surname{Bronner}}{73}
\name{\fname{A.} \surname{Bubak}}{55}
\name{\fname{M.} \surname{Buizza Avanzini}}{35}
\name{\fname{J.A.} \surname{Caballero}}{53}
\name{\fname{N.F.} \surname{Calabria}}{21}
\name{\fname{S.} \surname{Cao}}{19}
\name{\fname{S.} \surname{Cap}}{11}
\name{\fname{D.} \surname{Carabadjac}}{35,}\thanks{also at Universit\'e Paris-Saclay}
\name{\fname{S.L.} \surname{Cartwright}}{54}
\name{\fname{M.P.} \surname{Casado}}{17,}\thanks{also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain}
\name{\fname{M.G.} \surname{Catanesi}}{21}
\name{\fname{J.} \surname{Chakrani}}{34}
\name{\fname{A.} \surname{Chalumeau}}{57}
\name{\fname{D.} \surname{Cherdack}}{16}
\name{\fname{A.} \surname{Chvirova}}{25}
\name{\fname{J.} \surname{Coleman}}{36}
\name{\fname{G.} \surname{Collazuol}}{23}
\name{\fname{F.} \surname{Cormier}}{65}
\name{\fname{A.A.L.} \surname{Craplet}}{20}
\name{\fname{A.} \surname{Cudd}}{6}
\name{\fname{D.} \surname{D'Ago}}{23}
\name{\fname{C.} \surname{Dalmazzone}}{57}
\name{\fname{T.} \surname{Daret}}{5}
\name{\fname{P.} \surname{Dasgupta}}{17}
\name{\fname{C.} \surname{Davis}}{47}
\name{\fname{Yu.I.} \surname{Davydov}}{38}
\name{\fname{P.} \surname{de Perio}}{28}
\name{\fname{G.} \surname{De Rosa}}{22}
\name{\fname{T.} \surname{Dealtry}}{33}
\name{\fname{C.} \surname{Densham}}{43}
\name{\fname{A.} \surname{Dergacheva}}{25}
\name{\fname{R.} \surname{Dharmapal Banerjee}}{72}
\name{\fname{F.} \surname{Di Lodovico}}{30}
\name{\fname{G.} \surname{Diaz Lopez}}{57}
\name{\fname{S.} \surname{Dolan}}{10}
\name{\fname{D.} \surname{Douqa}}{11}
\name{\fname{T.A.} \surname{Doyle}}{46}
\name{\fname{O.} \surname{Drapier}}{35}
\name{\fname{K.E.} \surname{Duffy}}{46}
\name{\fname{J.} \surname{Dumarchez}}{57}
\name{\fname{P.} \surname{Dunne}}{20}
\name{\fname{K.} \surname{Dygnarowicz}}{69}
\name{\fname{A.} \surname{Eguchi}}{59}
\name{\fname{M.} \surname{El Baz}}{11}
\name{\fname{J.} \surname{Elias}}{49}
\name{\fname{S.} \surname{Emery-Schrenk}}{5}
\name{\fname{G.} \surname{Erofeev}}{25}
\name{\fname{A.} \surname{Ershova}}{35}
\name{\fname{G.} \surname{Eurin}}{5}
\name{\fname{M.} \surname{Fani}}{52}
\name{\fname{D.} \surname{Fedorova}}{25}
\name{\fname{S.} \surname{Fedotov}}{25}
\name{\fname{M.} \surname{Feltre}}{23}
\name{\fname{C.} \surname{Fengler}}{46}
\name{\fname{L.} \surname{Feng}}{32}
\name{\fname{D.} \surname{Ferlewicz}}{57}
\name{\fname{A.J.} \surname{Finch}}{33}
\name{\fname{M.D.} \surname{Fitton}}{43}
\name{\fname{C.} \surname{Forza}}{23}
\name{\fname{M.} \surname{Friend}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{Y.} \surname{Fujii}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{Y.} \surname{Fukuda}}{40}
\name{\fname{N.} \surname{Funayama}}{45}
\name{\fname{Y.} \surname{Furui}}{63}
\name{\fname{A.N.} \surname{Gaci\~no Olmedo}}{57}
\name{\fname{J.} \surname{Garc\'ia-Marcos}}{13}
\name{\fname{A.C.} \surname{Germer}}{47}
\name{\fname{L.} \surname{Giannessi}}{11}
\name{\fname{C.} \surname{Giganti}}{57}
\name{\fname{M.} \surname{Girgus}}{68}
\name{\fname{V.} \surname{Glagolev}}{38}
\name{\fname{P.} \surname{Golak}}{68}
\name{\fname{M.} \surname{Gonin}}{27}
\name{\fname{R.} \surname{Gonzalez Jimenez}}{53}
\name{\fname{J.} \surname{Gonz\'alez Rosa}}{53}
\name{\fname{E.A.G.} \surname{Goodman}}{12}
\name{\fname{K.} \surname{Gorshanov}}{25}
\name{\fname{P.} \surname{Govindaraj}}{68}
\name{\fname{M.} \surname{Grassi}}{23}
\name{\fname{M.} \surname{Guigue}}{57}
\name{\fname{F.Y.} \surname{Guo}}{42}
\name{\fname{D.R.} \surname{Hadley}}{71}
\name{\fname{S.} \surname{Han}}{32,61}
\name{\fname{D.A.} \surname{Harris}}{74}
\name{\fname{R.J.} \surname{Harris}}{33,43}
\name{\fname{M.} \surname{Hartz}}{65,28}
\name{\fname{K.} \surname{Hasegawa}}{32}
\name{\fname{T.} \surname{Hasegawa}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{C.M.} \surname{Hasnip}}{10}
\name{\fname{S.} \surname{Hassani}}{5}
\name{\fname{N.C.} \surname{Hastings}}{15}
\name{\fname{K.} \surname{Hayashi}}{32}
\name{\fname{Y.} \surname{Hayato}}{60,28}
\name{\fname{I.} \surname{Heitkamp}}{70}
\name{\fname{D.} \surname{Henaff}}{5}
\name{\fname{Y.} \surname{Hino}}{15}
\name{\fname{K.} \surname{Hiraide}}{60,28}
\name{\fname{J.} \surname{Holeczek}}{55}
\name{\fname{A.} \surname{Holin}}{43}
\name{\fname{T.} \surname{Holvey}}{46}
\name{\fname{N.T.} \surname{Hong Van}}{26}
\name{\fname{T.} \surname{Honjo}}{45}
\name{\fname{M.C.F.} \surname{Hooft}}{13}
\name{\fname{K.} \surname{Hosokawa}}{60}
\name{\fname{R.} \surname{Huang}}{34}
\name{\fname{J.} \surname{Hu}}{32}
\name{\fname{A.K.} \surname{Ichikawa}}{70}
\name{\fname{K.} \surname{Ieki}}{60}
\name{\fname{M.} \surname{Ikeda}}{60}
\name{\fname{K.} \surname{Indo}}{32}
\name{\fname{T.H.} \surname{Ishida}}{70}
\name{\fname{T.} \surname{Ishida}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Ishitsuka}}{64}
\name{\fname{H.} \surname{Ito}}{31}
\name{\fname{S.} \surname{Ito}}{73}
\name{\fname{A.} \surname{Izmaylov}}{25}
\name{\fname{N.} \surname{Jachowicz}}{13}
\name{\fname{B.} \surname{Jargowsky}}{2}
\name{\fname{S.J.} \surname{Jenkins}}{36}
\name{\fname{C.} \surname{Jes\'us-Valls}}{10}
\name{\fname{M.} \surname{Jia}}{42}
\name{\fname{J.J.} \surname{Jiang}}{42}
\name{\fname{J.Y.} \surname{Ji}}{42}
\name{\fname{T.P.} \surname{Jones}}{33}
\name{\fname{P.} \surname{Jonsson}}{20}
\name{\fname{S.} \surname{Joshi}}{42}
\name{\fname{C.K.} \surname{Jung}}{42,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Kabirnezhad}}{46}
\name{\fname{A.C.} \surname{Kaboth}}{50}
\name{\fname{K.} \surname{Kadota}}{31}
\name{\fname{H.} \surname{Kakuno}}{63}
\name{\fname{A.} \surname{Kamata}}{63}
\name{\fname{J.} \surname{Kameda}}{60}
\name{\fname{S.} \surname{Karpova}}{11}
\name{\fname{V.S.} \surname{Kasturi}}{11}
\name{\fname{Y.} \surname{Kataoka}}{60}
\name{\fname{T.} \surname{Katori}}{30}
\name{\fname{A.} \surname{Kawabata}}{29}
\name{\fname{R.} \surname{Kawabe}}{45}
\name{\fname{Y.} \surname{Kawamura}}{45}
\name{\fname{M.} \surname{Kawaue}}{32}
\name{\fname{E.} \surname{Kearns}}{2,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Khabibullin}}{25}
\name{\fname{N.V.} \surname{Khomutov}}{38}
\name{\fname{A.} \surname{Khotjantsev}}{25}
\name{\fname{T.} \surname{Kikawa}}{32}
\name{\fname{S.} \surname{King}}{30}
\name{\fname{V.} \surname{Kiseeva}}{38}
\name{\fname{J.} \surname{Kisiel}}{55}
\name{\fname{A.} \surname{Klustov\'a}}{20}
\name{\fname{L.} \surname{Kneale}}{54}
\name{\fname{H.} \surname{Kobayashi}}{59}
\name{\fname{S.R.} \surname{Kobayashi}}{70}
\name{\fname{T.} \surname{Kobayashi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{L.} \surname{Koch}}{18}
\name{\fname{S.} \surname{Kodama}}{59}
\name{\fname{M.} \surname{Kolupanova}}{25,}\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}
\name{\fname{A.} \surname{Konaka}}{65}
\name{\fname{L.L.} \surname{Kormos}}{33}
\name{\fname{Y.} \surname{Koshio}}{44,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{K.} \surname{Kowalik}}{41}
\name{\fname{R.} \surname{Kralik}}{30}
\name{\fname{Y.} \surname{Kudenko}}{25,}\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}
\name{\fname{Y.} \surname{Kudo}}{73}
\name{\fname{A.} \surname{Kumar Jha}}{13}
\name{\fname{R.} \surname{Kurjata}}{69}
\name{\fname{V.} \surname{Kurochka}}{25}
\name{\fname{T.} \surname{Kutter}}{37}
\name{\fname{L.} \surname{Labarga}}{1}
\name{\fname{M.} \surname{Lachat}}{49}
\name{\fname{K.} \surname{Lachner}}{8}
\name{\fname{J.} \surname{Lagoda}}{41}
\name{\fname{S.M.} \surname{Lakshmi}}{55}
\name{\fname{M.} \surname{Lamers James}}{71}
\name{\fname{A.} \surname{Langella}}{22}
\name{\fname{D.H.} \surname{Langridge}}{50}
\name{\fname{J.-F.} \surname{Laporte}}{5}
\name{\fname{D.} \surname{Last}}{49}
\name{\fname{N.} \surname{Latham}}{30}
\name{\fname{M.} \surname{Laveder}}{23}
\name{\fname{L.} \surname{Lavitola}}{22}
\name{\fname{M.} \surname{Lawe}}{33}
\name{\fname{A.} \surname{Leclerc}}{5}
\name{\fname{N.} \surname{Lemaire}}{35}
\name{\fname{D.} \surname{Leon Silverio}}{58}
\name{\fname{T.} \surname{Leplumey}}{35}
\name{\fname{S.} \surname{Levorato}}{23}
\name{\fname{S.V.} \surname{Lewis}}{30}
\name{\fname{B.} \surname{Li}}{8}
\name{\fname{C.} \surname{Lin}}{20}
\name{\fname{R.P.} \surname{Litchfield}}{12}
\name{\fname{S.L.} \surname{Liu}}{42}
\name{\fname{W.} \surname{Li}}{46}
\name{\fname{A.} \surname{Longhin}}{23}
\name{\fname{A.} \surname{Lopez Moreno}}{30}
\name{\fname{L.} \surname{Ludovici}}{24}
\name{\fname{X.} \surname{Lu}}{71}
\name{\fname{T.} \surname{Lux}}{17}
\name{\fname{L.N.} \surname{Machado}}{12}
\name{\fname{L.} \surname{Magaletti}}{21}
\name{\fname{K.} \surname{Mahn}}{39}
\name{\fname{K.K.} \surname{Mahtani}}{42}
\name{\fname{S.} \surname{Manly}}{49}
\name{\fname{A.D.} \surname{Marino}}{6}
\name{\fname{D.G.R.} \surname{Martin}}{20}
\name{\fname{D.A.} \surname{Martinez Caicedo}}{58}
\name{\fname{L.} \surname{Martinez}}{17}
\name{\fname{M.} \surname{Martini}}{57,}\thanks{also at IPSA-DRII, France}
\name{\fname{N.} \surname{Mashin}}{25}
\name{\fname{T.} \surname{Matsubara}}{15}
\name{\fname{R.} \surname{Matsumoto}}{62}
\name{\fname{V.} \surname{Matveev}}{25}
\name{\fname{C.} \surname{Mauger}}{47}
\name{\fname{K.} \surname{Mavrokoridis}}{36}
\name{\fname{N.} \surname{McCauley}}{36}
\name{\fname{K.S.} \surname{McFarland}}{49}
\name{\fname{C.} \surname{McGrew}}{42}
\name{\fname{J.} \surname{McKean}}{32}
\name{\fname{A.} \surname{Mefodiev}}{25}
\name{\fname{G.D.} \surname{Megias}}{53}
\name{\fname{L.} \surname{Mellet}}{39}
\name{\fname{C.} \surname{Metelko}}{36}
\name{\fname{M.} \surname{Mezzetto}}{23}
\name{\fname{S.} \surname{Miki}}{60}
\name{\fname{V.} \surname{Mikola}}{12}
\name{\fname{E.W.} \surname{Miller}}{20}
\name{\fname{A.} \surname{Minamino}}{73}
\name{\fname{O.} \surname{Mineev}}{25}
\name{\fname{S.} \surname{Mine}}{60,4}
\name{\fname{J.} \surname{Mirabito}}{2}
\name{\fname{M.} \surname{Miura}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{73}
\name{\fname{P.} \surname{Morrison}}{12}
\name{\fname{Th.A.} \surname{Mueller}}{35}
\name{\fname{D.} \surname{Munford}}{16}
\name{\fname{A.} \surname{Mu\~noz}}{18}
\name{\fname{L.} \surname{Munteanu}}{10}
\name{\fname{Y.} \surname{Nagai}}{15}
\name{\fname{T.} \surname{Nakadaira}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{K.} \surname{Nakagiri}}{60}
\name{\fname{M.} \surname{Nakahata}}{60,28}
\name{\fname{Y.} \surname{Nakajima}}{59}
\name{\fname{K.D.} \surname{Nakamura}}{70}
\name{\fname{A.} \surname{Nakano}}{70}
\name{\fname{Y.} \surname{Nakano}}{66}
\name{\fname{S.} \surname{Nakayama}}{60,28}
\name{\fname{T.} \surname{Nakaya}}{32,28}
\name{\fname{K.} \surname{Nakayoshi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{C.E.R.} \surname{Naseby}}{20}
\name{\fname{D.T.} \surname{Nguyen}}{9}
\name{\fname{V.Q.} \surname{Nguyen}}{35}
\name{\fname{K.} \surname{Niewczas}}{35,13}
\name{\fname{S.} \surname{Nishimori}}{59}
\name{\fname{Y.} \surname{Nishimura}}{29}
\name{\fname{Y.} \surname{Noguchi}}{60}
\name{\fname{T.} \surname{Nosek}}{41}
\name{\fname{F.} \surname{Nova}}{43}
\name{\fname{J.C.} \surname{Nugent}}{20}
\name{\fname{H.M.} \surname{O'Keeffe}}{33}
\name{\fname{L.} \surname{O'Sullivan}}{18}
\name{\fname{R.} \surname{Okazaki}}{29}
\name{\fname{W.} \surname{Okinaga}}{59}
\name{\fname{K.} \surname{Okumura}}{61,28}
\name{\fname{T.} \surname{Okusawa}}{45}
\name{\fname{N.} \surname{Onda}}{32}
\name{\fname{N.} \surname{Ospina}}{21}
\name{\fname{L.} \surname{Osu}}{35}
\name{\fname{N.} \surname{Otani}}{32}
\name{\fname{Y.} \surname{Oyama}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{V.} \surname{Paolone}}{48}
\name{\fname{J.} \surname{Pasternak}}{20}
\name{\fname{D.} \surname{Payne}}{36}
\name{\fname{T.P.D.} \surname{Peacock}}{54}
\name{\fname{M.} \surname{Pfaff}}{20}
\name{\fname{L.} \surname{Pickering}}{43}
\name{\fname{J.-B.} \surname{Plan\c{c}on}}{35}
\name{\fname{P.} \surname{Podlaski}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{B.} \surname{Popov}}{57,}\thanks{also at JINR, Dubna, Russia}
\name{\fname{A.J.} \surname{Portocarrero Yrey}}{15}
\name{\fname{M.} \surname{Posiadala-Zezula}}{68}
\name{\fname{Y.S.} \surname{Prabhu}}{68}
\name{\fname{H.} \surname{Prasad}}{72}
\name{\fname{F.} \surname{Pupilli}}{23}
\name{\fname{B.} \surname{Quilain}}{27,35}
\name{\fname{P.T.} \surname{Quyen}}{19,}\thanks{also at the Graduate University of Science and Technology, Vietnam Academy of Science and Technology}
\name{\fname{E.} \surname{Radicioni}}{21}
\name{\fname{B.} \surname{Radics}}{74}
\name{\fname{M.A.} \surname{Ramirez Delgado}}{47}
\name{\fname{R.} \surname{Ramsden}}{30}
\name{\fname{P.N.} \surname{Ratoff}}{33}
\name{\fname{M.} \surname{Reh}}{6}
\name{\fname{G.} \surname{Reina}}{18}
\name{\fname{L.} \surname{Restrepo}}{57}
\name{\fname{C.} \surname{Riccio}}{42}
\name{\fname{D.W.} \surname{Riley}}{12}
\name{\fname{E.} \surname{Rondio}}{41}
\name{\fname{D.} \surname{Ross}}{39}
\name{\fname{S.} \surname{Roth}}{51}
\name{\fname{N.} \surname{Roy}}{74}
\name{\fname{A.} \surname{Rubbia}}{8}
\name{\fname{L.} \surname{Russo}}{57}
\name{\fname{A.} \surname{Rychter}}{69}
\name{\fname{W.} \surname{Saenz}}{57}
\name{\fname{K.} \surname{Sakashita}}{67,15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{S.} \surname{Samani}}{11}
\name{\fname{F.} \surname{S\'anchez}}{11}
\name{\fname{E.M.} \surname{Sandford}}{36}
\name{\fname{Y.} \surname{Sato}}{64}
\name{\fname{T.} \surname{Schefke}}{37}
\name{\fname{K.} \surname{Scholberg}}{7,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Scott}}{20}
\name{\fname{Y.} \surname{Seiya}}{45,}\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}
\name{\fname{T.} \surname{Sekiguchi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{H.} \surname{Sekiya}}{60,28,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Sekiyama}}{59}
\name{\fname{T.} \surname{Sekiya}}{63}
\name{\fname{D.} \surname{Seppala}}{39}
\name{\fname{D.} \surname{Sgalaberna}}{8}
\name{\fname{A.} \surname{Shaikhiev}}{25}
\name{\fname{M.} \surname{Shiozawa}}{60,28}
\name{\fname{Y.} \surname{Shiraishi}}{44}
\name{\fname{N.} \surname{Shvarev}}{25}
\name{\fname{A.} \surname{Shvartsman}}{25}
\name{\fname{V.} \surname{Siccardi}}{30}
\name{\fname{N.} \surname{Skrobova}}{25}
\name{\fname{K.} \surname{Skwarczynski}}{50}
\name{\fname{D.} \surname{Smyczek}}{51}
\name{\fname{M.} \surname{Smy}}{4}
\name{\fname{J.T.} \surname{Sobczyk}}{72}
\name{\fname{H.} \surname{Sobel}}{4,28}
\name{\fname{F.J.P.} \surname{Soler}}{12}
\name{\fname{A.J.} \surname{Speers}}{33}
\name{\fname{R.} \surname{Spina}}{21}
\name{\fname{A.} \surname{Srivastava}}{18}
\name{\fname{P.} \surname{Stowell}}{54}
\name{\fname{Y.} \surname{Stroke}}{25}
\name{\fname{I.A.} \surname{Suslov}}{38}
\name{\fname{A.} \surname{Suzuki}}{31}
\name{\fname{M.} \surname{Suzuki}}{73}
\name{\fname{S.Y.} \surname{Suzuki}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Tada}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{S.} \surname{Tairafune}}{70}
\name{\fname{A.} \surname{Takeda}}{60}
\name{\fname{Y.} \surname{Takeuchi}}{31,28}
\name{\fname{K.} \surname{Takeya}}{44}
\name{\fname{H.K.} \surname{Tanaka}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{H.} \surname{Tanigawa}}{29}
\name{\fname{A.} \surname{Teklu}}{42}
\name{\fname{V.V.} \surname{Tereshchenko}}{38}
\name{\fname{N.} \surname{Thamm}}{51}
\name{\fname{C.} \surname{Touramanis}}{36}
\name{\fname{N.} \surname{Tran}}{19}
\name{\fname{T.} \surname{Tsukamoto}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Tzanov}}{37}
\name{\fname{Y.} \surname{Uchida}}{20}
\name{\fname{M.} \surname{Vagins}}{28,4}
\name{\fname{M.} \surname{Varghese}}{17}
\name{\fname{I.} \surname{Vasilyev}}{38}
\name{\fname{G.} \surname{Vasseur}}{5}
\name{\fname{E.} \surname{Villa}}{8}
\name{\fname{U.} \surname{Virginet}}{57}
\name{\fname{T.} \surname{Vladisavljevic}}{43}
\name{\fname{T.} \surname{Wachala}}{14}
\name{\fname{S.-i.} \surname{Wada}}{31}
\name{\fname{D.} \surname{Wakabayashi}}{70}
\name{\fname{H.T.} \surname{Wallace}}{54}
\name{\fname{J.G.} \surname{Walsh}}{39}
\name{\fname{D.} \surname{Wark}}{43,46}
\name{\fname{M.O.} \surname{Wascko}}{46,43}
\name{\fname{A.} \surname{Weber}}{18}
\name{\fname{R.} \surname{Wendell}}{32}
\name{\fname{M.J.} \surname{Wilking}}{52}
\name{\fname{C.} \surname{Wilkinson}}{34}
\name{\fname{J.R.} \surname{Wilson}}{30}
\name{\fname{C.} \surname{Winterstein}}{5}
\name{\fname{K.} \surname{Wood}}{34}
\name{\fname{C.} \surname{Wret}}{20}
\name{\fname{J.} \surname{Xia}}{56}
\name{\fname{Z.} \surname{Xie}}{52}
\name{\fname{K.} \surname{Yamamoto}}{45,}\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}
\name{\fname{T.} \surname{Yamamoto}}{45}
\name{\fname{T.} \surname{Yamazumi}}{59}
\name{\fname{C.} \surname{Yanagisawa}}{42,}\thanks{also at BMCC/CUNY, Science Department, New York, New York, U.S.A.}
\name{\fname{Y.} \surname{Yang}}{46}
\name{\fname{T.} \surname{Yano}}{60}
\name{\fname{N.} \surname{Yershov}}{25}
\name{\fname{U.} \surname{Yevarouskaya}}{42}
\name{\fname{M.} \surname{Yokoyama}}{59,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{Y.} \surname{Yoshimoto}}{59}
\name{\fname{N.} \surname{Yoshimura}}{32}
\name{\fname{R.} \surname{Zaki}}{74}
\name{\fname{A.} \surname{Zalewska}}{14}
\name{\fname{J.} \surname{Zalipska}}{41}
\name{\fname{G.} \surname{Zarnecki}}{14}
\name{\fname{J.} \surname{Zhang}}{65,3}
\name{\fname{X.Y.} \surname{Zhao}}{20}
\name{\fname{H.} \surname{Zheng}}{42}
\name{\fname{H.} \surname{Zhong}}{31}
\name{\fname{T.} \surname{Zhu}}{20}
\name{\fname{M.} \surname{Ziembicki}}{69}
\name{\fname{E.D.} \surname{Zimmerman}}{6}
\name{\fname{M.} \surname{Zito}}{57}
\name{\fname{S.} \surname{Zsoldos}}{30}
}

\address{
\affil{1}{University Autonoma Madrid, Department of Theoretical Physics, 28049 Madrid, Spain}
\affil{2}{Boston University, Department of Physics, Boston, Massachusetts, U.S.A.}
\affil{3}{University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada}
\affil{4}{University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.}
\affil{5}{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affil{6}{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}
\affil{7}{Duke University, Department of Physics, Durham, North Carolina, U.S.A.}
\affil{8}{ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland}
\affil{9}{VNU University of Science, Vietnam National University, Hanoi, Vietnam}
\affil{10}{CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland}
\affil{11}{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}
\affil{12}{University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom}
\affil{13}{Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium}
\affil{14}{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}
\affil{15}{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}
\affil{16}{University of Houston, Department of Physics, Houston, Texas, U.S.A.}
\affil{17}{Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}
\affil{18}{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Staudingerweg 7, 55128 Mainz, Germany}
\affil{19}{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}
\affil{20}{Imperial College London, Department of Physics, London, United Kingdom}
\affil{21}{INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}
\affil{22}{INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}
\affil{23}{INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}
\affil{24}{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy}
\affil{25}{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}
\affil{26}{International Centre of Physics, Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), 10 Dao Tan, Ba Dinh, Hanoi, Vietnam}
\affil{27}{ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}
\affil{28}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}
\affil{29}{Keio University, Department of Physics, Kanagawa, Japan}
\affil{30}{King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom}
\affil{31}{Kobe University, Kobe, Japan}
\affil{32}{Kyoto University, Department of Physics, Kyoto, Japan}
\affil{33}{Lancaster University, School of Physics and Astronomy, Lancaster, United Kingdom}
\affil{34}{Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.}
\affil{35}{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France}
\affil{36}{University of Liverpool, Department of Physics, Liverpool, United Kingdom}
\affil{37}{Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}
\affil{38}{Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia}
\affil{39}{Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.}
\affil{40}{Miyagi University of Education, Department of Physics, Sendai, Japan}
\affil{41}{National Centre for Nuclear Research, Warsaw, Poland}
\affil{42}{State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}
\affil{43}{STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}
\affil{44}{Okayama University, Department of Physics, Okayama, Japan}
\affil{45}{Osaka Metropolitan University, Department of Physics, Osaka, Japan}
\affil{46}{Oxford University, Department of Physics, Oxford, United Kingdom}
\affil{47}{University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.}
\affil{48}{University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.}
\affil{49}{University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}
\affil{50}{Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom}
\affil{51}{RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany}
\affil{52}{School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota, U.S.A.}
\affil{53}{Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain}
\affil{54}{University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom}
\affil{55}{University of Silesia, Institute of Physics, Katowice, Poland}
\affil{56}{SLAC National Accelerator Laboratory, Stanford University, Menlo Park, California, U.S.A.}
\affil{57}{Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}
\affil{58}{South Dakota School of Mines and Technology, 501 East Saint Joseph Street, Rapid City, SD 57701, United States}
\affil{59}{University of Tokyo, Department of Physics, Tokyo, Japan}
\affil{60}{University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}
\affil{61}{University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}
\affil{62}{Institute of Science Tokyo, Department of Physics, Tokyo}
\affil{63}{Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}
\affil{64}{Tokyo University of Science, Faculty of Science and Technology, Department of Physics, Noda, Chiba, Japan}
\affil{65}{TRIUMF, Vancouver, British Columbia, Canada}
\affil{66}{University of Toyama, Faculty of Science, Toyama, Japan}
\affil{67}{University of Tsukuba, Faculty of Pure and Applied Sciences, Tsukuba, Ibaraki, Japan}
\affil{68}{University of Warsaw, Faculty of Physics, Warsaw, Poland}
\affil{69}{Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland}
\affil{70}{Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan}
\affil{71}{University of Warwick, Department of Physics, Coventry, United Kingdom}
\affil{72}{Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}
\affil{73}{Yokohama National University, Department of Physics, Yokohama, Japan}
\affil{74}{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}
}


==> authorlist_backup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% T2K author list generated on Tue Jul 22 01:49:51 2025
% setting: extra = False
%         author list from archive (starting March 14 2025 until July 16 2025)
%         exemption(s) granted to: ashida,rgonzjim,jgrosa,gdmegias,jac,jgm,hmatthias,njachowicz,akumar,edatkin,martind,kniewczas,scap,vedantha,fcadoux,fsanchez,evila,amunoz,nova,pdunne,dlast,adrienblanchet,mkabirne,barker,morgan_wascko,bdl,vlglagolev,slava,mtzanov,kutter,lmachado,litchfieldp,egoodman,yyang,kiseevavi,akaboth,kmahtani,dseppala,acraplet,alex,kudenko,oleg,erofeev,kurochka,matveev,shaykhiev,greina,asrivast,nicklatham,nakahata,rubbiaa,laveder,mezzetto,Forza,mgrassi,damartin,denhaff,wilking
% Number of authors = 401
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\noaffiliation}{}

\newcommand{\INSTHD}{\affil{University Autonoma Madrid, Department of Theoretical Physics, 28049 Madrid, Spain}}
\newcommand{\INSTFE}{\affil{Boston University, Department of Physics, Boston, Massachusetts, U.S.A.}}
\newcommand{\INSTD}{\affil{University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada}}
\newcommand{\INSTGA}{\affil{University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.}}
\newcommand{\INSTI}{\affil{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}}
\newcommand{\INSTGB}{\affil{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}}
\newcommand{\INSTFH}{\affil{Duke University, Department of Physics, Durham, North Carolina, U.S.A.}}
\newcommand{\INSTJA}{\affil{E\"{o}tv\"{o}s Lor\'{a}nd University, Department of Atomic Physics, Budapest, Hungary}}
\newcommand{\INSTEF}{\affil{ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland}}
\newcommand{\INSTIG}{\affil{VNU University of Science, Vietnam National University, Hanoi, Vietnam}}
\newcommand{\INSTIE}{\affil{CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland}}
\newcommand{\INSTEG}{\affil{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}}
\newcommand{\INSTHJ}{\affil{University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom}}
\newcommand{\INSTJG}{\affil{Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium}}
\newcommand{\INSTDG}{\affil{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}}
\newcommand{\INSTCB}{\affil{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}}
\newcommand{\INSTIB}{\affil{University of Houston, Department of Physics, Houston, Texas, U.S.A.}}
\newcommand{\INSTED}{\affil{Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}}
\newcommand{\INSTJC}{\affil{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Staudingerweg 7, 55128 Mainz, Germany}}
\newcommand{\INSTHH}{\affil{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}}
\newcommand{\INSTEI}{\affil{Imperial College London, Department of Physics, London, United Kingdom}}
\newcommand{\INSTGF}{\affil{INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}}
\newcommand{\INSTBE}{\affil{INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}}
\newcommand{\INSTBF}{\affil{INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}}
\newcommand{\INSTBD}{\affil{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy}}
\newcommand{\INSTEB}{\affil{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}}
\newcommand{\INSTHI}{\affil{International Centre of Physics, Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), 10 Dao Tan, Ba Dinh, Hanoi, Vietnam}}
\newcommand{\INSTJD}{\affil{ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}}
\newcommand{\INSTHA}{\affil{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}}
\newcommand{\INSTID}{\affil{Keio University, Department of Physics, Kanagawa, Japan}}
\newcommand{\INSTIF}{\affil{King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom}}
\newcommand{\INSTCC}{\affil{Kobe University, Kobe, Japan}}
\newcommand{\INSTCD}{\affil{Kyoto University, Department of Physics, Kyoto, Japan}}
\newcommand{\INSTEJ}{\affil{Lancaster University, Physics Department, Lancaster, United Kingdom}}
\newcommand{\INSTII}{\affil{Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.}}
\newcommand{\INSTBA}{\affil{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France}}
\newcommand{\INSTFC}{\affil{University of Liverpool, Department of Physics, Liverpool, United Kingdom}}
\newcommand{\INSTFI}{\affil{Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}}
\newcommand{\INSTIH}{\affil{Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia}}
\newcommand{\INSTHB}{\affil{Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.}}
\newcommand{\INSTCE}{\affil{Miyagi University of Education, Department of Physics, Sendai, Japan}}
\newcommand{\INSTDF}{\affil{National Centre for Nuclear Research, Warsaw, Poland}}
\newcommand{\INSTFJ}{\affil{State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}}
\newcommand{\INSTEH}{\affil{STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}}
\newcommand{\INSTGJ}{\affil{Okayama University, Department of Physics, Okayama, Japan}}
\newcommand{\INSTCF}{\affil{Osaka Metropolitan University, Department of Physics, Osaka, Japan}}
\newcommand{\INSTGG}{\affil{Oxford University, Department of Physics, Oxford, United Kingdom}}
\newcommand{\INSTIC}{\affil{University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.}}
\newcommand{\INSTGC}{\affil{University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.}}
\newcommand{\INSTGD}{\affil{University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}}
\newcommand{\INSTHC}{\affil{Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom}}
\newcommand{\INSTBC}{\affil{RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany}}
\newcommand{\INSTJF}{\affil{School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota, U.S.A.}}
\newcommand{\INSTJB}{\affil{Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain}}
\newcommand{\INSTFB}{\affil{University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom}}
\newcommand{\INSTDI}{\affil{University of Silesia, Institute of Physics, Katowice, Poland}}
\newcommand{\INSTIA}{\affil{SLAC National Accelerator Laboratory, Stanford University, Menlo Park, California, U.S.A.}}
\newcommand{\INSTBB}{\affil{Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}}
\newcommand{\INSTJE}{\affil{South Dakota School of Mines and Technology, 501 East Saint Joseph Street, Rapid City, SD 57701, United States}}
\newcommand{\INSTCH}{\affil{University of Tokyo, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTBJ}{\affil{University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}}
\newcommand{\INSTCG}{\affil{University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}}
\newcommand{\INSTHF}{\affil{Institute of Science Tokyo, Department of Physics, Tokyo}}
\newcommand{\INSTGI}{\affil{Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}}
\newcommand{\INSTHG}{\affil{Tokyo University of Science, Faculty of Science and Technology, Department of Physics, Noda, Chiba, Japan}}
\newcommand{\INSTB}{\affil{TRIUMF, Vancouver, British Columbia, Canada}}
\newcommand{\INSTJH}{\affil{University of Toyama, Department of Physics, Toyama, Japan}}
\newcommand{\INSTDJ}{\affil{University of Warsaw, Faculty of Physics, Warsaw, Poland}}
\newcommand{\INSTDH}{\affil{Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland}}
\newcommand{\INSTIJ}{\affil{Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan}}
\newcommand{\INSTFD}{\affil{University of Warwick, Department of Physics, Coventry, United Kingdom}}
\newcommand{\INSTEA}{\affil{Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}}
\newcommand{\INSTHE}{\affil{Yokohama National University, Department of Physics, Yokohama, Japan}}
\newcommand{\INSTH}{\affil{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}}

\author{K.\,Abe}\INSTBJ
\author{S.\,Abe}\INSTBJ
\author{R.\,Akutsu}\INSTCB
\author{H.\,Alarakia-Charles}\INSTEJ
\author{Y.I.\,Alj Hakim}\INSTFB
\author{S.\,Alonso Monsalve}\INSTEF
\author{L.\,Anthony}\INSTEI
\author{S.\,Aoki}\INSTCC
\author{K.A.\,Apte}\INSTEI
\author{T.\,Arai}\INSTCH
\author{T.\,Arihara}\INSTGI
\author{S.\,Arimoto}\INSTCD
\author{Y.\,Ashida}\INSTIJ
\author{E.T.\,Atkin}\INSTEI
\author{N.\,Babu}\INSTFI
\author{V.\,Baranov}\INSTIH
\author{G.J.\,Barker}\INSTFD
\author{G.\,Barr}\INSTGG
\author{D.\,Barrow}\INSTGG
\author{P.\,Bates}\INSTFC
\author{L.\,Bathe-Peters}\INSTGG
\author{M.\,Batkiewicz-Kwasniak}\INSTDG
\author{N.\,Baudis}\INSTGG
\author{V.\,Berardi}\INSTGF
\author{L.\,Berns}\INSTIJ
\author{S.\,Bhattacharjee}\INSTFI
\author{A.\,Blanchet}\INSTIE
\author{A.\,Blondel}\INSTBB\INSTEG
\author{P.M.M.\,Boistier}\INSTI
\author{S.\,Bolognesi}\INSTI
\author{S.\,Bordoni }\INSTEG
\author{S.B.\,Boyd}\INSTFD
\author{C.\,Bronner}\INSTHE
\author{A.\,Bubak}\INSTDI
\author{M.\,Buizza Avanzini}\INSTBA
\author{J.A.\,Caballero}\INSTJB
\author{F.\,Cadoux}\INSTEG
\author{N.F.\,Calabria}\INSTGF
\author{S.\,Cao}\INSTHH
\author{S.\,Cap}\INSTEG
\author{D.\,Carabadjac\thanks{also at Universit\'e Paris-Saclay}}\INSTBA
\author{S.L.\,Cartwright}\INSTFB
\author{M.P.\,Casado\thanks{also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain}}\INSTED
\author{M.G.\,Catanesi}\INSTGF
\author{J.\,Chakrani}\INSTII
\author{A.\,Chalumeau}\INSTBB
\author{D.\,Cherdack}\INSTIB
\author{A.\,Chvirova}\INSTEB
\author{J.\,Coleman}\INSTFC
\author{G.\,Collazuol}\INSTBF
\author{F.\,Cormier}\INSTB
\author{A.A.L.\,Craplet}\INSTEI
\author{A.\,Cudd}\INSTGB
\author{D.\,D'ago}\INSTBF
\author{C.\,Dalmazzone}\INSTBB
\author{T.\,Daret}\INSTI
\author{P.\,Dasgupta}\INSTJA
\author{C.\,Davis}\INSTIC
\author{Yu.I.\,Davydov}\INSTIH
\author{P.\,de Perio}\INSTHA
\author{G.\,De Rosa}\INSTBE
\author{T.\,Dealtry}\INSTEJ
\author{C.\,Densham}\INSTEH
\author{A.\,Dergacheva}\INSTEB
\author{R.\,Dharmapal Banerjee}\INSTEA
\author{F.\,Di Lodovico}\INSTIF
\author{G.\,Diaz Lopez}\INSTBB
\author{S.\,Dolan}\INSTIE
\author{D.\,Douqa}\INSTEG
\author{T.A.\,Doyle}\INSTGG
\author{O.\,Drapier}\INSTBA
\author{K.E.\,Duffy}\INSTGG
\author{J.\,Dumarchez}\INSTBB
\author{P.\,Dunne}\INSTEI
\author{K.\,Dygnarowicz}\INSTDH
\author{A.\,Eguchi}\INSTCH
\author{J.\,Elias}\INSTGD
\author{S.\,Emery-Schrenk}\INSTI
\author{G.\,Erofeev}\INSTEB
\author{A.\,Ershova}\INSTBA
\author{G.\,Eurin}\INSTI
\author{D.\,Fedorova}\INSTEB
\author{S.\,Fedotov}\INSTEB
\author{M.\,Feltre}\INSTBF
\author{L.\,Feng}\INSTCD
\author{D.\,Ferlewicz}\INSTCH
\author{A.J.\,Finch}\INSTEJ
\author{M.D.\,Fitton}\INSTEH
\author{C.\,Forza}\INSTBF
\author{M.\,Friend\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{Y.\,Fujii\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{Y.\,Fukuda}\INSTCE
\author{Y.\,Furui}\INSTGI
\author{J.\,Garc\'ia-Marcos}\INSTJG
\author{A.C.\,Germer}\INSTIC
\author{L.\,Giannessi}\INSTEG
\author{C.\,Giganti}\INSTBB
\author{M.\,Girgus}\INSTDJ
\author{V.\,Glagolev}\INSTIH
\author{M.\,Gonin}\INSTJD
\author{R.\,Gonz\'alez Jim\'enez}\INSTJB
\author{J.\,Gonz\'alez Rosa}\INSTJB
\author{E.A.G.\,Goodman}\INSTHJ
\author{K.\,Gorshanov}\INSTEB
\author{P.\,Govindaraj}\INSTDJ
\author{M.\,Grassi}\INSTBF
\author{M.\,Guigue}\INSTBB
\author{F.Y.\,Guo}\INSTFJ
\author{D.R.\,Hadley}\INSTFD
\author{S.\,Han}\INSTCD\INSTCG
\author{D.A.\,Harris}\INSTH
\author{R.J.\,Harris}\INSTEJ\INSTEH
\author{T.\,Hasegawa\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{C.M.\,Hasnip}\INSTIE
\author{S.\,Hassani}\INSTI
\author{N.C.\,Hastings}\INSTCB
\author{Y.\,Hayato}\INSTBJ\INSTHA
\author{I.\,Heitkamp}\INSTIJ
\author{D.\,Henaff}\INSTI
\author{Y.\,Hino}\INSTCB
\author{J.\,Holeczek}\INSTDI
\author{A.\,Holin}\INSTEH
\author{T.\,Holvey}\INSTGG
\author{N.T.\,Hong Van}\INSTHI
\author{T.\,Honjo}\INSTCF
\author{M.C.F.\,Hooft}\INSTJG
\author{K.\,Hosokawa}\INSTBJ
\author{J.\,Hu}\INSTCD
\author{A.K.\,Ichikawa}\INSTIJ
\author{K.\,Ieki}\INSTBJ
\author{M.\,Ikeda}\INSTBJ
\author{T.H.\,Ishida}\INSTIJ
\author{T.\,Ishida\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{M.\,Ishitsuka}\INSTHG
\author{H.\,Ito}\INSTCC
\author{S.\,Ito}\INSTHE
\author{A.\,Izmaylov}\INSTEB
\author{N.\,Jachowicz}\INSTJG
\author{S.J.\,Jenkins}\INSTFC
\author{C.\,Jes\'us-Valls}\INSTIE
\author{M.\,Jia}\INSTFJ
\author{J.J.\,Jiang}\INSTFJ
\author{J.Y.\,Ji}\INSTFJ
\author{T.P.\,Jones}\INSTEJ
\author{P.\,Jonsson}\INSTEI
\author{S.\,Joshi}\INSTI
\author{M.\,Kabirnezhad}\INSTEI
\author{A.C.\,Kaboth}\INSTHC
\author{H.\,Kakuno}\INSTGI
\author{J.\,Kameda}\INSTBJ
\author{S.\,Karpova}\INSTEG
\author{V.S.\,Kasturi}\INSTEG
\author{Y.\,Kataoka}\INSTBJ
\author{T.\,Katori}\INSTIF
\author{A.\,Kawabata}\INSTID
\author{Y.\,Kawamura}\INSTCF
\author{M.\,Kawaue}\INSTCD
\author{E.\,Kearns\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}\INSTFE
\author{M.\,Khabibullin}\INSTEB
\author{A.\,Khotjantsev}\INSTEB
\author{T.\,Kikawa}\INSTCD
\author{S.\,King}\INSTIF
\author{V.\,Kiseeva}\INSTIH
\author{J.\,Kisiel}\INSTDI
\author{A.\,Klustov\'a}\INSTEI
\author{L.\,Kneale}\INSTFB
\author{H.\,Kobayashi}\INSTCH
\author{Sota.R\,Kobayashi}\INSTIJ
\author{L.\,Koch}\INSTJC
\author{S.\,Kodama}\INSTCH
\author{M.\,Kolupanova}\INSTEB
\author{A.\,Konaka}\INSTB
\author{L.L.\,Kormos}\INSTEJ
\author{Y.\,Koshio\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}\INSTGJ
\author{K.\,Kowalik}\INSTDF
\author{Y.\,Kudenko\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}}\INSTEB
\author{Y.\,Kudo}\INSTHE
\author{A.\,Kumar Jha}\INSTJG
\author{R.\,Kurjata}\INSTDH
\author{V.\,Kurochka}\INSTEB
\author{T.\,Kutter}\INSTFI
\author{L.\,Labarga}\INSTHD
\author{M.\,Lachat}\INSTGD
\author{K.\,Lachner}\INSTEF
\author{J.\,Lagoda}\INSTDF
\author{S.M.\,Lakshmi}\INSTDI
\author{M.\,Lamers James}\INSTFD
\author{A.\,Langella}\INSTBE
\author{D.H.\,Langridge}\INSTHC
\author{J.-F.\,Laporte}\INSTI
\author{D.\,Last}\INSTGD
\author{N.\,Latham}\INSTIF
\author{M.\,Laveder}\INSTBF
\author{L.\,Lavitola}\INSTBE
\author{M.\,Lawe}\INSTEJ
\author{D.\,Leon Silverio}\INSTJE
\author{S.\,Levorato}\INSTBF
\author{S.V.\,Lewis}\INSTIF
\author{B.\,Li}\INSTEF
\author{C.\,Lin}\INSTEI
\author{R.P.\,Litchfield}\INSTHJ
\author{S.L.\,Liu}\INSTFJ
\author{W.\,Li}\INSTGG
\author{A.\,Longhin}\INSTBF
\author{A.\,Lopez Moreno}\INSTIF
\author{L.\,Ludovici}\INSTBD
\author{X.\,Lu}\INSTFD
\author{T.\,Lux}\INSTED
\author{L.N.\,Machado}\INSTHJ
\author{L.\,Magaletti}\INSTGF
\author{K.\,Mahn}\INSTHB
\author{K.K.\,Mahtani}\INSTFJ
\author{S.\,Manly}\INSTGD
\author{A.D.\,Marino}\INSTGB
\author{D.G.R.\,Martin}\INSTEI
\author{D.A.\,Martinez Caicedo}\INSTJE
\author{L.\,Martinez}\INSTED
\author{M.\,Martini\thanks{also at IPSA-DRII, France}}\INSTBB
\author{T.\,Matsubara}\INSTCB
\author{R.\,Matsumoto}\INSTHF
\author{V.\,Matveev}\INSTEB
\author{C.\,Mauger}\INSTIC
\author{K.\,Mavrokoridis}\INSTFC
\author{N.\,McCauley}\INSTFC
\author{K.S.\,McFarland}\INSTGD
\author{C.\,McGrew}\INSTFJ
\author{J.\,McKean}\INSTEI
\author{A.\,Mefodiev}\INSTEB
\author{G.D.\,Megias }\INSTJB
\author{L.\,Mellet}\INSTHB
\author{C.\,Metelko}\INSTFC
\author{M.\,Mezzetto}\INSTBF
\author{S.\,Miki}\INSTBJ
\author{V.\,Mikola}\INSTHJ
\author{E.W.\,Miller}\INSTED
\author{A.\,Minamino}\INSTHE
\author{O.\,Mineev}\INSTEB
\author{S.\,Mine}\INSTBJ\INSTGA
\author{J.\,Mirabito}\INSTFE
\author{M.\,Miura\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}\INSTBJ
\author{S.\,Moriyama\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}\INSTBJ
\author{S.\,Moriyama}\INSTHE
\author{P.\,Morrison}\INSTHJ
\author{Th.A.\,Mueller}\INSTBA
\author{D.\,Munford}\INSTIB
\author{A.\,Mu\~noz}\INSTBA\INSTJD
\author{L.\,Munteanu}\INSTIE
\author{Y.\,Nagai}\INSTJA
\author{T.\,Nakadaira\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{K.\,Nakagiri}\INSTCH
\author{M.\,Nakahata}\INSTBJ\INSTHA
\author{Y.\,Nakajima}\INSTCH
\author{K.D.\,Nakamura}\INSTIJ
\author{A.\,Nakano}\INSTIJ
\author{Y.\,Nakano}\INSTJH
\author{S.\,Nakayama}\INSTBJ\INSTHA
\author{T.\,Nakaya}\INSTCD\INSTHA
\author{K.\,Nakayoshi\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{C.E.R.\,Naseby}\INSTEI
\author{D.T.\,Nguyen}\INSTIG
\author{V.Q.\,Nguyen}\INSTBA
\author{K.\,Niewczas}\INSTJG
\author{S.\,Nishimori}\INSTCB
\author{Y.\,Nishimura}\INSTID
\author{Y.\,Noguchi}\INSTBJ
\author{T.\,Nosek}\INSTDF
\author{F.\,Nova}\INSTEH
\author{J.C.\,Nugent}\INSTEI
\author{H.M.\,O'Keeffe}\INSTEJ
\author{L.\,O'Sullivan}\INSTJC
\author{R.\,Okazaki}\INSTID
\author{W.\,Okinaga}\INSTCH
\author{K.\,Okumura}\INSTCG\INSTHA
\author{T.\,Okusawa}\INSTCF
\author{N.\,Onda}\INSTCD
\author{N.\,Ospina}\INSTGF
\author{L.\,Osu}\INSTBA
\author{N.\,Otani}\INSTCD
\author{Y.\,Oyama\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{V.\,Paolone}\INSTGC
\author{J.\,Pasternak}\INSTEI
\author{D.\,Payne}\INSTFC
\author{T.P.D.\,Peacock}\INSTFB
\author{M.\,Pfaff}\INSTEI
\author{L.\,Pickering}\INSTEH
\author{B.\,Popov\thanks{also at JINR, Dubna, Russia}}\INSTBB
\author{A.J.\,Portocarrero Yrey}\INSTCB
\author{M.\,Posiadala-Zezula}\INSTDJ
\author{Y.S.\,Prabhu}\INSTDJ
\author{H.\,Prasad}\INSTEA
\author{F.\,Pupilli}\INSTBF
\author{B.\,Quilain}\INSTJD\INSTBA
\author{P.T.\,Quyen\thanks{also at the Graduate University of Science and Technology, Vietnam Academy of Science and Technology}}\INSTHH
\author{E.\,Radicioni}\INSTGF
\author{B.\,Radics}\INSTH
\author{M.A.\,Ramirez}\INSTIC
\author{R.\,Ramsden}\INSTIF
\author{P.N.\,Ratoff}\INSTEJ
\author{M.\,Reh}\INSTGB
\author{G.\,Reina}\INSTJC
\author{C.\,Riccio}\INSTFJ
\author{D.W.\,Riley}\INSTHJ
\author{E.\,Rondio}\INSTDF
\author{S.\,Roth}\INSTBC
\author{N.\,Roy}\INSTH
\author{A.\,Rubbia}\INSTEF
\author{L.\,Russo}\INSTBB
\author{A.\,Rychter}\INSTDH
\author{W.\,Saenz}\INSTBB
\author{K.\,Sakashita\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{S.\,Samani}\INSTEG
\author{F.\,S\'anchez}\INSTEG
\author{E.M.\,Sandford}\INSTFC
\author{Y.\,Sato}\INSTHG
\author{T.\,Schefke}\INSTFI
\author{K.\,Scholberg\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}\INSTFH
\author{M.\,Scott}\INSTEI
\author{Y.\,Seiya\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}}\INSTCF
\author{T.\,Sekiguchi\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{H.\,Sekiya\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}\INSTBJ\INSTHA
\author{T.\,Sekiya}\INSTGI
\author{D.\,Seppala}\INSTHB
\author{D.\,Sgalaberna}\INSTEF
\author{A.\,Shaikhiev}\INSTEB
\author{M.\,Shiozawa}\INSTBJ\INSTHA
\author{Y.\,Shiraishi}\INSTGJ
\author{A.\,Shvartsman}\INSTEB
\author{N.\,Skrobova}\INSTEB
\author{K.\,Skwarczynski}\INSTHC
\author{D.\,Smyczek}\INSTBC
\author{M.\,Smy}\INSTGA
\author{J.T.\,Sobczyk}\INSTEA
\author{H.\,Sobel}\INSTGA\INSTHA
\author{F.J.P.\,Soler}\INSTHJ
\author{A.J.\,Speers}\INSTEJ
\author{R.\,Spina}\INSTGF
\author{A.\,Srivastava}\INSTJC
\author{P.\,Stowell}\INSTFB
\author{Y.\,Stroke}\INSTEB
\author{I.A.\,Suslov}\INSTIH
\author{A.\,Suzuki}\INSTCC
\author{S.Y.\,Suzuki\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{M.\,Tada\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{S.\,Tairafune}\INSTIJ
\author{A.\,Takeda}\INSTBJ
\author{Y.\,Takeuchi}\INSTCC\INSTHA
\author{K.\,Takeya}\INSTGJ
\author{H.K.\,Tanaka\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}\INSTBJ
\author{H.\,Tanigawa}\INSTCB
\author{V.V.\,Tereshchenko}\INSTIH
\author{N.\,Thamm}\INSTBC
\author{C.\,Touramanis}\INSTFC
\author{N.\,Tran}\INSTCD
\author{T.\,Tsukamoto\thanks{also at J-PARC, Tokai, Japan}}\INSTCB
\author{M.\,Tzanov}\INSTFI
\author{Y.\,Uchida}\INSTEI
\author{M.\,Vagins}\INSTHA\INSTGA
\author{M.\,Varghese}\INSTED
\author{I.\,Vasilyev}\INSTIH
\author{G.\,Vasseur}\INSTI
\author{E.\,Villa}\INSTIE\INSTEG
\author{U.\,Virginet}\INSTBB
\author{T.\,Vladisavljevic}\INSTEH
\author{T.\,Wachala}\INSTDG
\author{S.-i.\,Wada}\INSTCC
\author{D.\,Wakabayashi}\INSTIJ
\author{H.T.\,Wallace}\INSTFB
\author{J.G.\,Walsh}\INSTHB
\author{D.\,Wark}\INSTEH\INSTGG
\author{M.O.\,Wascko}\INSTGG\INSTEH
\author{A.\,Weber}\INSTJC
\author{R.\,Wendell}\INSTCD
\author{M.J.\,Wilking}\INSTJF
\author{C.\,Wilkinson}\INSTII
\author{J.R.\,Wilson}\INSTIF
\author{K.\,Wood}\INSTII
\author{C.\,Wret}\INSTEI
\author{J.\,Xia}\INSTIA
\author{K.\,Yamamoto\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}}\INSTCF
\author{T.\,Yamamoto}\INSTCF
\author{C.\,Yanagisawa\thanks{also at BMCC/CUNY, Science Department, New York, New York, U.S.A.}}\INSTFJ
\author{Y.\,Yang}\INSTGG
\author{T.\,Yano}\INSTBJ
\author{N.\,Yershov}\INSTEB
\author{U.\,Yevarouskaya}\INSTFJ
\author{M.\,Yokoyama\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}}\INSTCH
\author{Y.\,Yoshimoto}\INSTCH
\author{N.\,Yoshimura}\INSTCD
\author{R.\,Zaki}\INSTH
\author{A.\,Zalewska}\INSTDG
\author{J.\,Zalipska}\INSTDF
\author{G.\,Zarnecki}\INSTDG
\author{J.\,Zhang}\INSTB\INSTD
\author{X.Y.\,Zhao}\INSTEF
\author{H.\,Zheng}\INSTFJ
\author{H.\,Zhong}\INSTCC
\author{T.\,Zhu}\INSTEI
\author{M.\,Ziembicki}\INSTDH
\author{E.D.\,Zimmerman}\INSTGB
\author{M.\,Zito}\INSTBB
\author{S.\,Zsoldos}\INSTIF

%\collaboration{The T2K Collaboration}\noaffiliation

==> authorlist_new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% T2K author list generated on Fri Jun 26 00:12:18 2026
% setting: extra = False
%         author list from archive (starting March 14 2025 until July 06 2026)
%         exemption(s) granted to: jacdz,akumar,alexrd,mccauley,mbuizza,munteanu,khomutov,melbaz,ateklu,alpinist,jgrosa,gdmegias,jac,jgm,hmatthias,edatkin,martind,kniewczas,adrienblanchet,mkabirne,morgan_wascko,bdl,vlglagolev,slava,kiseevavi,kurochka,shaykhiev,rubbiaa,laveder,damartin,wilking,ateklu,alpinist,naokiotani,tvngoc,ashida,rgonzjim,jgrosa,gdmegias,jac,jgm,hmatthias,njachowicz,akumar,edatkin,martind,kniewczas,scap,vedantha,fsanchez,evila,amunoz,nova,pdunne,dlast,adrienblanchet,mkabirne,barker,morgan_wascko,bdl,vlglagolev,slava,mtzanov,kutter,lmachado,litchfieldp,egoodman,yyang,kiseevavi,akaboth,kmahtani,dseppala,acraplet,alex,kudenko,oleg,erofeev,kurochka,matveev,shaykhiev,greina,asrivast,nicklatham,nakahata,rubbiaa,laveder,mezzetto,Forza,mgrassi,damartin,denhaff,wilking
% Number of authors = 438
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
\name{\fname{K.} \surname{Abe}}{60}
\name{\fname{S.} \surname{Abe}}{59}
\name{\fname{H.} \surname{Adhikary}}{67}
\name{\fname{R.} \surname{Akutsu}}{15}
\name{\fname{H.} \surname{Alarakia-Charles}}{33}
\name{\fname{Y.I.} \surname{Alj Hakim}}{54}
\name{\fname{S.} \surname{Alonso Monsalve}}{8}
\name{\fname{L.} \surname{Anthony}}{20}
\name{\fname{S.} \surname{Aoki}}{31}
\name{\fname{K.A.} \surname{Apte}}{20}
\name{\fname{T.} \surname{Arai}}{59}
\name{\fname{T.} \surname{Arihara}}{63}
\name{\fname{S.} \surname{Arimoto}}{32}
\name{\fname{Y.} \surname{Asami}}{63}
\name{\fname{Y.} \surname{Asaoka}}{60}
\name{\fname{Y.} \surname{Ashida}}{69}
\name{\fname{E.T.} \surname{Atkin}}{20}
\name{\fname{N.} \surname{Babu}}{37}
\name{\fname{V.} \surname{Baranov}}{38}
\name{\fname{G.J.} \surname{Barker}}{70}
\name{\fname{G.} \surname{Barr}}{46}
\name{\fname{D.} \surname{Barrow}}{46}
\name{\fname{P.} \surname{Bates}}{36}
\name{\fname{L.} \surname{Bathe-Peters}}{46}
\name{\fname{M.} \surname{Batkiewicz-Kwasniak}}{14}
\name{\fname{N.} \surname{Baudis}}{46}
\name{\fname{A.} \surname{Beliakova}}{25}
\name{\fname{V.} \surname{Berardi}}{21}
\name{\fname{L.} \surname{Berns}}{69}
\name{\fname{S.} \surname{Bhattacharjee}}{37}
\name{\fname{A.} \surname{Blanchet}}{57}
\name{\fname{A.} \surname{Blondel}}{57,11}
\name{\fname{L.} \surname{B{\o}e}}{16}
\name{\fname{P.M.M.} \surname{Boistier}}{5}
\name{\fname{S.} \surname{Bolognesi}}{5}
\name{\fname{B.} \surname{Bombin}}{25}
\name{\fname{S.} \surname{Bordoni }}{11}
\name{\fname{S.B.} \surname{Boyd}}{70}
\name{\fname{C.} \surname{Bronner}}{72}
\name{\fname{A.} \surname{Bubak}}{55}
\name{\fname{M.} \surname{Buizza Avanzini}}{35}
\name{\fname{J.A.} \surname{Caballero}}{53}
\name{\fname{N.F.} \surname{Calabria}}{21}
\name{\fname{S.} \surname{Cao}}{19}
\name{\fname{S.} \surname{Cap}}{11}
\name{\fname{D.} \surname{Carabadjac}}{35,}\thanks{also at Universit\'e Paris-Saclay}
\name{\fname{S.L.} \surname{Cartwright}}{54}
\name{\fname{M.P.} \surname{Casado}}{17,}\thanks{also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona, Spain}
\name{\fname{M.G.} \surname{Catanesi}}{21}
\name{\fname{J.} \surname{Chakrani}}{34}
\name{\fname{A.} \surname{Chalumeau}}{57}
\name{\fname{D.} \surname{Cherdack}}{16}
\name{\fname{A.} \surname{Chvirova}}{25}
\name{\fname{J.} \surname{Coleman}}{36}
\name{\fname{G.} \surname{Collazuol}}{23}
\name{\fname{F.} \surname{Cormier}}{65}
\name{\fname{A.A.L.} \surname{Craplet}}{20}
\name{\fname{A.} \surname{Cudd}}{6}
\name{\fname{D.} \surname{D'Ago}}{23}
\name{\fname{C.} \surname{Dalmazzone}}{57}
\name{\fname{T.} \surname{Daret}}{5}
\name{\fname{P.} \surname{Dasgupta}}{17}
\name{\fname{C.} \surname{Davis}}{47}
\name{\fname{Yu.I.} \surname{Davydov}}{38}
\name{\fname{P.} \surname{de Perio}}{28}
\name{\fname{G.} \surname{De Rosa}}{22}
\name{\fname{T.} \surname{Dealtry}}{33}
\name{\fname{C.} \surname{Densham}}{43}
\name{\fname{A.} \surname{Dergacheva}}{25}
\name{\fname{R.} \surname{Dharmapal Banerjee}}{71}
\name{\fname{F.} \surname{Di Lodovico}}{30}
\name{\fname{G.} \surname{Diaz Lopez}}{57}
\name{\fname{S.} \surname{Dolan}}{10}
\name{\fname{D.} \surname{Douqa}}{11}
\name{\fname{T.A.} \surname{Doyle}}{46}
\name{\fname{O.} \surname{Drapier}}{35}
\name{\fname{K.E.} \surname{Duffy}}{46}
\name{\fname{J.} \surname{Dumarchez}}{57}
\name{\fname{P.} \surname{Dunne}}{20}
\name{\fname{K.} \surname{Dygnarowicz}}{68}
\name{\fname{A.} \surname{Eguchi}}{59}
\name{\fname{M.} \surname{El Baz}}{11}
\name{\fname{J.} \surname{Elias}}{49}
\name{\fname{S.} \surname{Emery-Schrenk}}{5}
\name{\fname{G.} \surname{Erofeev}}{25}
\name{\fname{A.} \surname{Ershova}}{35}
\name{\fname{G.} \surname{Eurin}}{5}
\name{\fname{M.} \surname{Fani}}{52}
\name{\fname{D.} \surname{Fedorova}}{25}
\name{\fname{S.} \surname{Fedotov}}{25}
\name{\fname{M.} \surname{Feltre}}{23}
\name{\fname{L.} \surname{Feng}}{32}
\name{\fname{D.} \surname{Ferlewicz}}{57}
\name{\fname{A.J.} \surname{Finch}}{33}
\name{\fname{M.D.} \surname{Fitton}}{43}
\name{\fname{C.} \surname{Forza}}{23}
\name{\fname{M.} \surname{Friend}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{Y.} \surname{Fujii}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{Y.} \surname{Fukuda}}{40}
\name{\fname{N.} \surname{Funayama}}{45}
\name{\fname{Y.} \surname{Furui}}{63}
\name{\fname{A.N.} \surname{Gaci\~no Olmedo}}{57}
\name{\fname{J.} \surname{Garc\'ia-Marcos}}{13}
\name{\fname{A.C.} \surname{Germer}}{47}
\name{\fname{L.} \surname{Giannessi}}{11}
\name{\fname{C.} \surname{Giganti}}{57}
\name{\fname{M.} \surname{Girgus}}{67}
\name{\fname{V.} \surname{Glagolev}}{38}
\name{\fname{M.} \surname{Gonin}}{27}
\name{\fname{R.} \surname{Gonzalez Jimenez}}{53}
\name{\fname{J.} \surname{Gonz\'alez Rosa}}{53}
\name{\fname{E.A.G.} \surname{Goodman}}{12}
\name{\fname{K.} \surname{Gorshanov}}{25}
\name{\fname{P.} \surname{Govindaraj}}{67}
\name{\fname{M.} \surname{Grassi}}{23}
\name{\fname{M.} \surname{Guigue}}{57}
\name{\fname{F.Y.} \surname{Guo}}{42}
\name{\fname{D.R.} \surname{Hadley}}{70}
\name{\fname{S.} \surname{Han}}{32,61}
\name{\fname{D.A.} \surname{Harris}}{73}
\name{\fname{R.J.} \surname{Harris}}{33,43}
\name{\fname{M.} \surname{Hartz}}{65,28}
\name{\fname{T.} \surname{Hasegawa}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{C.M.} \surname{Hasnip}}{10}
\name{\fname{S.} \surname{Hassani}}{5}
\name{\fname{N.C.} \surname{Hastings}}{15}
\name{\fname{K.} \surname{Hayashi}}{32}
\name{\fname{Y.} \surname{Hayato}}{60,28}
\name{\fname{I.} \surname{Heitkamp}}{69}
\name{\fname{D.} \surname{Henaff}}{5}
\name{\fname{Y.} \surname{Hino}}{15}
\name{\fname{K.} \surname{Hiraide}}{60,28}
\name{\fname{J.} \surname{Holeczek}}{55}
\name{\fname{A.} \surname{Holin}}{43}
\name{\fname{T.} \surname{Holvey}}{46}
\name{\fname{N.T.} \surname{Hong Van}}{26}
\name{\fname{T.} \surname{Honjo}}{45}
\name{\fname{M.C.F.} \surname{Hooft}}{13}
\name{\fname{K.} \surname{Hosokawa}}{60}
\name{\fname{R.} \surname{Huang}}{34}
\name{\fname{J.} \surname{Hu}}{32}
\name{\fname{A.K.} \surname{Ichikawa}}{69}
\name{\fname{K.} \surname{Ieki}}{60}
\name{\fname{M.} \surname{Ikeda}}{60}
\name{\fname{T.H.} \surname{Ishida}}{69}
\name{\fname{T.} \surname{Ishida}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Ishitsuka}}{64}
\name{\fname{H.} \surname{Ito}}{31}
\name{\fname{S.} \surname{Ito}}{72}
\name{\fname{A.} \surname{Izmaylov}}{25}
\name{\fname{N.} \surname{Jachowicz}}{13}
\name{\fname{B.} \surname{Jargowsky}}{2}
\name{\fname{S.J.} \surname{Jenkins}}{36}
\name{\fname{C.} \surname{Jes\'us-Valls}}{10}
\name{\fname{M.} \surname{Jia}}{42}
\name{\fname{J.J.} \surname{Jiang}}{42}
\name{\fname{J.Y.} \surname{Ji}}{42}
\name{\fname{T.P.} \surname{Jones}}{33}
\name{\fname{P.} \surname{Jonsson}}{20}
\name{\fname{S.} \surname{Joshi}}{42}
\name{\fname{C.K.} \surname{Jung}}{42,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Kabirnezhad}}{46}
\name{\fname{A.C.} \surname{Kaboth}}{50}
\name{\fname{K.} \surname{Kadota}}{31}
\name{\fname{H.} \surname{Kakuno}}{63}
\name{\fname{A.} \surname{Kamata}}{63}
\name{\fname{J.} \surname{Kameda}}{60}
\name{\fname{S.} \surname{Karpova}}{11}
\name{\fname{V.S.} \surname{Kasturi}}{11}
\name{\fname{Y.} \surname{Kataoka}}{60}
\name{\fname{T.} \surname{Katori}}{30}
\name{\fname{A.} \surname{Kawabata}}{29}
\name{\fname{R.} \surname{Kawabe}}{45}
\name{\fname{Y.} \surname{Kawamura}}{45}
\name{\fname{M.} \surname{Kawaue}}{32}
\name{\fname{E.} \surname{Kearns}}{2,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Khabibullin}}{25}
\name{\fname{N.V.} \surname{Khomutov}}{38}
\name{\fname{A.} \surname{Khotjantsev}}{25}
\name{\fname{T.} \surname{Kikawa}}{32}
\name{\fname{S.} \surname{King}}{30}
\name{\fname{V.} \surname{Kiseeva}}{38}
\name{\fname{J.} \surname{Kisiel}}{55}
\name{\fname{A.} \surname{Klustov\'a}}{20}
\name{\fname{L.} \surname{Kneale}}{54}
\name{\fname{H.} \surname{Kobayashi}}{59}
\name{\fname{S.R.} \surname{Kobayashi}}{69}
\name{\fname{T.} \surname{Kobayashi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{L.} \surname{Koch}}{18}
\name{\fname{S.} \surname{Kodama}}{59}
\name{\fname{M.} \surname{Kolupanova}}{25,}\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}
\name{\fname{A.} \surname{Konaka}}{65}
\name{\fname{L.L.} \surname{Kormos}}{33}
\name{\fname{Y.} \surname{Koshio}}{44,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{K.} \surname{Kowalik}}{41}
\name{\fname{R.} \surname{Kralik}}{30}
\name{\fname{Y.} \surname{Kudenko}}{25,}\thanks{also at Moscow Institute of Physics and Technology (MIPT), Moscow region, Russia and National Research Nuclear University "MEPhI", Moscow, Russia}
\name{\fname{Y.} \surname{Kudo}}{72}
\name{\fname{A.} \surname{Kumar Jha}}{13}
\name{\fname{R.} \surname{Kurjata}}{68}
\name{\fname{V.} \surname{Kurochka}}{25}
\name{\fname{T.} \surname{Kutter}}{37}
\name{\fname{L.} \surname{Labarga}}{1}
\name{\fname{M.} \surname{Lachat}}{49}
\name{\fname{K.} \surname{Lachner}}{8}
\name{\fname{J.} \surname{Lagoda}}{41}
\name{\fname{S.M.} \surname{Lakshmi}}{55}
\name{\fname{M.} \surname{Lamers James}}{70}
\name{\fname{A.} \surname{Langella}}{22}
\name{\fname{D.H.} \surname{Langridge}}{50}
\name{\fname{J.-F.} \surname{Laporte}}{5}
\name{\fname{D.} \surname{Last}}{49}
\name{\fname{N.} \surname{Latham}}{30}
\name{\fname{M.} \surname{Laveder}}{23}
\name{\fname{L.} \surname{Lavitola}}{22}
\name{\fname{M.} \surname{Lawe}}{33}
\name{\fname{A.} \surname{Leclerc}}{5}
\name{\fname{N.} \surname{Lemaire}}{35}
\name{\fname{D.} \surname{Leon Silverio}}{58}
\name{\fname{T.} \surname{Leplumey}}{35}
\name{\fname{S.} \surname{Levorato}}{23}
\name{\fname{S.V.} \surname{Lewis}}{30}
\name{\fname{B.} \surname{Li}}{8}
\name{\fname{C.} \surname{Lin}}{20}
\name{\fname{R.P.} \surname{Litchfield}}{12}
\name{\fname{S.L.} \surname{Liu}}{42}
\name{\fname{W.} \surname{Li}}{46}
\name{\fname{A.} \surname{Longhin}}{23}
\name{\fname{A.} \surname{Lopez Moreno}}{30}
\name{\fname{L.} \surname{Ludovici}}{24}
\name{\fname{X.} \surname{Lu}}{70}
\name{\fname{T.} \surname{Lux}}{17}
\name{\fname{L.N.} \surname{Machado}}{12}
\name{\fname{L.} \surname{Magaletti}}{21}
\name{\fname{K.} \surname{Mahn}}{39}
\name{\fname{K.K.} \surname{Mahtani}}{42}
\name{\fname{S.} \surname{Manly}}{49}
\name{\fname{A.D.} \surname{Marino}}{6}
\name{\fname{D.G.R.} \surname{Martin}}{20}
\name{\fname{D.A.} \surname{Martinez Caicedo}}{58}
\name{\fname{L.} \surname{Martinez}}{17}
\name{\fname{M.} \surname{Martini}}{57,}\thanks{also at IPSA-DRII, France}
\name{\fname{N.} \surname{Mashin}}{25}
\name{\fname{T.} \surname{Matsubara}}{15}
\name{\fname{R.} \surname{Matsumoto}}{62}
\name{\fname{V.} \surname{Matveev}}{25}
\name{\fname{C.} \surname{Mauger}}{47}
\name{\fname{K.} \surname{Mavrokoridis}}{36}
\name{\fname{N.} \surname{McCauley}}{36}
\name{\fname{K.S.} \surname{McFarland}}{49}
\name{\fname{C.} \surname{McGrew}}{42}
\name{\fname{J.} \surname{McKean}}{32}
\name{\fname{A.} \surname{Mefodiev}}{25}
\name{\fname{G.D.} \surname{Megias }}{53}
\name{\fname{L.} \surname{Mellet}}{39}
\name{\fname{C.} \surname{Metelko}}{36}
\name{\fname{M.} \surname{Mezzetto}}{23}
\name{\fname{S.} \surname{Miki}}{60}
\name{\fname{V.} \surname{Mikola}}{12}
\name{\fname{E.W.} \surname{Miller}}{20}
\name{\fname{A.} \surname{Minamino}}{72}
\name{\fname{O.} \surname{Mineev}}{25}
\name{\fname{S.} \surname{Mine}}{60,4}
\name{\fname{J.} \surname{Mirabito}}{2}
\name{\fname{M.} \surname{Miura}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{S.} \surname{Moriyama}}{72}
\name{\fname{P.} \surname{Morrison}}{12}
\name{\fname{Th.A.} \surname{Mueller}}{35}
\name{\fname{D.} \surname{Munford}}{16}
\name{\fname{A.} \surname{Mu\~noz}}{35,27}
\name{\fname{L.} \surname{Munteanu}}{10}
\name{\fname{Y.} \surname{Nagai}}{15}
\name{\fname{T.} \surname{Nakadaira}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{K.} \surname{Nakagiri}}{60}
\name{\fname{M.} \surname{Nakahata}}{60,28}
\name{\fname{Y.} \surname{Nakajima}}{59}
\name{\fname{K.D.} \surname{Nakamura}}{69}
\name{\fname{A.} \surname{Nakano}}{69}
\name{\fname{Y.} \surname{Nakano}}{66}
\name{\fname{S.} \surname{Nakayama}}{60,28}
\name{\fname{T.} \surname{Nakaya}}{32,28}
\name{\fname{K.} \surname{Nakayoshi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{C.E.R.} \surname{Naseby}}{20}
\name{\fname{D.T.} \surname{Nguyen}}{9}
\name{\fname{V.Q.} \surname{Nguyen}}{35}
\name{\fname{K.} \surname{Niewczas}}{35,13}
\name{\fname{S.} \surname{Nishimori}}{59}
\name{\fname{Y.} \surname{Nishimura}}{29}
\name{\fname{Y.} \surname{Noguchi}}{60}
\name{\fname{T.} \surname{Nosek}}{41}
\name{\fname{F.} \surname{Nova}}{43}
\name{\fname{J.C.} \surname{Nugent}}{20}
\name{\fname{H.M.} \surname{O'Keeffe}}{33}
\name{\fname{L.} \surname{O'Sullivan}}{18}
\name{\fname{R.} \surname{Okazaki}}{29}
\name{\fname{W.} \surname{Okinaga}}{59}
\name{\fname{K.} \surname{Okumura}}{61,28}
\name{\fname{T.} \surname{Okusawa}}{45}
\name{\fname{N.} \surname{Onda}}{32}
\name{\fname{N.} \surname{Ospina}}{21}
\name{\fname{L.} \surname{Osu}}{35}
\name{\fname{N.} \surname{Otani}}{32}
\name{\fname{Y.} \surname{Oyama}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{V.} \surname{Paolone}}{48}
\name{\fname{J.} \surname{Pasternak}}{20}
\name{\fname{D.} \surname{Payne}}{36}
\name{\fname{T.P.D.} \surname{Peacock}}{54}
\name{\fname{M.} \surname{Pfaff}}{20}
\name{\fname{L.} \surname{Pickering}}{43}
\name{\fname{J.-B.} \surname{Plan\c{c}on}}{35}
\name{\fname{P.} \surname{Podlaski}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{B.} \surname{Popov}}{57,}\thanks{also at JINR, Dubna, Russia}
\name{\fname{A.J.} \surname{Portocarrero Yrey}}{15}
\name{\fname{M.} \surname{Posiadala-Zezula}}{67}
\name{\fname{Y.S.} \surname{Prabhu}}{67}
\name{\fname{H.} \surname{Prasad}}{71}
\name{\fname{F.} \surname{Pupilli}}{23}
\name{\fname{B.} \surname{Quilain}}{27,35}
\name{\fname{P.T.} \surname{Quyen}}{19,}\thanks{also at the Graduate University of Science and Technology, Vietnam Academy of Science and Technology}
\name{\fname{E.} \surname{Radicioni}}{21}
\name{\fname{B.} \surname{Radics}}{73}
\name{\fname{M.A.} \surname{Ramirez Delgado}}{47}
\name{\fname{R.} \surname{Ramsden}}{30}
\name{\fname{P.N.} \surname{Ratoff}}{33}
\name{\fname{M.} \surname{Reh}}{6}
\name{\fname{G.} \surname{Reina}}{18}
\name{\fname{L.} \surname{Restrepo}}{57}
\name{\fname{C.} \surname{Riccio}}{42}
\name{\fname{D.W.} \surname{Riley}}{12}
\name{\fname{E.} \surname{Rondio}}{41}
\name{\fname{D.} \surname{Ross}}{39}
\name{\fname{S.} \surname{Roth}}{51}
\name{\fname{N.} \surname{Roy}}{73}
\name{\fname{A.} \surname{Rubbia}}{8}
\name{\fname{L.} \surname{Russo}}{57}
\name{\fname{A.} \surname{Rychter}}{68}
\name{\fname{W.} \surname{Saenz}}{57}
\name{\fname{K.} \surname{Sakashita}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{S.} \surname{Samani}}{11}
\name{\fname{F.} \surname{S\'anchez}}{11}
\name{\fname{E.M.} \surname{Sandford}}{36}
\name{\fname{Y.} \surname{Sato}}{64}
\name{\fname{T.} \surname{Schefke}}{37}
\name{\fname{K.} \surname{Scholberg}}{7,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Scott}}{20}
\name{\fname{Y.} \surname{Seiya}}{45,}\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}
\name{\fname{T.} \surname{Sekiguchi}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{H.} \surname{Sekiya}}{60,28,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{M.} \surname{Sekiyama}}{59}
\name{\fname{T.} \surname{Sekiya}}{63}
\name{\fname{D.} \surname{Seppala}}{39}
\name{\fname{D.} \surname{Sgalaberna}}{8}
\name{\fname{A.} \surname{Shaikhiev}}{25}
\name{\fname{M.} \surname{Shiozawa}}{60,28}
\name{\fname{Y.} \surname{Shiraishi}}{44}
\name{\fname{N.} \surname{Shvarev}}{25}
\name{\fname{A.} \surname{Shvartsman}}{25}
\name{\fname{V.} \surname{Siccardi}}{30}
\name{\fname{N.} \surname{Skrobova}}{25}
\name{\fname{K.} \surname{Skwarczynski}}{50}
\name{\fname{D.} \surname{Smyczek}}{51}
\name{\fname{M.} \surname{Smy}}{4}
\name{\fname{J.T.} \surname{Sobczyk}}{71}
\name{\fname{H.} \surname{Sobel}}{4,28}
\name{\fname{F.J.P.} \surname{Soler}}{12}
\name{\fname{A.J.} \surname{Speers}}{33}
\name{\fname{R.} \surname{Spina}}{21}
\name{\fname{A.} \surname{Srivastava}}{18}
\name{\fname{P.} \surname{Stowell}}{54}
\name{\fname{Y.} \surname{Stroke}}{25}
\name{\fname{I.A.} \surname{Suslov}}{38}
\name{\fname{A.} \surname{Suzuki}}{31}
\name{\fname{M.} \surname{Suzuki}}{72}
\name{\fname{S.Y.} \surname{Suzuki}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Tada}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{S.} \surname{Tairafune}}{69}
\name{\fname{A.} \surname{Takeda}}{60}
\name{\fname{Y.} \surname{Takeuchi}}{31,28}
\name{\fname{K.} \surname{Takeya}}{44}
\name{\fname{H.K.} \surname{Tanaka}}{60,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{H.} \surname{Tanigawa}}{29}
\name{\fname{A.} \surname{Teklu}}{42}
\name{\fname{V.V.} \surname{Tereshchenko}}{38}
\name{\fname{N.} \surname{Thamm}}{51}
\name{\fname{C.} \surname{Touramanis}}{36}
\name{\fname{N.} \surname{Tran}}{19}
\name{\fname{T.} \surname{Tsukamoto}}{15,}\thanks{also at J-PARC, Tokai, Japan}
\name{\fname{M.} \surname{Tzanov}}{37}
\name{\fname{Y.} \surname{Uchida}}{20}
\name{\fname{M.} \surname{Vagins}}{28,4}
\name{\fname{M.} \surname{Varghese}}{17}
\name{\fname{I.} \surname{Vasilyev}}{38}
\name{\fname{G.} \surname{Vasseur}}{5}
\name{\fname{E.} \surname{Villa}}{8}
\name{\fname{U.} \surname{Virginet}}{57}
\name{\fname{T.} \surname{Vladisavljevic}}{43}
\name{\fname{T.} \surname{Wachala}}{14}
\name{\fname{S.-i.} \surname{Wada}}{31}
\name{\fname{D.} \surname{Wakabayashi}}{69}
\name{\fname{H.T.} \surname{Wallace}}{54}
\name{\fname{J.G.} \surname{Walsh}}{39}
\name{\fname{D.} \surname{Wark}}{43,46}
\name{\fname{M.O.} \surname{Wascko}}{46,43}
\name{\fname{A.} \surname{Weber}}{18}
\name{\fname{R.} \surname{Wendell}}{32}
\name{\fname{M.J.} \surname{Wilking}}{52}
\name{\fname{C.} \surname{Wilkinson}}{34}
\name{\fname{J.R.} \surname{Wilson}}{30}
\name{\fname{C.} \surname{Winterstein}}{5}
\name{\fname{K.} \surname{Wood}}{34}
\name{\fname{C.} \surname{Wret}}{20}
\name{\fname{J.} \surname{Xia}}{56}
\name{\fname{Z.} \surname{Xie}}{52}
\name{\fname{K.} \surname{Yamamoto}}{45,}\thanks{also at Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP)}
\name{\fname{T.} \surname{Yamamoto}}{45}
\name{\fname{T.} \surname{Yamazumi}}{59}
\name{\fname{C.} \surname{Yanagisawa}}{42,}\thanks{also at BMCC/CUNY, Science Department, New York, New York, U.S.A.}
\name{\fname{Y.} \surname{Yang}}{46}
\name{\fname{T.} \surname{Yano}}{60}
\name{\fname{N.} \surname{Yershov}}{25}
\name{\fname{U.} \surname{Yevarouskaya}}{42}
\name{\fname{M.} \surname{Yokoyama}}{59,}\thanks{affiliated member at Kavli IPMU (WPI), the University of Tokyo, Japan}
\name{\fname{Y.} \surname{Yoshimoto}}{59}
\name{\fname{N.} \surname{Yoshimura}}{32}
\name{\fname{R.} \surname{Zaki}}{73}
\name{\fname{A.} \surname{Zalewska}}{14}
\name{\fname{J.} \surname{Zalipska}}{41}
\name{\fname{G.} \surname{Zarnecki}}{14}
\name{\fname{J.} \surname{Zhang}}{65,3}
\name{\fname{X.Y.} \surname{Zhao}}{8}
\name{\fname{H.} \surname{Zheng}}{42}
\name{\fname{H.} \surname{Zhong}}{31}
\name{\fname{T.} \surname{Zhu}}{20}
\name{\fname{M.} \surname{Ziembicki}}{68}
\name{\fname{E.D.} \surname{Zimmerman}}{6}
\name{\fname{M.} \surname{Zito}}{57}
\name{\fname{S.} \surname{Zsoldos}}{30}
}

\address{
\affil{1}{University Autonoma Madrid, Department of Theoretical Physics, 28049 Madrid, Spain}
\affil{2}{Boston University, Department of Physics, Boston, Massachusetts, U.S.A.}
\affil{3}{University of British Columbia, Department of Physics and Astronomy, Vancouver, British Columbia, Canada}
\affil{4}{University of California, Irvine, Department of Physics and Astronomy, Irvine, California, U.S.A.}
\affil{5}{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affil{6}{University of Colorado at Boulder, Department of Physics, Boulder, Colorado, U.S.A.}
\affil{7}{Duke University, Department of Physics, Durham, North Carolina, U.S.A.}
\affil{8}{ETH Zurich, Institute for Particle Physics and Astrophysics, Zurich, Switzerland}
\affil{9}{VNU University of Science, Vietnam National University, Hanoi, Vietnam}
\affil{10}{CERN European Organization for Nuclear Research, CH-1211 Gen\'eve 23, Switzerland}
\affil{11}{University of Geneva, Section de Physique, DPNC, Geneva, Switzerland}
\affil{12}{University of Glasgow, School of Physics and Astronomy, Glasgow, United Kingdom}
\affil{13}{Ghent University, Department of Physics and Astronomy, Proeftuinstraat 86, B-9000 Gent, Belgium}
\affil{14}{H. Niewodniczanski Institute of Nuclear Physics PAN, Cracow, Poland}
\affil{15}{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki, Japan}
\affil{16}{University of Houston, Department of Physics, Houston, Texas, U.S.A.}
\affil{17}{Institut de Fisica d'Altes Energies (IFAE) - The Barcelona Institute of Science and Technology, Campus UAB, Bellaterra (Barcelona) Spain}
\affil{18}{Institut f\"ur Physik, Johannes Gutenberg-Universit\"at Mainz, Staudingerweg 7, 55128 Mainz, Germany}
\affil{19}{Institute For Interdisciplinary Research in Science and Education (IFIRSE), ICISE, Quy Nhon, Vietnam}
\affil{20}{Imperial College London, Department of Physics, London, United Kingdom}
\affil{21}{INFN Sezione di Bari and Universit\`a e Politecnico di Bari, Dipartimento Interuniversitario di Fisica, Bari, Italy}
\affil{22}{INFN Sezione di Napoli and Universit\`a di Napoli, Dipartimento di Fisica, Napoli, Italy}
\affil{23}{INFN Sezione di Padova and Universit\`a di Padova, Dipartimento di Fisica, Padova, Italy}
\affil{24}{INFN Sezione di Roma and Universit\`a di Roma ``La Sapienza'', Roma, Italy}
\affil{25}{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow, Russia}
\affil{26}{International Centre of Physics, Institute of Physics (IOP), Vietnam Academy of Science and Technology (VAST), 10 Dao Tan, Ba Dinh, Hanoi, Vietnam}
\affil{27}{ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}
\affil{28}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, University of Tokyo, Kashiwa, Chiba, Japan}
\affil{29}{Keio University, Department of Physics, Kanagawa, Japan}
\affil{30}{King's College London, Department of Physics, Strand, London WC2R 2LS, United Kingdom}
\affil{31}{Kobe University, Kobe, Japan}
\affil{32}{Kyoto University, Department of Physics, Kyoto, Japan}
\affil{33}{Lancaster University, Physics Department, Lancaster, United Kingdom}
\affil{34}{Lawrence Berkeley National Laboratory, Berkeley, California, U.S.A.}
\affil{35}{Ecole Polytechnique, IN2P3-CNRS, Laboratoire Leprince-Ringuet, Palaiseau, France}
\affil{36}{University of Liverpool, Department of Physics, Liverpool, United Kingdom}
\affil{37}{Louisiana State University, Department of Physics and Astronomy, Baton Rouge, Louisiana, U.S.A.}
\affil{38}{Joint Institute for Nuclear Research, Dubna, Moscow Region, Russia}
\affil{39}{Michigan State University, Department of Physics and Astronomy,  East Lansing, Michigan, U.S.A.}
\affil{40}{Miyagi University of Education, Department of Physics, Sendai, Japan}
\affil{41}{National Centre for Nuclear Research, Warsaw, Poland}
\affil{42}{State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, U.S.A.}
\affil{43}{STFC, Rutherford Appleton Laboratory, Harwell Oxford,  and  Daresbury Laboratory, Warrington, United Kingdom}
\affil{44}{Okayama University, Department of Physics, Okayama, Japan}
\affil{45}{Osaka Metropolitan University, Department of Physics, Osaka, Japan}
\affil{46}{Oxford University, Department of Physics, Oxford, United Kingdom}
\affil{47}{University of Pennsylvania, Department of Physics and Astronomy,  Philadelphia, Pennsylvania, U.S.A.}
\affil{48}{University of Pittsburgh, Department of Physics and Astronomy, Pittsburgh, Pennsylvania, U.S.A.}
\affil{49}{University of Rochester, Department of Physics and Astronomy, Rochester, New York, U.S.A.}
\affil{50}{Royal Holloway University of London, Department of Physics, Egham, Surrey, United Kingdom}
\affil{51}{RWTH Aachen University, III. Physikalisches Institut, Aachen, Germany}
\affil{52}{School of Physics and Astronomy, University of Minnesota, Minneapolis, Minnesota, U.S.A.}
\affil{53}{Departamento de F\'isica At\'omica, Molecular y Nuclear, Universidad de Sevilla, 41080 Sevilla, Spain}
\affil{54}{University of Sheffield, School of Mathematical and Physical Sciences, Sheffield, United Kingdom}
\affil{55}{University of Silesia, Institute of Physics, Katowice, Poland}
\affil{56}{SLAC National Accelerator Laboratory, Stanford University, Menlo Park, California, U.S.A.}
\affil{57}{Sorbonne Universit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}
\affil{58}{South Dakota School of Mines and Technology, 501 East Saint Joseph Street, Rapid City, SD 57701, United States}
\affil{59}{University of Tokyo, Department of Physics, Tokyo, Japan}
\affil{60}{University of Tokyo, Institute for Cosmic Ray Research, Kamioka Observatory, Kamioka, Japan}
\affil{61}{University of Tokyo, Institute for Cosmic Ray Research, Research Center for Cosmic Neutrinos, Kashiwa, Japan}
\affil{62}{Institute of Science Tokyo, Department of Physics, Tokyo}
\affil{63}{Tokyo Metropolitan University, Department of Physics, Tokyo, Japan}
\affil{64}{Tokyo University of Science, Faculty of Science and Technology, Department of Physics, Noda, Chiba, Japan}
\affil{65}{TRIUMF, Vancouver, British Columbia, Canada}
\affil{66}{University of Toyama, Faculty of Science, Toyama, Japan}
\affil{67}{University of Warsaw, Faculty of Physics, Warsaw, Poland}
\affil{68}{Warsaw University of Technology, Institute of Radioelectronics and Multimedia Technology, Warsaw, Poland}
\affil{69}{Tohoku University, Faculty of Science, Department of Physics, Miyagi, Japan}
\affil{70}{University of Warwick, Department of Physics, Coventry, United Kingdom}
\affil{71}{Wroclaw University, Faculty of Physics and Astronomy, Wroclaw, Poland}
\affil{72}{Yokohama National University, Department of Physics, Yokohama, Japan}
\affil{73}{York University, Department of Physics and Astronomy, Toronto, Ontario, Canada}
}

==> gundam.tex <==
%666\section{Validation of GUNDAM as ND fitter}
%\label{sec:GUNDAM}
%A comparison of the result of the fit to ND280 data of GUNDAM, BANFF, and MaCh3 is shown in \cref{fig:oa2023data_GMB_flux} and \cref{fig:oa2023data_GMB_xsec}. In general, the differences are minimal and any differences are known implementation differences between the fitters and are expected. It should be noted in these comparisons that for the cross-section parameters that are fixed in the fit, the error band and the mean value for GUNDAM are not added in the plots. Similarly, the differences in the parameter 2p2h\_shape\_C\_np is due to it being mirrored around -1 and the actual value passed to the far detector fitter agrees with MaCh3.  The full details of the GUNDAM analysis and validations compared to the BANFF can be found in \cite{TN458}.


%\begin{figure}[htbp]
%    \centering
%    \foreach \a in {2,...,5}
%    {
%        \includegraphics[page=\a, width=0.45\textwidth]{ND280_figs/MBG_comparison.pdf}
%    }
%    \caption{Comparison between BANFF GUNDAM and MaCh3 in terms of the cross-section parameters obtained from the data fit. The flux parameters errors are represented by black error bars for BANFF, blue error bands for GUNDAM, and yellow error bands for MaCh3. The blue, red, and black points correspond to the post-fit central values of GUNDAM, MaCh3, and BANFF, respectively.}
%    \label{fig:oa2023data_GMB_flux}
%\end{figure}
%
%\begin{figure}[htbp]
%   \centering
%   \foreach \a in {7,...,15}
%    {
%        \includegraphics[page=\a, width=0.38\textwidth]{ND280_figs/MBG_comparison.pdf}
%    }
%    \caption{Comparison between BANFF GUNDAM and MaCh3 in terms of the cross-section parameters obtained from the data fit. The cross-section parameter errors are represented by black error bars for BANFF, blue error bands for GUNDAM, and yellow error bands for MaCh3. The blue, red, and black points correspond to the post-fit central values of GUNDAM, MaCh3, and BANFF, respectively.}
%    \label{fig:oa2023data_GMB_xsec}
%\end{figure}



%Even though for OA23 the official ND fitter is still BANFF, the new GUNDAM fitter~\cite{TN458} is reaching its final steps of validation. As part of this analysis, an Asimov A22 sensitivity study was performed within P-Theta, using the GUNDAM OA23 ND data fit output. The full comparison is given in the P-Theta T2K-TN-461\cite{TN461} in Sec. 4.3. The relative difference in the predicted event rates is at a maximum of 0.12\% (for RHC 1Re). The differences within the contours obtained with BANFF and GUNDAM are negligible for our analysis sensitivity. An example taken from~\cite{TN461} is given in \cref{fig:GUNDAM_BANFF_PTheta} for \dcp~ and $\Delta m^2_{23}$ vs $\sin^2\theta_{23}$.
%\begin{figure}
%    \centering
%\includegraphics[width=0.5\textwidth]{Pthetasensi_figs/GUNDAM_figs/contour_dCP.pdf}%
%\includegraphics[width=0.5\textwidth]{Pthetasensi_figs/GUNDAM_figs/contour_dm2_32_th23.pdf}
%    \caption{P-Theta sensitivity plots at A22, with reactor constraints and with systematic parameters, comparison of the BANFF (orange) and GUNDAM (blue) outputs.}
%    \label{fig:GUNDAM_BANFF_PTheta}
%\end{figure}


==> old_ptephys_v1.tex <==
\newcommand\classname{styled}
\newcommand\lastmodifieddate{2004/07/05}
\newcommand\versionnumber{0.1}

\NeedsTeXFormat{LaTeX2e}[2000/06/01]
\ProvidesClass{ptephy_v1}

\setlength{\paperheight}{279truemm}
\setlength{\paperwidth}{216truemm}

\newif\if@numberedref \@numberedreftrue
\newif\if@endproofbox \@endproofboxtrue
\newif\ifcopyedit
\newif\ifunarticle
\newif\ifletterpaper
\newif\ifpreview
\newif\ifcolorfigs
\newif\ifendnotes
\newif\iffproof\fprooffalse %to make surname in magenta color
\newif\iffunding\fundingfalse % to make magenta color in funding text
\newif\ifnum@bib\num@bibtrue
\newif\iferratum
\newif\ifpteplogo
\newif\ifpreprint

\DeclareOption{erratum}{\erratumtrue}
\DeclareOption{letterpaper}{\letterpapertrue}
\DeclareOption{copyedit}{\copyedittrue}
\DeclareOption{preview}{\previewtrue}
\DeclareOption{draft}{\PassOptionsToPackage{draft}{graphicx}}
\DeclareOption{a3paper}{\PassOptionsToPackage{a3}{crop}}
\DeclareOption{centre}{\PassOptionsToPackage{center}{crop}}
\DeclareOption{info}{\PassOptionsToPackage{info}{crop}}
\DeclareOption{noinfo}{\PassOptionsToPackage{noinfo}{crop}}
\DeclareOption{numbered}{\global\@numberedreftrue}
\DeclareOption{named}{\global\@numberedreffalse}
\DeclareOption{noproofbox}{\global\@endproofboxfalse}
\DeclareOption{proofbox}{\global\@endproofboxtrue}
\DeclareOption{courier}{\def\verbatim@font{\normalfont\ttfamily}}
\DeclareOption{times}{\def\verbatim@font{\normalfont\rmfamily}}
\DeclareOption{bookreview}{\global\unarticletrue}
\DeclareOption{fproof}{\fprooftrue}
\DeclareOption{funding}{\fundingtrue}
\DeclareOption{endnotes}{\global\endnotestrue}
\DeclareOption{colorfigs}{\colorfigstrue}
\DeclareOption{numbib}{\num@bibtrue}
\DeclareOption{nonumbib}{\num@bibfalse}
\DeclareOption{pteplogo}{\pteplogotrue}
\DeclareOption{preprint}{\preprinttrue}
%\DeclareOption{preprint}{\InputIfFileExists{ptephy.clo}{\typeout{-----Reading ptephy.clo-----}}%
%{\ClassError{PTPTeX}{This class file needs the file named ``ptephy.clo'' in case the option `preprint' is specified.}{Please ensure the file is exist in proper location.}}}


\ExecuteOptions{a4paper,centre,info,proofbox}

\ProcessOptions

\RequirePackage{graphicx,array,amsthm,amsmath,amssymb,amsfonts,endnotes,rotating}

\ifendnotes
\RequirePackage{endnotes}
\let\footnote\endnote
\fi

\usepackage{multicol}

\usepackage{comment}
\usepackage{color}
\specialcomment{authorquery}{\begingroup\textcolor{red}}{\endgroup}

\newcommand\preprintnumber[2][30mm]{\gdef\@preprtnumwidth{#1}\gdef\@preprtnum{#2}}

% Not sure if needed.
\newcommand\@ptsize{0}

% Set twoside printing
\@twosidetrue

% Marginal notes are on the outside edge
\@mparswitchtrue

% Default font sizes
\def\normalsize{%
  \@setfontsize\normalsize{11\p@}{15\p@}%
  \abovedisplayskip 8\p@ \@plus 3\p@ \@minus4\p@
  \abovedisplayshortskip 2\p@ \@plus 3\p@ \@minus1\p@
  \belowdisplayshortskip 5\p@ \@plus 3\p@ \@minus2\p@
  \belowdisplayskip \abovedisplayskip
  \let\@listi\@listI}
\normalsize
\let\@bls\baselineskip

\def\small{%
  \@setfontsize\small{9\p@}{11\p@}%
  \abovedisplayskip 6\p@ \@plus1\p@ \@minus1\p@
  \abovedisplayshortskip 3\p@ \@plus 2\p@ \@minus1\p@
  \belowdisplayshortskip 2\p@ \@plus 1\p@ \@minus1\p@
  \def\@listi{\leftmargin\leftmargini
              \listparindent \parindent
              \topsep 6\p@ \@plus2\p@ \@minus1\p@
              \parsep \z@ \itemsep \z@}%
  \belowdisplayskip \abovedisplayskip}

\def\footnotesize{%
 \@setfontsize\footnotesize{8\p@}{10\p@}%
  \abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
  \abovedisplayshortskip \z@ \@plus \p@
  \belowdisplayshortskip 1\p@ \@plus2\p@ \@minus2\p@
  \def\@listi{\leftmargin\leftmargini
              \listparindent 1em
              \topsep 5\p@ \@plus 2\p@ \@minus 1\p@
              \parsep \z@ \itemsep \z@}%
  \belowdisplayskip \abovedisplayskip}

\def\scriptsize{\@setfontsize\scriptsize{7\p@}{9\p@}}
\def\tiny{\@setfontsize\tiny{6\p@}{7\p@}}
\def\little{\@setfontsize\little{5\p@}{6\p@}}
\def\large{\@setfontsize\large{12\p@}{14\p@}}
\def\Large{\@setfontsize\Large{14\p@}{16\p@}}
\def\LARGE{\@setfontsize\LARGE{16\p@}{18\p@}}
\def\huge{\@setfontsize\huge{24\p@}{26\p@}}
\def\Huge{\@setfontsize\Huge{25\p@}{27\p@}}

\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}

% Line spacing
\setlength\lineskip{1\p@}
\setlength\normallineskip{1\p@}
\renewcommand\baselinestretch{}

% Paragraph dimensions and inter-para spacing
\setlength\parskip{0\p@}
\setlength\parindent{9pt}

% Set inter-para skips
\setlength\smallskipamount{3\p@ \@plus 1\p@ \@minus 1\p@}
\setlength\medskipamount{6\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\bigskipamount{12\p@ \@plus 4\p@ \@minus 4\p@}

% Page break penalties
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301

% Disallow widows and orphans
\clubpenalty 10000
\widowpenalty 10000

% Disable page breaks before equations, allow pagebreaks after
% equations and discourage widow lines before equations.
\displaywidowpenalty 100
\predisplaypenalty   10000
\postdisplaypenalty  2500

% Allow breaking the page in the middle of a paragraph
\interlinepenalty 0

% Disallow breaking the page after a hyphenated line
\brokenpenalty 10000

% Hyphenation; don't split words into less than three characters
\lefthyphenmin=3
\righthyphenmin=3

%
% Set page layout dimensions
%
\setlength\headheight{7\p@}          % height of running head
\setlength\topmargin{2.3pc}            % top margin 3pc, 9pt
\addtolength\topmargin{8\p@}         %
\addtolength\topmargin{-1in}         % subtract out the 1 inch driver margin
%% \addtolength\topmargin{-\headheight} %  and the running head

\setlength\topskip{8\p@}            % height of first line of text%% {10\p@}
\setlength\headsep{30\p@}          % space below running head --
\addtolength\headsep{-\topskip}      %   base to base with first line of text

\setlength\footskip{18\p@}           % space above footer line
\setlength\maxdepth{.5\topskip}      % pages can be short or deep by half a line?

\setlength\textwidth{36.4pc}%41.4           % text measure excluding margins
%\addtolength\textwidth{9.89\p@}      % -> textwidth of 30pc, 9.89pt!

\setlength\textheight{44\@bls}       % text height of 48pc,
\addtolength\textheight{\topskip}    %  - including first line of text

% Set the margins
\setlength\marginparsep{16\p@} \setlength\marginparpush{8\p@}
\setlength\marginparwidth{4.1pc}

\setlength\oddsidemargin{88pt}%
\addtolength\oddsidemargin{-1in}    % subtract out the 1 inch driver margin
\setlength\@tempdima{\paperwidth}
\addtolength\@tempdima{-\textwidth}
\addtolength\@tempdima{-88pt}
\setlength\evensidemargin{\@tempdima}
\addtolength\evensidemargin{-1in}

\setlength\columnsep{18\p@}          % space between columns for double-column text
\setlength\columnseprule{0\p@}      % width of rule between two columns

% Footnotes
\setlength\footnotesep{0\p@}     % space between footnotes
% space between text and footnote
\setlength{\skip\footins}{24\p@ \@plus 6\p@ \@minus 1\p@}

% Float placement parameters

% The total number of floats that can be allowed on a page.
\setcounter{totalnumber}{10}
% The maximum number of floats at the top and bottom of a page.
\setcounter{topnumber}{5}
\setcounter{bottomnumber}{5}
% The maximum part of the top or bottom of a text page that can be
% occupied by floats. This is set so that at least four lines of text
% fit on the page.
\renewcommand\topfraction{.921}
\renewcommand\bottomfraction{.921}
% The minimum amount of a text page that must be occupied by text.
% This should accomodate four lines of text.
\renewcommand\textfraction{.079}
% The minimum amount of a float page that must be occupied by floats.
\renewcommand\floatpagefraction{.887}

% The same parameters repeated for double column output
\renewcommand\dbltopfraction{.88}
\renewcommand\dblfloatpagefraction{.88}

% Space between floats
\setlength\floatsep    {18\p@ \@plus 2\p@ \@minus 2\p@}
% Space between floats and text
\setlength\textfloatsep{20\p@ \@plus 2\p@ \@minus 4\p@}
% Space above and below an inline figure
\setlength\intextsep   {18\p@ \@plus 2\p@ \@minus 2\p@}

% For double column floats
\setlength\dblfloatsep    {12\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\dbltextfloatsep{20\p@ \@plus 2\p@ \@minus 4\p@}

% Space left at top, bottom and inbetween floats on a float page.
\setlength\@fptop{0\p@}         % no space above float page figures
\setlength\@fpsep{12\p@ \@plus 2fil}
\setlength\@fpbot{0\p@ \@plus 1fil}

% The same for double column
\setlength\@dblfptop{0\p@}
\setlength\@dblfpsep{12\p@ \@plus 1fil}
\setlength\@dblfpbot{0\p@ \@plus 2fil}

\AtEndDocument{%
\ifendnotes%
\theendnotes%
\fi%
   \message{Setting LastPage}%
   \clearpage\lastpage@putlabel%
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Article Identification %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@default@journal@title{Journal Title}
\let\@journal@title\@default@journal@title
\def\month@info{Month~}
\def\artid@info{00000}
\def\year@info{\the\year}
\def\eyear@info{00}
\def\vol@info{00}
\def\issue@info{00}
\def\@print@issn{0000-0000}
\def\@online@issn{0000-0000}
\def\ceby@info{}
\def\qaby@info{}
\def\mcby@info{}
\newcommand{\page@extent@info}{%
  \thepage--\pageref{LastPage}}
\gdef\pap#1{\gdef\@pap{#1}}\pap{}

\newcommand{\totalpage}{%
  \pageref{LastPage}}

\gdef\doi@string{0000000000}

\def\@doi@fixed@field{}
\def\@doi@variable@field{00000000000000000000}

\gdef\backack#1{\gdef\@backack{#1}}\backack{}

% Article information user commands
\def\Year#1{\gdef\year@info{#1}}
\def\ErrYear#1{\gdef\eyear@info{#1}}
\def\Vol#1{\gdef\vol@info{#1}}
\def\Issue#1{\gdef\issue@info{#1}}
\def\Month#1{\gdef\month@info{#1}}
\def\artid#1{\gdef\artid@info{#1}}
\def\ceby#1{\gdef\ceby@info{#1}}
\def\qaby#1{\gdef\qaby@info{#1}}
\def\mcby#1{\gdef\mcby@info{#1}}
\newcommand\DOI[2][\@doi@fixed@field]{%
  \gdef\@doi@variable@field{#1}%
  \setDOI{#1}{#2}}
\newcommand{\setDOI}[2]{%
  \gdef\doi@string{#1#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%% Page Styles %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ps@titlepage{%
\vskip-1.9pt
  \addtolength\headsep{3pt}      %   base to base with first line of text
  \def\@evenfoot{}
 \def\@evenhead{\fontsize{10}{12}\selectfont \titlepageheadline}
 \def\@oddhead{\fontsize{10}{12}\selectfont \titlepageheadline}%
  \def\@oddfoot{\titlepagefootline}%%
  \def\authormark##1{\def\leftmark{##1}}%
  \def\titlemark##1{\markboth{##1}{##1}}}

\def\ps@headings{%
  \def\@oddfoot{\vbox{\vskip16pt\hbox to \textwidth{}
  \hbox to \textwidth{\fontsize{10}{12}\selectfont\hfill \thepage/\pageref{LastPage}\hfill}}}%
  \def\@evenfoot{\vbox{\vskip16pt\hbox to \textwidth{}
  \hbox to \textwidth{\fontsize{10}{12}\selectfont\hfill\thepage/\pageref{LastPage}\hfill}}}%
  \def\@oddhead{\let\etal=\tetal{\vbox{\hbox to \textwidth{{\fontsize{10}{12}\selectfont\rightmark\hfill}}\vskip2pt
  \hbox to \textwidth{\rule{\textwidth}{.5pt}}
  }}}%
  \def\@evenhead{\let\etal=\tetal{\vbox{\hbox to \textwidth{{\fontsize{10}{12}\selectfont\leftmark\hfill}}\vskip2pt
  \hbox to \textwidth{\rule{\textwidth}{.5pt}}
  }}}%
  \def\authormark##1{\def\leftmark{##1}}%
  \def\titlemark##1{\markboth{##1}{##1}}}

\def\ps@myheadings{%
  \let\@oddfoot\@empty%
  \let\@evenfoot\@empty%
  \def\@evenhead{\hfil}%
  \def\@oddhead{\hfil}%
  \def\authormark##1{\def\leftmark{##1}}%
  \def\titlemark##1{\markboth{##1}{##1}}}

\newcommand{\titlepageheadline}{%
  \vbox to 2\baselineskip{%
    \hbox to \textwidth{%
      {\raisebox{3.85pt}{\parbox{79.5\p@}{%
\hbox to 3.3pc{\vbox{\begin{minipage}[t]{2.5pc}\includegraphics{Pepthy_logo}\hspace*{1.5pc}\end{minipage}}}}}}
      \parbox{396\p@}{\hfill%                   <- textwidth minus logo width
  \fontsize{10}{12}\selectfont
        {Prog. Theor. Exp. Phys.} {\bf \year@info},\ \artid@info\ (\pageref{LastPage} pages)\ \\
        \hspace*{\fill} DOI: 10.1093$/$ptep/\doi@string}\\[-3.5pt]
}\vspace*{6.25pt}
\hbox to \textwidth{\rule{\textwidth}{.5pt}}
%\rule{\textwidth}{.5pt}
}}

\def\today{\number\day/\ifcase\month\or
 1\or 2\or 3\or 4\or 5\or 6\or 7\or 8\or 9\or 10\or 11\or 12\fi/\number\year}

\newcommand{\titlepagefootline}{%
  \fontsize{6.5}{8.5}\selectfont
  \vbox{\vspace*{12pt}
\hbox to 436.9pt{\hspace*{-1.9pt}\hspace*{-1.4pt}}
\hbox to \textwidth{$\copyright$ The Author(s) 2012. Published by Oxford University Press on behalf of the Physical Society of Japan.\hfill}
\hbox to \textwidth{This is an Open Access article distributed under the terms of the Creative Commons Attribution License\hfill}
\hbox to \textwidth{(http://creativecommons.org/licenses/by-nc/3.0), which permits unrestricted use,\hfill}
\hbox to \textwidth{distribution, and reproduction in any medium, provided the original work is properly cited.\hfill}
 \vspace*{12pt}}}

\setcounter{footnote}{1}
\renewcommand\thefootnote{\@fnsymbol\c@footnote}

% Counters
\newcounter{part}
\newcounter{section}
\newcounter{subsection}[section]
\newcounter{subsubsection}[subsection]
\newcounter{paragraph}[subsubsection]
\newcounter{subparagraph}[paragraph]
\newcounter{refsection}[section]
\newcounter{acksection}[section]
\newcounter{scheme}

% Form of the numbers
\newcommand\thepage{\arabic{page}}
\renewcommand\thesection{\arabic{section}}
\renewcommand\thesubsection{{\thesection.\arabic{subsection}}}
\renewcommand\thesubsubsection{{\thesubsection.\arabic{subsubsection}}}
\renewcommand\theparagraph{\thesubsubsection.\arabic{paragraph}}
\renewcommand\thesubparagraph{\theparagraph.\arabic{subparagraph}}
\renewcommand\theequation{\arabic{equation}}

% Form of the words
\newcommand\contentsname{Contents}
\newcommand\guestname{GUEST EDITORS}
\newcommand\listfigurename{List of Figures}
\newcommand\listtablename{List of Tables}
\newcommand\partname{Part}
\newcommand\appendixname{Appendix}
\newcommand\abstractname{Abstract}
\newcommand\refname{References}
\newcommand\bibname{{{References}}}
\newcommand\normsname{Norms}
\newcommand\indexname{Index}
\newcommand\schemename{Scheme}
\newcommand\tablename{Table}

% Clearemptydoublepage should really clear the running heads too
\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}

\def\and{\MakeLowercase{and}\space\ignorespaces}

% Ifs for titling commands
\newif\if@supertitle@provided \@supertitle@providedfalse
\newif\if@specialissue@provided \@specialissue@providedfalse
\newif\if@guesteditor@provided \@guesteditor@providedfalse
\newif\if@subtitle@provided \@subtitle@providedfalse
\newif\if@date@provided \@date@providedfalse
\newif\if@dedi@provided \@dedi@providedfalse
\newif\if@classification@provided \@classification@providedfalse
\newif\if@abstract@provided \@abstract@providedfalse %%5/7/2004
\newif\if@keywords@provided \@keywords@providedfalse
\newif\if@subjectindex@provided \@subjectindex@providedfalse

\def\keywordsname{Keywords}
\def\subindexname{Subject Index}

\def\address#1{\gdef\@address{#1}}\address{}
\def\author#1{\gdef\@author{#1}}\author{}
\def\date#1{\gdef\@date{#1}\global\@date@providedtrue}
\def\dedi#1{\def\@dedi{#1}\global\@dedi@providedtrue}
\def\keywords#1{\gdef\@keywords{#1}\global\@keywords@providedtrue}
\def\subjectindex#1{\gdef\@subjectindex{#1}\global\@subjectindex@providedtrue}
\def\subtitle#1{\def\@subtitle{{#1}}\global\@subtitle@providedtrue}
\def\supertitle#1{\def\@supertitle{{\noindent #1}}\global\@supertitle@providedtrue}
\def\specialissue#1{\def\@specialissue{{\noindent SPECIAL ISSUE:~#1}}\global\@specialissue@providedtrue}
\def\guesteditor#1{\def\@guesteditor{{\noindent \guestname:~#1}}\global\@guesteditor@providedtrue}
\def\@abbreviations{}
\def\@classification{}
\newcommand\classification[2][Jel Classification]{%
     \global\@classification@providedtrue
     \gdef\@classification{{\leftskip=2pc\rightskip=2pc \noindent\textit{#1}:\enskip #2\par}}}

\newbox\@abstractbox%
\newenvironment{abstract}{\leftskip=4.7pc\rightskip=0pc\global\@abstract@providedtrue%%% 5/7/2004
  \global\setbox\@abstractbox\vbox\bgroup\fontsize{10}{12}\selectfont%
  \@hangfrom{\@afterindentfalse\@afterheading}}{\par\egroup}%

\def\@fnsymbol#1{\ifcase#1\or *\or \dagger\or \ddagger\or
    \S\or \P\or \|\or **\or \dagger\dagger
    \or \ddagger\ddagger \else\@ctrerr\fi}


\mathchardef\Register="20AE%
\mathchardef\ter="099%
\def\titdagger{\hbox{$\dagger$}}
\def\titddagger{\hbox{$\ddagger$}}
\def\titS{\hbox{$\S$}}
\def\titP{\hbox{$\P$}}

%% Reimplement Titling Layout
\newcommand\maketitle{\par
   \begingroup
\renewcommand{\@fnsymbol}[1]{\ifcase##1\or \hbox{*}\or \titdagger\or \titddagger\or
    \titS\or \titP\or $\|$\or \hbox{**}\or \titdagger\titdagger
    \or \titddagger\titddagger \else\@ctrerr\fi}
    \thispagestyle{titlepage}%
    \setcounter{footnote}{1}
    \renewcommand\thefootnote{\textsuperscript{\@fnsymbol\c@footnote}}%
    \def\@makefnmark{\rm\@thefnmark}%
    \long\def\@makefntext##1{%\noindent
      {${\@thefnmark}$}{##1}}%
    \global\@topnum\z@   % Prevents figures from going at top of page.
    \@maketitle
      \markboth{\@shortauthorlist}{\@shorttitle}
    \@thanks
  \endgroup
  \@afterindentfalse
  \@afterheading
  \setcounter{footnote}{0}%
  \global\let\maketitle\relax
  \global\let\@maketitle\relax}

\usepackage{authblk-TI}

\def\@maketitle{%
  \vspace*{2.5pt}%
\let\footnote\thanks
     \if@supertitle@provided%
 \vskip17pt
       {\fontfamily{\sfdefault}\fontsize{12}{14}\bfseries\selectfont\@supertitle\par%
 \vskip8pt}
    \else
       \vskip14pt%
     \fi
  \begingroup
    {\fontsize{20}{20}\fontseries{b}\selectfont\raggedright
      \mathversion{bold}%
      {\@title}%
      \par}%
     \if@subtitle@provided%
       \vspace{12.5\p@}%
       {\fontsize{12}{14}\fontseries{b}\selectfont\@subtitle\par
        %\vspace{1.5\p@}%
        }%
     \else
       \vspace{0\p@}%
%       \vspace{12.5\p@}%
     \fi
    \vspace{14pt}%
    {\fontsize{12}{14}\selectfont\raggedright
      \begingroup
      {\noindent\@author}%
    \vspace{6\p@}%
      \endgroup
      \par}%
    {\fontsize{10}{12}\fontshape{it}\selectfont\raggedright{\@address}\par}%
 \vspace{8\p@}%
     \if@date@provided%
         {\noindent\fontsize{9}{11}\fontshape{m}\selectfont{\@date\kern1pt}\par}%
\vspace{8.5\p@}%%
     \else
    \vspace{0\p@}%
     \fi
     \if@dedi@provided%
       {\fontsize{9}{10}\fontseries{rm}\selectfont{\@dedi}\par
        \vspace{18.25\p@}}%
     \else%
       \vspace{0\p@}%
     \fi%
\endgroup%
\if@abstract@provided%
    \vskip.1pt%
      {\hbox to 448.6pt{\hskip4.5pc\dotfill\hskip10pt}}\vskip3pt%
    {\fontsize{10}{12}\selectfont\noindent\unvbox\@abstractbox\par}%
    \vspace{1.5\p@}%
    \else%
       \vspace{0\p@}%
     \fi%
\if@subjectindex@provided%
\vspace*{-4.5pt}
      {\fontfamily{\sfdefault}\fontsize{9}{11}\selectfont\leftskip=4.7pc\parindent=0pt
      {\hbox to 448.6pt{\hskip4.5pc\dotfill\hskip10pt}}%
       \@hangfrom{{\begin{tabular}{@{}p{6pc}@{\hskip0.8pt}}{\subindexname}\end{tabular}}}\@subjectindex\par}\vspace*{-2pt}%
    \vspace{11\p@}%
\else%
       \vspace{0\p@}%
\fi%
    \if@classification@provided
      {\leftskip\z@\parfillskip=\z@ plus1fill%
        \fontsize{8}{9}\selectfont\@classification\par}%
    \fi
  \par
  \ifunarticle%
  \vspace{-.8pc plus 6\p@}%
  \else%
  \vspace{2pc plus 6\p@ minus 3\p@}%
  \fi\enlargethispage{-12pt}
 }
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Lastpage %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lastpage@putlabel{\addtocounter{page}{-1}%
   \immediate\write\@auxout{\string
   \newlabel{LastPage}{{}{\thepage}}}%
   \addtocounter{page}{1}
   }
\AtEndDocument{%
   \message{Setting LastPage}%
   \clearpage\lastpage@putlabel}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%% Sectioning macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Lowest level heading that takes a number by default
%\ifletterpaper
%\setcounter{secnumdepth}{0}
%\else
%\setcounter{secnumdepth}{3}
%\fi

\setcounter{secnumdepth}{3}

% Reset the default section macros to help with title casing
\def\@sect#1#2#3#4#5#6[#7]#8{%
  \ifnum #2>\c@secnumdepth
    \let\@svsec\@empty
  \else
    \refstepcounter{#1}%
    \protected@edef\@svsec{\@seccntformat{#1}\relax}%
  \fi
  \@tempskipa #5\relax
  \ifdim \@tempskipa>\z@
    \begingroup
      #6{%
        \@hangfrom{\hskip #3\relax\@svsec}%
          \interlinepenalty \@M
% Modified to uppercase H1's and titlecase the rest
          \ifnum #2=1\relax
             {#8}%
          \else
            {#8}%
          \fi
        \@@par}%
    \endgroup
    \csname #1mark\endcsname{#7}%
    \addcontentsline{toc}{#1}{%
      \ifnum #2>\c@secnumdepth \else
        \protect\numberline{\csname the#1\endcsname}%
      \fi
      #7}%
  \else
    \def\@svsechd{%
      #6{\hskip #3\relax
      \@svsec \ifletterpaper#8\else#8.\fi\quad}%
      \csname #1mark\endcsname{#7}%
      \addcontentsline{toc}{#1}{%
        \ifnum #2>\c@secnumdepth \else
          \protect\numberline{\csname the#1\endcsname}%
        \fi
        #7}}%
  \fi
  \@xsect{#5}}

% H1
\ifletterpaper
\def\section{%
\renewcommand{\@seccntformat}[1]{{{\rm\csname the##1\endcsname.\quad}}}
  \@startsection{section}{1}{\z@}
  {-15\p@ plus -3\p@ minus -3\p@}{-0.0001\p@}
  {\reset@font\fontsize{12}{14}\selectfont\itshape\selectfont
    \mathversion{bold}\raggedright%\setcounter{thm}{0}%
}}
\else
\def\section{%
\renewcommand{\@seccntformat}[1]{{{\csname the##1\endcsname.\quad}}}
  \@startsection{section}{1}{\z@}
  {-15\p@ plus -3\p@ minus -3\p@}{3\p@}
  {\reset@font\fontsize{12}{14}\selectfont\fontseries{b}\selectfont
    \mathversion{bold}\raggedright%\setcounter{thm}{0}%
}}
\fi

\def\ssection{%
\renewcommand{\@seccntformat}[1]{{{\csname the##1\endcsname.\quad}}}
  \@startsection{section}{1}{\z@}
  {-15\p@ plus -3\p@ minus -3\p@}{10\p@}
  {\reset@font\fontsize{12}{14}\selectfont\fontseries{b}\selectfont
    \mathversion{bold}\raggedright%\setcounter{thm}{0}%
}}

% H2
\def\subsection{%
\renewcommand{\@seccntformat}[1]{{{\it\csname the##1\endcsname.\quad}}}
  \@startsection{subsection}{2}{\z@}
  {-16.5\p@ plus -1\p@ minus -2\p@}{2\p@}
  {\reset@font\fontsize{12}{14}\fontseries{m}\fontshape{it}\selectfont
    \raggedright}}

\def\ssubsection{%
\renewcommand{\@seccntformat}[1]{{{\csname the##1\endcsname.\quad}}}
  \@startsection{subsection}{2}{\z@}
  {-16.5\p@ plus -1\p@ minus -2\p@}{14\p@}
  {\reset@font\fontsize{10}{12}\fontseries{b}\fontshape{m}\selectfont
    \mathversion{bold}\raggedright}}

% H3
\def\subsubsection{%
\renewcommand{\@seccntformat}[1]{{{\csname the##1\endcsname.\quad}}}
  \@startsection{subsubsection}{3}{\z@}
  {-12\p@ plus -1\p@ minus -2\p@}{0.0001\z@}
  {\reset@font\fontsize{11}{15}\fontseries{m}\fontshape{it}\selectfont
    \raggedright}}

\def\paragraph{%
\renewcommand{\@seccntformat}[1]{{{\csname the##1\endcsname.\quad}}}
  \@startsection{paragraph}{4}{\z@}
  {-1\@bls plus -1\p@}{-1em}
  {\reset@font\normalfont\normalsize\itshape}}


 % H5
 \def\subparagraph{%
   \@startsection{subparagraph}{5}{\z@}
   {-12\p@ plus -1\p@}{-1em}
   {\indent\reset@font\normalfont\normalsize%\bfseries
   }}


\def\acksection{%
  \@startsection{section}{1}{\z@}
  {-15\p@ plus -2\p@ minus -1\p@}{6\p@}
  {\reset@font\fontsize{12}{14}\selectfont\fontseries{b}\selectfont
    \mathversion{bold}\raggedright}}

\def\refsection{%
  \@startsection{section}{1}{\z@}
  {-17\p@ plus -2\p@ minus -1\p@}{1.5001\p@}
  {\reset@font\fontsize{12}{14}\selectfont\fontseries{b}\selectfont
    \mathversion{bold}\raggedright}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Footnotes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\@makefnmark{\parindent1em%
%\@textsuperscript{\normalfont\@thefnmark}}%
\renewcommand{\thefootnote}{\arabic{footnote}}
\def\@makefnmark{$^{\@thefnmark}$}%


%\renewcommand\footnoterule{\setcounter{footnote}{0}\leftskip\z@\noindent
%  \rule{8pc}{0.5\p@}\vspace{4\p@}}

\ifunarticle
\renewcommand\footnoterule{}
\else
\renewcommand\footnoterule{\leftskip\z@\noindent
\rule{6pc}{.5pt}
\vspace{2.5\p@}}
\fi
\newcommand\@makefntext[1]{%
 \begingroup
    \leftskip=\z@\rightskip=\z@
    \fontsize{10}{12}\selectfont
    \setlength\parindent{1em}%
    \@makefnmark\ignorespaces\,#1%
  \endgroup}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% From ifmtarg.sty
% Copyright Peter Wilson and Donald Arseneau, 2000
\begingroup
\catcode`\Q=3
\long\gdef\@ifmtarg#1{\@xifmtarg#1QQ\@secondoftwo\@firstoftwo\@nil}
\long\gdef\@xifmtarg#1#2Q#3#4#5\@nil{#4}
\long\gdef\@ifnotmtarg#1{\@xifmtarg#1QQ\@firstofone\@gobble\@nil}
\endgroup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%% PostScript Rotation Macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@rotate \@rotatefalse
\newif\if@rotatecenter \@rotatecenterfalse
\def\rotatecenter{\global\@rotatecentertrue}
\def\rotateendcenter{\global\@rotatecenterfalse}
\def\rotate{\global\@rotatetrue}
\def\endrotate{\global\@rotatefalse}
\newdimen\rotdimen
\def\rotstart#1{\special{ps: gsave currentpoint currentpoint translate
    #1 neg exch neg exch translate}}
\def\rotfinish{\special{ps: currentpoint grestore moveto}}
\def\rotl#1{\rotdimen=\ht#1\advance\rotdimen by \dp#1
    \hbox to \rotdimen{\vbox to\wd#1{\vskip \wd#1
    \rotstart{270 rotate}\box #1\vss}\hss}\rotfinish}
\def\rotr#1{\rotdimen=\ht #1\advance\rotdimen by \dp#1
    \hbox to \rotdimen{\vbox to \wd#1{\vskip \wd#1
    \rotstart{90 rotate}\box #1\vss}\hss}\rotfinish}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ********************
% Figures and tables *
% ********************

\setlength\arraycolsep{5\p@}
\setlength\tabcolsep{6\p@}
\setlength\arrayrulewidth{.4\p@}
\setlength\doublerulesep{2\p@}
\setlength\tabbingsep{\labelsep}
\skip\@mpfootins = \skip\footins
\setlength\fboxsep{3\p@}
\setlength\fboxrule{.4\p@}

\newcounter{figure}
\renewcommand \thefigure {\@arabic\c@figure}
\def\fps@figure{tbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\figurename\nobreakspace\thefigure}
\newenvironment{figure}
               {\@float{figure}}
               {\end@float}
\newenvironment{figure*}
               {\@dblfloat{figure}}
               {\end@dblfloat}
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{\tablename\nobreakspace\thetable}
\newenvironment{table}
               {\@float{table}}
               {\end@float}
\newenvironment{table*}
               {\@dblfloat{table}}
               {\end@dblfloat}
\newlength\abovecaptionskip
\newlength\belowcaptionskip
\setlength\abovecaptionskip{10\p@}
\setlength\belowcaptionskip{4\p@}
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{#1: #2}%
  \ifdim \wd\@tempboxa >\hsize
    #1: #2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}

\newcommand\figurename{Fig.}
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{\textbf{#1}\hspace*{1em}#2}%
  \ifdim \wd\@tempboxa >\hsize
    \textbf{#1}\hspace*{1em} #2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Lists %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\labelenumi{{\rm(\arabic{enumi})}}
\def\theenumi{\arabic{enumi}}
\def\labelenumii{{\rm(\alph{enumii})}}
\def\theenumii{\alph{enumii}}
\def\p@enumii{\theenumi}
\def\labelenumiii{{\rm(\arabic{enumiii})}}
\def\theenumiii{\roman{enumiii}}
\def\p@enumiii{\theenumi(\theenumii)}
\def\labelenumiv{{\rm(\arabic{enumiv})}}
\def\theenumiv{\Alph{enumiv}}
\def\p@enumiv{\p@enumiii\theenumiii}
\def\labelitemi{$\circ$}
\def\labelitemii{$\bullet$}
\def\labelitemiii{$\bullet$}
\def\labelitemiv{$\bullet$}

\setlength{\leftmargini}{9pt}
\setlength{\leftmarginii}{\z@}
\setlength{\leftmarginiii}{\z@}
\setlength{\leftmarginiv}{\z@}

\def\enumargs{%
   \partopsep     \z@
   \itemsep       \z@
   \parsep        \z@
   \rightmargin   \z@
   \labelsep      0.5em
   \listparindent \parindent
   \itemindent    \z@}

\def\enumerate{%
    \@ifnextchar[{\@numerate}{\@numerate[(3)]}}

\def\@numerate[#1]{%
     \ifnum \@enumdepth >3 \@toodeep\else
     \advance\@enumdepth \@ne
     \edef\@enumctr{enum\romannumeral\the\@enumdepth}
     \list{\csname label\@enumctr\endcsname}{%
       \enumargs
       \setlength{\leftmargin}{\csname leftmargin\romannumeral\the\@listdepth\endcsname}
       \usecounter{\@enumctr}
       \settowidth\labelwidth{#1}
       \addtolength{\leftmargin}{\labelwidth}
       \addtolength{\leftmargin}{\labelsep}
       \def\makelabel##1{\hss \llap{##1}}}%
     \fi
   }
\def\endenumerate{\endlist\advance \@listdepth -1}

% Changes to the list parameters for itemize
\def\itemargs{%
   \partopsep     \z@
   \itemsep       \z@
   \parsep        \z@
   \rightmargin   \z@
   \labelsep      0.5em
   \listparindent \parindent
   \itemindent    \z@}

\def\itemize{%
    \@ifnextchar[{\@itemize}{\@itemize[$\bullet$]}}

\def\@itemize[#1]{%
     \ifnum \@itemdepth >3 \@toodeep\else
     \advance\@itemdepth \@ne
     \edef\@itemctr{item\romannumeral\the\@itemdepth}
     \list{\csname label\@itemctr\endcsname}{%
       \itemargs
       \setlength{\leftmargin}{\csname leftmargin\romannumeral\the\@listdepth\endcsname}
       \settowidth\labelwidth{#1}
       \addtolength{\leftmargin}{\labelwidth}
       \addtolength{\leftmargin}{\labelsep}
       \def\makelabel##1{\hss \llap{##1}}}%
     \fi
   }
\let\enditemize\endlist

\setlength{\topsep}{6\p@}% \@plus 1\p@ \@minus 1\p@}
\setlength{\itemsep}{\z@}

\def\@listI{\leftmargin\leftmargini\topsep4\p@ plus 2\p@ minus 1\p@}
\let\@listi\@listI
\@listi
\def\@listii{\leftmargin\leftmarginii\topsep\z@}
\def\@listiii{\leftmargin\leftmarginiii\topsep\z@}
\def\@listiv{\leftmargin\leftmarginiv\topsep\z@}
\def\@listv{\leftmargin\leftmarginv\topsep\z@}
\def\@listvi{\leftmargin\leftmarginvi\topsep\z@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% unnumbered list %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{description}{%
  \begin{list}{}{%
      \usecounter{enumi}%
      \setlength{\itemsep}{\z@}%
      \setlength{\labelwidth}{\z@}%
      \setlength{\leftmargin}{2em}%
      \setlength{\itemindent}{-2em}}}%
{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Extracts %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\quotation{\par\begin{list}{}{\footnotesize%  Extracts in small type
      \setlength{\topsep}{\medskipamount}%
      \setlength{\itemsep}{\z@}%
      \setlength\labelwidth{\z@}%
      \setlength\labelsep{\z@}%
      \setlength\leftmargin{12pt}%
      \setlength\rightmargin{12pt}%
      \listparindent \parindent}%
  \item[\vrule width\z@ height 9\p@]}
\def\endquotation{\end{list}}
\let\quote\quotation
\let\endquote\endquotation
\newcommand{\source}[1]{\newline\hbox{}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\qedsymbol}{\ensuremath{\blacksquare}}
\renewenvironment{proof}[1][\proofname]{\par
  \if@endproofbox\pushQED{\qed}\fi%
  \normalfont
  \topsep\bigskipamount
  \labelsep=1em\relax
  \trivlist
  \item[\hskip\labelsep
        \itshape
    #1.]\ignorespaces
}{%
  \if@endproofbox\popQED\fi
  \endtrivlist\@endpefalse
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{thebibliography}[1]
     {\vbox{\vskip12pt\centering{\sc References}}
                  % \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}%
   \list{\ifnum@bib\@biblabel{\@arabic\c@enumiv}\fi}%
        {\settowidth\labelwidth{\@biblabel{#1}}%
           \topsep3.5pt
            \fontsize{9}{11}\selectfont  
            \parsep0pt        
            \ifnum@bib
            \itemsep0pt
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
          \else
            \leftmargin18pt
            \listparindent -18pt%
                         \leftmargin 18pt
                         \itemindent    \listparindent
                        \rightmargin 0pt
                        \itemsep 1pt
            \fi
           \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m
      }
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist
     }
       
      
\newcommand\newblock{\hskip .11em\@plus.33em\@minus.07em}
\let\@openbib@code\@empty

% Counter for saving the section numbering depth
\newcounter{savesecnumdepth}

%%%%%%%%%%%%%%%%%%%%%%%%%% Acknowledgments %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\providecommand{\ackname}{Acknowledgements}
\newcommand{\ack}[1][\ackname]{\fontsize{10}{12}\selectfont\par%
  \setcounter{savesecnumdepth}{\value{secnumdepth}}%
  \setcounter{secnumdepth}{0}%
  \acksection{#1}%
  \setcounter{secnumdepth}{\value{savesecnumdepth}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%% Nomenclature %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\providecommand{\nomenname}{Nomenclature}
\newcommand{\nomen}[1][\nomenname]{%
  \setcounter{savesecnumdepth}{\value{secnumdepth}}%
  \setcounter{secnumdepth}{0}%
  \section{#1}%
  \setcounter{secnumdepth}{\value{savesecnumdepth}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Notes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\enoteheading{\section*{\notesname
  \@mkboth{\uppercase{\notesname}}{\uppercase{\notesname}}}%
     \leavevmode\par}

\def\enoteformat{\rightskip\z@ \leftskip=16pt\parindent=0pt
     \leavevmode\llap{\hbox{${\@theenmark}$}.\enskip}}


\newenvironment{notes}[1][99]{%
  \begingroup%
 }%
{\endgroup}%

\ifnum@bib
\usepackage[sort&compress]{natbib}
\bibpunct{[}{]}{,}{n}{,}{;}
\else
\usepackage{natbib}
\bibpunct{(}{)}{;}{a}{,}{,}
\def\@biblabel#1{}
\fi

\renewenvironment{thebibliography}[1]
     {\vbox{\vskip12pt{\noindent\bf References}}
   \list{\ifnum@bib\@biblabel{\@arabic\c@enumiv}\fi}%
        {\settowidth\labelwidth{\@biblabel{#1}}%
           \topsep3.5pt
            \fontsize{9}{11}\selectfont  
            \parsep0pt        
            \ifnum@bib
            \itemsep0pt
            \leftmargin\labelwidth
                  \setlength{\labelsep}{0.7em}%%chgd. 1em to 0.5em on 21/7/2004 -- devi
            \advance\leftmargin\labelsep
          \else
            \leftmargin18pt
            \listparindent -18pt%
                         \leftmargin 18pt
                         \itemindent    \listparindent
                        \rightmargin 0pt
                        \itemsep 1pt
            \fi
           \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m
      }
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist
     }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  NORMES  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newskip\normskip
\setlength\normskip{6pt}

\newenvironment{normes}{%
  \begingroup
  \footnotesize\parindent=0pt
  \setcounter{secnumdepth}{0}
  \vskip\normskip
  {\fontsize{10}{12}\selectfont\bf\normsname}%
  \begin{list}{}{%
      \usecounter{enumi}%
      \setlength{\itemsep}{\z@}%
      \setlength{\labelwidth}{0pt}%
      \setlength{\leftmargin}{2em}%
      \setlength{\itemindent}{-2em}}}%
{\end{list}\endgroup}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Index %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@restonecol
\def\theindex{\@mainmatterfalse
  \@restonecoltrue\if@twocolumn\@restonecolfalse\fi
  \begingroup\parindent \z@
  \addcontentsline{toc}{section}{Index}
  \columnseprule \z@
  \columnsep 1pc\section*{\indexname} %Subject or Author here
  \parskip\z@ plus .3\p@\relax\let\item\idxitem\fontsize{8\p@}{10\p@}\selectfont}
\def\idxitem{\par\raggedright\hangindent 3em}
\def\subitem{\par\penalty1000\raggedright\hangindent 3em\hspace*{1em}}
\def\subsubitem{\par\penalty1000\raggedright\hangindent 3em\hspace*{2em}}
\def\endtheindex{\if@restonecol\endgroup\onecolumn\else\clearpage\fi}
\def\indexspace{\par \vskip 18\p@ plus 12\p@ minus 12\p@\relax}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%% Appendix %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifappend % Are we in the Appendix?
\def\appendix{%
\normalsize\selectfont\par%
  \setcounter{secnumdepth}{3}
\renewcommand{\thesection}{\Alph{section}}
\numberwithin{equation}{section}
\numberwithin{figure}{section}
\numberwithin{table}{section}
\def\theequation{\Alph{section}\@arabic\c@equation}
\def\thetable{\Alph{section}\@arabic\c@table}
\def\thefigure{\Alph{section}\@arabic\c@figure}
        \setcounter{section}{0}
        \setcounter{table}{0}
        \setcounter{figure}{0}
        \setcounter{equation}{0}
        \setcounter{subsection}{0}
        \appendtrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Override settings in MathTime back to TeX defaults
\DeclareMathSizes{5}     {5}   {5}  {5}
\DeclareMathSizes{6}     {6}   {5}  {5}
\DeclareMathSizes{7}     {7}   {5}  {5}
\DeclareMathSizes{8}     {8}   {6}  {5}
\DeclareMathSizes{9}     {9}   {7}  {5}
\DeclareMathSizes{10}   {10}   {7}  {5}
\DeclareMathSizes{12}   {12}   {9}  {7}

%Math parameters
\setlength{\jot}{5\p@}
\skip\@mpfootins = \skip\footins
\fboxsep=6\p@
\fboxrule=.25\p@

\medmuskip=4mu% plus 2mu minus 4mu
\thickmuskip=5mu% plus 5mu

\vbadness=9999
\tolerance=9999
\doublehyphendemerits=10000
\doublehyphendemerits 640000
\finalhyphendemerits  1000000

\flushbottom
\frenchspacing
\onecolumn
\pagestyle{headings}

% Author queries
\fboxsep=4\p@
\fboxrule=0.5\p@

% Short-form coding
\newcommand\tetal{{{\rm et~al.}}}
\newcommand\etal{\textit{et~al.}}
\newcommand\eg{\textit{e.g.}}
\newcommand\ie{\textit{i.e.}}
\let\endash\textendash

\def\dbond{\raise0.18ex\hbox{$=$}}
\def\bond{\raise0.18ex\hbox{$-$}}

\def\endash{--}
\def\emdash{\,--\,}
\def\sdot#1{{\buildrel{\scriptscriptstyle\bullet}\over{\hbox{$#1$}}}}
\def\ssdot#1{{\buildrel{\scriptscriptstyle\bullet\bullet}\over{\hbox{$#1$}}}}


\hyphenation{Table}
\hyphenation{Figure}
\hyphenation{Section}
\hyphenation{equation}
\hyphenation{Theorem}
\hyphenation{Lemma}
\hyphenation{Algorithm}
\hyphenation{Definition}
\hyphenation{Corollary}
\hyphenation{Proof}
\hyphenation{Remark}

\newcommand\@pnumwidth{13.5pt}
\newcommand\@dotsep{15}
\newcommand\@tocrmarg {3pt}
\setcounter{tocdepth}{3}

\def\@dottedtocline#1#2#3#4#5{% FROM LATEX.LTX
  \ifnum #1>\c@tocdepth \else
    \vskip \z@ \@plus.2\p@
    {\leftskip #2\relax \rightskip \@tocrmarg %\parfillskip -\rightskip
     \parfillskip -2.5pt% to give 20pt \rightskip
     \parindent #2\relax\@afterindenttrue
     \interlinepenalty\@M
     \leavevmode
     \@tempdima #3\relax
     \advance\leftskip \@tempdima \null\hskip -\leftskip
     {#4}\nobreak
     \leaders\hbox{}\hfill
     \nobreak
     {#5}%
     \par}%
  \fi
}

\def \twocolumn {%
  \global\columnwidth\textwidth
  \global\advance\columnwidth-\columnsep
  \global\divide\columnwidth\tw@
  \global\hsize\columnwidth
  \global\linewidth\columnwidth
  \global\@twocolumntrue
  \global\@firstcolumntrue
  \col@number \tw@
  \@ifnextchar [\@topnewpage\@floatplacement
}

\def\tocspace#1{\vphantom{\vrule height#1 width0pt}}

\newcommand\tableofcontents{%\setbox4=\hbox to \textwidth{%
  \@restonecoltrue
 \hsize\textwidth
  \section*{\hspace*{\fill}\centering Contents\hspace*{\fill}{\textsc{PAGE}\hspace*{23.5pt}}}%
  \@starttoc{toc}%
%  \if@restonecol\twocolumn\fi
  \par\addvspace{18\p@}}

\newcommand\guidetableofcontents{%
  \@restonecolfalse
  \if@twocolumn\@restonecoltrue\onecolumn\fi
  \section*{\contentsname\\[0.5\baselineskip]
    \footnotesize\textit{Note that authors are not asked to include a
    table of contents in their articles.\\ This is for reference only.}}%
  \@starttoc{toc}%
  \if@restonecol\twocolumn\fi
  \par\addvspace{\full@line}%
}

\newcommand*\l@part[2]{%
  \addpenalty{-\@highpenalty}%
  \addvspace{\baselineskip}%
  \begingroup
    \parindent \z@ \rightskip \@pnumwidth
    \parfillskip -\@pnumwidth
    \rightskip=33.5pt%
    {\small\normalfont\rmfamily
     \leavevmode
     \hspace*{33.5pt}%
     {\rm #1}\hfil \hb@xt@\@pnumwidth{\hss {\rm #2}}}\par
     \nobreak
    \global\@nobreaktrue
    \everypar{\global\@nobreakfalse\everypar{}}%
  \endgroup
}

\newcommand*\l@section[2]{%
  \addpenalty{\@secpenalty}%
  \@tempdima 17.5pt% (equiv 1.5em at 9pt)
  \begingroup
    \parindent \z@ \rightskip \@pnumwidth
    \parfillskip -\@pnumwidth
    \normalfont\rmfamily\leavevmode
    \advance\leftskip\@tempdima
    \leftskip=23pt\rightskip=35.5pt% added 24-jul-02
    #1\hfill{#2}\par
      \endgroup
}

\newcommand*\l@subsection[2]{%
  \addpenalty{\@secpenalty}%
  \@tempdima 28.5pt% (equiv 1.5em at 9pt)
  \begingroup
    \parindent \z@ \rightskip \@pnumwidth
    \parfillskip -\@pnumwidth
    \normalfont\rmfamily\leavevmode
    \advance\leftskip\@tempdima
    \leftskip=3.2pc\rightskip=35.5pt% added 24-jul-02
    #1\hfill{#2}\par
      \endgroup
}

\newcommand*\l@subsubsection[2]{%
  \addpenalty{\@secpenalty}%
  \@tempdima 32.5pt% (equiv 1.5em at 9pt)
  \begingroup
    \parindent \z@ \rightskip \@pnumwidth
    \parfillskip -\@pnumwidth
    \normalfont\rmfamily\leavevmode
    \advance\leftskip\@tempdima
  %  \hskip -\leftskip
    \leftskip=5.5pc\rightskip=35.5pt% added 24-jul-02
    #1\hfill{#2}\par
      \endgroup
}

\newcommand*\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
\newcommand*\l@subparagraph{\@dottedtocline{5}{10em}{5em}}

\newenvironment{tabenumerate}[1][10pc]{
\begin{minipage}[t]{#1}
\begin{enumerate}
}{\end{enumerate}
\end{minipage}}

\def\email#1{{\par $^{\ast}$E-mail: #1}}

\newenvironment{tabitemize}[1][10pc]{
\begin{minipage}[t]{#1}
\begin{itemize}
}{\end{itemize}
\end{minipage}}

\Year{2015}

\def\shortauthorlist#1{\gdef\@shortauthorlist{\uppercase{#1}}}
\let\@shortauthorlist\@empty
\def\shorttitle#1{\gdef\@shorttitle{\uppercase{#1}}}
\let\@shorttitle\@empty

%%%%%%%%%%%%%%%%%%%%%% Macros from PTPTEX %%%%%%%%%%%%%%%%%%%%
\newcommand\tocite[1]{$^{\hbox{--}}$\cite{#1}}%\cite{xx}\tocite{yy}
\def\halftext{.471\textwidth}
\def\@JLone<#1,#2>{#1}
\def\@JLtwo<#1,#2,#3>{#2}
\def\@JLyear<#1,#2,#3,#4>{#3}
\def\@JLpage<#1,#2,#3,#4>{#4}
\newcommand\JL[1]{\@JLone<#1>\ {\bfseries \@JLtwo<#1>}, \@JLyear<#1> (\@JLpage<#1>)}
\def\@Jpage<#1,#2,#3>{#3}
\newcommand\andvol[1]{{\bfseries \@JLone<#1>}, \@JLtwo<#1> (\@Jpage<#1>).}
\newcommand\PTP[1]{Prog.\ Theor.\ Phys.,\ \andvol{#1}}
\newcommand\PTPS[1]{Prog.\ Theor.\ Phys. Suppl.,\ \andvol{#1}} %%Modified by TD 12/06/14
\newcommand\JPSJ[1]{J.~Phys.\ Soc.\ Jpn.,\ \andvol{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\PR[1]{Phys.\ Rev.,\ \andvol{#1}}%Maybe deleted in future version
\newcommand\PRA[1]{Phys.\ Rev.\ A,\ \andvol{#1}}
\newcommand\PRB[1]{Phys.\ Rev.\ B,\ \andvol{#1}}
\newcommand\PRC[1]{Phys.\ Rev.\ C,\ \andvol{#1}}
\newcommand\PRD[1]{Phys.\ Rev.\ D,\ \andvol{#1}}
\newcommand\PRE[1]{Phys.\ Rev.\ E,\ \andvol{#1}}
\newcommand\PRX[1]{Phys.\ Rev.\ X,\ \andvol{#1}} %%Added by TD 12/06/14
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\PRL[1]{Phys.\ Rev.\ Lett.,\ \andvol{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\RMP[1]{Rev.\ Mod.\ Phys.,\ \andvol{#1}} %%Added by TD 12/06/14
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\PL[1]{Phys.\ Lett.,\ \andvol{#1}}%Maybe deleted in future version
\newcommand\PLA[1]{Phys.\ Lett.\ A,\ \andvol{#1}}
\newcommand\PLB[1]{Phys.\ Lett.\ B,\ \andvol{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\NP[1]{Nucl.\ Phys.,\ \andvol{#1}}%Maybe deleted in future version
\newcommand\NPA[1]{Nucl.\ Phys.\ A,\ \andvol{#1}}
\newcommand\NPB[1]{Nucl.\ Phys.\ B,\ \andvol{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\JMP[1]{J.~Math.\ Phys.,\ \andvol{#1}}
\newcommand\JMPNY[1]{J.~Math.\ Phys.\ (N.Y.),\ \andvol{#1}} %%Added by TD 12/06/14
\newcommand\JMPCA[1]{J.~Math.\ Phys.\ (Cambridge, Mass.),\ \andvol{#1}} %%Added by TD 12/06/14
\newcommand\IJMP[1]{Int.\ J.~Mod.\ Phys.,\ \andvol{#1}}
\newcommand\CMP[1]{Commun.\ Math.\ Phys.,\ \andvol{#1}}
\newcommand\JP[1]{J.~Phys.,\ \andvol{#1}} %%Modified by TD 12/06/14
\newcommand\JPA[1]{J.~Phys.\ A,\ \andvol{#1}} %%Added by TD 12/06/14
\newcommand\JPG[1]{J.~Phys.\ G,\ \andvol{#1}} %%Added by TD 12/06/14
\newcommand\JPCM[1]{J.~Phys.:\ Condens.\ Matter, \andvol{#1}} %%Added by TD 12/06/14
\newcommand\ANN[1]{Ann.\ Phys.,\ \andvol{#1}} %%Added by TD 12/06/14
\newcommand\ANNB[1]{Ann.\ Phys.\ (Berlin), \andvol{#1}} %%Added by TD 12/06/14
\newcommand\ANNNY[1]{Ann. Phys.\ (N.Y.), \andvol{#1}} %%Added by TD 12/06/14
\newcommand\NC[1]{Nuovo Cimento,\ \andvol{#1}} %%Modified by TD 12/06/14
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\AJ[1]{Astrophys. J.,\ \andvol{#1}}
\newcommand\PRP[1]{Phys. Rep.,\ \andvol{#1}}
\newcommand\JHEP[1]{J. High Energy Phys.,\ \andvol{#1}}
\mark{{}{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\name#1#2{#1$^{#2}$}

%\def\affil#1#2{$^{#1}$#2\par}

\def\fname#1{#1}
\def\surname#1{#1}
\def\midname#1{#1}
\def\collaborator#1{\textbf{#1}\par}

\newcommand{\PTPTeX}{\raisebox{-.2ex}{$\mathcal P$}\kern-.05em{$\mathcal T$}\kern-.18em\raisebox{-.2ex}{$\mathcal P$}\kern-.03em\TeX}
\newcommand{\@typeset}{typeset using \PTPTeX.cls}

\iferratum
\parindent0pt
\def\supertitle#1{\def\@supertitle{{\noindent{\sf\textbf{Erratum}: Prog. Theor. Exp. Phys. \textbf{\eyear@info}, #1}}}\global\@supertitle@providedtrue}
\Year{20xx}
\ErrYear{20xx}
\fi

\ifpreprint
\input preprint_v1.clo
\fi
\usepackage{lastpage}
\endinput

